A Comparison of Image Denoising Methods

The advancement of imaging devices and countless images generated everyday pose an increasingly high demand on image denoising, which still remains a challenging task in terms of both effectiveness and efficiency. To improve denoising quality, numerous denoising techniques and approaches have been proposed in the past decades, including different transforms, regularization terms, algebraic representations and especially advanced deep neural network (DNN) architectures. Despite their sophistication, many methods may fail to achieve desirable results for simultaneous noise removal and fine detail preservation. In this paper, to investigate the applicability of existing denoising techniques, we compare a variety of denoising methods on both synthetic and real-world datasets for different applications. We also introduce a new dataset for benchmarking, and the evaluations are performed from four different perspectives including quantitative metrics, visual effects, human ratings and computational cost. Our experiments demonstrate: (i) the effectiveness and efficiency of representative traditional denoisers for various denoising tasks, (ii) a simple matrix-based algorithm may be able to produce similar results compared with its tensor counterparts, and (iii) the notable achievements of DNN models, which exhibit impressive generalization ability and show state-of-the-art performance on various datasets. In spite of the progress in recent years, we discuss shortcomings and possible extensions of existing techniques. Datasets, code and results are made publicly available and will be continuously updated at https://github.com/ZhaomingKong/Denoising-Comparison.

==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Algorithm_M_SVD.tex <==
%\begin{algorithm}[ht]
%\caption{Modified SVD (M-SVD)}
%{\bf Input:} Noisy image $\mathcal{A}\in \mathbb{R}^{ps \times ps \times 3}$, patch size $ps$, number of similar patches $K$ and search window size $\Omega_{SR}$.\\
%{\bf Output:} Estimated clean image $\hat{\mathcal{A}}_c$.\\
%{\bf Step 1} (Grouping): For every reference patch of $\mathcal{A}$, stack $K$ similar patches in a group $\mathcal{G} \in \mathbb{R}^{ps \times ps \times 3 \times K}$ within $\Omega_{SR}$.\\
%{\bf Step 2} (Collaborative filtering):\\
% \hspace*{0.2in}(1) Obtain the group and patch level transform matrices $\mathbf{U}$ and $\mathbf{V}$ by performing SVD on $\mathbf{G}_{opp_{(3)}}$ and $\mathbf{G}_{(4)}^T$, respectively.\\
% \hspace*{0.2in}(2) Apply the hard-threshold technique to $\mathbf{C} = \mathbf{U}^T \mathbf{G}_{(4)} \mathbf{V}$ via $\mathbf{C}_{trun} = \text{hard-threshold}(\mathbf{C})$.\\
% \hspace*{0.2in}(3) Take the inverse transform to obtain estimated clean group via $\hat{\mathbf{G}}_{c} = \mathbf{U} \mathbf{C}_{trun} \mathbf{V}^T$.\\
%{\bf Step 4} (Aggregation): Averagely write back all image patches in $\hat{\mathbf{G}}_{c}$ to their original locations.
%\label{m-svd}
%\end{algorithm}

\begin{algorithm}[ht]
\caption{Modified SVD (M-SVD)}
{\bf Input:} Noisy image $\mathcal{A}$, patch size $ps$, number of similar patches $K$ and search window size $\Omega_{SR}$.\\
{\bf Output:} Estimated clean image $\hat{\mathcal{A}}_c$.\\
{\bf Step 1} (Grouping): For every reference patch of $\mathcal{A}$, stack $K$ similar patches in a group $\mathcal{G}$ within $\Omega_{SR}$.\\
{\bf Step 2} (Collaborative filtering):\\
 \hspace*{0.18in}(1) Obtain the group and patch level transform $\mathbf{U}$ and $\mathbf{V}$ by performing SVD on $\mathbf{G}_{opp_{(3)}}$ and $\mathbf{G}_{(4)}^T$, respectively.\\
 \hspace*{0.18in}(2) Apply the hard-threshold technique to $\mathbf{C} = \mathbf{U}^T \mathbf{G}_{(4)} \mathbf{V}$ via $\mathbf{C}_{trun} = \text{hard-threshold}(\mathbf{C})$.\\
 \hspace*{0.18in}(3) Take the inverse transform to obtain estimated clean group via $\hat{\mathbf{G}}_{c} = \mathbf{U} \mathbf{C}_{trun} \mathbf{V}^T$.\\
{\bf Step 3} (Aggregation): Averagely write back all image patches in $\hat{\mathbf{G}}_{c}$ to their original locations.
\label{m-svd}
\end{algorithm}
 \vspace{-0.3cm}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/FIg_compare_MRI_NLSVD_HOSVD.tex <==
%\begin{figure}[htbp]
%\graphicspath{{Figs/combine_real_MRI_in_Supplementary/}}
%\centering
%%\subfigure[MRI\_0092]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{MRI_0092_Noisy_slice48_combine_marked}}
%\subfigure[SVD]{
%\label{Fig4}
%\includegraphics[MRI_0092_NLPCA_slice48_combined}}
%\subfigure[HOSVD]{
%\label{Fig4}
%\includegraphics[width=0.78in]{MRI_0092_HOSVD_slice48_combined}}
%
%
%\caption{Comparison of SVD and HOSVD transforms for real MRI denoising.}
%
%\label{Fig_compare_MRI_NLSVD_HOSVD}
%\end{figure}

\begin{figure}[htbp]
\graphicspath{{Figs/combine_real_MRI_in_Supplementary/}}
\centering
\subfigure[MRI\_0092]{
\label{Fig4}
\includegraphics[width=1.08in]{MRI_0092_Noisy_slice48_combine_marked}}
\subfigure[SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{MRI_0092_NLPCA_slice48_combined}}
\subfigure[HOSVD]{
\label{Fig4}
\includegraphics[width=1.08in]{MRI_0092_HOSVD_slice48_combined}}


\caption{Comparison of SVD and HOSVD for real MRI denoising.}
\label{Fig_compare_MRI_NLSVD_HOSVD}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_Brainweb.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_Brainweb/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.81in]{Clean_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.81in]{Noisy}}
\subfigure[NLPCA]{
\label{Fig4}
\includegraphics[width=0.81in]{NLPCA}}
\subfigure[PRINLM]{
\label{Fig4}
\includegraphics[width=0.81in]{PRINLM}}
\subfigure[PRI-NLPCA]{
\label{Fig4}
\includegraphics[width=0.81in]{PRI_NLPCA_marked}}
\subfigure[ILR-HOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{HOSVDR_S}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.81in]{MStSVD}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.81in]{BM4D2}}


\caption{Visual evaluation of compared methods on the Brainweb T1w data with noise level $\sigma$ = 19\%.}
\label{Fig_Brainweb}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_CAVE.tex <==
%%\begin{figure}[htbp]
%%\graphicspath{{Figs/combine_CAVE/}}
%%\centering
%%\subfigure[Clean]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{Clean_combined_marked}}
%%\subfigure[Noisy]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{Noisy}}
%%\subfigure[BM4D2]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{BM4D2_combined}}
%%\subfigure[NGMeet]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{NGMeet_combined}}\\
%%
%%\subfigure[4DHOSVD]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{4DHOSVD_combined}}
%%\subfigure[MSt-SVD]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{MStSVD_combined}}
%%\subfigure[LTDL]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{LTDL_combined}}
%%\subfigure[LLRT]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{LLRT_combined}}
%%
%%
%%
%%\caption{Visual evaluation of the CAVE dataset with noise level $\sigma = 100$.}
%%\label{Fig_CAVE}
%%\end{figure}
%
%
%\begin{figure}[htbp]
%\graphicspath{{Figs/combine_CAVE/}}
%\centering
%\subfigure[Clean]{
%\label{Fig4}
%\includegraphics[width=0.78in]{Clean_combined_marked}}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=0.78in]{Noisy}}
%\subfigure[4DHOSVD]{
%\label{Fig4}
%\includegraphics[width=0.78in]{4DHOSVD_combined}}
%\subfigure[BM4D2]{
%\label{Fig4}
%\includegraphics[width=0.78in]{BM4D2_combined}}\\
%\subfigure[LLRT]{
%\label{Fig4}
%\includegraphics[width=0.78in]{LLRT_combined}}
%\subfigure[LTDL]{
%\label{Fig4}
%\includegraphics[width=0.78in]{LTDL_combined}}
%\subfigure[MSt-SVD]{
%\label{Fig4}
%\includegraphics[width=0.78in]{MStSVD_combined}}
%\subfigure[NGMeet]{
%\label{Fig4}
%\includegraphics[width=0.78in]{NGMeet_combined}}
%
%
%\caption{Visual evaluation of the CAVE dataset with noise level $\sigma = 100$.}
%\label{Fig_CAVE}
%\end{figure}

%\begin{figure}[htbp]
%\graphicspath{{Figs/combine_CAVE/}}
%\centering
%\subfigure[Clean]{
%\label{Fig4}
%\includegraphics[width=0.78in]{Clean_combined_marked}}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=0.78in]{Noisy}}
%\subfigure[BM4D2]{
%\label{Fig4}
%\includegraphics[width=0.78in]{BM4D2_combined}}
%\subfigure[NGMeet]{
%\label{Fig4}
%\includegraphics[width=0.78in]{NGMeet_combined}}\\
%
%\subfigure[4DHOSVD]{
%\label{Fig4}
%\includegraphics[width=0.78in]{4DHOSVD_combined}}
%\subfigure[MSt-SVD]{
%\label{Fig4}
%\includegraphics[width=0.78in]{MStSVD_combined}}
%\subfigure[LTDL]{
%\label{Fig4}
%\includegraphics[width=0.78in]{LTDL_combined}}
%\subfigure[LLRT]{
%\label{Fig4}
%\includegraphics[width=0.78in]{LLRT_combined}}
%
%
%
%\caption{Visual evaluation of the CAVE dataset with noise level $\sigma = 100$.}
%\label{Fig_CAVE}
%\end{figure}


\begin{figure}[htbp]
\graphicspath{{Figs/combine_CAVE/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.78in]{Clean_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.78in]{Noisy}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.78in]{BM4D2_combined}}
\subfigure[LLRT]{
\label{Fig4}
\includegraphics[width=0.78in]{LLRT_combined}} \\
\subfigure[LTDL]{
\label{Fig4}
\includegraphics[width=0.78in]{LTDL_combined}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.78in]{MStSVD_combined}}
\subfigure[NGMeet]{
\label{Fig4}
\includegraphics[width=0.78in]{NGMeet_combined}}
\subfigure[OLRT]{
\label{Fig4}
\includegraphics[width=0.78in]{OLRT_combined_marked}}


\caption{Visual evaluation of the CAVE dataset with noise level $\sigma = 100$.}
\label{Fig_CAVE}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_CBM3D_noise_level_influence.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_discussion/}}
\centering
\subfigure[PSNR]{
\label{Fig4}
\includegraphics[width=1.65in]{CBM3D1_PSNR_change_new2}}
\subfigure[SSIM]{
\label{Fig4}
\includegraphics[width=1.699in]{CBM3D1_SSIM_change_new}}


\caption{PSNR and SSIM change of CBM3D1 with noise level $\sigma \in [10, 30]$ on five real-world color image datasets.}
\label{Fig_CBM3D_noise_level_influence}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_CC15.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_CC15/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_Origin}}
\subfigure[Noisy (33.26)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_Noisy}}
\subfigure[NI (38.78)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_NI_mark}}
\subfigure[DeNoiseAI (36.63)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_Topaz_marked}}
\subfigure[DBF (41.42)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_DeepBoosting}}
\subfigure[DRUNet (40.85)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_DRUNet}}\\

\subfigure[FFDNet (40.15)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_FFDNet}}
\subfigure[FCCF (41.21)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_FCCF}}
\subfigure[CBM3D2 (39.59)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_CBM3D2}}
\subfigure[CMSt-SVD (39.98)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_MS-TSVD}}
\subfigure[TWSC (40.27)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_TWSC}}
\subfigure[NLH (40.21)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_NLH}}


\caption{Visual evaluations of compared methods (PSNR) on CC15 dataset.}
\label{Fig_CC15}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_CNN.tex <==
\begin{figure}[htbp]
  \centering
  \graphicspath{{Figs/Fig_frameworks/}}
  \includegraphics[width=2.866in, height=1.399in]{CNN_denoising_new}\\
  \caption{A plain CNN denoising framework with three convolutional layers.}
  \label{Fig_CNN}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_CRVD.tex <==
\begin{figure}[htbp]
\graphicspath{{C:/Users/KZM11/Desktop/Figs_Video/result_images_sample/selected_for_comparison/Combined/CRVD/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}\\
\subfigure[DVDNet]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}

\caption{Visual evaluation of compared methods (PSNR) on our IOCI's IPHONE 5S dataset.}
\label{Fig_CRVD}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_CRVD_plus_Set8.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/Figs_Video/result_images_sample/selected_for_comparison/Combined/CRVD_plus_Set8/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.828in]{Clean_combined_CRVD_Set8_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.828in]{Noisy_combined_CRVD_Set8}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.828in]{CVMStSVD_combined_CRVD_Set8}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=0.828in]{VBM4D2_combined_CRVD_Set8}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=0.828in]{FastDVDNet_combined_CRVD_Set8}}
\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=0.828in]{FloRNN_combined_CRVD_Set8}}
\subfigure[RVRT]{
\label{Fig4}
\includegraphics[width=0.828in]{RVRT_combined_CRVD_Set8}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=0.828in]{VNLNet_combined_CRVD_Set8}}

\caption{Visual evaluation of compared methods on synthetic and real-world video data. First row: Set8 ($\sigma = 40$), second row: CRVD (ISO = 6400).}
\label{Fig_CRVD_plus_Set8}
\end{figure*}



%\begin{figure*}[htbp]
%\graphicspath{{Figs/Figs_Video/result_images_sample/selected_for_comparison/Combined/CRVD_plus_Set8/}}
%\centering
%\subfigure[Mean]{
%\label{Fig4}
%\includegraphics[width=0.828in]{Clean_combined_CRVD_Set8_marked}}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=0.828in]{Noisy_combined_CRVD_Set8}}
%\subfigure[CVMSt-SVD]{
%\label{Fig4}
%\includegraphics[width=0.828in]{CVMStSVD_combined_CRVD_Set8}}
%\subfigure[VBM4D2]{
%\label{Fig4}
%\includegraphics[width=0.828in]{VBM4D2_combined_CRVD_Set8}}
%\subfigure[DVDNet]{
%\label{Fig4}
%\includegraphics[width=0.828in]{DVDNet_combined_CRVD_Set8}}
%\subfigure[FastDVDNet]{
%\label{Fig4}
%\includegraphics[width=0.828in]{FastDVDNet_combined_CRVD_Set8}}
%\subfigure[FloRNN]{
%\label{Fig4}
%\includegraphics[width=0.828in]{FloRNN_combined_CRVD_Set8}}
%\subfigure[VNLNet]{
%\label{Fig4}
%\includegraphics[width=0.828in]{VNLNet_combined_CRVD_Set8}}
%
%\caption{Visual evaluation of compared methods on synthetic and real-world video data. First row: Set8 ($\sigma = 40$), second row: CRVD (ISO = 6400).}
%\label{Fig_CRVD_plus_Set8}
%\end{figure*}

%\begin{figure*}[htbp]
%\graphicspath{{C:/Users/KZM11/Desktop/Figs_Video/result_images_sample/selected_for_comparison/Combined/CRVD_plus_Set8/}}
%\centering
%\subfigure[Bitonic]{
%\label{Fig4}
%\includegraphics[width=0.728in]{Clean_combined_CRVD_Set8_marked}}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=0.728in]{Noisy_combined_CRVD_Set8}}
%\subfigure[CMSt-SVD]{
%\label{Fig4}
%\includegraphics[width=0.728in]{CVMStSVD_combined_CRVD_Set8}}
%\subfigure[VBM4D2]{
%\label{Fig4}
%\includegraphics[width=0.728in]{VBM4D2_combined_CRVD_Set8}}
%\subfigure[DVDNet]{
%\label{Fig4}
%\includegraphics[width=0.728in]{DVDNet_combined_CRVD_Set8}}
%\subfigure[Restormer]{
%\label{Fig4}
%\includegraphics[width=0.728in]{FastDVDNet_combined_CRVD_Set8}}
%\subfigure[FloRNN]{
%\label{Fig4}
%\includegraphics[width=0.728in]{FloRNN_combined_CRVD_Set8}}
%\subfigure[VNLNet]{
%\label{Fig4}
%\includegraphics[width=0.728in]{VNLNet_combined_CRVD_Set8}}
%\subfigure[VNLNet]{
%\label{Fig4}
%\includegraphics[width=0.728in]{VNLNet_combined_CRVD_Set8}}
%
%\caption{Visual evaluation of compared methods on synthetic and real-world data. First row: Set8 ($\sigma = 40$), second row: CRVD (ISO = 6400).}
%\label{Fig_CRVD_plus_Set8}
%\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_DND_plus_SIDD.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/Figs_Image(sRGB)/result_images_sample/selected_for_comparison/Combined/DND_plus_SIDD/}}
\centering
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_Noisy_marked}}
\subfigure[Bitonic]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_Bitonic}}
\subfigure[CBM3D2]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_CBM3D2}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_CMStSVD}}
\subfigure[NLHCC]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_NLHCC}}
\subfigure[AINDNet]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_AINDNet}}
\subfigure[NAFNet]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_NAFNet}}
\subfigure[PNGAN]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_PNGAN}}
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.728in]{DND_plus_SIDD_Restormer}}

\caption{Visual evaluation of compared methods on DnD (first row) and SIDD (second row) datsets.}
%\caption{Visual evaluation of compared methods on real-world datasets. First row: DND, second row: SIDD.}
\label{Fig_DND_plus_SIDD}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_HHD.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/combine_HHD/Combine_new/}}
\centering
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=1.08in]{imga4_combined}}
%\subfigure[BM4D1]{
%\label{Fig4}
%\includegraphics[width=1.08in]{imga4_BM4D1_combined}}
%\subfigure[MSt-SVD]{
%\label{Fig4}
%\includegraphics[width=1.08in]{imga4_MStSVD_combined}}\\

%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=1.08in]{imgc6_combined_marked}}
%\subfigure[BM4D1]{
%\label{Fig4}
%\includegraphics[width=1.08in]{imgc6_BM4D1_combined_marked}}
%\subfigure[MSt-SVD]{
%\label{Fig4}
%\includegraphics[width=1.08in]{imgc6_MStSVD_combined}}

\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{imgc6_combine_new_marked}}
\subfigure[BM4D1]{
\label{Fig4}
\includegraphics[width=1.08in]{imgc6_BM4D1_combine_new_marked}}
\subfigure[TDL]{
\label{Fig4}
\includegraphics[width=1.08in]{imgc6_TDL_combine_new}}\\
%\subfigure[FastHyDe]{
%\label{Fig4}
%\includegraphics[width=1.08in]{imgc6_FastHyDe_combine_new}}
\subfigure[QRNN3D]{
\label{Fig4}
\includegraphics[width=1.08in]{imgc6_QRNN3D_combine_new}}
\subfigure[NGMeet]{
\label{Fig4}
\includegraphics[width=1.08in]{imgc6_NGMeet_combine_new_marked}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{imgc6_MStSVD_combine_new}}


\caption{Visual evaluation of the real-world HHD dataset.}
\label{Fig_HHD}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_HUAWEI-Mate40Pro_IPHONE13_compare.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[HUAWEI Mate40Pro]{
\label{Fig4}
\includegraphics[width=1.28in]{Huawei_Mate40Pro_IMG15_6_noisy_combined}}
\subfigure[IPHONE 13]{
\label{Fig4}
\includegraphics[width=1.28in]{IPHONE13_IMG39_9_noisy_combined}}

\caption{Images captured by two popular smartphone cameras of the same objects in the dark environment.}
\label{Fig_HUAWEI-Mate40Pro_IPHONE13_compare}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_HUAWEI-Mate40Pro_dark_environment_demo.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_images_Supp_proposed_dataset/}}
\centering
\subfigure[Trees]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo1}}
\subfigure[Streetlight]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo2}}
\subfigure[Grass]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo3}}

\caption{Images captured by HUAWEI Mate40Pro in dark environments.}
\label{Fig_HUAWEI-Mate40Pro_dark_environment_demo}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_HUAWEI-Mate40Pro_different_environment_demo.tex <==
%\begin{figure}[htbp]
%\graphicspath{{C:/Users/KZM11/Desktop/Fig_images_Supp_proposed_dataset/Combined/}}
%\centering
%\subfigure[Morning]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_sufficient-light_combined_marked}}
%\subfigure[Afternoon]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_low-light_combined}}
%\subfigure[Midnight]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_dark_combined}}
%
%\caption{Images of HUAWEI Mate40Pro under different lighting conditions.}
%\label{Fig_HUAWEI-Mate40Pro_different_environment_demo}
%\end{figure}


\begin{figure}[htbp]
\graphicspath{{Figs/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[Morning]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_sufficient-light_combined_marked}}
\subfigure[Afternoon]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_low-light_combined}}
\subfigure[Midnight]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_dark_combined}}

\caption{Images of IPHONE13 under different lighting conditions.}
\label{Fig_HUAWEI-Mate40Pro_different_environment_demo}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_HUAWEI-Mate40Pro_noise_pattern_compare.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[Cups]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG4_2_noisy_combined}}
\subfigure[Streetlight]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG13_3_noisy_combined}}
\subfigure[Building A]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG30_6_noisy_combined}}
\subfigure[Building B]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG28_1_noisy_combined}}

\caption{Images captured by HUAWEI Mate40Pro of different scenes.}
\label{Fig_HUAWEI-Mate40Pro_noise_pattern_compare}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_IOCV_new.tex <==
%\begin{figure*}[htbp]
%\graphicspath{{Figs/combined_IOCV/}}
%\centering
%\subfigure[Mean]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Clean_sclice1_combined}}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Noisy_sclice1_combined}}
%\subfigure[CVMSt-SVD]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_CVMStSVD_combined}}
%\subfigure[VBM4D2]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_VBM4D2_combined}}
%\subfigure[DVDNet]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_DVDNet_sig15_combined}}
%\subfigure[FastDVDNet]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_fastdvdnet_sig10_combined}}\\
%
%\subfigure[FloRNN]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_FloRNN_sig40_combined}}
%\subfigure[MAP-VDNet]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_MAP-VDNet_sig15_combined}}
%\subfigure[RFR]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_RFR_sig25_combined}}
%\subfigure[UDVD]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_UDVD_sig30_combined}}
%\subfigure[ViDeNN]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_ViDeNN_ckpt_videnn_combined}}
%\subfigure[VNLNet]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_vnlnet_sig20_combined}}
%
%
%\caption{Visual evaluation of video denoising on the IOCV dataset. The camera device is OPPO R11s.}
%\label{Fig_IOCV_new}
%\end{figure*}
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_IOCV/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Clean_sclice1_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Noisy_sclice1_combined}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_CVMStSVD_combined}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_VBM4D2_combined}}
\subfigure[DVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_DVDNet_sig15_combined}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_fastdvdnet_sig10_combined}}\\

\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_FloRNN_sig40_combined}}
\subfigure[MAP-VDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_MAP-VDNet_sig15_combined}}
\subfigure[RVRT]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_RVRT_sig20_combined}}
\subfigure[UDVD]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_UDVD_sig30_combined}}
\subfigure[ViDeNN]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_ViDeNN_ckpt_videnn_combined}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_vnlnet_sig20_combined}}


\caption{Visual evaluation of video denoising on the IOCV dataset. The camera device is OPPO R11s.}
\label{Fig_IOCV_new}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_Kong_dataset.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_dataset_illus/}}
\centering
\subfigure[The proposed IOCI dataset]{
\label{Fig4}
\includegraphics[width=3.38in]{Kong-Image}}
\subfigure[The proposed IOCV dataset]{
\label{Fig4}
\includegraphics[width=3.38in]{Kong-Video}}


\caption{Illustration of the proposed IOCI and IOCV dataset.}
\label{Fig_Kong_dataset}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_My_dataset_IPHONE13.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/Figs_Image(sRGB)/result_images_sample/selected_for_comparison/Combined/My_dataset/IPHONE13/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.829in]{Clean_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.829in]{Noisy_combined}}
\subfigure[Bitonic]{
\label{Fig4}
\includegraphics[width=0.829in]{Bitonic_combined}}
\subfigure[CBM3D2]{
\label{Fig4}
\includegraphics[width=0.829in]{CBM3D2_combined}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.829in]{CMSt-SVD_combined}}
\subfigure[MCWNNM]{
\label{Fig4}
\includegraphics[width=0.829in]{MCWNNM_combined}}
\subfigure[NLHCC]{
\label{Fig4}
\includegraphics[width=0.829in]{NLHCC_combined}}
\subfigure[TWSC]{
\label{Fig4}
\includegraphics[width=0.829in]{TWSC_combined}}\\

\subfigure[AINDNet]{
\label{Fig4}
\includegraphics[width=0.829in]{AINDNet_combined}}
\subfigure[DIDN]{
\label{Fig4}
\includegraphics[width=0.829in]{DIDN_combined}}
\subfigure[DRUNet]{
\label{Fig4}
\includegraphics[width=0.829in]{DRUNet_combined}}
\subfigure[FCCF]{
\label{Fig4}
\includegraphics[width=0.829in]{FCCF_combined}}
\subfigure[NAFNet]{
\label{Fig4}
\includegraphics[width=0.829in]{NAFNet_combined}}
\subfigure[PNGAN]{
\label{Fig4}
\includegraphics[width=0.829in]{PNGAN_combined_marked}}
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.829in]{Restormer_combined}}
\subfigure[VDIR]{
\label{Fig4}
\includegraphics[width=0.829in]{VDIR_combined}}


\caption{Visual evaluation of compared methods on the real-world IOCI dataset. The camera device is IPHONE 13.}
\label{Fig_My_dataset_IPHONE13}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_NSS.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_frameworks/}}
\centering
\subfigure[Image data]{
\label{Fig4}
\includegraphics[width=0.81in]{Color_image}}
\subfigure[Video data]{
\label{Fig4}
\includegraphics[width=0.81in]{Color_video}}
\subfigure[MRI data]{
\label{Fig4}
\includegraphics[width=0.81in]{MRI}}
\subfigure[MSI data]{
\label{Fig4}
\includegraphics[width=0.81in]{MSI}}




\caption{The nonlocal self-similarity (NLSS) prior and patch representation of different imaging sensors, techniques and applications.}
\label{Fig_NSS}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_PSNR_diff_Fujifilm_test.tex <==
\begin{figure}[htbp]
%\setlength{\abovecaptionskip}{0.cm}
%\setlength{\belowcaptionskip}{-0.8cm}

\graphicspath{{Figs/Fig_discussion/}}

%\centering
%\includegraphics[width=2.36in]{PSNR_diff}
\centering
\subfigure[PSNR]{
\label{Fig4}
\includegraphics[width=1.66in]{PSNR_diff_new}}
\subfigure[SSIM]{
\label{Fig4}
\includegraphics[width=1.66in]{SSIM_diff_new}}

\caption{PSNR and SSIM difference of six implementations compared with 'Mean\_3' on the FUJI dataset.}

\label{Fig_PSNR_diff_Fujifilm_test}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_PolyU_new.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/Figs_Image(sRGB)/result_images_sample/selected_for_comparison/Combined/PolyU/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.829in]{Clean_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.829in]{Noisy_combined}}
\subfigure[Bitonic]{
\label{Fig4}
\includegraphics[width=0.829in]{Bitonic_combined}}
\subfigure[CBM3D2]{
\label{Fig4}
\includegraphics[width=0.829in]{CBM3D2_combined}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.829in]{CMSt-SVD_combined}}
\subfigure[MCWNNM]{
\label{Fig4}
\includegraphics[width=0.829in]{MCWNNM_combined}}
\subfigure[NLHCC]{
\label{Fig4}
\includegraphics[width=0.829in]{NLHCC_combined}}
\subfigure[TWSC]{
\label{Fig4}
\includegraphics[width=0.829in]{TWSC_combined}}\\

\subfigure[AINDNet]{
\label{Fig4}
\includegraphics[width=0.829in]{AINDNet_combined_marked}}
\subfigure[DIDN]{
\label{Fig4}
\includegraphics[width=0.829in]{DIDN_combined}}
\subfigure[DRUNet]{
\label{Fig4}
\includegraphics[width=0.829in]{DRUNet_combined}}
\subfigure[FCCF]{
\label{Fig4}
\includegraphics[width=0.829in]{FCCF_combined}}
\subfigure[NAFNet]{
\label{Fig4}
\includegraphics[width=0.829in]{NAFNet_combined}}
\subfigure[PNGAN]{
\label{Fig4}
\includegraphics[width=0.829in]{PNGAN_combined}}
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.829in]{Restormer_combined}}
\subfigure[VDIR]{
\label{Fig4}
\includegraphics[width=0.829in]{VDIR_combined}}


\caption{Visual evaluation of compared methods on the real-world PolyU dataset. The camera device is NIKON D800.}
\label{Fig_PolyU_new}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_Real_HSI.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/combined_Real_HSI/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.8in]{Clean_img_57_slice_26_enhanced_combined_with_arrow_and_square}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.8in]{Noisy_img_57_slice_26_enhanced_combined}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.8in]{BM4D2_img_57_slice_26_enhanced_combined}}
%\subfigure[LLRT]{
%\label{Fig4}
%\includegraphics[width=0.78in]{LLRT_img_57_slice_26_enhanced_1.8_combined}}
\subfigure[LTDL]{
\label{Fig4}
\includegraphics[width=0.8in]{LTDL_img_57_slice_26_enhanced_combined}} \\
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.8in]{MStSVD_img_57_slice_26_enhanced_combined_with_arrow}}
\subfigure[NGMeet]{
\label{Fig4}
\includegraphics[width=0.8in]{NGMeet_img_57_slice_26_enhanced_combined}}
\subfigure[OLRT]{
\label{Fig4}
\includegraphics[width=0.8in]{OLRT_img_57_slice_26_enhanced_combined}}
\subfigure[QRNN3D]{
\label{Fig4}
\includegraphics[width=0.8in]{QRNN3D_img_57_slice_26_enhanced_combined}}


\caption{Visual evaluation of the real-world Real-HSI dataset.}
\label{Fig_Real_HSI}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_SIDD_validate_test_similar.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Figs_Supp_Experiments_Image_dataset/}}
\centering
\subfigure[Validation]{
\label{Fig4}
\includegraphics[width=1.28in]{SIDD_Validate_noisysRGB_19_23_sigma_0}}
\subfigure[Test]{
\label{Fig4}
\includegraphics[width=1.28in]{SIDD_Benchmark_noisysRGB_19_2_sigma_0}}

\caption{Sample images from the validation and test sets of SIDD.}
\label{Fig_SIDD_validate_test_similar}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_Set8.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_Set8/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.828in]{Clean_Motorbike_slice18_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.828in]{Noisy_Motorbike_slice18_sig40_combined}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.828in]{18_CVMStSVD_sig40_combined}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=0.828in]{18_VBM4D2_sig40_combined}}
\subfigure[DVDNet]{
\label{Fig4}
\includegraphics[width=0.828in]{18_DVDNet_sig40_combined}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=0.828in]{18_FastDVDNet_sig40_combined}}
\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=0.828in]{18_FloRNN_sig40_combined}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=0.828in]{18_vnlnet_sig40_combined}}

\caption{Visual evaluation of compared methods on the Set8 dataset.}
\label{Fig_Set8}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_Video_slider.tex <==
\begin{figure}[htbp]

\graphicspath{{Figs/Fig_frameworks/}}

\centering
\includegraphics[width=3.58in]{Video_slider}


\caption{The procedure of generating mean video sequences with a motorized slider. The camera is fixed to a rotatable tripod ball-head placed on
top of the slider.}

\label{Fig_Video_slider}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_Xu_100.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_Xu_100/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_Origin}}
\subfigure[Noisy (36.68)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_Noisy}}
\subfigure[NI (36.78)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_NI}}
\subfigure[DeNoiseAI (36.01)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_Topaz}}
\subfigure[DBF (36.62)]{
\label{Fig4}
\includegraphics[width=1.1in]{Figs/combined_Xu_100/NikonD800_4-5_160_1800_classroom_5_real_DeepBoosting_mark.png}}
\subfigure[DRUNet (37.57)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_DRUNet}}\\
\subfigure[FFDNet (36.95)]{
\label{Fig4}
\includegraphics[width=1.1in]{Figs/combined_Xu_100/NikonD800_4-5_160_1800_classroom_5_real_FFDNet.png}}
\subfigure[FCCF (37.48)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_FCCF}}
\subfigure[CBM3D2 (37.81)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_CBM3D2}}
\subfigure[CMSt-SVD (37.80)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_MS-TSVD}}
\subfigure[TWSC (37.16)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_TWSC}}
\subfigure[NLH (37.14)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_NLH}}


\caption{Visual evaluation of compared methods (PSNR) on PolyU dataset.}
\label{Fig_Xu_100}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_choose_N_noisy_for_mean_image.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Figs_Supp_Experiments_Image_dataset/}}
\centering
\subfigure[Relative error]{
\label{Fig4}
\includegraphics[width=1.696in]{Fig_Compare_mean_GT_img_relative_error}}
\subfigure[SSIM]{
\label{Fig4}
\includegraphics[width=1.696in]{Fig_Compare_mean_GT_img_SSIM}}

\caption{Relative error and SSIM of different mean images compared to the ground-truth. The camera device is IPHONE 13.}
\label{Fig_choose_N_noisy_for_mean_image}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_color_video.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/combined_real_video/combine/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.08in]{Clean}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{CVMStSVD}}\\
\subfigure[VBM4D1]{
\label{Fig4}
\includegraphics[width=1.08in]{VBM4D1}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{Fastdvdnet}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=1.08in]{Vnlnet}}\\


\caption{Visual evaluation of video denoising on the IOCV dataset.}
\label{Fig_color_video}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_dataset_illus.tex <==
%\begin{figure}[htbp]
%
%\graphicspath{{Figs/Fig_dataset_illus/}}
%
%\centering
%\includegraphics[width=3.39in]{Dataset_illus_all_new2}
%
%
%\caption{Illustration of datasets for different applications. From the first row to the fourth row: grayscale/color image, video, MSI and MRI data.}
%
%\label{Fig_dataset_illus}
%\end{figure}

\begin{figure}[htbp]

\graphicspath{{Figs/Fig_dataset_illus/}}

\centering
\includegraphics[width=3.39in]{Fig_illus_dataset}


\caption{Illustration of datasets for different applications. From the first row to the fourth row: grayscale/color image, video, MSI/HSI and MRI data.}

\label{Fig_dataset_illus}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_discussion_visual_enhancement.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_discussion/}}
\centering
\subfigure[Noisy (RENOIR)]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy_demo_combine_marked}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{denoised_demo_combine}}
\subfigure[CMSt-SVD\_R]{
\label{Fig4}
\includegraphics[width=1.08in]{resized_demo_combine}}

\subfigure[Noisy (DND)]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy_demo2_combine_marked}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{denoised_demo2_combine}}
\subfigure[CMSt-SVD\_R]{
\label{Fig4}
\includegraphics[width=1.08in]{resized_demo2_combine}}


\caption{Visual evaluation of CMSt-SVD with and without the image resizing strategy on RENOIR (first row) and DND (second row) datasets.}
\label{Fig_discussion_visual_enhancement}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_fastMRI.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_fastMRI/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.81in]{Clean_img_9_slice_26_combined}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.81in]{Noisy_img_9_slice_26_combined}}
\subfigure[4DHOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{4DHOSVD1_img_9_slice_26_combined}}
\subfigure[AONLM]{
\label{Fig4}
\includegraphics[width=0.81in]{AONLM_img_9_slice_26_combined}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.81in]{BM4D2_img_9_slice_26_combined}}
\subfigure[ILR-HOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{ILRHOSVD_img_9_slice_26_combined}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.81in]{MStSVD_img_9_slice_26_combined}}
\subfigure[ODCT]{
\label{Fig4}
\includegraphics[width=0.81in]{ODCT_img_9_slice_26_combined}}


\caption{Visual evaluation of compared methods on the fastMRI dataset with noise level $\sigma$ = 19\%.}
\label{Fig_fastMRI}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_illus_PSNR_SSIM_MRI.tex <==
%\begin{figure}[htbp]
%\graphicspath{{Figs/Fig_others/}}
%\centering
%\subfigure[PSNR]{
%\label{Fig4}
%\includegraphics[width=1.69in]{PSNR_MRI}}
%\subfigure[SSIM]{
%\label{Fig4}
%\includegraphics[width=1.69in]{SSIM_MRI}}
%
%
%\caption{Average PSNR and SSIM values of representative compared methods on the Brainweb data at high noise levels ($\sigma \geq 11\%$).}
%\label{Fig_illus_PSNR_SSIM_MRI}
%\end{figure}

\begin{figure}[htbp]
\graphicspath{{Figs/Fig_MRI_PSNR_SSIM/}}
\centering
\subfigure[PSNR of Brainweb]{
\label{Fig_MRI_results_a}
\includegraphics[width=1.69in]{Fig_Brainweb_PSNR}}
\subfigure[PSNR of fastMRI]{
\label{Fig_MRI_results_b}
\includegraphics[width=1.69in]{Fig_FastMRI-Knee_PSNR}}


\caption{Average PSNR values of compared methods on the Brainweb and fastMRI data at high noise levels ($\sigma \geq 11\%$).}
\label{Fig_illus_PSNR_SSIM_MRI}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_my_dataset_SONYA6500.tex <==
%\begin{figure*}[htbp]
%\graphicspath{{Figs/combined_my_dataset_SonyA6500/}}
%\centering
%\subfigure[Mean]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_clean_combined_marked}}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_combined}}
%\subfigure[4DHOSVD]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_4DHOSVD_combined}}
%\subfigure[mSVD]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_mSVD_combined}}
%\subfigure[Bitonic]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_bitonic_combined}}
%\subfigure[CBM3D2]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_CBM3D2_combined}} \\
%
%\subfigure[CMSt-SVD]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_CMSt-SVD_combined}}
%\subfigure[MCWNNM]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_MCWNNM_combined}}
%\subfigure[NLHCC]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_NLHCC_combined}}
%\subfigure[TWSC]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_TWSC_combined}}
%\subfigure[DIDN]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_DIDN_combined}}
%\subfigure[DRUNet]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_DPIR_combined}}\\
%
%\subfigure[FCCF]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_FCCF_combined}}
%\subfigure[FFDNet]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_FFDNet_combined}}
%\subfigure[NAFNet]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_NAFNet_combined}}
%\subfigure[PNGAN]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_PNGAN_combined}}
%\subfigure[Restormer]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_Restormer_combined}}
%\subfigure[VDIR]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_VDIR_combined}}
%
%
%\caption{Visual evaluation of compared methods on the IOCI dataset. The camera device is SONYA6500.}
%\label{Fig_my_dataset_SONYA6500}
%\end{figure*}


\begin{figure*}[htbp]
\graphicspath{{Figs/combined_my_dataset_SonyA6500/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_clean_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_combined}}
\subfigure[Bitonic]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_bitonic_combined}}
\subfigure[CBM3D2]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_CBM3D2_combined}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_CMSt-SVD_combined}}
\subfigure[MCWNNM]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_MCWNNM_combined}}
\subfigure[4DHOSVD]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_4DHOSVD_combined}}
\subfigure[mSVD]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_mSVD_combined}}
\subfigure[NLHCC]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_NLHCC_combined}}\\

\subfigure[TWSC]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_TWSC_combined}}
\subfigure[DIDN]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_DIDN_combined}}
\subfigure[DRUNet]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_DPIR_combined}}
\subfigure[FCCF]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_FCCF_combined}}
\subfigure[FFDNet]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_FFDNet_combined}}
\subfigure[NAFNet]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_NAFNet_combined}}
\subfigure[PNGAN]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_PNGAN_combined}}
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_Restormer_combined}}
\subfigure[VDIR]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_VDIR_combined}}


\caption{Visual evaluation of compared methods on the IOCI dataset. The camera device is SONYA6500.}
\label{Fig_my_dataset_SONYA6500}
\end{figure*} 



==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_my_own.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_my_own/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_Origin}}
\subfigure[Noisy (41.23)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_Noisy}}
\subfigure[NI (42.89)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_NI}}
\subfigure[DeNoiseAI (41.06)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_Topaz_marked}}
\subfigure[DBF (42.66)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_DeepBoosting}}
\subfigure[DRUNet (44.47)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_DRUNet}}\\
\subfigure[FFDNet (44.77)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_FFDNet}}
\subfigure[FCCF (43.40)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_FCCF}}
\subfigure[CBM3D2 (44.54)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_CBM3D2}}
\subfigure[CMSt-SVD (44.81)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_MS-TSVD}}
\subfigure[TWSC (42.60)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_TWSC}}
\subfigure[NLH (44.47)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_NLH}}


\caption{Visual evaluation of compared methods (PSNR) on our IOCI's IPHONE 5S dataset.}
\label{Fig_my_own}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_oversmooth.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_appendix/}}
\centering
\subfigure[Origin]{
\label{Fig4}
\includegraphics[width=1.10in]{Origin}}
\subfigure[T-HOSVD]{
\label{Fig4}
\includegraphics[width=1.10in]{Over_smooth}}
\subfigure[Origin - T-HOSVD]{
\label{Fig4}
\includegraphics[width=1.10in]{Difference}}


\caption{Illustration of over-smooth effects produced by truncated HOSVD (T-HOSVD) when all the patches in a group are the same.}
\label{Fig_oversmooth}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_pre_train.tex <==
\begin{figure}[htbp]
%\setlength{\abovecaptionskip}{0.cm}
%\setlength{\belowcaptionskip}{-0.8cm}

\graphicspath{{Figs/Fig_discussion/}}

%\centering
%\includegraphics[width=2.36in]{PSNR_diff}
\centering
\subfigure[PSNR]{
\label{Fig4}
\includegraphics[width=1.69in]{PSNR_pre_train}}
\subfigure[SSIM]{
\label{Fig4}
\includegraphics[width=1.69in]{SSIM_pre_train}}

\caption{PSNR and SSIM values of DANet on the PolyU test set w.r.t different training epochs.}

\label{Fig_pre_train}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_real_MRI.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/combine_real_MRI/}}
\centering
\subfigure[MRI\_0092]{
\label{Fig4}
\includegraphics[width=0.78in]{Noisy_0092_combine_marked}}
\subfigure[NLPCA]{
\label{Fig4}
\includegraphics[width=0.78in]{NLPCA_0092_combine_marked}}
\subfigure[PRINLM]{
\label{Fig4}
\includegraphics[width=0.78in]{PRINLM_0092_combine}}
\subfigure[PRI-NLPCA]{
\label{Fig4}
\includegraphics[width=0.78in]{PRI_NLPCA_0092_combine}}\\

\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.78in]{MStSVD_0092_combine}}
\subfigure[ILR-HOSVD]{
\label{Fig4}
\includegraphics[width=0.78in]{HOSVDR_S_0092_combine}}
\subfigure[BM4D1]{
\label{Fig4}
\includegraphics[width=0.78in]{BM4D1_0092_combine}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.78in]{BM4D2_0092_combine}}


\caption{Visual evaluation of compared methods on the real OAS1\_0092 T1w data with estimated noise level $\sigma$ = 4.5\%.}
%\caption{Results on the real OAS1\_0092 T1w data ($\sigma$ = 4.5\%).}
\label{Fig_real_MRI}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_real_MRI_0112.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/combine_real_MRI/}}
\centering
\subfigure[MRI\_0112]{
\label{Fig4}
\includegraphics[width=0.78in]{Noisy_0112_combine_marked}}
\subfigure[NLPCA]{
\label{Fig4}
\includegraphics[width=0.78in]{NLPCA_0112_combine}}
\subfigure[PRINLM]{
\label{Fig4}
\includegraphics[width=0.78in]{PRINLM_0112_combine}}
\subfigure[PRI-NLPCA]{
\label{Fig4}
\includegraphics[width=0.78in]{PRI_NLPCA_0112_combine}}\\

\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.78in]{MStSVD_0112_combine}}
\subfigure[ILR-HOSVD]{
\label{Fig4}
\includegraphics[width=0.78in]{HOSVDR_S_0112_combine}}
\subfigure[BM4D1]{
\label{Fig4}
\includegraphics[width=0.78in]{BM4D1_0112_combine}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.78in]{BM4D2_0112_combine}}

\caption{Visual evaluation of compared methods on the real OAS1\_0092 T1w data with estimated noise level $\sigma$ = 3\%.}
\label{Fig_real_MRI_0112}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_timeline.tex <==
\begin{figure*}[htbp]
%\setlength{\abovecaptionskip}{0.cm}
%\setlength{\belowcaptionskip}{-0.8cm}

\graphicspath{{Figs/Fig_frameworks/}}

\centering
\includegraphics[width=6.999in]{time_line}


\caption{Timeline of representative multi-dimensional image denoising methods and datasets.}

\label{Fig_timeline}
\end{figure*}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Fig_traditional_framework.tex <==
\begin{figure}[htbp]
  \centering
  \graphicspath{{Figs/Fig_frameworks/}}
  \includegraphics[width=3.46in]{Fig_framework_Traditional_denoisers}\\
  \caption{Illustration of the grouping-collaborative filtering-aggregation framework for traditional denoisers.}
  \label{Fig_traditional_framework}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Figs_IOCV.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/combined_IOCV/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Clean_sclice1_combined}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Noisy_sclice1_combined}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_CVMStSVD_combined}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_VBM4D2_combined}}
\subfigure[DVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_DVDNet_sig15_combined}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_fastdvdnet_sig10_combined}}\\

\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_FloRNN_sig40_combined}}
\subfigure[MAP-VDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_MAP-VDNet_sig15_combined}}
\subfigure[RFR]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_RFR_sig25_combined}}
\subfigure[UDVD]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_UDVD_sig30_combined}}
\subfigure[ViDeNN]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_ViDeNN_ckpt_videnn_combined}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_vnlnet_sig20_combined}}


\caption{Visual evaluation of video denoising on the IOCV dataset. The camera device is OPPO R11s.}
\label{Fig_IOCV_new}
\end{figure}


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_CC15.tex <==
%% Table generated by Excel2LaTeX from sheet 'Results_all'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Psnr results and average computational time(s) of compared methods on CC15 dataset. The best results are bolded and the second best are underlined.}
%    \begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|c|c|}
%    \toprule
%    \multicolumn{2}{|c|}{Methods} & \multicolumn{3}{c|}{CANON 5D ISO = 3200} & \multicolumn{3}{c|}{CANON D600 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 1600} & \multicolumn{3}{c|}{NIKON D800 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 6400} & Average & Time(s) \\
%    \midrule
%    \multicolumn{2}{|c|}{Noisy} & 37.00  & 33.88  & 33.83  & 33.28  & 33.77  & 34.93  & 35.47  & 35.71  & 34.81  & 33.26  & 32.89  & 32.91  & 29.63  & 29.97  & 29.87  & 33.41  & / \\
%    \midrule
%    \multirow{15}[30]{*}{Deep Learning} & TNRD  & 39.51  & 36.47  & 36.45  & 34.79  & 36.37  & 39.49  & 38.11  & 40.52  & 38.17  & 37.69  & 35.90  & 38.21  & 32.81  & 32.33  & 32.29  & 36.61  & 0.63  \\
%\cmidrule{2-19}          & MLP   & 39.01  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & 1.28  \\
%\cmidrule{2-19}          & FFD-Net & 39.40  & 37.02  & 36.53  & 34.97  & 36.73  & 41.02  & 38.66  & 41.53  & 38.80  & 40.15  & 37.61  & 41.18  & 34.13  & 33.66  & 33.69  & 37.67  & 1.99  \\
%\cmidrule{2-19}          & CBDNet & 38.63  & 36.18  & 36.10  & 34.83  & 35.69  & 38.32  & 38.44  & 39.98  & 37.29  & 37.78  & 37.15  & 37.39  & 32.58  & 33.01  & 32.01  & 36.36  & 3.58  \\
%\cmidrule{2-19}          & DeepBoosting & 39.74  & 37.23  & 36.87  & 35.39  & 36.98  & 41.08  & 39.72  & 42.02  & 39.68  & 41.42  & 38.76  & 42.34  & 35.78  & 34.48  & 34.27  & 38.38  & 0.32  \\
%\cmidrule{2-19}          & DIDN  & 35.45  & 36.16  & 35.10  & 34.34  & 35.25  & 37.88  & 38.52  & 36.82  & 39.50  & 38.62  & 37.61  & 38.15  & 32.16  & 32.46  & 32.56  & 36.04  & 0.18  \\
%\cmidrule{2-19}          & FCCF  & 41.41  & 37.63  & 37.49  & 36.94  & 39.07  & 42.71  & 39.88  & 42.37  & 40.03  & 41.21  & 38.73  & 41.67  & 36.22  & 35.10  & 35.09  & \textbf{39.04} & 36.36  \\
%\cmidrule{2-19}          & NLNet & 40.57  & 37.05  & 36.86  & 35.26  & 36.80  & 40.47  & 39.03  & 41.53  & 39.19  & 39.37  & 37.13  & 39.83  & 33.68  & 33.33  & 33.26  & 37.56  & 49.98  \\
%\cmidrule{2-19}          & Unet  & 39.72  & 36.75  & 36.54  & 35.28  & 36.53  & 40.47  & 39.09  & 41.13  & 39.33  & 38.50  & 36.89  & 38.75  & 31.69  & 31.88  & 31.74  & 36.95  & 5.69  \\
%\cmidrule{2-19}          & VDNet & 35.68  & 35.32  & 34.93  & 33.73  & 34.92  & 37.55  & 38.27  & 37.23  & 38.56  & 38.19  & 37.69  & 38.54  & 32.45  & 32.26  & 32.65  & 35.86  & 0.21  \\
%\cmidrule{2-19}          & AINDNet & 37.57  & 36.10  & 36.04  & 34.91  & 35.90  & 37.81  & 38.22  & 38.73  & 37.00  & 36.68  & 36.85  & 35.70  & 31.86  & 32.96  & 31.93  & 35.88  & 1.29  \\
%\cmidrule{2-19}          & Noise2Noise & 36.93  & 33.79  & 33.78  & 32.99  & 33.46  & 34.71  & 35.57  & 35.83  & 34.91  & 33.20  & 33.02  & 32.98  & 29.62  & 29.94  & 29.81  & 33.37  & 0.98  \\
%\cmidrule{2-19}          & CycleISP & 36.83  & 35.38  & 35.75  & 34.36  & 35.42  & 37.82  & 38.19  & 39.26  & 37.56  & 35.79  & 35.37  & 35.35  & 31.17  & 31.42  & 31.32  & 35.40  & 0.38  \\
%\cmidrule{2-19}          & SADNet & 38.40  & 37.51  & 36.35  & 35.98  & 37.26  & 41.00  & 39.65  & 41.23  & 39.59  & 39.67  & 37.94  & 41.35  & 33.65  & 34.08  & 33.27  & 37.80  & 0.33  \\
%\cmidrule{2-19}          & DnCNN & 39.51  & 36.92  & 36.54  & 35.02  & 36.46  & 40.59  & 38.94  & 41.33  & 39.05  & 39.57  & 37.43  & 40.18  & 33.56  & 33.53  & 33.41  & 37.47  & 3.28  \\
%    \midrule
%    \midrule
%    \multirow{13}[26]{*}{Traditional Gaussian} & LCSD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 6.45  \\
%\cmidrule{2-19}          & LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & $>$1000 \\
%\cmidrule{2-19}          & WTR1  & 41.09  & 36.92  & 36.25  & 34.68  & 36.48  & 40.52  & 38.26  & 41.40  & 38.61  & 39.98  & 37.70  & 41.36  & 35.16  & 34.22  & 34.43  & 37.80  & $>$1000 \\
%\cmidrule{2-19}          & GID   & 40.82  & 37.19  & 36.92  & 35.32  & 36.62  & 38.68  & 38.88  & 40.66  & 39.20  & 37.92  & 36.62  & 37.64  & 33.01  & 32.93  & 32.96  & 37.02  & 38.88  \\
%\cmidrule{2-19}          & MCWNNM & 41.21  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & 37.72  & 228.16  \\
%\cmidrule{2-19}          & NLH\_CC & 41.57  & 37.39  & 36.68  & 35.51  & 37.21  & 41.34  & 39.67  & 42.66  & 40.04  & 40.21  & 37.30  & 42.02  & 36.19  & 34.70  & 34.83  & 38.49  & 51.86  \\
%\cmidrule{2-19}          & TWSC  & 40.55  & 35.92  & 35.15  & 35.36  & 37.09  & 41.13  & 39.36  & 41.91  & 38.81  & 40.27  & 37.22  & 42.09  & 35.53  & 34.15  & 33.93  & 37.90  & 368.68  \\
%\cmidrule{2-19}          & CBM3D1 & 40.23  & 37.02  & 36.18  & 34.78  & 36.61  & 40.44  & 38.58  & 41.34  & 39.15  & 39.57  & 37.35  & 39.79  & 34.59  & 33.84  & 33.94  & 37.56  & 0.95  \\
%\cmidrule{2-19}          & CBM3D2 & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & 37.70  & 4.38  \\
%\cmidrule{2-19}          & CBM3D\_best & 40.96  & 37.31  & 37.15  & 35.38  & 36.81  & 40.45  & 39.25  & 41.65  & 39.59  & 39.86  & 37.54  & 40.38  & 34.85  & 33.92  & 34.16  & 37.95  & 4.38  \\
%\cmidrule{2-19}          & M-SVD & 41.43  & 37.17  & 36.84  & 35.20  & 36.97  & 40.23  & 38.90  & 41.75  & 39.60  & 39.33  & 37.26  & 38.70  & 34.52  & 33.53  & 33.74  & 37.68  & 75.88  \\
%\cmidrule{2-19}          & 4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 86.69  \\
%\cmidrule{2-19}          & CMSt-SVD & 40.79  & 37.37  & 37.01  & 35.29  & 36.95  & 40.93  & 39.21  & 41.98  & 39.54  & 39.98  & 37.65  & 40.05  & 34.50  & 33.93  & 34.01  & 37.95  & 6.18  \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:addlabel}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Results_all'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Psnr results and average computational time(s) of compared methods on CC15 dataset. The best results are bolded and the second best are underlined.}
    \begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|c|c|}
    \toprule
    \multicolumn{2}{|c|}{Methods} & \multicolumn{3}{c|}{CANON 5D ISO = 3200} & \multicolumn{3}{c|}{CANON D600 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 1600} & \multicolumn{3}{c|}{NIKON D800 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 6400} & Average & Time(s) \\
    \midrule
    \multicolumn{2}{|c|}{Noisy} & 37.00  & 33.88  & 33.83  & 33.28  & 33.77  & 34.93  & 35.47  & 35.71  & 34.81  & 33.26  & 32.89  & 32.91  & 29.63  & 29.97  & 29.87  & 33.41  & / \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{15}[30]{*}{Deep Learning models}} & TNRD  & 39.51  & 36.47  & 36.45  & 34.79  & 36.37  & 39.49  & 38.11  & 40.52  & 38.17  & 37.69  & 35.90  & 38.21  & 32.81  & 32.33  & 32.29  & 36.61  & 0.63  \\
\cmidrule{2-19}          & MLP   & 39.01  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & 1.28  \\
\cmidrule{2-19}          & FFDNet & 39.40  & 37.02  & 36.53  & 34.97  & 36.73  & 41.02  & 38.66  & 41.53  & 38.80  & 40.15  & 37.61  & 41.18  & 34.13  & 33.66  & 33.69  & 37.67  & 1.99  \\
\cmidrule{2-19}          & CBDNet & 38.63  & 36.18  & 36.10  & 34.83  & 35.69  & 38.32  & 38.44  & 39.98  & 37.29  & 37.78  & 37.15  & 37.39  & 32.58  & 33.01  & 32.01  & 36.36  & 3.58  \\
\cmidrule{2-19}          & DeepBoosting & 39.74  & 37.23  & 36.87  & 35.39  & 36.98  & 41.08  & 39.72  & 42.02  & 39.68  & 41.42  & 38.76  & 42.34  & 35.78  & 34.48  & 34.27  & 38.38  & 0.32  \\
\cmidrule{2-19}          & DIDN  & 35.45  & 36.16  & 35.10  & 34.34  & 35.25  & 37.88  & 38.52  & 36.82  & 39.50  & 38.62  & 37.61  & 38.15  & 32.16  & 32.46  & 32.56  & 36.04  & 0.18  \\
\cmidrule{2-19}          & FCCF  & 41.41  & 37.63  & 37.49  & 36.94  & 39.07  & 42.71  & 39.88  & 42.37  & 40.03  & 41.21  & 38.73  & 41.67  & 36.22  & 35.10  & 35.09  & \textbf{39.04} & 36.36  \\
\cmidrule{2-19}          & NLNet & 40.57  & 37.05  & 36.86  & 35.26  & 36.80  & 40.47  & 39.03  & 41.53  & 39.19  & 39.37  & 37.13  & 39.83  & 33.68  & 33.33  & 33.26  & 37.56  & 49.98  \\
\cmidrule{2-19}          & Unet  & 39.72  & 36.75  & 36.54  & 35.28  & 36.53  & 40.47  & 39.09  & 41.13  & 39.33  & 38.50  & 36.89  & 38.75  & 31.69  & 31.88  & 31.74  & 36.95  & 5.69  \\
\cmidrule{2-19}          & VDNet & 35.68  & 35.32  & 34.93  & 33.73  & 34.92  & 37.55  & 38.27  & 37.23  & 38.56  & 38.19  & 37.69  & 38.54  & 32.45  & 32.26  & 32.65  & 35.86  & 0.21  \\
\cmidrule{2-19}          & AINDNet & 37.57  & 36.10  & 36.04  & 34.91  & 35.90  & 37.81  & 38.22  & 38.73  & 37.00  & 36.68  & 36.85  & 35.70  & 31.86  & 32.96  & 31.93  & 35.88  & 1.29  \\
\cmidrule{2-19}          & Noise2Noise & 36.93  & 33.79  & 33.78  & 32.99  & 33.46  & 34.71  & 35.57  & 35.83  & 34.91  & 33.20  & 33.02  & 32.98  & 29.62  & 29.94  & 29.81  & 33.37  & 0.98  \\
\cmidrule{2-19}          & CycleISP & 36.83  & 35.38  & 35.75  & 34.36  & 35.42  & 37.82  & 38.19  & 39.26  & 37.56  & 35.79  & 35.37  & 35.35  & 31.17  & 31.42  & 31.32  & 35.40  & 0.38  \\
\cmidrule{2-19}          & SADNet & 38.40  & 37.51  & 36.35  & 35.98  & 37.26  & 41.00  & 39.65  & 41.23  & 39.59  & 39.67  & 37.94  & 41.35  & 33.65  & 34.08  & 33.27  & 37.80  & 0.33  \\
\cmidrule{2-19}          & DnCNN & 39.51  & 36.92  & 36.54  & 35.02  & 36.46  & 40.59  & 38.94  & 41.33  & 39.05  & 39.57  & 37.43  & 40.18  & 33.56  & 33.53  & 33.41  & 37.47  & 3.28  \\
    \midrule
    \midrule
    \multicolumn{1}{|c|}{\multirow{13}[26]{*}{Traditional Gaussian Denoiser}} & LCSD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 6.45  \\
\cmidrule{2-19}          & LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & $>$1000 \\
\cmidrule{2-19}          & WTR1  & 41.09  & 36.92  & 36.25  & 34.68  & 36.48  & 40.52  & 38.26  & 41.40  & 38.61  & 39.98  & 37.70  & 41.36  & 35.16  & 34.22  & 34.43  & 37.80  & $>$2000 \\
\cmidrule{2-19}          & GID   & 40.82  & 37.19  & 36.92  & 35.32  & 36.62  & 38.68  & 38.88  & 40.66  & 39.20  & 37.92  & 36.62  & 37.64  & 33.01  & 32.93  & 32.96  & 37.02  & 38.88  \\
\cmidrule{2-19}          & MCWNNM & 41.21  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & 37.72  & 228.16  \\
\cmidrule{2-19}          & NLH\_CC & 41.57  & 37.39  & 36.68  & 35.51  & 37.21  & 41.34  & 39.67  & 42.66  & 40.04  & 40.21  & 37.30  & 42.02  & 36.19  & 34.70  & 34.83  & 38.49  & 51.86  \\
\cmidrule{2-19}          & TWSC  & 40.55  & 35.92  & 35.15  & 35.36  & 37.09  & 41.13  & 39.36  & 41.91  & 38.81  & 40.27  & 37.22  & 42.09  & 35.53  & 34.15  & 33.93  & 37.90  & 368.68  \\
\cmidrule{2-19}          & CBM3D1 & 40.23  & 37.02  & 36.18  & 34.78  & 36.61  & 40.44  & 38.58  & 41.34  & 39.15  & 39.57  & 37.35  & 39.79  & 34.59  & 33.84  & 33.94  & 37.56  & 0.95  \\
\cmidrule{2-19}          & CBM3D2 & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & 37.70  & 4.38  \\
\cmidrule{2-19}          & CBM3D\_best & 40.96  & 37.31  & 37.15  & 35.38  & 36.81  & 40.45  & 39.25  & 41.65  & 39.59  & 39.86  & 37.54  & 40.38  & 34.85  & 33.92  & 34.16  & 37.95  & 4.38  \\
\cmidrule{2-19}          & M-SVD & 41.43  & 37.17  & 36.84  & 35.20  & 36.97  & 40.23  & 38.90  & 41.75  & 39.60  & 39.33  & 37.26  & 38.70  & 34.52  & 33.53  & 33.74  & 37.68  & 75.88  \\
\cmidrule{2-19}          & 4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 86.69  \\
\cmidrule{2-19}          & CMSt-SVD & 40.79  & 37.37  & 37.01  & 35.29  & 36.95  & 40.93  & 39.21  & 41.98  & 39.54  & 39.98  & 37.65  & 40.05  & 34.50  & 33.93  & 34.01  & 37.95  & 6.18  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_Color_other_datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'Results_all'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Psnr results of compared methods on CC60, Xu-100 and Kong-Image dataset. The three best results are bolded.}
    \begin{tabular}{c|cccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{11}{c}{Dataset} \\
\cmidrule{3-13}    \multicolumn{2}{c}{} & CC60  & Xu-100 & CANON 100D & CANON 600D & HUAWEI & IPHONE 5S & IPHONE 6S & SONY & XIAOMI & OPPO & FUJIFILM \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  \\
    \midrule
    \multirow{12}[24]{*}{Deep Learning Models} & FFD-Net & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  \\
\cmidrule{2-13}          & CBDNet & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  \\
\cmidrule{2-13}          & DeepBoosting & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  \\
\cmidrule{2-13}          & DIDN  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  \\
\cmidrule{2-13}          & FCCF  & 40.89  & 38.85 & 41.91  & 43.07  & 40.11  & 40.39  & 40.65  & 45.38  & 36.67  & 40.93  & 42.78  \\
\cmidrule{2-13}          & NLNet & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  \\
\cmidrule{2-13}          & Unet  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  \\
\cmidrule{2-13}          & VDNet & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  \\
\cmidrule{2-13}          & AINDNet & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  \\
\cmidrule{2-13}          & CycleISP & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  \\
\cmidrule{2-13}          & SADNet & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  \\
\cmidrule{2-13}          & DnCNN & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  \\
    \midrule
    \midrule
    \multicolumn{1}{c|}{\multirow{11}[22]{*}{Traditional Gaussian Denoisers}} & LCSD  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  \\
\cmidrule{2-13}          & LLRT  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  \\
\cmidrule{2-13}          & GID   & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  \\
\cmidrule{2-13}          & MCWNNM & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  \\
\cmidrule{2-13}          & NLH\_CC & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & 46.00  & 35.73  & 40.69  & 42.80  \\
\cmidrule{2-13}          & TWSC  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  \\
\cmidrule{2-13}          & CBM3D1 & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  \\
\cmidrule{2-13}          & CBM3D2 & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  \\
\cmidrule{2-13}          & CBM3D\_best & 39.68 & 38.81 & 42.08 & 42.89 & 40.48 & 41.25 & 41.16 & 45.81 & 36.66  & 40.89  & 43.14  \\
\cmidrule{2-13}          & 4DHOSVD1 & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  \\
\cmidrule{2-13}          & CMSt-SVD & 39.75 & 38.82 & 41.99  & 42.75  & 40.08  & 40.84  & 40.53  & 45.89  & 36.40  & 40.85  & 42.68  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_DNN_method.tex <==
%\begin{table*}[htbp]
%\scriptsize
%\centering
%\caption{Related DNN denoising methods for multi-dimensional image data with different noise modeling techniques and applications. 'CI': color image, 'CV': color video, 'MSI': multispectral imaging, 'HSI': hyperspectral imaging, 'MRI': magnetic resonance imaging.}
%\scalebox{0.869}{
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%\textbf{Category}                      & \textbf{Network  Architectures}   & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                  \\
%\hline
%\multirow{38}{*}{\shortstack[l]{DNN \\ methods}}         & \multirow{36}{*}{CNN/NN}   & MLP \cite{burger2012image}          & AWGN                        & CI                & A multilayer perceptron model                                 \\
%
%\cline{3-6}
%                              &                          & TNRD \cite{chen2016trainable}         & AWGN                        & CI                & A trainable nonlinear difussion model                         \\
%\cline{3-6}
%                              &                          & DnCNN \cite{zhang2017beyond, jiang2018denoising}          & AWGN                        & CI, MRI                 & CNN with Residual learning and batch normalization                       \\
%\cline{3-6}
%                              &                          & NLNet \cite{lefkimmiatis2017non}         & AWGN                        & CI                & A nonlocal CNN model                                          \\
%\cline{3-6}
%                              &                          & UDNet \cite{Lefkimmiatis_2018_CVPR}        & AWGN                        & CI                & A robust and flexible CNN model                               \\
%\cline{3-6}
%                              &                          & FFDNet \cite{zhang2018ffdnet}       & AWGN                        & CI                & A flexible model with tunable input noise levels              \\
%\cline{3-6}
%                              &                          & HSID-CNN \cite{yuan2018hyperspectral}      & AWGN                        & MSI, HSI          & A 2D and 3D combined CNN model                                \\
%\cline{3-6}
%                              &                          & HSI-SDeCNN \cite{maffei2019single}    & AWGN                        & MSI, HSI          & A single CNN model with spatial and spectral information      \\
%\cline{3-6}
%                              &                          & VNLNet \cite{davy2018non}       & AWGN                        & CV                & The first nonlocal CNN model for video                        \\
%\cline{3-6}
%                              &                          & ViDeNN \cite{claus2019videnn}       & AWGN                        & CV                & Combination of spatial and temporal filtering with CNN        \\
%\cline{3-6}
%                              &                          & SADNet \cite{chang2020spatial}        & AWGN                        & CI                & A novel spatial-adaptive CNN model                            \\
%\cline{3-6}
%                              &                          & FastDVDNet \cite{Tassano_2020_CVPR}   & AWGN                        & CV                & Real-time video denoising without flow estimation                    \\
%\cline{3-6}
%                              &                          & LIDIA \cite{Vaksman_2020_CVPR_Workshops}        & AWGN                        & CI                & A lightweight denoiser with instance adaptation               \\
%\cline{3-6}
%                              &                          & DRUNet \cite{zhang2020plug}     & AWGN                   & CI                & A plug-and-play method with deep denoiser prior     \\
%\cline{3-6}
%                              &                          & ADRN \cite{zhao2020adrn}          & AWGN                   & MSI, HSI                & A deep residual network model with channel attention scheme            \\
%\cline{3-6}
%                              &                          & HSI-DeNet \cite{chang2018hsi}    & AWGN and Strip              & MSI, HSI          & A CNN method with mixed noise modeling                        \\
%\cline{3-6}
%                              &                          & Noise2noise \cite{lehtinen2018noise2noise}       & AWGN and Poisson                     & CI              & A CNN model trained only with noisy data.                         \\
%\cline{3-6}
%                              &                          & VDNet \cite{yue2019variational}        & AWGN and Realistic          & CI                & A variational inference method with noise estimation          \\
%\cline{3-6}
%                              &                          & CBDNet \cite{guo2019toward}       & Realistic                   & CI                & a convolutional blind denoising network                       \\
%\cline{3-6}
%                              &                          & PRI-PB-CNN \cite{manjon2018mri}   & AWGN an Rician              & MRI               & Combination of sliding window scheme and 3D CNN               \\
%\cline{3-6}
%                              &                          & MIFCN \cite{abbasi2019three}        & Realistic                   & MRI               & A fully convolutional network model                           \\
%\cline{3-6}
%                              &                          & DIDN \cite{yu2019deep}         & AWGN and Realistic          & CI                & A deep iterative down-up CNN model                            \\
%\cline{3-6}
%                              &                          & DRDN \cite{song2019dynamic}         & Realistic                   & CI                & A dynamic residual dense network model                        \\
%\cline{3-6}
%                              &                          & SGN \cite{gu2019self}          & Realistic                   & CI                & A self-guided network with top-down architecture              \\
%\cline{3-6}
%                              &                          & FCCF \cite{yue2019high}         & AWGN and Realistic          & CI                & Fusion of collaborative filtering (CBM3D) and CNN                     \\
%\cline{3-6}
%                              &                          & DBF \cite{chen2019real}          & AWGN and Realistic          & CI                & Integration of CNN into a boosting algorithm                    \\
%\cline{3-6}
%                              &                          & RIDNet \cite{anwar2019real}       & AWGN and Realistic          & CI                & A single stage model with feature attention                   \\
%\cline{3-6}
%                              &                          & AINDNet \cite{Kim_2020_CVPR}      & AWGN and Realistic          & CI                & Transfer learning with adaptive instance normalization        \\
%\cline{3-6}
%                              &                          & Self2Self \cite{quan2020self2self}      & AWGN and Realistic          & CI                & A self-supervised model trained only with noisy images        \\
%\cline{3-6}
%                              &                          & QRNN3D \cite{wei20203}          & AWGN and Stripe                   & MSI, HSI                & A deep recurrent neural network model with 3D convolution           \\
%\cline{3-6}
%                              &                          & CycleISP \cite{zamir2020cycleisp}     & Realistic                   & CI                & A camera pipeline model in forward and reverse directions     \\
%\cline{3-6}
%                              &                          & DANet \cite{yue2020dual}        & Realistic                   & CI                & A Bayesian framework for noise removal and generation.                    \\
%\cline{3-6}
%                              &                          & MIRNet \cite{Zamir2020MIRNet}        & Realistic                   & CI                & A multi-scale model with parallel convolution streams                   \\
%\cline{3-6}
%                              &                          & GCDN \cite{valsesia2020deep}        & AWGN and Realistic                   & CI                & A graph convolution denoising network                  \\
%\cline{2-6}
%                              & \multirow{5}{*}{CNN + GAN} & GCBD \cite{chen2018image}         & AWGN and Realistic          & CI                & A GAN-based blind denoiser                               \\
%\cline{3-6}
%                              &                          & SCGAN \cite{yan2019unsupervised}        & AWGN                        & CI                & Unsupervised modeling with self-consistent GAN                \\
%\cline{3-6}
%                              &                          & DnGAN \cite{yeh2018image}        & AWGN and Blur               & CI                & GAN with  maximum a posteriori (MAP) framework                \\
%%\cline{3-6}
%%                              &                          & RED-WGAN \cite{ran2019denoising}     & AWGN and Rician             & MRI               & A residual encoder decoder Wasserstein GAN model              \\
%\cline{3-6}
%                              &                          & ADGAN \cite{Lin_2019_CVPR_Workshops}        & Realistic                   & CI                & Attentive GAN with noise domain adaptation                    \\
%\hline
%\end{tabular}
%}
%\label{Table_DNN_method}
%\end{table*}


% Table generated by Excel2LaTeX from sheet 'DNN Methods'
\begin{table*}[htbp]
    \renewcommand{\arraystretch}{0.098}
    \scriptsize
    \centering
    \caption{Representative DNN denoising methods with different noise modeling techniques and training strategy.}
    \scalebox{0.8468}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Category & Training srategy & Methods & Year  & Noise modeling & Key words \\
    \hline
    \multirow{198}[136]{*}{DNN Methods} & \multirow{136}[100]{*}{Supervised} & MLP\cite{burger2012image} & 2012  & AWGN  & A multilayer perceptron model \\
\cline{3-6}          &       & TNRD\cite{chen2016trainable} & 2016  & AWGN  & A trainable nonlinear diffusion model \\
\cline{3-6}          &       & DnCNN\cite{zhang2017beyond} & 2017  & AWGN  & A CNN model with batch normalization and residual learning \\
%\cline{3-6}          &       & IRCNN\cite{zhang2017learning} & 2017  & AWGN  & A CNN model with BN and dilated filters \\
\cline{3-6}          &       & NLNet\cite{lefkimmiatis2017non} & 2017  & AWGN  & A nonlocal CNN model for grayscale/color image denoising \\
\cline{3-6}          &       & UDNet\cite{Lefkimmiatis_2018_CVPR} & 2018  & AWGN  & A robust and flexible CNN model using UNet \\
\cline{3-6}          &       & HSID-CNN\cite{yuan2018hyperspectral} & 2018  & AWGN  & A 2D and 3D combined CNN model \\
\cline{3-6}          &       & VNLNet\cite{davy2018non} & 2018  & AWGN  & The first nonlocal CNN model for video denoising\\
\cline{3-6}          &       & FFDNet\cite{zhang2018ffdnet} & 2018  & AWGN  & A flexible CNN model with tunable input noise levels \\
\cline{3-6}          &       & HSI-DeNet\cite{chang2018hsi} & 2018  & AWGN and Stripe & A CNN model for mixed noise removal \\
\cline{3-6}          &       & PRI-PB-CNN\cite{manjon2018mri} & 2018  & AWGN an Rician & A combination of sliding window scheme and 3D CNN \\
\cline{3-6}          &       & GCBD\cite{chen2018image} & 2018  & AWGN and Realistic & A GAN-based blind denoiser \\
\cline{3-6}          &       & DnGAN\cite{yeh2018image} & 2018  & AWGN and Blur & A GAN model with maximum a posteriori (MAP) framework \\
\cline{3-6}          &       & DBF\cite{chen2019real} & 2019  & AWGN and Realistic & Integration of CNN into a boosting algorithm \\
\cline{3-6}          &       & FCCF\cite{yue2019high} & 2019  & AWGN and Realistic & A deep fusion scheme of collaborative filtering (CBM3D) and CNN \\
\cline{3-6}          &       & DIDN\cite{yu2019deep} & 2019  & AWGN and Realistic & A deep iterative down-up CNN model \\
\cline{3-6}          &       & CBDNet\cite{guo2019toward} & 2019  & Realistic & A convolutional blind denoising network \\
\cline{3-6}          &       & ViDeNN\cite{claus2019videnn} & 2019  & AWGN  & A combination of spatial and temporal filtering with CNN \\
\cline{3-6}          &       & RIDNet\cite{anwar2019real} & 2019  & AWGN and Realistic & A single stage model with feature attention \\
\cline{3-6}          &       & MIFCN\cite{abbasi2019three} & 2019  & Realistic & A fully convolutional network model \\
\cline{3-6}          &       & DRDN\cite{song2019dynamic} & 2019  & Realistic & A dynamic residual dense network model \\
\cline{3-6}          &       & SGN\cite{gu2019self} & 2019  & Realistic & A self-guided network with top-down architecture \\
\cline{3-6}          &       & ADGAN\cite{Lin_2019_CVPR_Workshops} & 2019  & Realistic & An attentive GAN model with noise domain adaptation \\
\cline{3-6}          &       & QRNN3D\cite{wei20203} & 2020  & AWGN and Stripe & A deep recurrent neural network model with 3D convolution \\
\cline{3-6}          &       & CycleISP\cite{zamir2020cycleisp} & 2020  & Realistic & A GAN based framework modeling the camera pipeline \\
\cline{3-6}          &       & GCDN\cite{valsesia2020deep} & 2020  & AWGN and Realistic & A graph convolution network based denoising model \\
\cline{3-6}          &       & FastDVDNet \cite{Tassano_2020_CVPR}& 2020  & AWGN  & A real-time video denoising network without flow estimation \\
\cline{3-6}          &       & DANet\cite{yue2020dual} & 2020  & Realistic & A Bayesian framework for noise removal and generation \\
\cline{3-6}          &       & LIDIA \cite{Vaksman_2020_CVPR_Workshops} & 2020  & AWGN  & A lightweight model with instance adaptation \\
\cline{3-6}          &       & SADNet\cite{chang2020spatial} & 2020  & AWGN  & A CNN model with residual spatial-adaptive blocks \\
\cline{3-6}          &       & AINDNet\cite{Kim_2020_CVPR} & 2020  & AWGN and Realistic & A CNN model based on a transfer learning scheme \\
\cline{3-6}          &       & MIRNet\cite{Zamir2020MIRNet} & 2020  & Realistic & A multi-scale model with parallel convolution streams \\
\cline{3-6}          &       & PD-denosing\cite{zhou2020awgn} & 2020  & AWGN and Realistic & A CNN model with pixel-shuffle down-sampling adaptation \\
\cline{3-6}          &       & ADRN\cite{zhao2020adrn} & 2020  & AWGN  & A deep residual network model with channel attention scheme \\
\cline{3-6}          &       & MPRNet\cite{zamir2021multi} & 2021  & Realistic & A multi-stage network with cross-stage feature fusion and attention modules \\
\cline{3-6}          &       & DRUNet\cite{zhang2021plug} & 2021  & AWGN  & A plug-and-play method with deep denoiser prior \\
\cline{3-6}          &       & DudeNet\cite{tian2021designing} & 2021  & AWGN and Realistic & A dual network with four different blocks and sparse mechanism \\
\cline{3-6}          &       & InvDN\cite{liu2021invertible} & 2021  & Realistic & An invertible denoising network with wavelet transformation \\
\cline{3-6}          &       & Restormer\cite{liu2021invertible} & 2021  & AWGN and Realistic & An efficient Transformer model with multi-head attention networks \\
\cline{3-6}          &       & DCDicL\cite{zheng2021deep} & 2021  & AWGN  & A deep convolution dictionary learning denoising network \\
\cline{3-6}          &       & NBNet\cite{cheng2021nbnet} & 2021  & AWGN and Realistic & A UNet based model that learns subspace basis and image projection \\
\cline{3-6}          &       & DeamNet\cite{ren2021adaptive} & 2021  & AWGN and Realistic & A CNN model with adaptive consistency prior and self-attention mechanism \\
\cline{3-6}          &       & PNGAN\cite{cai2021learning} & 2021  & AWGN and Realistic & A GAN based model for real image synthesis with domain alignment \\
\cline{3-6}          &       & SwinIR\cite{liang2021swinir} & 2021 & AWGN & A shifted window (Swin) Transformer model with self-attention mechanism \\
\cline{3-6}          &       & NAFNet\cite{chen2022simple} & 2022  & Realistic & A UNet based model without nonlinear activation layers \\
\cline{3-6}          &       & MalleNet\cite{jiang2022fast} & 2022  & AWGN and Realistic & A CNN with spatially-varying convolution kernels \\
\cline{3-6}          &       & Masked\cite{chen2023masked} & 2023 & AWGN and Realistic & A novel training approach that randomly masks pixels of the input image\\
\cline{3-6}          &       & SERT\cite{li2023spectral} & 2023 & AWGN, Mixed and Realistic & A Transformer framework with rectangle self-attention modeling\\
% \cline{3-6}          &       & RIDFnF & 2023  & AWGN  & A combination model denoise no-flash images with flash image pairs \\
\cline{2-6}          & \multirow{89}[22]{*}{\shortstack[l]{Self-supervised/\\Unsupervised}} & Noise2Noise\cite{lehtinen2018noise2noise} & 2018  & AWGN and Poisson & A model trained on noisy image pairs of the same scene \\
\cline{3-6}          &       & SCGAN\cite{yan2019unsupervised} & 2019  & AWGN  & Unsupervised modeling with self-consistent GAN \\
\cline{3-6}          &       & Noise2Void \cite{krull2019noise2void} & 2019  & AWGN  & A blind-spot masking strategy that excludes central pixels of the input \\
\cline{3-6}          &       & Self2Self\cite{quan2020self2self} & 2020  & AWGN and Realistic & A dropout based strategy that generates noisy pairs with the Bernoulli sampler \\
\cline{3-6}          &       & C2N\cite{jang2021c2n} & 2021  & Realistic & A GAN based model that generates real noisy images from arbitrary clean ones \\
\cline{3-6}          &       & UDVD\cite{sheth2021unsupervised} & 2021  & AWGN & An unsupervised video denoising network based on blind-spot strategy \\
\cline{3-6}          &       & R2R\cite{pang2021recorrupted} & 2021  & AWGN and Realistic & A model trained on recorrupted noisy pairs \\
\cline{3-6}          &       & Neighbor2Neighbor \cite{huang2021neighbor2neighbor} & 2021  & AWGN and Realistic & A model trained on noisy pairs generated by the downsampling strategy \\
\cline{3-6}          &       & IDR\cite{zhang2022idr} & 2022  & AWGN and Realistic & A model trained on noisy pairs with an iterative refinement strategy \\
\cline{3-6}          &       & CVF-SID\cite{neshatavar2022cvf} & 2022  & Realistic & A CNN model with a self-supervised cycle \\
\cline{3-6}          &       & Blind2Unblind\cite{wang2022blind2unblind} & 2022  & AWGN and Realistic & A blind-spot network with a global-aware mask mapper \\
\cline{3-6}          &       & AP-BSN\cite{lee2022ap} & 2022  & Realistic & A blind-spot network (BSN) with an asymmetric pixel-shuffle downsampling strategy \\
\cline{3-6}          &       & DDS2M \cite{miao2023dds2m} & 2023  & AWGN & A deep diffusion model with a variational spatio-spectral module \\
\cline{3-6}          &       & C-BSN \cite{jang2023self} & 2023  & Realistic & A conditional BSN with downsampled invariance loss \\
\cline{3-6}          &       & MM-BSN \cite{zhang2023mm} & 2023  & Realistic & A BSN method with multiple masks of different shapes \\
\cline{3-6}          &       & LGBPN \cite{wang2023lgbpn} & 2023  & Realistic & A BSN with a patch-masked convolution module and a dilated Transformer block \\
\cline{3-6}          &       & SASL \cite{li2023spatially} & 2023  & Realistic & A BSN with spatially adaptive supervision \\
    \hline
    \end{tabular}}%
  \label{Table_DNN_method}%
\end{table*}%



==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_ICVL.tex <==
%\begin{table}[htbp]
%  \centering
%  \caption{Average PSNR/SSIM of representative denoising methods under i.i.d Gaussian noise $\sigma \in \{10,20,40\}$ with ICVL dataset.}
%    \begin{tabular}{cccc}
%    \toprule
%    Methods & $\sigma = 10$    & $\sigma = 20$    & $\sigma = 40$ \\
%    \midrule
%    MSt-SVD & 46.58/0.9868 & 42.98/0.9746 & 39.32/0.9525 \\
%    \midrule
%    QRNN3D & 47.37/0.9908 & 45.08/0.9842 & 42.38/0.9731 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_ICVL}%
%\end{table}%


% Table generated by Excel2LaTeX from sheet 'ICVL'
\begin{table}[htbp]
\scriptsize
  \centering
  \caption{Average PSNR/SSIM and computational time (minutes) of MSt-SVD and QRNN3D under i.i.d Gaussian noise $\sigma \in \{10,20,40\}$ on the first 20 MSI data of ICVL dataset.}
    \begin{tabular}{ccccc}
    \toprule
    Methods & $\sigma = 10$    & $\sigma = 20$    & $\sigma = 40$    & Time (m) \\
    \midrule
    MSt-SVD & 46.58/0.9868 & 42.98/0.9746 & 39.32/0.9525 & 10.1 \\
    \midrule
    QRNN3D & \textbf{47.37/0.9908} & \textbf{45.08/0.9842} & \textbf{42.38/0.9731} & \textbf{0.16} \\
    \bottomrule
    \end{tabular}%
  \label{Table_ICVL}%
\end{table}%


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_MRI.tex <==
% Table generated by Excel2LaTeX from sheet 'All'
%\begin{table*}[htbp]
%\scriptsize
%  \centering
%  \caption{Average PSNR (left value in each cell), SSIM and computational time (s) of different methods with T1w, T2w, and PDw data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
%  \renewcommand{\arraystretch}{0.98}
%  \scalebox{0.83}{
%    \begin{tabular}{ccccccccccccc}
%    \toprule
%    $\sigma$ ($\%$) & Noisy & AONLM & ODCT  & ONLM  & PRINLM & BM4D1 & BM4D2 & NLPCA & PRI-NLPCA & ILR-HOSVD & 4DHOSVD & MSt-SVD \\
%    \midrule
%    1    & 40.0/0.971 & 41.9/0.991 & 43.3/0.992 & 41.7/0.991 & 43.3/0.993 & 43.2/0.992 & 43.4/0.992 & 44.1/0.994 & 44.3/0.994 & \textbf{44.4/0.994} & 43.9/0.993 & 44.0/0.993 \\
%    \midrule
%    3     & 30.5/0.822 & 36.5/0.971 & 36.4/0.970 & 36.4/0.969 & 36.9/0.975 & 36.6/0.972 & 37.2/0.975 & 37.7/0.977 & \textbf{38.1/0.981} & 38.0/0.978 & 37.5/0.976 & 37.5/0.975 \\
%    \midrule
%    5     & 26.1/0.676 & 33.8/0.947 & 33.6/0.949 & 33.3/0.940 & 34.0/0.955 & 33.7/0.950 & 34.6/0.959 & 33.8/0.940 & \textbf{35.3/0.967} & 35.2/0.963 & 34.6/0.959 & 34.6/0.958 \\
%    \midrule
%    7     & 23.2/0.564 & 31.9/0.921 & 31.7/0.927 & 31.2/0.911 & 32.0/0.934 & 31.8/0.926 & 32.8/0.943 & 31.9/0.912 & \textbf{33.4/0.951} & 33.4/0.948 & 32.9/0.941 & 32.8/0.940 \\
%    \midrule
%    9     & 21.0/0.479 & 30.5/0.894 & 30.2/0.905 & 29.4/0.880 & 30.5/0.911 & 30.3/0.899 & 31.5/0.928 & 31.2/0.908 & \textbf{31.9/0.934} & \textbf{32.0/0.933} & 31.5/0.922 & 31.3/0.924 \\
%    \midrule
%    11    & 19.3/0.414 & 29.3/0.865 & 29.1/0.883 & 27.8/0.847 & 29.3/0.888 & 29.2/0.873 & 30.5/0.912 & 30.0/0.883 & 30.7/0.916 & \textbf{30.9/0.917} & 30.4/0.903 & 30.2/0.906 \\
%    \midrule
%    13    & 17.8/0.361 & 28.3/0.836 & 28.1/0.861 & 26.3/0.811 & 28.2/0.864 & 28.1/0.844 & 29.6/0.895 & 29.0/0.855 & 29.6/0.898 & \textbf{29.9/0.902} & 29.4/0.883 & 29.3/0.888 \\
%    \midrule
%    15    & 16.6/0.319 & 27.4/0.807 & 27.3/0.840 & 24.9/0.771 & 27.4/0.841 & 27.3/0.814 & 28.8/0.879 & 28.1/0.826 & 28.8/0.879 & \textbf{29.1/0.886} & 28.6/0.863 & 28.5/0.871 \\
%    \midrule
%    17    & 15.5/0.284 & 26.5/0.775 & 26.5/0.820 & 23.4/0.729 & 26.6/0.817 & 26.5/0.785 & \textbf{28.1/0.862} & 27.3/0.798 & 28.0/0.860 & 27.7/0.838 & 27.8/0.842 & 27.7/0.853 \\
%    \midrule
%    19    & 14.6/0.254 & 25.7/0.744 & 25.8/0.799 & 22.0/0.684 & 25.9/0.797 & 25.7/0.755 & \textbf{27.4/0.845} & 26.6/0.772 & 27.3/0.841 & 27.0/0.819 & 27.1/0.822 & 27.1/0.835 \\
%    \midrule
%    Implementation & /     & Mex   & Mex   & Mex   & Mex   & Mex   & Mex   & MATLAB & MEX   & MATLAB & MATLAB & MEX \\
%    \midrule
%    Time (s) & /     & 868.1 & \textbf{10.5}  & 139.9 & 18.6  & 69.9  & 211.3 & 638.8 & 868.9 & 1896.3 & 706.9 & 99.6 \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_MRI}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'All'
\begin{table*}[htbp]
\scriptsize
  \centering
  \caption{Average PSNR/SSIM and computational time (s) of different methods with T1w, T2w, and PDw data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
  \renewcommand{\arraystretch}{0.99}
  \scalebox{0.839}{
    \begin{tabular}{ccccccccccccc}
    \toprule
    $\sigma (\%)$ & Noisy & ONLM  & AONLM & ODCT  & PRINLM & BM4D1 & BM4D2 & NLPCA & PRI-NLPCA & ILR-HOSVD & 4DHOSVD & MSt-SVD \\
    \midrule
    1     & 40.0/0.971 & 41.7/0.991 & 41.9/0.991 & 43.3/0.992 & 43.3/0.993 & 43.2/0.992 & 43.4/0.992 & 44.1/0.994 & 44.3/0.994 & \textbf{44.4/0.994} & 43.9/0.993 & 44.0/0.993 \\
    \midrule
    3     & 30.5/0.822 & 36.4/0.969 & 36.5/0.971 & 36.4/0.970 & 36.9/0.975 & 36.6/0.972 & 37.2/0.975 & 37.7/0.977 & \textbf{38.1/0.981} & 38.0/0.978 & 37.5/0.976 & 37.5/0.975 \\
    \midrule
    5     & 26.1/0.676 & 33.3/0.940 & 33.8/0.947 & 33.6/0.949 & 34.0/0.955 & 33.7/0.950 & 34.6/0.959 & 33.8/0.940 & \textbf{35.3/0.967} & 35.2/0.963 & 34.6/0.959 & 34.6/0.958 \\
    \midrule
    7     & 23.2/0.564 & 31.2/0.911 & 31.9/0.921 & 31.7/0.927 & 32.0/0.934 & 31.8/0.926 & 32.8/0.943 & 31.9/0.912 & \textbf{33.4/0.951} & 33.4/0.948 & 32.9/0.941 & 32.8/0.940 \\
    \midrule
    9     & 21.0/0.479 & 29.4/0.880 & 30.5/0.894 & 30.2/0.905 & 30.5/0.911 & 30.3/0.899 & 31.5/0.928 & 31.2/0.908 & \textbf{31.9/0.934} & \textbf{32.0/0.933} & 31.5/0.922 & 31.3/0.924 \\
    \midrule
    11    & 19.3/0.414 & 27.8/0.847 & 29.3/0.865 & 29.1/0.883 & 29.3/0.888 & 29.2/0.873 & 30.5/0.912 & 30.0/0.883 & 30.7/0.916 & \textbf{30.9/0.917} & 30.4/0.903 & 30.2/0.906 \\
    \midrule
    13    & 17.8/0.361 & 26.3/0.811 & 28.3/0.836 & 28.1/0.861 & 28.2/0.864 & 28.1/0.844 & 29.6/0.895 & 29.0/0.855 & 29.6/0.898 & \textbf{29.9/0.902} & 29.4/0.883 & 29.3/0.888 \\
    \midrule
    15    & 16.6/0.319 & 24.9/0.771 & 27.4/0.807 & 27.3/0.840 & 27.4/0.841 & 27.3/0.814 & 28.8/0.879 & 28.1/0.826 & 28.8/0.879 & \textbf{29.1/0.886} & 28.6/0.863 & 28.5/0.871 \\
    \midrule
    17    & 15.5/0.284 & 23.4/0.729 & 26.5/0.775 & 26.5/0.820 & 26.6/0.817 & 26.5/0.785 & \textbf{28.1/0.862} & 27.3/0.798 & 28.0/0.860 & 27.7/0.838 & 27.8/0.842 & 27.7/0.853 \\
    \midrule
    19    & 14.6/0.254 & 22.0/0.684 & 25.7/0.744 & 25.8/0.799 & 25.9/0.797 & 25.7/0.755 & \textbf{27.4/0.845} & 26.6/0.772 & 27.3/0.841 & 27.0/0.819 & 27.1/0.822 & 27.1/0.835 \\
    \midrule
    Implementation & /     & Mex   & Mex   & Mex   & Mex   & Mex   & Mex   & MATLAB & MEX   & MATLAB & MATLAB & MEX \\
    \midrule
    Time (s) & /     & 139.9 & 868.1 & \textbf{10.5} & 18.6  & 69.9  & 211.3 & 638.8 & 868.9 & 1896.3 & 706.9 & 99.6 \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_MRI}%
\end{table*}%



==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_Method_all.tex <==
%\begin{table*}
%\scriptsize
%\centering
%\caption{aa}
%\scalebox{0.88}{
%\renewcommand{\arraystretch}{1.02}
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%Category                      & Representation           & Methods       & Noise Modeling Experiments      & Applications     & Key Words                                                     \\
%\hline
%\multirow{41}{*}{Traditional} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color, othman2006noise}           & AWGN                            & CI, MSI          & Adaptive wavelet thresholding with thresholding techniques    \\
%\cline{3-6}
%                              &                          & NLM \cite{buades2005review, dai2013multichannel}          & AWGN                            & CI               & NLM algorithm with Gaussian kernels                           \\
%\cline{3-6}
%                              &                          & WSM \cite{coupe20083d}          & AWGN                            & MRI              & 3D wavelet subbands mixing for image denoising                \\
%\cline{3-6}
%                              &                          & TCVD \cite{liu2010high}         & AWGN                            & CV               & Integration of robust optical flow into NLM                   \\
%\cline{3-6}
%                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                            & CI, MRI          & Applications of SVD decomposition                             \\
%\cline{3-6}
%                              &                          & LRMR \cite{zhang2013hyperspectral}          & AWGN                            & MRI              & A low-rank matrix decomposition model                         \\
%\cline{3-6}
%                              &                          & GID \cite{xu2018external}          & AWGN                            & CI               & External data guided and internal prior learning              \\
%\cline{3-6}
%                              &                          & SPTWO \cite{buades2016patch}        & AWGN                            & CV               & NLPCA with optical flow estimation                            \\
%\cline{3-6}
%                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                            & CI, MSI          & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                            & CV               & Efficient approximate global patch search                     \\
%\cline{3-6}
%                              &                          & MCWNNM \cite{xu2017multi}       & AWGN                            & CI               & Extension of WNNM to color images                             \\
%\cline{3-6}
%                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                            & CV               & ~A trilateral weighted sparse coding scheme                   \\
%\cline{3-6}
%                              &                          & NLH\_CC \cite{hou2020nlh}      & AWGN                            & CI               & Nonlocal pixel similarity with Haar transform                 \\
%\cline{3-6}
%                              &                          & AMF \cite{chan2005salt}          & Impulsive                       & CI               & Impulsive noise removal by adaptive median filter             \\
%\cline{3-6}
%                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                       & CI               & Impulsive noise removal by iterative adaptive fuzzy filter    \\
%\cline{3-6}
%                              &                          & LSM-NLR \cite{huang2017mixed}      & Gaussian, Poisson and Impulsive & CV               & Low-rank with laplacian scale mixture modeling                \\
%\cline{3-6}
%                              &                          & FastHyde \cite{zhuang2018fast}     & Gaussian and Poisson        & MSI              & Low-rank and sparse representation                            \\
%\cline{3-6}
%                              &                          & NMoG \cite{chen2017denoising}         & Gaussian, Stripe and Impulsive  & MSI              & Low-rank matrix model with non i.i.d Gaussian noise           \\
%\cline{3-6}
%                              &                          & ODCT \cite{manjon2012new}         & AWGN and Rician                 & MRI              & A 3D DCT implementation                                       \\
%\cline{3-6}
%                              &                          & OBNLM \cite{coupe2008optimized}        & AWGN and Rician                 & MRI              & An optimized blockwise NLM Filter                             \\
%\cline{3-6}
%                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician                 & MRI              & Adaptive NLM with spatially varying noise levels              \\
%\cline{3-6}
%                              &                          & RLMMSE \cite{aja2008noise}       & Rician                          & MRI              & A novel linear minimum mean square error (LMMSE) estimator    \\
%\cline{3-6}
%                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician                 & MRI              & A rotationally invariant version of the NLM filter            \\
%\cline{3-6}
%                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician                 & MRI              & A two stage filter based on NLPCA and PRI-NLM                 \\
%\cline{2-6}
%                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                            & CI               & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}       & AWGN                            & CV               & Extention of CBM3D to color videos                            \\
%\cline{3-6}
%                              &                          & LRTA \cite{renard2008denoising}         & AWGN                            & MSI              & A low Tucker rank tensor decomposition  model                 \\
%\cline{3-6}
%                              &                          & PARAFAC \cite{liu2012denoising}      & AWGN                            & MSI              & A rank-one CP decomposition model                             \\
%\cline{3-6}
%                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                            & CV               & Extention of BM3D to color videos using 3D patch              \\
%\cline{3-6}
%                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                            & MSI, MRI         & Extention of BM4D to MSI and MRI using 3D patch               \\
%\cline{3-6}
%                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising}      & AWGN                            & CI, MSI, MRI     & Applications of 4DHOSVD transform                             \\
%\cline{3-6}
%                              &                          & TDL \cite{peng2014decomposable}           & AWGN                            & MSI              & A Tucker based tensor dictionary learning algorithm           \\
%\cline{3-6}
%                              &                          & KTSVD \cite{Zhang2015KTSVD}        & AWGN                            & MSI              & A t-SVD based tensor dictionary learning algorithm            \\
%\cline{3-6}
%                              &                          & ITSReg \cite{xie2016multispectral}       & AWGN                            & MSI              & Intrinsic Tensor Sparsity Regularization                      \\
%\cline{3-6}
%                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                            & MSI              & Low Tucker rank decomposition with total variation            \\
%\cline{3-6}
%                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                            & CI               & A weighted rank-one CP decomposition model                    \\
%\cline{3-6}
%                              &                          & HOSVDR\_S \cite{lv2019denoising}    & AWGN                            & MRI              & A recursive low Tucker rank model with rank estimation        \\
%\cline{3-6}
%                              &                          & MSt-SVD \cite{kong2017new, kong2019color}      & AWGN                            & CI, CV, MRI, MSI & An efficient one-stage multi-diemsional t-SVD implementation  \\
%\cline{3-6}
%                              &                          & NGMeet \cite{he2019non}        & AWGN                            & MSI              & Low-rank tensor model with iterative regularization           \\
%\cline{3-6}
%                              &                          & LTDL \cite{gong2020low}         & AWGN                            & MSI              & A low-rank tensor dictionary learning method                  \\
%\cline{3-6}
%                              &                          & NLTA-LSM \cite{dong2015low}     & Gaussian and Poisson         & MSI, MRI         & Low Tucker rank with laplacian scale mixture modeling         \\
%\hline
%\end{tabular}
%}
%\end{table*}

% \usepackage{multirow}

\begin{table*}[htbp]
\scriptsize
\centering
\caption{Related multi-dimensional image denoising methods with different noise modeling techniques and applications. 'CI': color image, 'CV': color video, 'MSI': multispectral imaging, 'MRI': magnetic resonance imaging.}
\scalebox{0.84}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Category}                      & \textbf{Representation}           & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                     \\
\hline
\multirow{41}{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color,othman2006noise}           & AWGN                        & CI, MSI, HSI      & Adaptive wavelet thresholding with thresholding techniques    \\
\cline{3-6}
                              &                          & DCT \cite{yaroslavsky1996local, foi2007pointwise}           & AWGN                        & CI                & high-quality denoising with discrete cosine transform (DCT)   \\
\cline{3-6}
                              &                          & NLM \cite{buades2005review, dai2013multichannel}           & AWGN                        & CI                & NLM algorithm with Gaussian kernels                           \\
\cline{3-6}
                              &                          & WSM \cite{coupe20083d}           & AWGN                        & MRI               & 3D wavelet subbands mixing for image denoising                \\
\cline{3-6}
                              &                          & K-SVD \cite{mairal2007sparse, fu2015adaptive}           & AWGN                        & CI, MSI               & 3D wavelet over-complete dictionary learning and sparse coding                \\
\cline{3-6}
                              &                          & TCVD \cite{liu2010high}         & AWGN                        & CV                & Integration of robust optical flow into NLM                   \\
\cline{3-6}
                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                        & CI, MRI           & Applications of SVD decomposition                             \\
\cline{3-6}
                              &                          & EPLL \cite{zoran2011learning, hurault2018epll}           & AWGN                        & CI                & A Bayesian patch-based method for whole image restoration                          \\
\cline{3-6}
                              &                          & LRMR \cite{zhang2013hyperspectral}         & AWGN                        & MRI               & A low-rank matrix decomposition model                         \\
\cline{3-6}
                              &                          & GID \cite{xu2018external}          & AWGN                        & CI                & External data guided and internal prior learning              \\
\cline{3-6}
                              &                          & SPTWO \cite{buades2016patch}         & AWGN                        & CV                & NLPCA with optical flow estimation                            \\
\cline{3-6}
                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                        & CI, MSI, HSI      & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                        & CV                & Efficient approximate global patch search                     \\
\cline{3-6}
                              &                          & MCWNNM \cite{xu2017multi}        & AWGN                        & CI                & Extension of WNNM to color images                             \\
\cline{3-6}
                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                        & CI              & A trilateral weighted sparse coding scheme                   \\
\cline{3-6}
                              &                          & VNLB \cite{arias2018video}         & AWGN                        & CV                & A patch-based Bayesian model for video denoising                   \\
\cline{3-6}
                              &                          & NLH \cite{hou2020nlh}      & AWGN                        & CI                & Nonlocal pixel similarity with Haar transform                 \\
\cline{3-6}
                              &                          & AMF \cite{chan2005salt}          & Impulsive                   & CI                & Impulsive noise removal by adaptive median filter             \\
\cline{3-6}
                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                   & CI                & Impulsive noise removal by iterative adaptive fuzzy filter    \\
\cline{3-6}
                              &                          & NoiseClinic \cite{lebrun2015multiscale}         & AWGN and Realistic                   & CI                & A multiscale blind Bayes denoising algorithm    \\
\cline{3-6}
                              &                          & LSM-NLR \cite{huang2017mixed}      & AWGN, Poisson and Impulsive & CV                & Low-rank with laplacian scale mixture modeling                \\
\cline{3-6}
                              &                          & FastHyde \cite{zhuang2018fast}     & AWGN and Poisson            & MSI, HSI          & Low-rank and sparse representation                            \\
\cline{3-6}
                              &                          & NMoG \cite{chen2017denoising}         & AWGN, Stripe and Impulsive  & MSI, HSI          & Low-rank matrix model with non i.i.d Gaussian noise           \\
\cline{3-6}
                              &                          & ODCT \cite{manjon2012new}          & AWGN and Rician             & MRI               & A 3D DCT implementation                                       \\
\cline{3-6}
                              &                          & OBNLM \cite{coupe2008optimized}         & AWGN and Rician             & MRI               & An optimized blockwise NLM Filter                             \\
\cline{3-6}
                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician             & MRI               & Adaptive NLM with spatially varying noise levels              \\
\cline{3-6}
                              &                          & RLMMSE \cite{aja2008noise}       & Rician                      & MRI               & A novel linear minimum mean square error (LMMSE) estimator    \\
\cline{3-6}
                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician             & MRI               & A rotationally invariant version of the NLM filter            \\
\cline{3-6}
                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician             & MRI               & A two stage filter based on NLPCA and PRI-NLM                 \\
\cline{2-6}
                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                        & CI, CV                & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}        & AWGN                        & CV                & Extention of CBM3D to color videos                            \\
\cline{3-6}
                              &                          & LRTA \cite{renard2008denoising}         & AWGN                        & MSI, HSI          & A low Tucker rank tensor decomposition  model                 \\
\cline{3-6}
                              &                          & PARAFAC \cite{liu2012denoising}       & AWGN                        & MSI               & A rank-one CP decomposition model                             \\
\cline{3-6}
                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                        & CV                & Extention of BM3D to color videos using 3D patch              \\
\cline{3-6}
                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                        & MSI, HSI, MRI     & Extention of BM4D to MSI and MRI using 3D patch               \\
\cline{3-6}
                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising, zhang2017denoise}      & AWGN                        & CI, MSI, HSI, MRI & Applications of 4DHOSVD transform                             \\
\cline{3-6}
                              &                          & TDL \cite{peng2014decomposable}           & AWGN                        & MSI, HSI          & A Tucker based tensor dictionary learning algorithm           \\
\cline{3-6}
                              &                          & KTSVD \cite{Zhang2015KTSVD}         & AWGN                        & MSI, HSI          & A t-SVD based tensor dictionary learning algorithm            \\
\cline{3-6}
                              &                          & LRTV \cite{he2015total}         & AWGN                        & MSI, HSI          & Low-rank model with total variation (TV) regularization            \\
\cline{3-6}
                              &                          & ITSReg \cite{xie2016multispectral}        & AWGN                        & MSI, HSI          & Intrinsic Tensor Sparsity Regularization                      \\
\cline{3-6}
                              &                          & LLRT \cite{chang2017hyper}        & AWGN                        & CI, MSI          & low-rank tensor with hyper-laplacian regularization                      \\
\cline{3-6}
                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                        & MSI, HSI          & Low Tucker rank decomposition with total variation            \\
\cline{3-6}
                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                        & CI                & A weighted rank-one CP decomposition model                    \\
\cline{3-6}
                              &                          & ILR-HOSVD \cite{lv2019denoising}    & AWGN                        & MRI               & A recursive low Tucker rank model with rank estimation        \\
\cline{3-6}
                              &                          & MSt-SVD \cite{kong2017new, kong2019color}       & AWGN                        & CI, MRI, MSI, HSI & An efficient one-stage t-SVD implementation  \\
\cline{3-6}
                              &                          & NGMeet \cite{he2019non}       & AWGN                        & MSI, HSI          & Low-rank tensor model with iterative regularization           \\
\cline{3-6}
                              &                          & LTDL \cite{gong2020low}         & AWGN                        & MSI, HSI          & A low-rank tensor dictionary learning method                  \\
\cline{3-6}
                              &                          & NLTA-LSM \cite{dong2015low}      & AWGN and Poisson            & MSI, HSI, MRI     & Low Tucker rank with laplacian scale mixture modeling         \\
\hline
\textbf{Category}                      & \textbf{Network  Architectures}   & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                  \\
\hline
\multirow{32}{*}{\shortstack[l]{DNN \\ methods}}         & \multirow{22}{*}{CNN}    & DnCNN \cite{zhang2017beyond, jiang2018denoising}       & AWGN                        & CI, MRI           & Residual learning and batch normalization                     \\
\cline{3-6}
                              &                          & NLNet \cite{lefkimmiatis2017non}         & AWGN                        & CI                & A nonlocal CNN model                                          \\
\cline{3-6}
                              &                          & UDNet \cite{Lefkimmiatis_2018_CVPR}        & AWGN                        & CI                & A robust and flexible CNN model                               \\
\cline{3-6}
                              &                          & FFDNet \cite{zhang2018ffdnet}       & AWGN                        & CI                & A flexible model with tunable input noise levels              \\
\cline{3-6}
                              &                          & HSID-CNN \cite{yuan2018hyperspectral}      & AWGN                        & MSI, HSI          & A 2D and 3D combined CNN model                                \\
\cline{3-6}
                              &                          & HSI-SDeCNN \cite{maffei2019single}    & AWGN                        & MSI, HSI          & A single CNN model with spatial and spectral information      \\
\cline{3-6}
                              &                          & VNLNet \cite{davy2018non}       & AWGN                        & CV                & The first nonlocal CNN model for video                        \\
\cline{3-6}
                              &                          & ViDeNN \cite{claus2019videnn}       & AWGN                        & CV                & Combination of spatial and temporal filtering with CNN        \\
\cline{3-6}
                              &                          & SADNet \cite{chang2020spatial}        & AWGN                        & CI                & A novel spatial-adaptive CNN model                            \\
\cline{3-6}
                              &                          & FastDVDNet \cite{Tassano_2020_CVPR}   & AWGN                        & CV                & A real-time method without flow estimation                    \\
\cline{3-6}
                              &                          & LIDIA \cite{Vaksman_2020_CVPR_Workshops}        & AWGN                        & CI                & A lightweight denoiser with instance adaptation               \\
\cline{3-6}
                              &                          & DRUNet \cite{zhang2020plug}     & AWGN                   & CI                & A plug-and-play method with deep denoiser prior     \\
\cline{3-6}
                              &                          & HSI-DeNet \cite{chang2018hsi}    & AWGN and Strip              & MSI, HSI          & A CNN method with mixed noise modeling                        \\
\cline{3-6}
                              &                          & Noise2noise \cite{lehtinen2018noise2noise}       & AWGN and Poisson                     & CI              & A CNN model trained only with noisy data.                         \\
\cline{3-6}
                              &                          & VDNet \cite{yue2019variational}        & AWGN and Realistic          & CI                & A variational inference method with noise estimation          \\
\cline{3-6}
                              &                          & CBDNet \cite{guo2019toward}       & Realistic                   & CI                & a convolutional blind denoising network                       \\
\cline{3-6}
                              &                          & PRI-PB-CNN \cite{manjon2018mri}   & AWGN an Rician              & MRI               & Combination of sliding window scheme and 3D CNN               \\
\cline{3-6}
                              &                          & DIDN \cite{yu2019deep}         & AWGN and Realistic          & CI                & A deep iterative down-up CNN model                            \\
\cline{3-6}
                              &                          & DRDN \cite{song2019dynamic}         & Realistic                   & CI                & A dynamic residual dense network model                        \\
\cline{3-6}
                              &                          & FCCF \cite{yue2019high}         & AWGN and Realistic          & CI                & Fusion of collaborative filtering and CNN                     \\
\cline{3-6}
                              &                          & DBF \cite{chen2019real}          & AWGN and Realistic          & CI                & Integration of CNN into a boosting algorithm                    \\
\cline{3-6}
                              &                          & RIDNet \cite{anwar2019real}       & AWGN and Realistic          & CI                & A single stage model with feature attention                   \\
\cline{3-6}
                              &                          & AINDNet \cite{Kim_2020_CVPR}      & AWGN and Realistic          & CI                & Transfer learning with adaptive instance normalization        \\
\cline{3-6}
                              &                          & QRNN3D \cite{wei20203}          & AWGN and Stripe                   & MSI, HSI                & A deep recurrent neural network model with 3D convolution           \\
\cline{3-6}
                              &                          & CycleISP \cite{zamir2020cycleisp}     & Realistic                   & CI                & A camera pipeline model in forward and reverse directions     \\
\cline{3-6}
                              &                          & MIRNet \cite{Zamir2020MIRNet}        & Realistic                   & CI                & A multi-scale model with parallel convolution streams                   \\
\cline{2-6}
                              & \multirow{10}{*}{Others} & MLP \cite{burger2012image}          & AWGN                        & CI                & A multilayer perceptron model                                 \\
\cline{3-6}
                              &                          & TNRD \cite{chen2016trainable}         & AWGN                        & CI                & A trainable nonlinear difussion model                         \\
\cline{3-6}
                              &                          & SCGAN \cite{yan2019unsupervised}        & AWGN                        & CI                & Unsupervised modeling with self-consistent GAN                \\
\cline{3-6}
                              &                          & ADRN \cite{zhao2020adrn}          & AWGN                   & MSI, HSI                & A deep residual network model with channel attention scheme            \\
%\cline{3-6}
%                              &                          & LLRefineNet \cite{jiang2018deep}  & AWGN and Impulsive          & CI                & Encoder-decoder network with skip connections                 \\
\cline{3-6}
                              &                          & GCBD \cite{Chen_2018_CVPR}         & AWGN and Realistic          & CI                & A GAN-based blind denoiser                               \\
\cline{3-6}
                              &                          & DnGAN \cite{yeh2018image}        & AWGN and Blur               & CI                & GAN with  maximum a posteriori (MAP) framework                \\
\cline{3-6}
                              &                          & RED-WGAN \cite{ran2019denoising}     & AWGN and Rician             & MRI               & A residual encoder decoder Wasserstein GAN model              \\
\cline{3-6}
                              &                          & ADGAN \cite{Lin_2019_CVPR_Workshops}        & Realistic                   & CI                & Attentive GAN with noise domain adaptation                    \\
\cline{3-6}
                              &                          & MIFCN \cite{abbasi2019three}        & Realistic                   & MRI               & A fully convolutional network model                           \\
\cline{3-6}
                              &                          & SGN \cite{gu2019self}          & Realistic                   & CI                & A self-guided network with top-down architecture              \\
\cline{3-6}
                              &                          & DANet \cite{yue2020dual}        & Realistic                   & CI                & A Bayesian framework for noise removal and generation.                    \\
\hline
\end{tabular}
}
\label{Table_Method_all}
\end{table*}



==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_Method_all_new.tex <==
\begin{table*}[htbp]
\scriptsize
\centering
\caption{Related multi-dimensional image denoising methods with different noise modeling techniques and applications. 'CI': color image, 'CV': color video, 'MSI': multispectral imaging, 'HSI': hyperspectral imaging, 'MRI': magnetic resonance imaging.}
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Category}                      & \textbf{Representation}           & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                     \\
\hline
\multirow{41}{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color,othman2006noise}           & AWGN                        & CI, MSI, HSI      & Adaptive wavelet thresholding with thresholding techniques    \\
\cline{3-6}
                              &                          & DCT \cite{yaroslavsky1996local, foi2007pointwise}           & AWGN                        & CI                & high-quality denoising with discrete cosine transform (DCT)   \\
\cline{3-6}
                              &                          & NLM \cite{buades2005review, dai2013multichannel}           & AWGN                        & CI                & NLM algorithm with Gaussian kernels                           \\
\cline{3-6}
                              &                          & K-SVD \cite{mairal2007sparse, fu2015adaptive}           & AWGN                        & CI, MSI               & 3D wavelet over-complete dictionary learning and sparse coding                \\
\cline{3-6}
                              &                          & TCVD \cite{liu2010high}         & AWGN                        & CV                & Combination of robust optical flow with NLM                   \\
\cline{3-6}
                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                        & CI, MRI           & Applications of SVD decomposition                             \\
\cline{3-6}
                              &                          & EPLL \cite{zoran2011learning, hurault2018epll}           & AWGN                        & CI                & A Bayesian patch-based method for whole image restoration                          \\
\cline{3-6}
                              &                          & LRMR \cite{zhang2013hyperspectral}         & AWGN                        & MRI               & A low-rank matrix decomposition model                         \\
\cline{3-6}
                              &                          & GID \cite{xu2018external}          & AWGN                        & CI                & External data guided and internal prior learning              \\
\cline{3-6}
                              &                          & SPTWO \cite{buades2016patch}         & AWGN                        & CV                & NLPCA with optical flow estimation                            \\
\cline{3-6}
                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                        & CI, MSI, HSI      & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                        & CV                & Efficient approximate global patch search                     \\
\cline{3-6}
                              &                          & MCWNNM \cite{xu2017multi}        & AWGN                        & CI                & Extension of WNNM to color images                             \\
\cline{3-6}
                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                        & CI              & A trilateral weighted sparse coding scheme                   \\
\cline{3-6}
                              &                          & VNLB \cite{arias2018video}         & AWGN                        & CV                & A patch-based Bayesian model for video denoising                   \\
\cline{3-6}
                              &                          & NLH \cite{hou2020nlh}      & AWGN                        & CI                & Nonlocal pixel similarity with Haar transform                 \\
\cline{3-6}
                              &                          & AMF \cite{chan2005salt}          & Impulsive                   & CI                & Impulsive noise removal by adaptive median filter             \\
%\cline{3-6}
%                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                   & CI                & Impulsive noise removal by iterative adaptive fuzzy filter    \\
\cline{3-6}
                              &                          & NoiseClinic \cite{lebrun2015multiscale}         & AWGN and Realistic                   & CI                & A multiscale blind Bayes denoising algorithm    \\
\cline{3-6}
                              &                          & LSM-NLR \cite{huang2017mixed}      & AWGN, Poisson and Impulsive & CV                & Low-rank with laplacian scale mixture modeling                \\
\cline{3-6}
                              &                          & FastHyde \cite{zhuang2018fast}     & AWGN and Poisson            & MSI, HSI          & Low-rank and sparse representation                            \\
\cline{3-6}
                              &                          & NMoG \cite{chen2017denoising}         & AWGN, Stripe and Impulsive  & MSI, HSI          & Low-rank matrix model with non i.i.d Gaussian noise           \\
\cline{3-6}
                              &                          & ODCT \cite{manjon2012new}          & AWGN and Rician             & MRI               & A 3D DCT implementation                                       \\
\cline{3-6}
                              &                          & OBNLM \cite{coupe2008optimized}         & AWGN and Rician             & MRI               & An optimized blockwise NLM Filter                             \\
\cline{3-6}
                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician             & MRI               & Adaptive NLM with spatially varying noise levels              \\
\cline{3-6}
                              &                          & RLMMSE \cite{aja2008noise}       & Rician                      & MRI               & A novel linear minimum mean square error (LMMSE) estimator    \\
\cline{3-6}
                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician             & MRI               & A rotationally invariant version of the NLM filter            \\
\cline{3-6}
                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician             & MRI               & A two stage filter based on NLPCA and PRI-NLM                 \\
\cline{2-6}
                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                        & CI, CV                & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}        & AWGN                        & CV                & Extention of CBM3D to color videos                            \\
\cline{3-6}
                              &                          & LRTA \cite{renard2008denoising}         & AWGN                        & MSI, HSI          & A low Tucker rank tensor decomposition  model                 \\
\cline{3-6}
                              &                          & PARAFAC \cite{liu2012denoising}       & AWGN                        & MSI               & A rank-one CP decomposition model                             \\
\cline{3-6}
                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                        & CV                & Extention of BM3D to color videos using 3D patch              \\
\cline{3-6}
                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                        & MSI, HSI, MRI     & Extention of BM4D to MSI and MRI using 3D patch               \\
\cline{3-6}
                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising, zhang2017denoise}      & AWGN                        & CI, MSI, HSI, MRI & Applications of 4DHOSVD transform                             \\
\cline{3-6}
                              &                          & TDL \cite{peng2014decomposable}           & AWGN                        & MSI, HSI          & A Tucker based tensor dictionary learning algorithm           \\
\cline{3-6}
                              &                          & KTSVD \cite{Zhang2015KTSVD}         & AWGN                        & MSI, HSI          & A t-SVD based tensor dictionary learning algorithm            \\
\cline{3-6}
                              &                          & LRTV \cite{he2015total}         & AWGN                        & MSI, HSI          & Low-rank model with total variation (TV) regularization            \\
\cline{3-6}
                              &                          & ITSReg \cite{xie2016multispectral}        & AWGN                        & MSI, HSI          & Intrinsic Tensor Sparsity Regularization                      \\
\cline{3-6}
                              &                          & LLRT \cite{chang2017hyper}        & AWGN                        & CI, MSI          & low-rank tensor with hyper-laplacian regularization                      \\
\cline{3-6}
                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                        & MSI, HSI          & Low Tucker rank decomposition with total variation            \\
\cline{3-6}
                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                        & CI                & A weighted rank-one CP decomposition model                    \\
\cline{3-6}
                              &                          & ILR-HOSVD \cite{lv2019denoising}    & AWGN                        & MRI               & A recursive low Tucker rank model with rank estimation        \\
\cline{3-6}
                              &                          & MSt-SVD \cite{kong2017new, kong2019color}       & AWGN                        & CI, MRI, MSI, HSI & An efficient one-stage t-SVD implementation  \\
\cline{3-6}
                              &                          & NGMeet \cite{he2019non}       & AWGN                        & MSI, HSI          & Low-rank tensor model with iterative regularization           \\
\cline{3-6}
                              &                          & LTDL \cite{gong2020low}         & AWGN                        & MSI, HSI          & A low-rank tensor dictionary learning method                  \\
\cline{3-6}
                              &                          & NLTA-LSM \cite{dong2015low}      & AWGN and Poisson            & MSI, HSI, MRI     & Low Tucker rank with laplacian scale mixture modeling         \\
\hline
\textbf{Category}                      & \textbf{Network  Architectures}   & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                  \\
\hline
\multirow{32}{*}{\shortstack[l]{DNN \\ methods}}         & \multirow{29}{*}{CNN/NN}   & MLP \cite{burger2012image}          & AWGN                        & CI                & A multilayer perceptron model                                 \\

\cline{3-6}
                              &                          & TNRD \cite{chen2016trainable}         & AWGN                        & CI                & A trainable nonlinear difussion model                         \\
\cline{3-6}
                              &                          & DnCNN \cite{zhang2017beyond, jiang2018denoising}          & AWGN                        & CI, MRI                 & CNN with Residual learning and batch normalization                       \\
\cline{3-6}
                              &                          & NLNet \cite{lefkimmiatis2017non}         & AWGN                        & CI                & A nonlocal CNN model                                          \\
\cline{3-6}
                              &                          & UDNet \cite{Lefkimmiatis_2018_CVPR}        & AWGN                        & CI                & A robust and flexible CNN model                               \\
\cline{3-6}
                              &                          & FFDNet \cite{zhang2018ffdnet}       & AWGN                        & CI                & A flexible model with tunable input noise levels              \\
\cline{3-6}
                              &                          & HSID-CNN \cite{yuan2018hyperspectral}      & AWGN                        & MSI, HSI          & A 2D and 3D combined CNN model                                \\
\cline{3-6}
                              &                          & HSI-SDeCNN \cite{maffei2019single}    & AWGN                        & MSI, HSI          & A single CNN model with spatial and spectral information      \\
\cline{3-6}
                              &                          & VNLNet \cite{davy2018non}       & AWGN                        & CV                & The first nonlocal CNN model for video                        \\
\cline{3-6}
                              &                          & ViDeNN \cite{claus2019videnn}       & AWGN                        & CV                & Combination of spatial and temporal filtering with CNN        \\
\cline{3-6}
                              &                          & SADNet \cite{chang2020spatial}        & AWGN                        & CI                & A novel spatial-adaptive CNN model                            \\
\cline{3-6}
                              &                          & FastDVDNet \cite{Tassano_2020_CVPR}   & AWGN                        & CV                & A real-time method without flow estimation                    \\
\cline{3-6}
                              &                          & LIDIA \cite{Vaksman_2020_CVPR_Workshops}        & AWGN                        & CI                & A lightweight denoiser with instance adaptation               \\
\cline{3-6}
                              &                          & DRUNet \cite{zhang2020plug}     & AWGN                   & CI                & A plug-and-play method with deep denoiser prior     \\
\cline{3-6}
                              &                          & ADRN \cite{zhao2020adrn}          & AWGN                   & MSI, HSI                & A deep residual network model with channel attention scheme            \\
\cline{3-6}
                              &                          & HSI-DeNet \cite{chang2018hsi}    & AWGN and Strip              & MSI, HSI          & A CNN method with mixed noise modeling                        \\
\cline{3-6}
                              &                          & Noise2noise \cite{lehtinen2018noise2noise}       & AWGN and Poisson                     & CI              & A CNN model trained only with noisy data.                         \\
\cline{3-6}
                              &                          & VDNet \cite{yue2019variational}        & AWGN and Realistic          & CI                & A variational inference method with noise estimation          \\
\cline{3-6}
                              &                          & CBDNet \cite{guo2019toward}       & Realistic                   & CI                & a convolutional blind denoising network                       \\
\cline{3-6}
                              &                          & PRI-PB-CNN \cite{manjon2018mri}   & AWGN an Rician              & MRI               & Combination of sliding window scheme and 3D CNN               \\
\cline{3-6}
                              &                          & MIFCN \cite{abbasi2019three}        & Realistic                   & MRI               & A fully convolutional network model                           \\
\cline{3-6}
                              &                          & DIDN \cite{yu2019deep}         & AWGN and Realistic          & CI                & A deep iterative down-up CNN model                            \\
\cline{3-6}
                              &                          & DRDN \cite{song2019dynamic}         & Realistic                   & CI                & A dynamic residual dense network model                        \\
\cline{3-6}
                              &                          & FCCF \cite{yue2019high}         & AWGN and Realistic          & CI                & Fusion of collaborative filtering and CNN                     \\
\cline{3-6}
                              &                          & DBF \cite{chen2019real}          & AWGN and Realistic          & CI                & Integration of CNN into a boosting algorithm                    \\
\cline{3-6}
                              &                          & RIDNet \cite{anwar2019real}       & AWGN and Realistic          & CI                & A single stage model with feature attention                   \\
\cline{3-6}
                              &                          & AINDNet \cite{Kim_2020_CVPR}      & AWGN and Realistic          & CI                & Transfer learning with adaptive instance normalization        \\
\cline{3-6}
                              &                          & QRNN3D \cite{wei20203}          & AWGN and Stripe                   & MSI, HSI                & A deep recurrent neural network model with 3D convolution           \\
\cline{3-6}
                              &                          & CycleISP \cite{zamir2020cycleisp}     & Realistic                   & CI                & A camera pipeline model in forward and reverse directions     \\
\cline{3-6}
                              &                          & MIRNet \cite{Zamir2020MIRNet}        & Realistic                   & CI                & A multi-scale model with parallel convolution streams                   \\
\cline{2-6}
                              & \multirow{8}{*}{CNN + GAN} & GCBD \cite{Chen_2018_CVPR}         & AWGN and Realistic          & CI                & A GAN-based blind denoiser                               \\
\cline{3-6}
                              &                          & SCGAN \cite{yan2019unsupervised}        & AWGN                        & CI                & Unsupervised modeling with self-consistent GAN                \\
\cline{3-6}
                              &                          & DnGAN \cite{yeh2018image}        & AWGN and Blur               & CI                & GAN with  maximum a posteriori (MAP) framework                \\
\cline{3-6}
                              &                          & RED-WGAN \cite{ran2019denoising}     & AWGN and Rician             & MRI               & A residual encoder decoder Wasserstein GAN model              \\
\cline{3-6}
                              &                          & ADGAN \cite{Lin_2019_CVPR_Workshops}        & Realistic                   & CI                & Attentive GAN with noise domain adaptation                    \\
\cline{3-6}
                              &                          & SGN \cite{gu2019self}          & Realistic                   & CI                & A self-guided network with top-down architecture              \\
\cline{3-6}
                              &                          & DANet \cite{yue2020dual}        & Realistic                   & CI                & A Bayesian framework for noise removal and generation.                    \\
\hline
\end{tabular}
}
\label{Table_Method_all}
\end{table*}



==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_Results_Color_image_all.tex <==
%\begin{table*}[htbp]
%  \centering
%  \caption{Average PSNR, SSIM values on real-world color image datasets. The average time is calculated based on the PolyU dataset. `-' means the results are not available. `C: CANON', `F: FUJIFILM', `H: HUAWEI', `I: IPHONE', 'N: NIKON', `O: OPPO', `S: SONY', `X: XIAOMI'.}
%  \vspace{-9pt}
%  \renewcommand{\arraystretch}{0.138}
%  \scalebox{0.5806}{
%    \begin{tabular}{cccccccccccccccccccccc}
%    \toprule
%    \multicolumn{2}{c}{\multirow{2}[3]{*}{Methods/Models}} & \multirow{2}[3]{*}{DnD} & \multirow{2}[3]{*}{SIDD} & \multirow{2}[3]{*}{CC15} & \multirow{2}[3]{*}{CC60} & \multirow{2}[3]{*}{PolyU} & \multirow{2}[3]{*}{HighISO} & \multicolumn{13}{c}{IOCI}                                                                             & \multirow{3}[5]{*}{Time (s)} \\
%    \cmidrule{9-21}    \multicolumn{2}{c}{} &       &       &       &       &       &       & C-100D & C-600D & C-5DMark4 & F-X100T & H-Honor6X & H-Mate40Pro & I-5S & I-6S & I-13 & N-D5300 & O-R11s & S-A6500 & X-MI8 \\
%\cmidrule{1-21}    -     & \# Images & 1000  & 1280  & 15    & 60    & 100   & 100   & 55    & 25    & 83    & 71    & 30    & 126   & 36    & 67    & 174   & 56    & 39    & 36    & 50    &  \\
%     \midrule
%    \multirow{96}[52]{*}{\shortstack[c]{Traditional \\ denoisers}} & \multirow{2}[4]{*}{4DHOSVD} & 37.58  & 34.49  & 37.52  & 39.15  & 38.54  & 40.27  & 41.40  & 42.19  & 44.49  & 42.60  & 39.82  & 38.88  & 40.59  & 40.37  & 41.75  & 41.82  & 40.71  & 45.58  & 36.27  & \multirow{2}[4]{*}{123.06 } \\
%\cmidrule{3-21}          &       & 0.929  & 0.911  & 0.956  & 0.973  & 0.968  & 0.973  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.965  & 0.967  & 0.980  & 0.977  & 0.974  & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Bitonic} & 37.85  & 36.67  & 35.22  & 35.98  & 36.64  & 37.37  & 39.38  & 39.63  & 40.76  & 41.05  & 37.71  & 37.41  & 38.98  & 38.04  & 39.09  & 39.22  & 38.87  & 43.25  & 34.92  & \multirow{2}[4]{*}{2.57 } \\
%\cmidrule{3-21}          &       & 0.936  & 0.933  & 0.925  & 0.931  & 0.940  & 0.943  & 0.959  & 0.952  & 0.965  & 0.964  & 0.940  & 0.956  & 0.947  & 0.939  & 0.952  & 0.954  & 0.959  & 0.979  & 0.941  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CBM3D1} & 38.04  & 35.00  & 37.58  & 39.21  & 38.60  & 40.11  & 41.58  & 42.40  & 44.43  & 42.53  & 39.93  & 38.84  & 40.56  & 40.41  & 41.93  & 42.29  & 40.62  & 45.58  & 36.24  & \multirow{2}[4]{*}{1.02 } \\
%\cmidrule{3-21}          &       & 0.938  & 0.925  & 0.955  & 0.971  & 0.969  & 0.972  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.967  & \textcolor{blue}{\textbf{0.970}} & 0.982  & 0.979  & 0.973  & 0.990  & 0.959  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CBM3D2} & 37.73  & 34.74  & 37.70  & 39.41  & 38.69  & 40.35  & 41.69  & 42.54  & 44.74  & 42.65  & 39.97  & 38.97  & 40.77  & 40.55  & 42.03  & 42.20  & 40.75  & 45.72  & 36.38  & \multirow{2}[4]{*}{2.94 } \\
%\cmidrule{3-21}          &       & 0.934  & 0.922  & 0.957  & 0.975  & 0.970  & 0.974  & 0.978  & 0.984  & 0.992  & 0.977  & 0.967  & 0.974  & 0.967  & 0.969  & 0.983  & 0.979  & 0.974  & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CMSt-SVD} & 38.25  & 34.38  & 37.95  & 39.76  & 38.85  & 40.49  & 41.99  & 42.75  & 44.65  & 42.68  & 40.08  & 38.95  & \textcolor{blue}{\textbf{40.84}} & 40.53  & 42.06  & 42.72  & \textcolor{blue}{\textbf{40.88}} & 45.91  & 36.40  & \multirow{2}[4]{*}{4.95} \\
%\cmidrule{3-21}          &       & 0.940  & 0.900  & 0.959  & 0.976  & 0.971  & 0.974  & 0.979  & 0.984  & 0.991  & 0.977  & 0.967  & 0.973  & 0.967  & 0.967  & 0.982  & 0.980  & \textcolor{blue}{\textbf{0.974}} & 0.991  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{GID} & 34.32  & 27.16  & 37.17  & 38.41  & 38.37  & 39.63  & 40.86  & 41.60  & 44.11  & 42.31  & 39.52  & 38.66  & 40.12  & 40.16  & 41.50  & 41.09  & 40.50  & 44.96  & 36.11  & \multirow{2}[4]{*}{49.99 } \\
%\cmidrule{3-21}          &       & 0.817  & 0.634  & 0.946  & 0.963  & 0.967  & 0.967  & 0.974  & 0.979  & 0.989  & 0.975  & 0.965  & 0.972  & 0.964  & 0.967  & 0.979  & 0.973  & 0.973  & 0.989  & 0.960  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{LLRT} & 35.45  & 30.74  & 37.77  & 39.76  & 38.28  & 39.59  & 41.60  & 42.24  & 42.68  & 42.22  & 37.91  & 38.80  & 38.01  & 39.87  & 42.02  & 41.76  & 38.69  & 45.17  & 35.71  & \multirow{2}[4]{*}{285.62 } \\
%\cmidrule{3-21}          &       & 0.897  & 0.766  & 0.957  & 0.977  & 0.970  & 0.972  & 0.977  & 0.983  & 0.992  & 0.975  & 0.969  & 0.973  & 0.965  & 0.971  & 0.984  & 0.979  & 0.972  & 0.989  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{LSCD} & -     & -     & 36.20  & 37.69  & 37.97  & 38.64  & 40.65  & 41.45  & -     & -     & 39.22  & -     & 39.84  & 39.53  & -     & 40.83  & -     & 44.34  & 35.86  & \multirow{2}[4]{*}{3.19 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.942  & 0.963  & 0.964  & 0.962  & 0.973  & 0.979  & -     & -     & 0.963  & -     & 0.963  & 0.963  & -     & 0.973  & -     & 0.987  & 0.957  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{MCWNNM} & 37.38  & 29.54  & 37.02  & 38.54  & 38.26  & 39.89  & 41.47  & 42.07  & 44.22  & 42.48  & 39.46  & 38.78  & 39.87  & 40.18  & 41.33  & 41.74  & 40.71  & 45.38  & 35.84  & \multirow{2}[4]{*}{237.57 } \\
%\cmidrule{3-21}          &       & 0.929  & 0.888  & 0.950  & 0.967  & 0.965  & 0.970  & 0.977  & 0.979  & 0.988  & 0.976  & 0.961  & 0.971  & 0.957  & 0.963  & 0.976  & 0.975  & 0.973  & 0.990  & 0.952  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{M-SVD} & 37.45  & 33.51  & 37.63  & 39.36  & 38.57  & 40.27  & 41.81  & 42.55  & 44.39  & 42.68  & 39.99  & 38.93  & 40.78  & 40.52  & 41.72  & 42.18  & 40.73  & 45.71  & 36.37  & \multirow{2}[4]{*}{104.24 } \\
%\cmidrule{3-21}          &       & 0.924  & 0.867  & 0.954  & 0.971  & 0.967  & 0.971  & 0.979  & 0.983  & 0.989  & 0.976  & 0.967  & 0.973  & 0.969  & 0.969  & 0.977  & 0.977  & 0.974  & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{NLH-CC} & 38.85  & 35.31  & 38.49  & 39.86  & 38.36  & 40.29  & 41.77  & 42.72  & 43.66  & \textcolor{blue}{\textbf{42.80}} & 38.84  & 38.31  & 40.44  & 39.94  & 41.13  & \textcolor{blue}{\textbf{43.25}} & -     & \textcolor{blue}{\textbf{46.02}} & 35.73  & \multirow{2}[4]{*}{40.32} \\
%\cmidrule{3-21}          &       & 0.953  & 0.930  & 0.965  & 0.976  & 0.965  & 0.971  & 0.979  & 0.984  & 0.986  & \textcolor{blue}{\textbf{0.978}} & 0.959  & 0.968  & 0.964  & 0.963  & 0.976  & \textcolor{blue}{\textbf{0.981}} & -     & \textcolor{blue}{\textbf{0.991}} & 0.955  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{TWSC} & 37.96  & -     & 37.90  & 39.66  & 38.62  & 40.62  & 41.65  & 42.52  & 44.94  & 42.26  & 38.71  & 38.81  & 38.77  & 40.12  & 41.71  & 42.23  & 40.65  & 45.49  & 35.40  & \multirow{2}[4]{*}{350.30 } \\
%\cmidrule{3-21}          &       & 0.942  & -     & 0.959  & 0.976  & 0.967  & 0.975  & 0.977  & 0.982  & 0.992  & 0.973  & 0.945  & 0.972  & 0.938  & 0.962  & 0.980  & 0.975  & 0.972  & 0.990  & 0.939  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{WTR1} & -     & -     & 37.80  & 37.32  & 38.20  & 38.19  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{600.33} \\
%\cmidrule{3-21}          &       & -     & -     & 0.958  & 0.944  & 0.965  & 0.940  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
%    \midrule
%    \midrule
%    \multirow{418}[148]{*}{\shortstack[c]{DNN \\ methods}} & \multirow{2}[4]{*}{AINDNet\cite{Kim_2020_CVPR}} & 39.77  & 39.08  & 36.14  & 37.19  & 37.33  & 38.00  & 38.54  & 39.33  & 39.49  & 38.50  & 36.53  & 36.24  & 36.93  & 36.83  & 37.27  & 38.11  & 37.44  & 40.17  & 34.65  & \multirow{2}[4]{*}{0.33} \\
%\cmidrule{3-21}          &       & 0.959  & 0.953  & 0.935  & 0.949  & 0.954  & 0.946  & 0.975  & 0.976  & 0.979  & 0.966  & 0.954  & 0.965  & 0.958  & 0.953  & 0.964  & 0.961  & 0.968  & 0.981  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{AP-BSN\cite{lee2022ap}} & 37.29  & 35.97  & 35.44  & 36.76  & 36.99  & 38.26  & 40.23  & 41.29  & 42.72  & 41.40  & 37.87  & 37.62  & 37.47  & 38.29  & 40.83  & 40.86  & 39.55  & 43.73  & 34.37  & \multirow{2}[4]{*}{3.56 } \\
%\cmidrule{3-21}          &       & 0.932  & 0.925  & 0.936  & 0.956  & 0.956  & 0.965  & 0.973  & 0.979  & 0.986  & 0.970  & 0.949  & 0.966  & 0.939  & 0.960  & 0.977  & 0.973  & 0.969  & 0.983  & 0.937  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Blind2Unblind\cite{wang2022blind2unblind}} & -     & -     & 36.51  & 38.18  & 38.25  & 39.03  & 40.71  & 41.72  & 43.11  & 41.17  & 39.35  & 38.27  & 39.39  & 39.04  & 40.88  & 40.90  & 39.76  & 43.78  & 35.75  & \multirow{2}[4]{*}{0.74 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.935  & 0.958  & 0.968  & 0.962  & 0.974  & 0.981  & 0.990  & 0.970  & 0.967  & 0.971  & 0.962  & 0.958  & 0.976  & 0.970  & 0.971  & 0.986  & 0.956  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{BRDNet\cite{tian2020image}} & 33.80  & -     & 37.27  & 39.16  & 38.04  & 39.64  & 39.85  & 40.95  & 43.54  & 40.27  & 39.48  & 38.66  & 38.19  & 40.07  & 41.92  & 41.34  & 39.66  & 42.76  & 36.08  & \multirow{2}[4]{*}{14.66 } \\
%\cmidrule{3-21}          &       & 0.897  & -     & 0.953  & 0.974  & 0.960  & 0.969  & 0.965  & 0.974  & 0.989  & 0.958  & 0.958  & 0.973  & 0.943  & 0.969  & 0.981  & 0.972  & 0.965  & 0.979  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{C2N\cite{jang2021c2n}} & 37.28  & -     & 37.02  & -     & 37.69  & 38.86  & 41.12  & 41.95  & 42.61  & 41.33  & 38.73  & 38.15  & 38.95  & 38.67  & 40.50  & 40.78  & 40.05  & 44.64  & 35.53  & \multirow{2}[4]{*}{88.00 } \\
%\cmidrule{3-21}          &       & 0.924  & -     & 0.945  & -     & 0.958  & 0.960  & 0.976  & 0.980  & 0.980  & 0.966  & 0.954  & 0.965  & 0.956  & 0.945  & 0.977  & 0.964  & 0.970  & 0.987  & 0.952  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CBDNet\cite{guo2019toward}} & 38.06  & 33.26  & 36.20  & 37.67  & 37.81  & 38.18  & 41.43  & 42.41  & 42.55  & 41.88  & 38.35  & 38.17  & 39.80  & 39.07  & 40.63  & 40.92  & 39.54  & 44.38  & 35.54  & \multirow{2}[4]{*}{0.04 } \\
%\cmidrule{3-21}          &       & 0.942  & 0.869  & 0.919  & 0.940  & 0.956  & 0.942  & 0.977  & 0.981  & 0.980  & 0.971  & 0.946  & 0.964  & 0.960  & 0.951  & 0.968  & 0.963  & 0.965  & 0.981  & 0.950  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CVF-SID\cite{neshatavar2022cvf}} & 36.31  & 34.43  & 29.13  & 31.02  & 33.08  & 33.35  & 36.68  & 39.08  & 39.73  & 36.40  & 33.13  & 33.16  & 32.07  & 33.33  & 36.92  & 38.40  & 35.22  & 38.56  & 29.89  & \multirow{2}[4]{*}{0.12 } \\
%\cmidrule{3-21}          &       & 0.923  & 0.912  & 0.853  & 0.898  & 0.912  & 0.929  & 0.933  & 0.974  & 0.976  & 0.929  & 0.895  & 0.920  & 0.857  & 0.917  & 0.946  & 0.961  & 0.927  & 0.952  & 0.849  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CycleISP\cite{zamir2020cycleisp}} & 39.57  & 39.42  & 35.40  & 36.87  & 37.61  & 37.70  & 41.26  & 41.84  & 42.64  & 41.59  & 38.47  & 38.01  & 38.79  & 38.67  & 40.61  & 40.03  & 39.86  & 44.75  & 35.54  & \multirow{2}[4]{*}{0.26 } \\
%\cmidrule{3-21}          &       & 0.955  & 0.956  & 0.916  & 0.939  & 0.955  & 0.936  & 0.977  & 0.977  & 0.978  & 0.969  & 0.952  & 0.966  & 0.961  & 0.952  & 0.970  & 0.953  & 0.968  & 0.987  & 0.949  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DANet\cite{yue2020dual}} & 39.55  & 39.43  & 37.17  & 38.63  & \textcolor{blue}{\textbf{41.49}} & 38.92  & 41.59  & 42.59  & 42.83  & 41.70  & 37.91  & 38.17  & 39.23  & 38.74  & 41.58  & 41.54  & 39.58  & 44.03  & 36.21  & \multirow{2}[4]{*}{0.02} \\
%\cmidrule{3-21}          &       & 0.953  & 0.956  & 0.953  & 0.969  & \textcolor{blue}{\textbf{0.977}} & 0.960  & 0.979  & 0.985  & 0.979  & 0.977  & 0.963  & 0.970  & 0.964  & 0.962  & 0.980  & 0.976  & 0.972  & 0.989  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DBF\cite{chen2019real}} & -     & -     & 38.48  & 40.59  & 38.87  & 40.09  & 41.56  & 42.87  & 44.85  & 42.36  & 39.98  & 38.86  & 40.17  & 40.26  & 42.12  & 43.17  & 40.67  & 44.75  & 36.45  & \multirow{2}[4]{*}{0.34 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.960  & 0.981  & 0.970  & 0.970  & 0.979  & 0.984  & 0.992  & 0.975  & 0.967  & 0.972  & 0.966  & 0.966  & 0.982  & 0.982  & 0.973  & 0.987  & 0.963  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DCDicL\cite{zheng2021deep}} & -     & -     & 36.61  & -     & 37.45  & 38.12  & 37.77  & 38.24  & 38.39  & 38.62  & 35.87  & 36.07  & 35.83  & 36.25  & 39.84  & 39.38  & 37.04  & 40.24  & 34.72  & \multirow{2}[4]{*}{1.24 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.945  & -     & 0.972  & 0.965  & 0.970  & 0.977  & 0.990  & 0.968  & 0.968  & 0.975  & 0.956  & 0.971  & 0.984  & 0.976  & 0.969  & 0.980  & 0.955  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DeamNet\cite{ren2021adaptive}} & 39.63  & 39.35  & 36.63  & -     & 37.70  & 36.93  & 40.90  & 40.86  & 41.22  & 39.72  & 33.67  & 36.40  & 37.87  & 35.07  & 40.25  & 38.92  & 39.56  & 40.52  & 34.61  & \multirow{2}[4]{*}{0.18 } \\
%\cmidrule{3-21}          &       & 0.953  & 0.955  & 0.936  & -     & 0.958  & 0.944  & 0.977  & 0.978  & 0.979  & 0.967  & 0.953  & 0.964  & 0.961  & 0.948  & 0.966  & 0.957  & 0.969  & 0.980  & 0.952  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DIDN\cite{yu2019deep}} & 39.64  & 39.78  & 36.06  & -     & 37.36  & 38.24  & 40.74  & 41.68  & 42.35  & 41.17  & 38.15  & 37.87  & 38.27  & 38.58  & 40.03  & 40.32  & 39.73  & 44.07  & 35.28  & \multirow{2}[4]{*}{7.25 } \\
%\cmidrule{3-21}          &       & 0.953  & 0.958  & 0.946  & -     & 0.953  & 0.950  & 0.975  & 0.977  & 0.975  & 0.966  & 0.951  & 0.965  & 0.954  & 0.950  & 0.963  & 0.959  & 0.966  & 0.985  & 0.949  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DnCNN\cite{zhang2017beyond}} & 37.90  & 37.73  & 37.47  & 39.32  & 38.51  & 40.01  & 40.81  & 41.91  & 44.16  & 41.57  & 39.92  & 38.72  & 39.34  & 40.22  & 42.03  & 42.12  & 40.26  & 43.97  & 36.30  & \multirow{2}[4]{*}{3.23 } \\
%\cmidrule{3-21}          &       & 0.943  & 0.941  & 0.954  & 0.974  & 0.966  & 0.971  & 0.972  & 0.979  & 0.991  & 0.969  & 0.962  & 0.973  & 0.964  & 0.969  & 0.983  & 0.977  & 0.970  & 0.984  & 0.960  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DRUNet \cite{zhang2020plug}} & -     & -     & 38.30  & 40.33  & 38.93  & 40.77  & 41.94  & 42.62  & \textcolor{blue}{\textbf{45.36}} & 42.78  & 40.35 & \textcolor{blue}{\textbf{39.17}} & 40.80  & \textcolor{blue}{\textbf{40.80}} & \textcolor{blue}{\textbf{42.86}} & 42.86  & \textcolor{blue}{\textbf{40.88}} & 45.76  & 36.61  & \multirow{2}[4]{*}{0.17} \\
%\cmidrule{3-21}          &       & -     & -     & 0.961  & 0.979  & 0.970  & 0.974  & 0.978  & 0.982  & \textcolor{blue}{\textbf{0.993}} & 0.977  & 0.969 & \textcolor{blue}{\textbf{0.975}} & 0.966  & 0.970  & \textcolor{blue}{\textbf{0.985}} & 0.980  & \textcolor{blue}{\textbf{0.974}} & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DudeNet\cite{tian2021designing}} & 33.18  & 27.55  & 36.03  & 37.44  & 39.92  & 38.18  & 39.94  & 41.13  & 42.97  & 41.06  & 38.63  & 37.83  & 39.09  & 38.58  & 40.73  & 40.63  & 39.71  & 43.34  & 35.44  & \multirow{2}[4]{*}{0.18 } \\
%\cmidrule{3-21}          &       & 0.810  & 0.645  & 0.933  & 0.953  & 0.973  & 0.955  & 0.972  & 0.977  & 0.988  & 0.971  & 0.962  & 0.969  & 0.962  & 0.961  & 0.976  & 0.969  & 0.972  & 0.985  & 0.955  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{FCCF\cite{yue2019high}} & 36.30  & -  & \textcolor{blue}{\textbf{39.02}} & \textcolor{blue}{\textbf{40.89}} & 38.87  & \textcolor{blue}{\textbf{41.20}} & \textcolor{blue}{\textbf{42.03}} & 43.07  & 45.15  & \textcolor{blue}{\textbf{42.80}} & 40.14  & 39.04  & 40.61  & 40.66  & 42.31  & 43.05  & \textcolor{blue}{\textbf{40.88}} & 45.47  & \textcolor{blue}{\textbf{36.72}} & \multirow{2}[4]{*}{11.20} \\
%\cmidrule{3-21}          &       & 0.885  & - & \textcolor{blue}{\textbf{0.968}} & \textcolor{blue}{\textbf{0.982}} & 0.971  & \textcolor{blue}{\textbf{0.978}} & \textcolor{blue}{\textbf{0.980}} & \textcolor{blue}{\textbf{0.985}} & 0.993  & \textcolor{blue}{\textbf{0.978}} & 0.966  & 0.974  & 0.967  & 0.969  & 0.984  & 0.982  & \textcolor{blue}{\textbf{0.974}} & 0.989  & \textcolor{blue}{\textbf{0.964}} &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{FFDNet\cite{zhang2018ffdnet}} & 37.61  & 38.27  & 37.67  & 39.73  & 38.76  & 40.28  & 41.67  & 42.55  & 44.77  & 42.44  & 40.05  & 38.96  & 40.60  & 40.50  & 42.43  & 42.44  & 40.75  & 45.71  & 36.47  & \multirow{2}[4]{*}{0.02} \\
%\cmidrule{3-21}          &       & 0.942  & 0.948  & 0.956  & 0.977  & 0.970  & 0.973  & 0.977  & 0.982  & 0.992  & 0.976  & 0.967  & 0.974  & 0.964  & 0.971  & 0.984  & 0.979  & 0.973  & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{IDR\cite{zhang2022idr}} & -     & -     & 34.26  & 36.18  & 36.28  & 36.44  & 39.33  & 40.31  & 40.94  & 39.74  & 37.38  & 37.39  & 38.30  & 38.15  & 39.68  & 38.22  & 38.01  & 43.15  & 34.64  & \multirow{2}[4]{*}{0.32 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.877  & 0.923  & 0.925  & 0.910  & 0.955  & 0.962  & 0.961  & 0.935  & 0.927  & 0.957  & 0.938  & 0.944  & 0.951  & 0.913  & 0.941  & 0.978  & 0.929  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{InvDN\cite{liu2021invertible}} & 39.57  & 39.28  & 34.55  & 36.33  & 35.94  & 38.01  & 38.95  & 40.09  & 42.03  & 40.02  & 33.32  & 37.00  & 36.64  & 37.66  & 40.06  & 40.98  & 39.10  & 40.74  & 34.15  & \multirow{2}[4]{*}{0.74 } \\
%\cmidrule{3-21}          &       & 0.952  & 0.955  & 0.937  & 0.953  & 0.947  & 0.952  & 0.965  & 0.973  & 0.978  & 0.960  & 0.930  & 0.965  & 0.939  & 0.955  & 0.966  & 0.971  & 0.964  & 0.969  & 0.935  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{IRCNN\cite{zhang2017learning}} & 34.78  & 33.50  & 37.26  & 37.25  & 37.49  & 39.66  & 41.24  & 41.85  & 43.89  & 41.78  & 39.91  & 38.63  & 40.14  & 40.12  & 41.87  & 41.86  & 40.26  & 44.38  & 36.22  & \multirow{2}[4]{*}{2.15 } \\
%\cmidrule{3-21}          &       & 0.907  & 0.887  & 0.954  & 0.956  & 0.956  & 0.970  & 0.978  & 0.981  & 0.991  & 0.973  & 0.969  & 0.972  & 0.965  & 0.969  & 0.983  & 0.977  & 0.972  & 0.988  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{MIRNet\cite{Zamir2020MIRNet}} & 39.88  & 39.55  & 36.06  & 37.25  & 37.49  & 38.10  & 40.72  & 41.68  & 42.76  & 41.05  & 38.28  & 37.80  & 38.60  & 38.55  & 40.28  & 40.46  & 39.73  & 43.66  & 35.42  & \multirow{2}[4]{*}{0.71 } \\
%\cmidrule{3-21}          &       & 0.956  & 0.957  & 0.942  & 0.956  & 0.956  & 0.952  & 0.975  & 0.978  & 0.980  & 0.968  & 0.954  & 0.967  & 0.959  & 0.952  & 0.966  & 0.964  & 0.967  & 0.983  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{MPRNet\cite{zamir2021multi}} & 39.82  & 39.57  & 35.94  & -     & 37.50  & 38.04  & 40.59  & 41.30  & 42.59  & 41.23  & 38.35  & 37.92  & 38.95  & 38.62  & 40.21  & 40.20  & 39.77  & 44.05  & 35.49  & \multirow{2}[4]{*}{35.97 } \\
%\cmidrule{3-21}          &       & 0.954  & 0.958  & 0.935  & -     & 0.954  & 0.946  & 0.974  & 0.974  & 0.978  & 0.969  & 0.952  & 0.966  & 0.960  & 0.949  & 0.965  & 0.960  & 0.967  & 0.986  & 0.951  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{NAFNet\cite{chen2022simple}} & 38.36  & \textcolor{blue}{\textbf{40.15}} & 34.39  & -     & 36.38  & 37.88  & 40.12  & 40.23  & 40.66  & 40.01  & 36.13  & 35.87  & 36.66  & 36.79  & 36.53  & 39.93  & 39.32  & 40.45  & 34.82  & \multirow{2}[4]{*}{0.35} \\
%\cmidrule{3-21}          &       & 0.943  & \textcolor{blue}{\textbf{0.960}} & 0.923  & -     & 0.947  & 0.954  & 0.973  & 0.943  & 0.936  & 0.962  & 0.919  & 0.927  & 0.948  & 0.927  & 0.884  & 0.951  & 0.966  & 0.924  & 0.948  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{NBNet\cite{cheng2021nbnet}} & 39.89  & 39.64  & 35.89  & -     & 37.37  & 38.32  & 40.95  & 41.91  & 42.92  & 41.17  & 38.02  & 37.87  & 37.79  & 38.45  & 40.51  & 40.45  & 39.73  & 43.96  & 35.37  & \multirow{2}[4]{*}{0.12 } \\
%\cmidrule{3-21}          &       & 0.955  & 0.958  & 0.935  & -     & 0.957  & 0.955  & 0.977  & 0.980  & 0.982  & 0.971  & 0.955  & 0.967  & 0.956  & 0.955  & 0.972  & 0.967  & 0.969  & 0.984  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Neigh2Neigh\cite{huang2021neighbor2neighbor}} & -     & -     & 34.47  & 35.65  & 37.10  & 36.59  & 40.22  & 40.41  & 41.29  & 41.24  & 38.13  & 37.94  & 39.71  & 38.50  & 39.63  & 38.05  & 39.17  & 44.49  & 35.30  & \multirow{2}[4]{*}{2.48} \\
%\cmidrule{3-21}          &       & -     & -     & 0.883  & 0.907  & 0.942  & 0.908  & 0.967  & 0.960  & 0.966  & 0.958  & 0.940  & 0.961  & 0.956  & 0.936  & 0.952  & 0.919  & 0.958  & 0.984  & 0.944  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{NLNet\cite{lefkimmiatis2017non}} & -     & -     & 37.56  & 39.32  & 38.58  & 40.17  & 41.43  & 42.18  & 44.53  & 42.19  & 39.96  & 38.89  & 40.06  & 40.61  & 42.14  & 42.16  & 40.63  & 44.87  & 36.34  & \multirow{2}[4]{*}{39.06 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.955  & 0.974  & 0.968  & 0.973  & 0.976  & 0.981  & 0.991  & 0.974  & 0.969 & 0.973  & 0.964  & \textcolor{blue}{\textbf{0.971}} & 0.983  & 0.978  & 0.973  & 0.988  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Noise2Noise\cite{lehtinen2018noise2noise}} & -     & -     & 33.55  & 34.67  & 35.91  & 35.28  & 38.88  & 39.07  & 39.34  & 39.26  & 36.81  & 36.99  & 38.04  & 37.21  & 38.00  & 36.35  & 37.67  & 42.59  & 34.44  & \multirow{2}[4]{*}{0.03 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.850  & 0.874  & 0.913  & 0.875  & 0.950  & 0.940  & 0.938  & 0.931  & 0.919  & 0.948  & 0.936  & 0.916  & 0.924  & 0.876  & 0.936  & 0.975  & 0.926  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{PD-Denoising\cite{zhou2020awgn}} & 38.40  & 33.99  & 35.85  & 37.13  & 37.13  & 37.12  & 40.85  & 41.38  & 41.13  & 41.05  & 37.72  & 37.57  & 39.03  & 38.01  & 39.18  & 39.64  & 38.80  & 43.73  & 35.05  & \multirow{2}[4]{*}{0.61 } \\
%\cmidrule{3-21}          &       & 0.943  & 0.896  & 0.924  & 0.944  & 0.944  & 0.921  & 0.974  & 0.974  & 0.966  & 0.959  & 0.935  & 0.956  & 0.948  & 0.929  & 0.948  & 0.946  & 0.955  & 0.981  & 0.940  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{PNGAN\cite{cai2021learning}} & 39.38  & 39.81  & 38.44  & -     & 39.57  & 40.51  & 41.79  & \textcolor{blue}{\textbf{43.13}} & 44.73  & 42.55  & 39.84  & 38.78  & 40.63  & 40.20  & 41.85  & 43.15  & \textcolor{blue}{\textbf{40.88}} & 45.32  & 36.40  & \multirow{2}[4]{*}{1.53} \\
%\cmidrule{3-21}          &       & 0.953  & 0.959  & 0.963  & -     & 0.974  & 0.974  & 0.979  & \textcolor{blue}{\textbf{0.985}} & 0.992  & 0.977  & 0.964  & 0.970  & \textcolor{blue}{\textbf{0.969}} & 0.962  & 0.981  & 0.982  & \textcolor{blue}{\textbf{0.974}} & 0.988  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{R2R\cite{pang2021recorrupted}} & -     & 34.78     & 36.32  & 38.11  & 38.47  & 38.71  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{4481.98 } \\
%\cmidrule{3-21}          &       & -     & 0.844     & 0.937  & 0.961  & 0.965  & 0.958  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Restormer\cite{zamir2022restormer}} & \textcolor{blue}{\textbf{40.03}} & 40.02  & 36.33  & -     & 37.66  & 38.29  & 41.10  & 41.84  & 42.49  & 41.47  & 38.42  & 38.08  & 39.05  & 38.77  & 40.13  & 40.53  & 39.56  & 44.19  & 35.65  & \multirow{2}[4]{*}{0.77} \\
%\cmidrule{3-21}          &       & \textcolor{blue}{\textbf{0.956}} & \textcolor{blue}{\textbf{0.960}}  & 0.941  & -     & 0.956  & 0.948  & 0.977  & 0.979  & 0.976  & 0.968  & 0.952  & 0.966  & 0.960  & 0.949  & 0.963  & 0.962  & 0.963  & 0.986  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{RIDNet\cite{anwar2019real}} & 39.26  & 38.70  & 36.84  & 38.11  & 38.57  & 38.60  & 41.09  & 42.15  & 42.39  & 41.59  & 38.88  & 38.21  & 38.67  & 39.02  & 40.91  & 41.01  & 40.07  & 44.40  & 35.76  & \multirow{2}[4]{*}{0.11 } \\
%\cmidrule{3-21}          &       & 0.953  & 0.950  & 0.941  & 0.961  & 0.970  & 0.956  & 0.977  & 0.980  & 0.989  & 0.975  & 0.962  & 0.970  & 0.963  & 0.959  & 0.978  & 0.977  & 0.972  & 0.987  & 0.957  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{SADNet\cite{chang2020spatial}} & 39.59  & -     & 37.76  & 38.11  & 39.22  & 38.90  & 40.82  & 42.02  & 44.25  & 41.85  & 39.53  & 38.33  & 39.83  & 39.69  & 39.81  & 41.64  & 40.70  & 44.61  & 36.36  & \multirow{2}[4]{*}{0.04 } \\
%\cmidrule{3-21}          &       & 0.952  & -     & 0.952  & 0.961  & 0.972  & 0.965  & 0.976  & 0.980  & 0.992  & 0.975  & 0.965  & 0.970  & 0.965  & 0.963  & 0.965  & 0.979  & \textcolor{blue}{\textbf{0.974}} & 0.988  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{SASL\cite{li2023spatially}} & 38.00  &  37.41   & 34.93  &  -  & 37.13  & 38.24  & 40.04  & 41.86  & 43.07  & 40.29  & 37.22  & 37.38  & 36.45  & 37.64  & 40.85  & 41.64  & 39.10  & 42.89  & 34.25  & \multirow{2}[4]{*}{0.06 } \\
%\cmidrule{3-21}          &       & 0.936  &  0.934  & 0.936  & -  & 0.954  & 0.964  & 0.966  & 0.982  & 0.987  & 0.963  & 0.947  & 0.965  & 0.933  & 0.958  & 0.977  & 0.976  & 0.965  & 0.980  & 0.930  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{SCUNet\cite{zhang2022practical}} & 38.96     & 35.31     & 37.44  & 39.29  & 38.08  & 39.47  & 40.96  & 42.24  & 44.02  & 41.93  & \textcolor{blue}{\textbf{40.74}}  & 38.75  & 39.97  & 40.37  & 41.79  & 42.61  & 40.64  & 44.24  & 36.13  & \multirow{2}[4]{*}{0.62} \\
%\cmidrule{3-21}          &       & 0.953   & 0.901   & 0.958  & 0.972  & 0.962  & 0.971  & 0.972  & 0.980  & 0.991  & 0.966  & \textcolor{blue}{\textbf{0.974}}  & 0.971  & 0.968  & 0.975  & 0.970  & 0.978  & 0.973  & 0.981  & 0.956  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Self2Self\cite{quan2020self2self}} & -     & -     & 36.26  & 38.23  & -     & 39.49  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{4100.76 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.947  & 0.969  & -     & 0.963  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{UDnet \cite{lefkimmiatis2018universal}} & -     & -     & 36.95  & 38.96  & 38.05  & 39.62  & 40.40  & 41.36  & 43.58  & 41.12  & 39.35  & 38.25  & 38.94  & 39.95  & 41.32  & 41.70  & 39.51  & 43.17  & 36.09  & \multirow{2}[4]{*}{3.68 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.943  & 0.971  & 0.962  & 0.968  & 0.968  & 0.977  & 0.989  & 0.968  & 0.963  & 0.971  & 0.959  & 0.968  & 0.979  & 0.974  & 0.966  & 0.981  & 0.958  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Uformer\cite{Wang_2022_CVPR}} & \textcolor{blue}{\textbf{40.05}}  & 39.74  & 35.97  & -  & 37.44  & 38.12  & 40.83  & 41.37  & 42.45  & 41.35  & 38.36  & 37.83  & 38.95  & 38.69  & 40.30  & 40.36  & 39.69  & 43.93  & 35.50  & \multirow{2}[4]{*}{1.46} \\
%\cmidrule{3-21}          &       & \textcolor{blue}{\textbf{0.956}}  & 0.958  & 0.941  & -  & 0.956  & 0.950  & 0.976  & 0.977  & 0.978  & 0.968  & 0.954  & 0.966  & 0.960  & 0.953  & 0.966  & 0.964  & 0.967  & 0.985  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{VDIR \cite{soh2022variational}} & 39.63     & 39.26  & 34.90  & 36.51  & 37.01  & 36.84  & 40.84  & 41.40  & 41.29  & 40.81  & 37.65  & 37.84  & 39.09  & 38.17  & 39.20  & 39.41  & 38.98  & 44.40  & 35.04  & \multirow{2}[4]{*}{2.03 } \\
%\cmidrule{3-21}          &       & 0.953     & 0.955  & 0.894  & 0.925  & 0.940  & 0.911  & 0.973  & 0.970  & 0.965  & 0.953  & 0.936  & 0.960  & 0.951  & 0.931  & 0.946  & 0.938  & 0.956  & 0.985  & 0.939  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{VDNet\cite{yue2019variational}} & -     & -     & 35.86  & -     & 37.58  & 38.43  & 40.97  & 42.37  & 43.08  & 41.19  & 38.23  & 37.95  & 37.88  & 38.60  & 40.81  & 41.21  & 39.93  & 44.27  & 35.49  & \multirow{2}[4]{*}{0.05 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.945  & -     & 0.957  & 0.955  & 0.976  & 0.983  & 0.983  & 0.970  & 0.956  & 0.968  & 0.956  & 0.956  & 0.973  & 0.970  & 0.970  & 0.984  & 0.953  &  \\
%    \bottomrule
%    \end{tabular}%
% }
%  \label{Table_Results_Color_image_all}%
%\end{table*}%
%

%\begin{table*}[htbp]
%  \centering
%  \caption{Average PSNR, SSIM values on real-world color image datasets. The average time is calculated based on the PolyU dataset. `-' means the results are not available. `C: CANON', `F: FUJIFILM', `H: HUAWEI', `I: IPHONE', 'N: NIKON', `O: OPPO', `S: SONY', `X: XIAOMI'.}
%  \vspace{-9pt}
%  \renewcommand{\arraystretch}{0.138}
%  \scalebox{0.5806}{
%    \begin{tabular}{cccccccccccccccccccccc}
%    \toprule
%    \multicolumn{2}{c}{\multirow{2}[3]{*}{Methods/Models}} & \multirow{2}[3]{*}{DnD} & \multirow{2}[3]{*}{SIDD} & \multirow{2}[3]{*}{CC15} & \multirow{2}[3]{*}{CC60} & \multirow{2}[3]{*}{PolyU} & \multirow{2}[3]{*}{HighISO} & \multicolumn{13}{c}{IOCI}                                                                             & \multirow{3}[5]{*}{Time (s)} \\
%    \cmidrule{9-21}    \multicolumn{2}{c}{} &       &       &       &       &       &       & C-100D & C-600D & C-5DMark4 & F-X100T & H-Honor6X & H-Mate40Pro & I-5S & I-6S & I-13 & N-D5300 & O-R11s & S-A6500 & X-MI8 \\
%\cmidrule{1-21}    -     & \# Images & 1000  & 1280  & 15    & 60    & 100   & 100   & 55    & 25    & 83    & 71    & 30    & 126   & 36    & 67    & 174   & 56    & 39    & 36    & 50    &  \\
%     \midrule
%    \multirow{96}[52]{*}{\shortstack[c]{Traditional \\ denoisers}} & \multirow{2}[4]{*}{4DHOSVD \cite{rajwade2012image}} & 37.58  & 34.49  & 37.52  & 39.15  & 38.54  & 40.27  & 41.40  & 42.19  & 44.49  & 42.60  & 39.82  & 38.88  & 40.59  & 40.37  & 41.75  & 41.82  & 40.71  & 45.58  & 36.27  & \multirow{2}[4]{*}{123.06 } \\
%\cmidrule{3-21}          &       & 0.929  & 0.911  & 0.956  & 0.973  & 0.968  & 0.973  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.965  & 0.967  & 0.980  & 0.977  & 0.974  & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Bitonic \cite{treece2022real}} & 37.85  & 36.67  & 35.22  & 35.98  & 36.64  & 37.37  & 39.38  & 39.63  & 40.76  & 41.05  & 37.71  & 37.41  & 38.98  & 38.04  & 39.09  & 39.22  & 38.87  & 43.25  & 34.92  & \multirow{2}[4]{*}{2.57 } \\
%\cmidrule{3-21}          &       & 0.936  & 0.933  & 0.925  & 0.931  & 0.940  & 0.943  & 0.959  & 0.952  & 0.965  & 0.964  & 0.940  & 0.956  & 0.947  & 0.939  & 0.952  & 0.954  & 0.959  & 0.979  & 0.941  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CBM3D1 \cite{dabov2007image}} & 38.04  & 35.00  & 37.58  & 39.21  & 38.60  & 40.11  & 41.58  & 42.40  & 44.43  & 42.53  & 39.93  & 38.84  & 40.56  & 40.41  & 41.93  & 42.29  & 40.62  & 45.58  & 36.24  & \multirow{2}[4]{*}{1.02 } \\
%\cmidrule{3-21}          &       & 0.938  & 0.925  & 0.955  & 0.971  & 0.969  & 0.972  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.967  & {\textbf{0.970}} & 0.982  & 0.979  & 0.973  & 0.990  & 0.959  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CBM3D2 \cite{dabov2007image}} & 37.73  & 34.74  & 37.70  & 39.41  & 38.69  & 40.35  & 41.69  & 42.54  & 44.74  & 42.65  & 39.97  & 38.97  & 40.77  & 40.55  & 42.03  & 42.20  & 40.75  & 45.72  & 36.38  & \multirow{2}[4]{*}{2.94 } \\
%\cmidrule{3-21}          &       & 0.934  & 0.922  & 0.957  & 0.975  & 0.970  & 0.974  & 0.978  & 0.984  & 0.992  & 0.977  & 0.967  & 0.974  & 0.967  & 0.969  & 0.983  & 0.979  & 0.974  & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CMSt-SVD \cite{kong2019color}} & 38.25  & 34.38  & 37.95  & 39.76  & 38.85  & 40.49  & 41.99  & 42.75  & 44.65  & 42.68  & 40.08  & 38.95  & {\textbf{40.84}} & 40.53  & 42.06  & 42.72  & {\textbf{40.88}} & 45.91  & 36.40  & \multirow{2}[4]{*}{4.95} \\
%\cmidrule{3-21}          &       & 0.940  & 0.900  & 0.959  & 0.976  & 0.971  & 0.974  & 0.979  & 0.984  & 0.991  & 0.977  & 0.967  & 0.973  & 0.967  & 0.967  & 0.982  & 0.980  & {\textbf{0.974}} & 0.991  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{GID\cite{xu2018external}} & 34.32  & 27.16  & 37.17  & 38.41  & 38.37  & 39.63  & 40.86  & 41.60  & 44.11  & 42.31  & 39.52  & 38.66  & 40.12  & 40.16  & 41.50  & 41.09  & 40.50  & 44.96  & 36.11  & \multirow{2}[4]{*}{49.99 } \\
%\cmidrule{3-21}          &       & 0.817  & 0.634  & 0.946  & 0.963  & 0.967  & 0.967  & 0.974  & 0.979  & 0.989  & 0.975  & 0.965  & 0.972  & 0.964  & 0.967  & 0.979  & 0.973  & 0.973  & 0.989  & 0.960  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{LLRT \cite{chang2017hyper}} & 35.45  & 30.74  & 37.77  & 39.76  & 38.28  & 39.59  & 41.60  & 42.24  & 42.68  & 42.22  & 37.91  & 38.80  & 38.01  & 39.87  & 42.02  & 41.76  & 38.69  & 45.17  & 35.71  & \multirow{2}[4]{*}{285.62 } \\
%\cmidrule{3-21}          &       & 0.897  & 0.766  & 0.957  & 0.977  & 0.970  & 0.972  & 0.977  & 0.983  & 0.992  & 0.975  & 0.969  & 0.973  & 0.965  & 0.971  & 0.984  & 0.979  & 0.972  & 0.989  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{LSCD \cite{rizkinia2016local}} & -     & -     & 36.20  & 37.69  & 37.97  & 38.64  & 40.65  & 41.45  & -     & -     & 39.22  & -     & 39.84  & 39.53  & -     & 40.83  & -     & 44.34  & 35.86  & \multirow{2}[4]{*}{3.19 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.942  & 0.963  & 0.964  & 0.962  & 0.973  & 0.979  & -     & -     & 0.963  & -     & 0.963  & 0.963  & -     & 0.973  & -     & 0.987  & 0.957  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{MCWNNM\cite{xu2017multi}} & 37.38  & 29.54  & 37.02  & 38.54  & 38.26  & 39.89  & 41.47  & 42.07  & 44.22  & 42.48  & 39.46  & 38.78  & 39.87  & 40.18  & 41.33  & 41.74  & 40.71  & 45.38  & 35.84  & \multirow{2}[4]{*}{237.57 } \\
%\cmidrule{3-21}          &       & 0.929  & 0.888  & 0.950  & 0.967  & 0.965  & 0.970  & 0.977  & 0.979  & 0.988  & 0.976  & 0.961  & 0.971  & 0.957  & 0.963  & 0.976  & 0.975  & 0.973  & 0.990  & 0.952  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{M-SVD} & 37.45  & 33.51  & 37.63  & 39.36  & 38.57  & 40.27  & 41.81  & 42.55  & 44.39  & 42.68  & 39.99  & 38.93  & 40.78  & 40.52  & 41.72  & 42.18  & 40.73  & 45.71  & 36.37  & \multirow{2}[4]{*}{104.24 } \\
%\cmidrule{3-21}          &       & 0.924  & 0.867  & 0.954  & 0.971  & 0.967  & 0.971  & 0.979  & 0.983  & 0.989  & 0.976  & 0.967  & 0.973  & 0.969  & 0.969  & 0.977  & 0.977  & 0.974  & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{NLHCC\cite{hou2020nlh}} & 38.85  & 35.31  & 38.49  & 39.86  & 38.36  & 40.29  & 41.77  & 42.72  & 43.66  & {\textbf{42.80}} & 38.84  & 38.31  & 40.44  & 39.94  & 41.13  & {\textbf{43.25}} & -     & {\textbf{46.02}} & 35.73  & \multirow{2}[4]{*}{40.32} \\
%\cmidrule{3-21}          &       & 0.953  & 0.930  & 0.965  & 0.976  & 0.965  & 0.971  & 0.979  & 0.984  & 0.986  & {\textbf{0.978}} & 0.959  & 0.968  & 0.964  & 0.963  & 0.976  & {\textbf{0.981}} & -     & {\textbf{0.991}} & 0.955  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{TWSC\cite{xu2018trilateral}} & 37.96  & -     & 37.90  & 39.66  & 38.62  & 40.62  & 41.65  & 42.52  & 44.94  & 42.26  & 38.71  & 38.81  & 38.77  & 40.12  & 41.71  & 42.23  & 40.65  & 45.49  & 35.40  & \multirow{2}[4]{*}{350.30 } \\
%\cmidrule{3-21}          &       & 0.942  & -     & 0.959  & 0.976  & 0.967  & 0.975  & 0.977  & 0.982  & 0.992  & 0.973  & 0.945  & 0.972  & 0.938  & 0.962  & 0.980  & 0.975  & 0.972  & 0.990  & 0.939  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{WTR1 \cite{wu2018weighted}} & -     & -     & 37.80  & 37.32  & 38.20  & 38.19  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{600.33} \\
%\cmidrule{3-21}          &       & -     & -     & 0.958  & 0.944  & 0.965  & 0.940  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
%    \midrule
%    \midrule
%    \multirow{418}[148]{*}{\shortstack[c]{DNN \\ methods}} & \multirow{2}[4]{*}{AINDNet\cite{Kim_2020_CVPR}} & 39.77  & 39.08  & 36.14  & 37.19  & 37.33  & 38.00  & 38.54  & 39.33  & 39.49  & 38.50  & 36.53  & 36.24  & 36.93  & 36.83  & 37.27  & 38.11  & 37.44  & 40.17  & 34.65  & \multirow{2}[4]{*}{0.33} \\
%\cmidrule{3-21}          &       & 0.959  & 0.953  & 0.935  & 0.949  & 0.954  & 0.946  & 0.975  & 0.976  & 0.979  & 0.966  & 0.954  & 0.965  & 0.958  & 0.953  & 0.964  & 0.961  & 0.968  & 0.981  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{AP-BSN\cite{lee2022ap}} & 37.29  & 35.97  & 35.44  & 36.76  & 36.99  & 38.26  & 40.23  & 41.29  & 42.72  & 41.40  & 37.87  & 37.62  & 37.47  & 38.29  & 40.83  & 40.86  & 39.55  & 43.73  & 34.37  & \multirow{2}[4]{*}{3.56 } \\
%\cmidrule{3-21}          &       & 0.932  & 0.925  & 0.936  & 0.956  & 0.956  & 0.965  & 0.973  & 0.979  & 0.986  & 0.970  & 0.949  & 0.966  & 0.939  & 0.960  & 0.977  & 0.973  & 0.969  & 0.983  & 0.937  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Blind2Unblind\cite{wang2022blind2unblind}} & -     & -     & 36.51  & 38.18  & 38.25  & 39.03  & 40.71  & 41.72  & 43.11  & 41.17  & 39.35  & 38.27  & 39.39  & 39.04  & 40.88  & 40.90  & 39.76  & 43.78  & 35.75  & \multirow{2}[4]{*}{0.74 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.935  & 0.958  & 0.968  & 0.962  & 0.974  & 0.981  & 0.990  & 0.970  & 0.967  & 0.971  & 0.962  & 0.958  & 0.976  & 0.970  & 0.971  & 0.986  & 0.956  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{BRDNet\cite{tian2020image}} & 33.80  & -     & 37.27  & 39.16  & 38.04  & 39.64  & 39.85  & 40.95  & 43.54  & 40.27  & 39.48  & 38.66  & 38.19  & 40.07  & 41.92  & 41.34  & 39.66  & 42.76  & 36.08  & \multirow{2}[4]{*}{14.66 } \\
%\cmidrule{3-21}          &       & 0.897  & -     & 0.953  & 0.974  & 0.960  & 0.969  & 0.965  & 0.974  & 0.989  & 0.958  & 0.958  & 0.973  & 0.943  & 0.969  & 0.981  & 0.972  & 0.965  & 0.979  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{C2N\cite{jang2021c2n}} & 37.28  & -     & 37.02  & -     & 37.69  & 38.86  & 41.12  & 41.95  & 42.61  & 41.33  & 38.73  & 38.15  & 38.95  & 38.67  & 40.50  & 40.78  & 40.05  & 44.64  & 35.53  & \multirow{2}[4]{*}{88.00 } \\
%\cmidrule{3-21}          &       & 0.924  & -     & 0.945  & -     & 0.958  & 0.960  & 0.976  & 0.980  & 0.980  & 0.966  & 0.954  & 0.965  & 0.956  & 0.945  & 0.977  & 0.964  & 0.970  & 0.987  & 0.952  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CBDNet\cite{guo2019toward}} & 38.06  & 33.26  & 36.20  & 37.67  & 37.81  & 38.18  & 41.43  & 42.41  & 42.55  & 41.88  & 38.35  & 38.17  & 39.80  & 39.07  & 40.63  & 40.92  & 39.54  & 44.38  & 35.54  & \multirow{2}[4]{*}{0.04 } \\
%\cmidrule{3-21}          &       & 0.942  & 0.869  & 0.919  & 0.940  & 0.956  & 0.942  & 0.977  & 0.981  & 0.980  & 0.971  & 0.946  & 0.964  & 0.960  & 0.951  & 0.968  & 0.963  & 0.965  & 0.981  & 0.950  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CVF-SID\cite{neshatavar2022cvf}} & 36.31  & 34.43  & 29.13  & 31.02  & 33.08  & 33.35  & 36.68  & 39.08  & 39.73  & 36.40  & 33.13  & 33.16  & 32.07  & 33.33  & 36.92  & 38.40  & 35.22  & 38.56  & 29.89  & \multirow{2}[4]{*}{0.12 } \\
%\cmidrule{3-21}          &       & 0.923  & 0.912  & 0.853  & 0.898  & 0.912  & 0.929  & 0.933  & 0.974  & 0.976  & 0.929  & 0.895  & 0.920  & 0.857  & 0.917  & 0.946  & 0.961  & 0.927  & 0.952  & 0.849  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{CycleISP\cite{zamir2020cycleisp}} & 39.57  & 39.42  & 35.40  & 36.87  & 37.61  & 37.70  & 41.26  & 41.84  & 42.64  & 41.59  & 38.47  & 38.01  & 38.79  & 38.67  & 40.61  & 40.03  & 39.86  & 44.75  & 35.54  & \multirow{2}[4]{*}{0.26 } \\
%\cmidrule{3-21}          &       & 0.955  & 0.956  & 0.916  & 0.939  & 0.955  & 0.936  & 0.977  & 0.977  & 0.978  & 0.969  & 0.952  & 0.966  & 0.961  & 0.952  & 0.970  & 0.953  & 0.968  & 0.987  & 0.949  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DANet\cite{yue2020dual}} & 39.55  & 39.43  & 37.17  & 38.63  & {\textbf{41.49}} & 38.92  & 41.59  & 42.59  & 42.83  & 41.70  & 37.91  & 38.17  & 39.23  & 38.74  & 41.58  & 41.54  & 39.58  & 44.03  & 36.21  & \multirow{2}[4]{*}{0.02} \\
%\cmidrule{3-21}          &       & 0.953  & 0.956  & 0.953  & 0.969  & {\textbf{0.977}} & 0.960  & 0.979  & 0.985  & 0.979  & 0.977  & 0.963  & 0.970  & 0.964  & 0.962  & 0.980  & 0.976  & 0.972  & 0.989  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DBF\cite{chen2019real}} & -     & -     & 38.48  & 40.59  & 38.87  & 40.09  & 41.56  & 42.87  & 44.85  & 42.36  & 39.98  & 38.86  & 40.17  & 40.26  & 42.12  & 43.17  & 40.67  & 44.75  & 36.45  & \multirow{2}[4]{*}{0.34 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.960  & 0.981  & 0.970  & 0.970  & 0.979  & 0.984  & 0.992  & 0.975  & 0.967  & 0.972  & 0.966  & 0.966  & 0.982  & 0.982  & 0.973  & 0.987  & 0.963  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DCDicL\cite{zheng2021deep}} & -     & -     & 36.61  & -     & 37.45  & 38.12  & 37.77  & 38.24  & 38.39  & 38.62  & 35.87  & 36.07  & 35.83  & 36.25  & 39.84  & 39.38  & 37.04  & 40.24  & 34.72  & \multirow{2}[4]{*}{1.24 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.945  & -     & 0.972  & 0.965  & 0.970  & 0.977  & 0.990  & 0.968  & 0.968  & 0.975  & 0.956  & 0.971  & 0.984  & 0.976  & 0.969  & 0.980  & 0.955  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DeamNet\cite{ren2021adaptive}} & 39.63  & 39.35  & 36.63  & -     & 37.70  & 36.93  & 40.90  & 40.86  & 41.22  & 39.72  & 33.67  & 36.40  & 37.87  & 35.07  & 40.25  & 38.92  & 39.56  & 40.52  & 34.61  & \multirow{2}[4]{*}{0.18 } \\
%\cmidrule{3-21}          &       & 0.953  & 0.955  & 0.936  & -     & 0.958  & 0.944  & 0.977  & 0.978  & 0.979  & 0.967  & 0.953  & 0.964  & 0.961  & 0.948  & 0.966  & 0.957  & 0.969  & 0.980  & 0.952  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DIDN\cite{yu2019deep}} & 39.64  & 39.78  & 36.06  & -     & 37.36  & 38.24  & 40.74  & 41.68  & 42.35  & 41.17  & 38.15  & 37.87  & 38.27  & 38.58  & 40.03  & 40.32  & 39.73  & 44.07  & 35.28  & \multirow{2}[4]{*}{7.25 } \\
%\cmidrule{3-21}          &       & 0.953  & 0.958  & 0.946  & -     & 0.953  & 0.950  & 0.975  & 0.977  & 0.975  & 0.966  & 0.951  & 0.965  & 0.954  & 0.950  & 0.963  & 0.959  & 0.966  & 0.985  & 0.949  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DnCNN\cite{zhang2017beyond}} & 37.90  & 37.73  & 37.47  & 39.32  & 38.51  & 40.01  & 40.81  & 41.91  & 44.16  & 41.57  & 39.92  & 38.72  & 39.34  & 40.22  & 42.03  & 42.12  & 40.26  & 43.97  & 36.30  & \multirow{2}[4]{*}{3.23 } \\
%\cmidrule{3-21}          &       & 0.943  & 0.941  & 0.954  & 0.974  & 0.966  & 0.971  & 0.972  & 0.979  & 0.991  & 0.969  & 0.962  & 0.973  & 0.964  & 0.969  & 0.983  & 0.977  & 0.970  & 0.984  & 0.960  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DRUNet \cite{zhang2020plug}} & -     & -     & 38.30  & 40.33  & 38.93  & 40.77  & 41.94  & 42.62  & {\textbf{45.36}} & 42.78  & 40.35 & {\textbf{39.17}} & 40.80  & {\textbf{40.80}} & {\textbf{42.86}} & 42.86  & {\textbf{40.88}} & 45.76  & 36.61  & \multirow{2}[4]{*}{0.17} \\
%\cmidrule{3-21}          &       & -     & -     & 0.961  & 0.979  & 0.970  & 0.974  & 0.978  & 0.982  & {\textbf{0.993}} & 0.977  & 0.969 & {\textbf{0.975}} & 0.966  & 0.970  & {\textbf{0.985}} & 0.980  & {\textbf{0.974}} & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{DudeNet\cite{tian2021designing}} & 33.18  & 27.55  & 36.03  & 37.44  & 39.92  & 38.18  & 39.94  & 41.13  & 42.97  & 41.06  & 38.63  & 37.83  & 39.09  & 38.58  & 40.73  & 40.63  & 39.71  & 43.34  & 35.44  & \multirow{2}[4]{*}{0.18 } \\
%\cmidrule{3-21}          &       & 0.810  & 0.645  & 0.933  & 0.953  & 0.973  & 0.955  & 0.972  & 0.977  & 0.988  & 0.971  & 0.962  & 0.969  & 0.962  & 0.961  & 0.976  & 0.969  & 0.972  & 0.985  & 0.955  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{FCCF\cite{yue2019high}} & 36.30  & -  & {\textbf{39.02}} & {\textbf{40.89}} & 38.87  & {\textbf{41.20}} & {\textbf{42.03}} & 43.07  & 45.15  & {\textbf{42.80}} & 40.14  & 39.04  & 40.61  & 40.66  & 42.31  & 43.05  & {\textbf{40.88}} & 45.47  & {\textbf{36.72}} & \multirow{2}[4]{*}{11.20} \\
%\cmidrule{3-21}          &       & 0.885  & - & {\textbf{0.968}} & {\textbf{0.982}} & 0.971  & {\textbf{0.978}} & {\textbf{0.980}} & {\textbf{0.985}} & 0.993  & {\textbf{0.978}} & 0.966  & 0.974  & 0.967  & 0.969  & 0.984  & 0.982  & {\textbf{0.974}} & 0.989  & {\textbf{0.964}} &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{FFDNet\cite{zhang2018ffdnet}} & 37.61  & 38.27  & 37.67  & 39.73  & 38.76  & 40.28  & 41.67  & 42.55  & 44.77  & 42.44  & 40.05  & 38.96  & 40.60  & 40.50  & 42.43  & 42.44  & 40.75  & 45.71  & 36.47  & \multirow{2}[4]{*}{0.02} \\
%\cmidrule{3-21}          &       & 0.942  & 0.948  & 0.956  & 0.977  & 0.970  & 0.973  & 0.977  & 0.982  & 0.992  & 0.976  & 0.967  & 0.974  & 0.964  & 0.971  & 0.984  & 0.979  & 0.973  & 0.990  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{IDR\cite{zhang2022idr}} & -     & -     & 34.26  & 36.18  & 36.28  & 36.44  & 39.33  & 40.31  & 40.94  & 39.74  & 37.38  & 37.39  & 38.30  & 38.15  & 39.68  & 38.22  & 38.01  & 43.15  & 34.64  & \multirow{2}[4]{*}{0.32 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.877  & 0.923  & 0.925  & 0.910  & 0.955  & 0.962  & 0.961  & 0.935  & 0.927  & 0.957  & 0.938  & 0.944  & 0.951  & 0.913  & 0.941  & 0.978  & 0.929  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{InvDN\cite{liu2021invertible}} & 39.57  & 39.28  & 34.55  & 36.33  & 35.94  & 38.01  & 38.95  & 40.09  & 42.03  & 40.02  & 33.32  & 37.00  & 36.64  & 37.66  & 40.06  & 40.98  & 39.10  & 40.74  & 34.15  & \multirow{2}[4]{*}{0.74 } \\
%\cmidrule{3-21}          &       & 0.952  & 0.955  & 0.937  & 0.953  & 0.947  & 0.952  & 0.965  & 0.973  & 0.978  & 0.960  & 0.930  & 0.965  & 0.939  & 0.955  & 0.966  & 0.971  & 0.964  & 0.969  & 0.935  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{IRCNN\cite{zhang2017learning}} & 34.78  & 33.50  & 37.26  & 37.25  & 37.49  & 39.66  & 41.24  & 41.85  & 43.89  & 41.78  & 39.91  & 38.63  & 40.14  & 40.12  & 41.87  & 41.86  & 40.26  & 44.38  & 36.22  & \multirow{2}[4]{*}{2.15 } \\
%\cmidrule{3-21}          &       & 0.907  & 0.887  & 0.954  & 0.956  & 0.956  & 0.970  & 0.978  & 0.981  & 0.991  & 0.973  & 0.969  & 0.972  & 0.965  & 0.969  & 0.983  & 0.977  & 0.972  & 0.988  & 0.961  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{MIRNet\cite{Zamir2020MIRNet}} & 39.88  & 39.55  & 36.06  & 37.25  & 37.49  & 38.10  & 40.72  & 41.68  & 42.76  & 41.05  & 38.28  & 37.80  & 38.60  & 38.55  & 40.28  & 40.46  & 39.73  & 43.66  & 35.42  & \multirow{2}[4]{*}{0.71 } \\
%\cmidrule{3-21}          &       & 0.956  & 0.957  & 0.942  & 0.956  & 0.956  & 0.952  & 0.975  & 0.978  & 0.980  & 0.968  & 0.954  & 0.967  & 0.959  & 0.952  & 0.966  & 0.964  & 0.967  & 0.983  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{MPRNet\cite{zamir2021multi}} & 39.82  & 39.57  & 35.94  & -     & 37.50  & 38.04  & 40.59  & 41.30  & 42.59  & 41.23  & 38.35  & 37.92  & 38.95  & 38.62  & 40.21  & 40.20  & 39.77  & 44.05  & 35.49  & \multirow{2}[4]{*}{35.97 } \\
%\cmidrule{3-21}          &       & 0.954  & 0.958  & 0.935  & -     & 0.954  & 0.946  & 0.974  & 0.974  & 0.978  & 0.969  & 0.952  & 0.966  & 0.960  & 0.949  & 0.965  & 0.960  & 0.967  & 0.986  & 0.951  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{NAFNet\cite{chen2022simple}} & 38.36  & {\textbf{40.15}} & 34.39  & -     & 36.38  & 37.88  & 40.12  & 40.23  & 40.66  & 40.01  & 36.13  & 35.87  & 36.66  & 36.79  & 36.53  & 39.93  & 39.32  & 40.45  & 34.82  & \multirow{2}[4]{*}{0.35} \\
%\cmidrule{3-21}          &       & 0.943  & {\textbf{0.960}} & 0.923  & -     & 0.947  & 0.954  & 0.973  & 0.943  & 0.936  & 0.962  & 0.919  & 0.927  & 0.948  & 0.927  & 0.884  & 0.951  & 0.966  & 0.924  & 0.948  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{NBNet\cite{cheng2021nbnet}} & 39.89  & 39.64  & 35.89  & -     & 37.37  & 38.32  & 40.95  & 41.91  & 42.92  & 41.17  & 38.02  & 37.87  & 37.79  & 38.45  & 40.51  & 40.45  & 39.73  & 43.96  & 35.37  & \multirow{2}[4]{*}{0.12 } \\
%\cmidrule{3-21}          &       & 0.955  & 0.958  & 0.935  & -     & 0.957  & 0.955  & 0.977  & 0.980  & 0.982  & 0.971  & 0.955  & 0.967  & 0.956  & 0.955  & 0.972  & 0.967  & 0.969  & 0.984  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Neigh2Neigh\cite{huang2021neighbor2neighbor}} & -     & -     & 34.47  & 35.65  & 37.10  & 36.59  & 40.22  & 40.41  & 41.29  & 41.24  & 38.13  & 37.94  & 39.71  & 38.50  & 39.63  & 38.05  & 39.17  & 44.49  & 35.30  & \multirow{2}[4]{*}{2.48} \\
%\cmidrule{3-21}          &       & -     & -     & 0.883  & 0.907  & 0.942  & 0.908  & 0.967  & 0.960  & 0.966  & 0.958  & 0.940  & 0.961  & 0.956  & 0.936  & 0.952  & 0.919  & 0.958  & 0.984  & 0.944  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{NLNet\cite{lefkimmiatis2017non}} & -     & -     & 37.56  & 39.32  & 38.58  & 40.17  & 41.43  & 42.18  & 44.53  & 42.19  & 39.96  & 38.89  & 40.06  & 40.61  & 42.14  & 42.16  & 40.63  & 44.87  & 36.34  & \multirow{2}[4]{*}{39.06 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.955  & 0.974  & 0.968  & 0.973  & 0.976  & 0.981  & 0.991  & 0.974  & 0.969 & 0.973  & 0.964  & {\textbf{0.971}} & 0.983  & 0.978  & 0.973  & 0.988  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Noise2Noise\cite{lehtinen2018noise2noise}} & -     & -     & 33.55  & 34.67  & 35.91  & 35.28  & 38.88  & 39.07  & 39.34  & 39.26  & 36.81  & 36.99  & 38.04  & 37.21  & 38.00  & 36.35  & 37.67  & 42.59  & 34.44  & \multirow{2}[4]{*}{0.03 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.850  & 0.874  & 0.913  & 0.875  & 0.950  & 0.940  & 0.938  & 0.931  & 0.919  & 0.948  & 0.936  & 0.916  & 0.924  & 0.876  & 0.936  & 0.975  & 0.926  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{PD-Denoising\cite{zhou2020awgn}} & 38.40  & 33.99  & 35.85  & 37.13  & 37.13  & 37.12  & 40.85  & 41.38  & 41.13  & 41.05  & 37.72  & 37.57  & 39.03  & 38.01  & 39.18  & 39.64  & 38.80  & 43.73  & 35.05  & \multirow{2}[4]{*}{0.61 } \\
%\cmidrule{3-21}          &       & 0.943  & 0.896  & 0.924  & 0.944  & 0.944  & 0.921  & 0.974  & 0.974  & 0.966  & 0.959  & 0.935  & 0.956  & 0.948  & 0.929  & 0.948  & 0.946  & 0.955  & 0.981  & 0.940  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{PNGAN\cite{cai2021learning}} & 39.38  & 39.81  & 38.44  & -     & 39.57  & 40.51  & 41.79  & {\textbf{43.13}} & 44.73  & 42.55  & 39.84  & 38.78  & 40.63  & 40.20  & 41.85  & 43.15  & {\textbf{40.88}} & 45.32  & 36.40  & \multirow{2}[4]{*}{1.53} \\
%\cmidrule{3-21}          &       & 0.953  & 0.959  & 0.963  & -     & 0.974  & 0.974  & 0.979  & {\textbf{0.985}} & 0.992  & 0.977  & 0.964  & 0.970  & {\textbf{0.969}} & 0.962  & 0.981  & 0.982  & {\textbf{0.974}} & 0.988  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{R2R\cite{pang2021recorrupted}} & -     & 34.78     & 36.32  & 38.11  & 38.47  & 38.71  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{4481.98 } \\
%\cmidrule{3-21}          &       & -     & 0.844     & 0.937  & 0.961  & 0.965  & 0.958  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Restormer\cite{zamir2022restormer}} & {\textbf{40.03}} & 40.02  & 36.33  & -     & 37.66  & 38.29  & 41.10  & 41.84  & 42.49  & 41.47  & 38.42  & 38.08  & 39.05  & 38.77  & 40.13  & 40.53  & 39.56  & 44.19  & 35.65  & \multirow{2}[4]{*}{0.77} \\
%\cmidrule{3-21}          &       & {\textbf{0.956}} & {\textbf{0.960}}  & 0.941  & -     & 0.956  & 0.948  & 0.977  & 0.979  & 0.976  & 0.968  & 0.952  & 0.966  & 0.960  & 0.949  & 0.963  & 0.962  & 0.963  & 0.986  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{RIDNet\cite{anwar2019real}} & 39.26  & 38.70  & 36.84  & 38.11  & 38.57  & 38.60  & 41.09  & 42.15  & 42.39  & 41.59  & 38.88  & 38.21  & 38.67  & 39.02  & 40.91  & 41.01  & 40.07  & 44.40  & 35.76  & \multirow{2}[4]{*}{0.11 } \\
%\cmidrule{3-21}          &       & 0.953  & 0.950  & 0.941  & 0.961  & 0.970  & 0.956  & 0.977  & 0.980  & 0.989  & 0.975  & 0.962  & 0.970  & 0.963  & 0.959  & 0.978  & 0.977  & 0.972  & 0.987  & 0.957  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{SADNet\cite{chang2020spatial}} & 39.59  & -     & 37.76  & 38.11  & 39.22  & 38.90  & 40.82  & 42.02  & 44.25  & 41.85  & 39.53  & 38.33  & 39.83  & 39.69  & 39.81  & 41.64  & 40.70  & 44.61  & 36.36  & \multirow{2}[4]{*}{0.04 } \\
%\cmidrule{3-21}          &       & 0.952  & -     & 0.952  & 0.961  & 0.972  & 0.965  & 0.976  & 0.980  & 0.992  & 0.975  & 0.965  & 0.970  & 0.965  & 0.963  & 0.965  & 0.979  & {\textbf{0.974}} & 0.988  & 0.962  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{SASL\cite{li2023spatially}} & 38.00  &  37.41   & 34.93  &  -  & 37.13  & 38.24  & 40.04  & 41.86  & 43.07  & 40.29  & 37.22  & 37.38  & 36.45  & 37.64  & 40.85  & 41.64  & 39.10  & 42.89  & 34.25  & \multirow{2}[4]{*}{0.06 } \\
%\cmidrule{3-21}          &       & 0.936  &  0.934  & 0.936  & -  & 0.954  & 0.964  & 0.966  & 0.982  & 0.987  & 0.963  & 0.947  & 0.965  & 0.933  & 0.958  & 0.977  & 0.976  & 0.965  & 0.980  & 0.930  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{SCUNet\cite{zhang2022practical}} & 38.96     & 35.31     & 37.44  & 39.29  & 38.08  & 39.47  & 40.96  & 42.24  & 44.02  & 41.93  & {\textbf{40.74}}  & 38.75  & 39.97  & 40.37  & 41.79  & 42.61  & 40.64  & 44.24  & 36.13  & \multirow{2}[4]{*}{0.62} \\
%\cmidrule{3-21}          &       & 0.953   & 0.901   & 0.958  & 0.972  & 0.962  & 0.971  & 0.972  & 0.980  & 0.991  & 0.966  & {\textbf{0.974}}  & 0.971  & 0.968  & 0.975  & 0.970  & 0.978  & 0.973  & 0.981  & 0.956  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Self2Self\cite{quan2020self2self}} & -     & -     & 36.26  & 38.23  & -     & 39.49  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{4100.76 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.947  & 0.969  & -     & 0.963  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{UDnet \cite{lefkimmiatis2018universal}} & -     & -     & 36.95  & 38.96  & 38.05  & 39.62  & 40.40  & 41.36  & 43.58  & 41.12  & 39.35  & 38.25  & 38.94  & 39.95  & 41.32  & 41.70  & 39.51  & 43.17  & 36.09  & \multirow{2}[4]{*}{3.68 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.943  & 0.971  & 0.962  & 0.968  & 0.968  & 0.977  & 0.989  & 0.968  & 0.963  & 0.971  & 0.959  & 0.968  & 0.979  & 0.974  & 0.966  & 0.981  & 0.958  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{Uformer\cite{Wang_2022_CVPR}} & {\textbf{40.05}}  & 39.74  & 35.97  & -  & 37.44  & 38.12  & 40.83  & 41.37  & 42.45  & 41.35  & 38.36  & 37.83  & 38.95  & 38.69  & 40.30  & 40.36  & 39.69  & 43.93  & 35.50  & \multirow{2}[4]{*}{1.46} \\
%\cmidrule{3-21}          &       & {\textbf{0.956}}  & 0.958  & 0.941  & -  & 0.956  & 0.950  & 0.976  & 0.977  & 0.978  & 0.968  & 0.954  & 0.966  & 0.960  & 0.953  & 0.966  & 0.964  & 0.967  & 0.985  & 0.953  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{VDIR \cite{soh2022variational}} & 39.63     & 39.26  & 34.90  & 36.51  & 37.01  & 36.84  & 40.84  & 41.40  & 41.29  & 40.81  & 37.65  & 37.84  & 39.09  & 38.17  & 39.20  & 39.41  & 38.98  & 44.40  & 35.04  & \multirow{2}[4]{*}{2.03 } \\
%\cmidrule{3-21}          &       & 0.953     & 0.955  & 0.894  & 0.925  & 0.940  & 0.911  & 0.973  & 0.970  & 0.965  & 0.953  & 0.936  & 0.960  & 0.951  & 0.931  & 0.946  & 0.938  & 0.956  & 0.985  & 0.939  &  \\
%\cmidrule{2-22}          & \multirow{2}[4]{*}{VDNet\cite{yue2019variational}} & -     & -     & 35.86  & -     & 37.58  & 38.43  & 40.97  & 42.37  & 43.08  & 41.19  & 38.23  & 37.95  & 37.88  & 38.60  & 40.81  & 41.21  & 39.93  & 44.27  & 35.49  & \multirow{2}[4]{*}{0.05 } \\
%\cmidrule{3-21}          &       & -     & -     & 0.945  & -     & 0.957  & 0.955  & 0.976  & 0.983  & 0.983  & 0.970  & 0.956  & 0.968  & 0.956  & 0.956  & 0.973  & 0.970  & 0.970  & 0.984  & 0.953  &  \\
%    \bottomrule
%    \end{tabular}%
% }
%  \label{Table_Results_Color_image_all}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'All in One-Supplementary'
\begin{table*}[htbp]
\centering
    \caption{Average PSNR, SSIM values on real-world color image datasets. The average time is calculated based on the PolyU dataset. `-' means the results are not available. `C: CANON', `F: FUJIFILM', `H: HUAWEI', `I: IPHONE', 'N: NIKON', `O: OPPO', `S: SONY', `X: XIAOMI'. Results marked with $\ast$ are from the original papers or the official websites.}
    \vspace{-9pt}
    \renewcommand{\arraystretch}{0.2818}
    \scalebox{0.5399}{
    \begin{tabular}{ccccccccccccccccccccccc}
    \toprule
    \multicolumn{3}{c}{\multirow{2}[4]{*}{Methods/Models}} & \multirow{2}[4]{*}{DnD} & \multirow{2}[4]{*}{SIDD} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multirow{2}[4]{*}{HighISO} & \multicolumn{13}{c}{IOCI}                                                                             & \multirow{3}[6]{*}{Time (s)} \\
\cmidrule{10-22}    \multicolumn{3}{c}{}  &       &       &       &       &       &       & C-100D & C-600D & C-5DMark4 & F-X100T & H-Honor6X & H-Mate40Pro & I-5S & I-6S & I-13 & N-D5300 & O-R11s & S-A6500 & X-MI8 \\
\cmidrule{1-22}    Category     & Schemes & \# Images & 1000  & 1280  & 15    & 60    & 100   & 100   & 55    & 25    & 83    & 71    & 30    & 126   & 36    & 67    & 174   & 56    & 39    & 36    & 50    &  \\
    \midrule
    \multirow{66}[52]{*}{\shortstack[c]{Traditional \\ denoisers}} & \multirow{39}[32]{*}{Matrix} & \multirow{2}[4]{*}{Bitonic \cite{treece2022real}} & 37.85  & 36.67  & 35.22  & 35.98  & 36.64  & 37.37  & 39.38  & 39.63  & 40.76  & 41.05  & 37.71  & 37.41  & 38.98  & 38.04  & 39.09  & 39.22  & 38.87  & 43.25  & 34.92  & \multirow{2}[4]{*}{2.57} \\
\cmidrule{4-22}          &       &       & 0.936  & 0.933  & 0.925  & 0.931  & 0.940  & 0.943  & 0.959  & 0.952  & 0.965  & 0.964  & 0.940  & 0.956  & 0.947  & 0.939  & 0.952  & 0.954  & 0.959  & 0.979  & 0.941  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{GID\cite{xu2018external}} & 34.32  & 27.16  & 37.17  & 38.41  & 38.37  & 39.63  & 40.86  & 41.60  & 44.11  & 42.31  & 39.52  & 38.66  & 40.12  & 40.16  & 41.50  & 41.09  & 40.50  & 44.96  & 36.11  & \multirow{2}[4]{*}{49.99} \\
\cmidrule{4-22}          &       &       & 0.817  & 0.634  & 0.946  & 0.963  & 0.967  & 0.967  & 0.974  & 0.979  & 0.989  & 0.975  & 0.965  & 0.972  & 0.964  & 0.967  & 0.979  & 0.973  & 0.973  & 0.989  & 0.960  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{LSCD \cite{rizkinia2016local}} & -     & -     & 36.20  & 37.69  & 37.97  & 38.64  & 40.65  & 41.45  & -     & -     & 39.22  & -     & 39.84  & 39.53  & -     & 40.83  & -     & 44.34  & 35.86  & \multirow{2}[4]{*}{3.19} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.942  & 0.963  & 0.964  & 0.962  & 0.973  & 0.979  & -     & -     & 0.963  & -     & 0.963  & 0.963  & -     & 0.973  & -     & 0.987  & 0.957  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{MCWNNM \cite{xu2017multi}} & 37.38$^\ast$  & -  & 37.02  & 38.54  & 38.26  & 39.89  & 41.47  & 42.07  & 44.22  & 42.48  & 39.46  & 38.78  & 39.87  & 40.18  & 41.33  & 41.74  & 40.71  & 45.38  & 35.84  & \multirow{2}[4]{*}{237.57} \\
\cmidrule{4-22}          &       &       & 0.929$^\ast$  & -  & 0.950  & 0.967  & 0.965  & 0.970  & 0.977  & 0.979  & 0.988  & 0.976  & 0.961  & 0.971  & 0.957  & 0.963  & 0.976  & 0.975  & 0.973  & 0.990  & 0.952  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{M-SVD} & 37.45  & 33.51  & 37.63  & 39.36  & 38.57  & 40.27  & 41.81  & 42.55  & 44.39  & 42.68  & 39.99  & 38.93  & 40.78  & 40.52  & 41.72  & 42.18  & 40.73  & 45.71  & 36.37  & \multirow{2}[4]{*}{104.24} \\
\cmidrule{4-22}          &       &       & 0.924  & 0.867  & 0.954  & 0.971  & 0.967  & 0.971  & 0.979  & 0.983  & 0.989  & 0.976  & 0.967  & 0.973  & 0.969  & 0.969  & 0.977  & 0.977  & 0.974  & 0.990  & 0.961  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{NLHCC\cite{hou2020nlh}} & 38.85  & 35.31  & 38.49  & 39.86  & 38.36  & 40.29  & 41.77  & 42.72  & 43.66  & {\textbf{42.80}} & 38.84  & 38.31  & 40.44  & 39.94  & 41.13  & {\textbf{43.25}} & -     & {\textbf{46.02}} & 35.73  & \multirow{2}[4]{*}{40.32} \\
\cmidrule{4-22}          &       &       & 0.953  & 0.930  & 0.965  & 0.976  & 0.965  & 0.971  & 0.979  & 0.984  & 0.986  & {\textbf{0.978}} & 0.959  & 0.968  & 0.964  & 0.963  & 0.976  & {\textbf{0.981}} & -     & {\textbf{0.991}} & 0.955  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{TWSC\cite{xu2018trilateral}} & 37.96$^\ast$  & -     & 37.90  & 39.66  & 38.62  & 40.62  & 41.65  & 42.52  & 44.94  & 42.26  & 38.71  & 38.81  & 38.77  & 40.12  & 41.71  & 42.23  & 40.65  & 45.49  & 35.40  & \multirow{2}[4]{*}{350.30} \\
\cmidrule{4-22}          &       &       & 0.942$^\ast$  & -     & 0.959  & 0.976  & 0.967  & 0.975  & 0.977  & 0.982  & 0.992  & 0.973  & 0.945  & 0.972  & 0.938  & 0.962  & 0.980  & 0.975  & 0.972  & 0.990  & 0.939  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{WTR1\cite{wu2018weighted}} & -     & -     & 37.80  & 37.32  & 38.20  & 38.19  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{600.33} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.958  & 0.944  & 0.965  & 0.940  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
\cmidrule{2-23}          & \multirow{26}[20]{*}{Tensor} & \multirow{2}[4]{*}{4DHOSVD\cite{rajwade2012image}} & 37.58  & 34.49  & 37.52  & 39.15  & 38.54  & 40.27  & 41.40  & 42.19  & 44.49  & 42.60  & 39.82  & 38.88  & 40.59  & 40.37  & 41.75  & 41.82  & 40.71  & 45.58  & 36.27  & \multirow{2}[4]{*}{123.06} \\
\cmidrule{4-22}          &       &       & 0.929  & 0.911  & 0.956  & 0.973  & 0.968  & 0.973  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.965  & 0.967  & 0.980  & 0.977  & 0.974  & 0.990  & 0.961  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{CBM3D1\cite{dabov2007image}} & 38.04  & 35.00  & 37.58  & 39.21  & 38.60  & 40.11  & 41.58  & 42.40  & 44.43  & 42.53  & 39.93  & 38.84  & 40.56  & 40.41  & 41.93  & 42.29  & 40.62  & 45.58  & 36.24  & \multirow{2}[4]{*}{1.02} \\
\cmidrule{4-22}          &       &       & 0.938  & 0.925  & 0.955  & 0.971  & 0.969  & 0.972  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.967  & {\textbf{0.970}} & 0.982  & 0.979  & 0.973  & 0.990  & 0.959  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{CBM3D2\cite{dabov2007image}} & 37.73  & 34.74  & 37.70  & 39.41  & 38.69  & 40.35  & 41.69  & 42.54  & 44.74  & 42.65  & 39.97  & 38.97  & 40.77  & 40.55  & 42.03  & 42.20  & 40.75  & 45.72  & 36.38  & \multirow{2}[4]{*}{2.94} \\
\cmidrule{4-22}          &       &       & 0.934  & 0.922  & 0.957  & 0.975  & 0.970  & 0.974  & 0.978  & 0.984  & 0.992  & 0.977  & 0.967  & 0.974  & 0.967  & 0.969  & 0.983  & 0.979  & 0.974  & 0.990  & 0.961  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{CMSt-SVD\cite{kong2019color}} & 38.25  & 34.38  & 37.95  & 39.76  & 38.85  & 40.49  & 41.99  & 42.75  & 44.65  & 42.68  & 40.08  & 38.95  & {\textbf{40.84}} & 40.53  & 42.06  & 42.72  & {\textbf{40.88}} & 45.91  & 36.40  & \multirow{2}[4]{*}{4.95} \\
\cmidrule{4-22}          &       &       & 0.940  & 0.900  & 0.959  & 0.976  & 0.971  & 0.974  & 0.979  & 0.984  & 0.991  & 0.977  & 0.967  & 0.973  & 0.967  & 0.967  & 0.982  & 0.980  & {\textbf{0.974}} & 0.991  & 0.962  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{LLRT\cite{chang2017hyper}} & 35.45  & 30.74  & 37.77  & 39.76  & 38.28  & 39.59  & 41.60  & 42.24  & 42.68  & 42.22  & 37.91  & 38.80  & 38.01  & 39.87  & 42.02  & 41.76  & 38.69  & 45.17  & 35.71  & \multirow{2}[4]{*}{285.62} \\
\cmidrule{4-22}          &       &       & 0.897  & 0.766  & 0.957  & 0.977  & 0.970  & 0.972  & 0.977  & 0.983  & 0.992  & 0.975  & 0.969  & 0.973  & 0.965  & 0.971  & 0.984  & 0.979  & 0.972  & 0.989  & 0.962  &  \\
    \midrule
    \midrule
    \multirow{218}[148]{*}{\shortstack[c]{DNN \\ methods}} & \multirow{216}[124]{*}{Supervised} & \multirow{2}[4]{*}{AINDNet\cite{Kim_2020_CVPR}} & 39.77  & 39.08  & 36.14  & 37.19  & 37.33  & 38.00  & 38.54  & 39.33  & 39.49  & 38.50  & 36.53  & 36.24  & 36.93  & 36.83  & 37.27  & 38.11  & 37.44  & 40.17  & 34.65  & \multirow{2}[4]{*}{0.33} \\
\cmidrule{4-22}          &       &       & 0.959  & 0.953  & 0.935  & 0.949  & 0.954  & 0.946  & 0.975  & 0.976  & 0.979  & 0.966  & 0.954  & 0.965  & 0.958  & 0.953  & 0.964  & 0.961  & 0.968  & 0.981  & 0.953  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{BRDNet\cite{tian2020image}} & 33.80  & -     & 37.27  & 39.16  & 38.04  & 39.64  & 39.85  & 40.95  & 43.54  & 40.27  & 39.48  & 38.66  & 38.19  & 40.07  & 41.92  & 41.34  & 39.66  & 42.76  & 36.08  & \multirow{2}[4]{*}{14.66} \\
\cmidrule{4-22}          &       &       & 0.897  & -     & 0.953  & 0.974  & 0.960  & 0.969  & 0.965  & 0.974  & 0.989  & 0.958  & 0.958  & 0.973  & 0.943  & 0.969  & 0.981  & 0.972  & 0.965  & 0.979  & 0.953  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{CBDNet\cite{guo2019toward}} & 38.06  & 33.26  & 36.20  & 37.67  & 37.81  & 38.18  & 41.43  & 42.41  & 42.55  & 41.88  & 38.35  & 38.17  & 39.80  & 39.07  & 40.63  & 40.92  & 39.54  & 44.38  & 35.54  & \multirow{2}[4]{*}{0.04} \\
\cmidrule{4-22}          &       &       & 0.942  & 0.869  & 0.919  & 0.940  & 0.956  & 0.942  & 0.977  & 0.981  & 0.980  & 0.971  & 0.946  & 0.964  & 0.960  & 0.951  & 0.968  & 0.963  & 0.965  & 0.981  & 0.950  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{CycleISP\cite{zamir2020cycleisp}} & 39.57  & 39.42  & 35.40  & 36.87  & 37.61  & 37.70  & 41.26  & 41.84  & 42.64  & 41.59  & 38.47  & 38.01  & 38.79  & 38.67  & 40.61  & 40.03  & 39.86  & 44.75  & 35.54  & \multirow{2}[4]{*}{0.26} \\
\cmidrule{4-22}          &       &       & 0.955  & 0.956  & 0.916  & 0.939  & 0.955  & 0.936  & 0.977  & 0.977  & 0.978  & 0.969  & 0.952  & 0.966  & 0.961  & 0.952  & 0.970  & 0.953  & 0.968  & 0.987  & 0.949  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{DANet\cite{yue2020dual}} & 39.55  & 39.43  & 37.17  & 38.63  & {\textbf{41.49}} & 38.92  & 41.59  & 42.59  & 42.83  & 41.70  & 37.91  & 38.17  & 39.23  & 38.74  & 41.58  & 41.54  & 39.58  & 44.03  & 36.21  & \multirow{2}[4]{*}{0.02} \\
\cmidrule{4-22}          &       &       & 0.953  & 0.956  & 0.953  & 0.969  & {\textbf{0.977}} & 0.960  & 0.979  & 0.985  & 0.979  & 0.977  & 0.963  & 0.970  & 0.964  & 0.962  & 0.980  & 0.976  & 0.972  & 0.989  & 0.961  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{DBF\cite{chen2019real}} & -     & -     & 38.48  & 40.59  & 38.87  & 40.09  & 41.56  & 42.87  & 44.85  & 42.36  & 39.98  & 38.86  & 40.17  & 40.26  & 42.12  & 43.17  & 40.67  & 44.75  & 36.45  & \multirow{2}[4]{*}{0.34} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.960  & 0.981  & 0.970  & 0.970  & 0.979  & 0.984  & 0.992  & 0.975  & 0.967  & 0.972  & 0.966  & 0.966  & 0.982  & 0.982  & 0.973  & 0.987  & 0.963  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{DCDicL\cite{zheng2021deep}} & 35.86  & -     & 36.61  & -     & 37.45  & 38.12  & 37.77  & 38.24  & 38.39  & 38.62  & 35.87  & 36.07  & 35.83  & 36.25  & 39.84  & 39.38  & 37.04  & 40.24  & 34.72  & \multirow{2}[4]{*}{1.24} \\
\cmidrule{4-22}          &       &       & 0.918  & -     & 0.945  & -     & 0.972  & 0.965  & 0.970  & 0.977  & 0.990  & 0.968  & 0.968  & 0.975  & 0.956  & 0.971  & 0.984  & 0.976  & 0.969  & 0.980  & 0.955  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{DeamNet\cite{ren2021adaptive}} & 39.63  & 39.35  & 36.63  & -     & 37.70  & 36.93  & 40.90  & 40.86  & 41.22  & 39.72  & 33.67  & 36.40  & 37.87  & 35.07  & 40.25  & 38.92  & 39.56  & 40.52  & 34.61  & \multirow{2}[4]{*}{0.18} \\
\cmidrule{4-22}          &       &       & 0.953  & 0.955  & 0.936  & -     & 0.958  & 0.944  & 0.977  & 0.978  & 0.979  & 0.967  & 0.953  & 0.964  & 0.961  & 0.948  & 0.966  & 0.957  & 0.969  & 0.980  & 0.952  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{DIDN\cite{yu2019deep}} & 39.64  & 39.78  & 36.06  & -     & 37.36  & 38.24  & 40.74  & 41.68  & 42.35  & 41.17  & 38.15  & 37.87  & 38.27  & 38.58  & 40.03  & 40.32  & 39.73  & 44.07  & 35.28  & \multirow{2}[4]{*}{7.25} \\
\cmidrule{4-22}          &       &       & 0.953  & 0.958  & 0.946  & -     & 0.953  & 0.950  & 0.975  & 0.977  & 0.975  & 0.966  & 0.951  & 0.965  & 0.954  & 0.950  & 0.963  & 0.959  & 0.966  & 0.985  & 0.949  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{DnCNN\cite{zhang2017beyond}} & 37.90$^\ast$  & 37.73$^\ast$  & 37.47  & 39.32  & 38.51  & 40.01  & 40.81  & 41.91  & 44.16  & 41.57  & 39.92  & 38.72  & 39.34  & 40.22  & 42.03  & 42.12  & 40.26  & 43.97  & 36.30  & \multirow{2}[4]{*}{3.23} \\
\cmidrule{4-22}          &       &       & 0.943$^\ast$  & 0.941$^\ast$  & 0.954  & 0.974  & 0.966  & 0.971  & 0.972  & 0.979  & 0.991  & 0.969  & 0.962  & 0.973  & 0.964  & 0.969  & 0.983  & 0.977  & 0.970  & 0.984  & 0.960  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{DRUNet\cite{zhang2020plug}} & -     & -     & 38.30  & 40.33  & 38.93  & 40.77  & 41.94  & 42.62  & {\textbf{45.36}} & 42.78  & {\textbf{40.35}} & {\textbf{39.17}} & 40.80  & {\textbf{40.80}} & {\textbf{42.86}} & 42.86  & {\textbf{40.88}} & 45.76  & 36.61  & \multirow{2}[4]{*}{0.17} \\
\cmidrule{4-22}          &       &       & -     & -    & 0.961  & 0.979  & 0.970  & 0.974  & 0.978  & 0.982  & {\textbf{0.993}} & 0.977  & {\textbf{0.969}} & {\textbf{0.975}} & 0.966  & {\textbf{0.970}}  & {\textbf{0.985}} & 0.980  & {\textbf{0.974}} & 0.990  & 0.961  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{DudeNet\cite{tian2021designing}} & 33.18  & 27.55  & 36.03  & 37.44  & 39.92  & 38.18  & 39.94  & 41.13  & 42.97  & 41.06  & 38.63  & 37.83  & 39.09  & 38.58  & 40.73  & 40.63  & 39.71  & 43.34  & 35.44  & \multirow{2}[4]{*}{0.18} \\
\cmidrule{4-22}          &       &       & 0.810  & 0.645  & 0.933  & 0.953  & 0.973  & 0.955  & 0.972  & 0.977  & 0.988  & 0.971  & 0.962  & 0.969  & 0.962  & 0.961  & 0.976  & 0.969  & 0.972  & 0.985  & 0.955  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{FCCF\cite{yue2019high}} & 36.30  & 23.32  & {\textbf{39.02}} & {\textbf{40.89}} & 38.87  & {\textbf{41.20}} & {\textbf{42.03}} & 43.07  & 45.15  & {\textbf{42.80}} & 40.14  & 39.04  & 40.61  & 40.66  & 42.31  & 43.05  & {\textbf{40.88}} & 45.47  & {\textbf{36.72}} & \multirow{2}[4]{*}{11.20} \\
\cmidrule{4-22}          &       &       & 0.885  & 0.461  & {\textbf{0.968}} & {\textbf{0.982}} & 0.971  & {\textbf{0.978}} & {\textbf{0.980}} & {\textbf{0.985}} & 0.993  & {\textbf{0.978}} & 0.966  & 0.974  & 0.967  & 0.969  & 0.984  & 0.982  & {\textbf{0.974}} & 0.989  & {\textbf{0.964}} &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{FFDNet\cite{zhang2018ffdnet}} & 37.61$^\ast$  & 38.27$^\ast$  & 37.67  & 39.73  & 38.76  & 40.28  & 41.67  & 42.55  & 44.77  & 42.44  & 40.05  & 38.96  & 40.60  & 40.50  & 42.43  & 42.44  & 40.75  & 45.71  & 36.47  & \multirow{2}[4]{*}{0.02} \\
\cmidrule{4-22}          &       &       & 0.942$^\ast$  & 0.948$^\ast$  & 0.956  & 0.977  & 0.970  & 0.973  & 0.977  & 0.982  & 0.992  & 0.976  & 0.967  & 0.974  & 0.964  & 0.971  & 0.984  & 0.979  & 0.973  & 0.990  & 0.961  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{InvDN\cite{liu2021invertible}} & 39.57  & 39.28  & 34.55  & 36.33  & 35.94  & 38.01  & 38.95  & 40.09  & 42.03  & 40.02  & 33.32  & 37.00  & 36.64  & 37.66  & 40.06  & 40.98  & 39.10  & 40.74  & 34.15  & \multirow{2}[4]{*}{0.74} \\
\cmidrule{4-22}          &       &       & 0.952  & 0.955  & 0.937  & 0.953  & 0.947  & 0.952  & 0.965  & 0.973  & 0.978  & 0.960  & 0.930  & 0.965  & 0.939  & 0.955  & 0.966  & 0.971  & 0.964  & 0.969  & 0.935  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{IRCNN\cite{zhang2017learning}} & 34.78  & 33.50  & 37.26  & 37.25  & 37.49  & 39.66  & 41.24  & 41.85  & 43.89  & 41.78  & 39.91  & 38.63  & 40.14  & 40.12  & 41.87  & 41.86  & 40.26  & 44.38  & 36.22  & \multirow{2}[4]{*}{2.15} \\
\cmidrule{4-22}          &       &       & 0.907  & 0.887  & 0.954  & 0.956  & 0.956  & 0.970  & 0.978  & 0.981  & 0.991  & 0.973  & 0.969  & 0.972  & 0.965  & 0.969  & 0.983  & 0.977  & 0.972  & 0.988  & 0.961  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{MIRNet\cite{Zamir2020MIRNet}} & 39.88  & 39.55  & 36.06  & 37.25  & 37.49  & 38.10  & 40.72  & 41.68  & 42.76  & 41.05  & 38.28  & 37.80  & 38.60  & 38.55  & 40.28  & 40.46  & 39.73  & 43.66  & 35.42  & \multirow{2}[4]{*}{0.71} \\
\cmidrule{4-22}          &       &       & 0.956  & 0.957  & 0.942  & 0.956  & 0.956  & 0.952  & 0.975  & 0.978  & 0.980  & 0.968  & 0.954  & 0.967  & 0.959  & 0.952  & 0.966  & 0.964  & 0.967  & 0.983  & 0.953  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{MPRNet\cite{zamir2021multi}} & 39.82  & 39.57  & 35.94  & -     & 37.50  & 38.04  & 40.59  & 41.30  & 42.59  & 41.23  & 38.35  & 37.92  & 38.95  & 38.62  & 40.21  & 40.20  & 39.77  & 44.05  & 35.49  & \multirow{2}[4]{*}{35.97} \\
\cmidrule{4-22}          &       &       & 0.954  & 0.958  & 0.935  & -     & 0.954  & 0.946  & 0.974  & 0.974  & 0.978  & 0.969  & 0.952  & 0.966  & 0.960  & 0.949  & 0.965  & 0.960  & 0.967  & 0.986  & 0.951  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{NAFNet\cite{chen2022simple}} & 38.36  & {\textbf{40.15}} & 34.39  & -     & 36.38  & 37.88  & 40.12  & 40.23  & 40.66  & 40.01  & 36.13  & 35.87  & 36.66  & 36.79  & 36.53  & 39.93  & 39.32  & 40.45  & 34.82  & \multirow{2}[4]{*}{0.35} \\
\cmidrule{4-22}          &       &       & 0.943  & {\textbf{0.960}} & 0.923  & -     & 0.947  & 0.954  & 0.973  & 0.943  & 0.936  & 0.962  & 0.919  & 0.927  & 0.948  & 0.927  & 0.884  & 0.951  & 0.966  & 0.924  & 0.948  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{NBNet\cite{cheng2021nbnet}} & 39.89  & 39.64  & 35.89  & -     & 37.37  & 38.32  & 40.95  & 41.91  & 42.92  & 41.17  & 38.02  & 37.87  & 37.79  & 38.45  & 40.51  & 40.45  & 39.73  & 43.96  & 35.37  & \multirow{2}[4]{*}{0.12} \\
\cmidrule{4-22}          &       &       & 0.955  & 0.958  & 0.935  & -     & 0.957  & 0.955  & 0.977  & 0.980  & 0.982  & 0.971  & 0.955  & 0.967  & 0.956  & 0.955  & 0.972  & 0.967  & 0.969  & 0.984  & 0.953  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{NLNet\cite{lefkimmiatis2017non}} & -     & -     & 37.56  & 39.32  & 38.58  & 40.17  & 41.43  & 42.18  & 44.53  & 42.19  & 39.96  & 38.89  & 40.06  & 40.61  & 42.14  & 42.16  & 40.63  & 44.87  & 36.34  & \multirow{2}[4]{*}{39.06} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.955  & 0.974  & 0.968  & 0.973  & 0.976  & 0.981  & 0.991  & 0.974  & {\textbf{0.969}} & 0.973  & 0.964  & {\textbf{0.971}} & 0.983  & 0.978  & 0.973  & 0.988  & 0.962  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{PD-Denoising\cite{zhou2020awgn}} & 38.40  & 33.99  & 35.85  & 37.13  & 37.13  & 37.12  & 40.85  & 41.38  & 41.13  & 41.05  & 37.72  & 37.57  & 39.03  & 38.01  & 39.18  & 39.64  & 38.80  & 43.73  & 35.05  & \multirow{2}[4]{*}{0.61} \\
\cmidrule{4-22}          &       &       & 0.943  & 0.896  & 0.924  & 0.944  & 0.944  & 0.921  & 0.974  & 0.974  & 0.966  & 0.959  & 0.935  & 0.956  & 0.948  & 0.929  & 0.948  & 0.946  & 0.955  & 0.981  & 0.940  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{PNGAN\cite{cai2021learning}} & 39.38  & 39.81  & 38.44  & -     & 39.57  & 40.51  & 41.79  & {\textbf{43.13}} & 44.73  & 42.55  & 39.84  & 38.78  & 40.63  & 40.20  & 41.85  & 43.15  & {\textbf{40.88}} & 45.32  & 36.40  & \multirow{2}[4]{*}{1.53} \\
\cmidrule{4-22}          &       &       & 0.953  & 0.959  & 0.963  & -     & 0.974  & 0.974  & 0.979  & {\textbf{0.985}} & 0.992  & 0.977  & 0.964  & 0.970  & {\textbf{0.969}} & 0.962  & 0.981  & 0.982  & \textbf{0.974} & 0.988  & 0.962  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{Restormer\cite{zamir2022restormer}} & {\textbf{40.03}} & 40.02  & 36.33  & -     & 37.66  & 38.29  & 41.10  & 41.84  & 42.49  & 41.47  & 38.42  & 38.08  & 39.05  & 38.77  & 40.13  & 40.53  & 39.56  & 44.19  & 35.65  & \multirow{2}[4]{*}{0.77} \\
\cmidrule{4-22}          &       &       & {\textbf{0.956}} & 0.960  & 0.941  & -     & 0.956  & 0.948  & 0.977  & 0.979  & 0.976  & 0.968  & 0.952  & 0.966  & 0.960  & 0.949  & 0.963  & 0.962  & 0.963  & 0.986  & 0.953  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{RIDNet\cite{anwar2019real}} & 39.26  & 38.70  & 36.84  & 38.11  & 38.57  & 38.60  & 41.09  & 42.15  & 42.39  & 41.59  & 38.88  & 38.21  & 38.67  & 39.02  & 40.91  & 41.01  & 40.07  & 44.40  & 35.76  & \multirow{2}[4]{*}{0.11} \\
\cmidrule{4-22}          &       &       & 0.953  & 0.950  & 0.941  & 0.961  & 0.970  & 0.956  & 0.977  & 0.980  & 0.989  & 0.975  & 0.962  & 0.970  & 0.963  & 0.959  & 0.978  & 0.977  & 0.972  & 0.987  & 0.957  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{SADNet\cite{chang2020spatial}} & 39.59$^\ast$  & -     & 37.76  & 38.11  & 39.22  & 38.90  & 40.82  & 42.02  & 44.25  & 41.85  & 39.53  & 38.33  & 39.83  & 39.69  & 39.81  & 41.64  & 40.70  & 44.61  & 36.36  & \multirow{2}[4]{*}{0.04} \\
\cmidrule{4-22}          &       &       & 0.952$^\ast$  & -     & 0.952  & 0.961  & 0.972  & 0.965  & 0.976  & 0.980  & 0.992  & 0.975  & 0.965  & 0.970  & 0.965  & 0.963  & 0.965  & 0.979  & {\textbf{0.974}} & 0.988  & 0.962  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{SCUNet\cite{zhang2022practical}} & -     & -     & 37.44  & 39.29  & 38.08  & 39.47  & 40.96  & 42.24  & 44.02  & 41.93  & 40.74  & 38.75  & 39.97  & 40.37  & 41.79  & 42.61  & 40.64  & 44.24  & 36.13  & \multirow{2}[4]{*}{0.62} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.958  & 0.972  & 0.962  & 0.971  & 0.972  & 0.980  & 0.991  & 0.966  & 0.974  & 0.971  & 0.967  & 0.975  & 0.970  & 0.978  & 0.973  & 0.981  & 0.956  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{Uformer\cite{Wang_2022_CVPR}} & 40.05  & 39.74  & 35.97  & -     & 37.44  & 38.12  & 40.83  & 41.37  & 42.45  & 41.35  & 38.36  & 37.83  & 38.95  & 38.69  & 40.30  & 40.36  & 39.69  & 43.93  & 35.50  & \multirow{2}[4]{*}{1.46} \\
\cmidrule{4-22}          &       &       & 0.956  & 0.958  & 0.941  & -     & 0.956  & 0.950  & 0.976  & 0.977  & 0.978  & 0.968  & 0.954  & 0.966  & 0.960  & 0.953  & 0.966  & 0.964  & 0.967  & 0.985  & 0.953  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{UDNet\cite{lefkimmiatis2018universal}} & -     & -     & 36.95  & 38.96  & 38.05  & 39.62  & 40.40  & 41.36  & 43.58  & 41.12  & 39.35  & 38.25  & 38.94  & 39.95  & 41.32  & 41.70  & 39.51  & 43.17  & 36.09  & \multirow{2}[4]{*}{3.68} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.943  & 0.971  & 0.962  & 0.967  & 0.968  & 0.977  & 0.989  & 0.968  & 0.963  & 0.971  & 0.959  & 0.968  & 0.979  & 0.974  & 0.966  & 0.981  & 0.958  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{VDIR\cite{soh2022variational}} & 39.63  & 39.26  & 34.90  & 36.51  & 37.01  & 36.84  & 40.84  & 41.40  & 41.29  & 40.81  & 37.65  & 37.84  & 39.09  & 38.17  & 39.20  & 39.41  & 38.98  & 44.40  & 35.04  & \multirow{2}[4]{*}{2.03} \\
\cmidrule{4-22}          &       &       & 0.953  & 0.955  & 0.894  & 0.925  & 0.940  & 0.911  & 0.973  & 0.970  & 0.965  & 0.953  & 0.936  & 0.960  & 0.951  & 0.931  & 0.946  & 0.938  & 0.956  & 0.985  & 0.939  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{VDNet\cite{yue2019variational}} & -     & -     & 35.86  & -     & 37.58  & 38.43  & 40.97  & 42.37  & 43.08  & 41.19  & 38.23  & 37.95  & 37.88  & 38.60  & 40.81  & 41.21  & 39.93  & 44.27  & 35.49  & \multirow{2}[4]{*}{0.05} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.945  & -     & 0.957  & 0.955  & 0.976  & 0.983  & 0.983  & 0.970  & 0.956  & 0.968  & 0.956  & 0.956  & 0.973  & 0.970  & 0.970  & 0.984  & 0.953  &  \\
\cmidrule{2-23}          & \multirow{66}[40]{*}{Self-supervised} & \multirow{2}[4]{*}{AP-BSN\cite{lee2022ap}} & 37.29  & 35.97  & 35.44  & 36.76  & 36.99  & 38.26  & 40.23  & 41.29  & 42.72  & 41.40  & 37.87  & 37.62  & 37.47  & 38.29  & 40.83  & 40.86  & 39.55  & 43.73  & 34.37  & \multirow{2}[4]{*}{3.56} \\
\cmidrule{4-22}          &       &       & 0.932  & 0.925  & 0.936  & 0.956  & 0.956  & 0.965  & 0.973  & 0.979  & 0.986  & 0.970  & 0.949  & 0.966  & 0.939  & 0.960  & 0.977  & 0.973  & 0.969  & 0.983  & 0.937  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{Blind2Unblind\cite{wang2022blind2unblind}} & -     & -     & 36.51  & 38.18  & 38.25  & 39.03  & 40.71  & 41.72  & 43.11  & 41.17  & 39.35  & 38.27  & 39.39  & 39.04  & 40.88  & 40.90  & 39.76  & 43.78  & 35.75  & \multirow{2}[4]{*}{0.74} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.935  & 0.958  & 0.968  & 0.962  & 0.974  & 0.981  & 0.990  & 0.970  & 0.967  & 0.971  & 0.962  & 0.958  & 0.976  & 0.970  & 0.971  & 0.986  & 0.956  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{C2N\cite{jang2021c2n}} & 37.28  & -     & 37.02  & -     & 37.69  & 38.86  & 41.12  & 41.95  & 42.61  & 41.33  & 38.73  & 38.15  & 38.95  & 38.67  & 40.50  & 40.78  & 40.05  & 44.64  & 35.53  & \multirow{2}[4]{*}{88.00} \\
\cmidrule{4-22}          &       &       & 0.924  & -     & 0.945  & -     & 0.958  & 0.960  & 0.976  & 0.980  & 0.980  & 0.966  & 0.954  & 0.965  & 0.956  & 0.945  & 0.977  & 0.964  & 0.970  & 0.987  & 0.952  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{CVF-SID\cite{neshatavar2022cvf}} & 36.31  & 34.43  & 29.13  & 31.02  & 33.08  & 33.35  & 36.68  & 39.08  & 39.73  & 36.40  & 33.13  & 33.16  & 32.07  & 33.33  & 36.92  & 38.40  & 35.22  & 38.56  & 29.89  & \multirow{2}[4]{*}{0.12} \\
\cmidrule{4-22}          &       &       & 0.923  & 0.912  & 0.853  & 0.898  & 0.912  & 0.929  & 0.933  & 0.974  & 0.976  & 0.929  & 0.895  & 0.920  & 0.857  & 0.917  & 0.946  & 0.961  & 0.927  & 0.952  & 0.849  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{IDR\cite{zhang2022idr}} & -     & -     & 34.26  & 36.18  & 36.28  & 36.44  & 39.33  & 40.31  & 40.94  & 39.74  & 37.38  & 37.39  & 38.30  & 38.15  & 39.68  & 38.22  & 38.01  & 43.15  & 34.64  & \multirow{2}[4]{*}{0.32} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.877  & 0.923  & 0.925  & 0.910  & 0.955  & 0.962  & 0.961  & 0.935  & 0.927  & 0.957  & 0.938  & 0.944  & 0.951  & 0.913  & 0.941  & 0.978  & 0.929  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{LGBPN\cite{wang2023lgbpn}} & 38.43$^\ast$   & 37.28$^\ast$   & -  & -  & -    & -  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{-} \\
\cmidrule{4-22}          &       &       & 0.942$^\ast$     & 0.936$^\ast$     & -  & -  & -     & -  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{Neigh2Neigh\cite{huang2021neighbor2neighbor}} & -     & -     & 34.47  & 35.65  & 37.10  & 36.59  & 40.22  & 40.41  & 41.29  & 41.24  & 38.13  & 37.94  & 39.71  & 38.50  & 39.63  & 38.05  & 39.17  & 44.49  & 35.30  & \multirow{2}[4]{*}{2.48} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.883  & 0.907  & 0.942  & 0.908  & 0.967  & 0.960  & 0.966  & 0.958  & 0.940  & 0.961  & 0.956  & 0.936  & 0.952  & 0.919  & 0.958  & 0.984  & 0.944  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{Noise2Noise\cite{lehtinen2018noise2noise}} & -     & -     & 33.55  & 34.67  & 35.91  & 35.28  & 38.88  & 39.07  & 39.34  & 39.26  & 36.81  & 36.99  & 38.04  & 37.21  & 38.00  & 36.35  & 37.67  & 42.59  & 34.44  & \multirow{2}[4]{*}{0.03} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.850  & 0.874  & 0.913  & 0.875  & 0.950  & 0.940  & 0.938  & 0.931  & 0.919  & 0.948  & 0.936  & 0.916  & 0.924  & 0.876  & 0.936  & 0.975  & 0.926  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{R2R\cite{pang2021recorrupted}} & -     & 34.78$^\ast$     & 36.32  & 38.11  & 38.47$^\ast$  & 38.71  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{4481.98} \\
\cmidrule{4-22}          &       &       & -     & 0.844$^\ast$     & 0.937  & 0.961  & 0.965$^\ast$  & 0.958  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{SASL\cite{li2023spatially}} & 38.00  & 37.41     & 34.93  & -     & 37.13  & 38.24  & 40.04  & 41.86  & 43.07  & 40.29  & 37.22  & 37.38  & 36.45  & 37.64  & 40.85  & 41.64  & 39.10  & 42.89  & 34.25  & \multirow{2}[4]{*}{0.06} \\
\cmidrule{4-22}          &       &       & 0.936  & 0.934     & 0.936  & -     & 0.954  & 0.964  & 0.966  & 0.982  & 0.987  & 0.963  & 0.947  & 0.965  & 0.933  & 0.958  & 0.977  & 0.976  & 0.965  & 0.980  & 0.930  &  \\
\cmidrule{3-23}          &       & \multirow{2}[4]{*}{Self2Self\cite{quan2020self2self}} & -     & -     & 36.26  & 38.23  & -     & 39.49  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & \multirow{2}[4]{*}{4100.76} \\
\cmidrule{4-22}          &       &       & -     & -     & 0.947  & 0.969  & -     & 0.963  & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     &  \\
    \bottomrule
    \end{tabular}}%
  \label{Table_Results_Color_image_all}%
\end{table*}%









==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_Results_Color_image_all_detailed.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%  \centering
%  \caption{Add caption}
%  \scalebox{0.59}{
%  \renewcommand{\arraystretch}{0.118}
%    \begin{tabular}{ccccccccccccccccccccc}
%    \toprule
%    \multicolumn{2}{c}{\multirow{2}[4]{*}{Methods/Models}} & \multirow{2}[4]{*}{DnD} & \multirow{2}[4]{*}{SIDD} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multirow{2}[4]{*}{HighISO} & \multicolumn{13}{c}{IOCI} \\
%    \cmidrule{9-21}    \multicolumn{2}{c}{} &       &       &       &       &       &       & C-100D & C-600D & C-5DMark4 & F-X100T & H-Honor6X & H-Mate40Pro & I-5S & I-6S & I-13 & N-D5300 & O-R11s & S-A6500 & X-MI8 \\
%    \midrule
%    /     & \# Images & 1000  & 1280  & 15    & 60    & 100   & 100   & 55    & 25    & 83    & 71    & 30    & 126   & 36    & 67    & 174   & 56    & 39    & 36    & 50 \\
%    \midrule
%    \multirow{128}[56]{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{2}[4]{*}{LSCD} & /     & /     & 36.20  & 37.69  & 37.97  & 38.64  & 40.65  & 41.45  & /     & /     & 39.22  & /     & 39.84  & 39.53  & /     & 40.83  & /     & 44.34  & 35.86  \\
%\cmidrule{3-21}          &       & /     & /     & 0.942  & 0.963  & 0.964  & 0.962  & 0.973  & 0.979  & /     & /     & 0.963  & /     & 0.963  & 0.963  & /     & 0.973  & /     & 0.987  & 0.957  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{GID} & 34.32  & 27.16  & 37.17  & 38.41  & 38.37  & 39.63  & 40.86  & 41.60  & 44.11  & 42.31  & 39.52  & 38.66  & 40.12  & 40.16  & 41.50  & 41.09  & 40.50  & 44.96  & 36.11  \\
%\cmidrule{3-21}          &       & 0.817  & 0.634  & 0.946  & 0.963  & 0.967  & 0.967  & 0.974  & 0.979  & 0.989  & 0.975  & 0.965  & 0.972  & 0.964  & 0.967  & 0.979  & 0.973  & 0.973  & 0.989  & 0.960  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Bitonic} & 37.85  & 36.67  & 35.22  & 35.98  & 36.64  & 37.37  & 39.38  & 39.63  & 40.76  & 41.05  & 37.71  & 37.41  & 38.98  & 38.04  & 39.09  & 39.22  & 38.87  & 43.25  & 34.92  \\
%\cmidrule{3-21}          &       & 0.936  & 0.933  & 0.925  & 0.931  & 0.940  & 0.943  & 0.959  & 0.952  & 0.965  & 0.964  & 0.940  & 0.956  & 0.947  & 0.939  & 0.952  & 0.954  & 0.959  & 0.979  & 0.941  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{LLRT} & 35.45  & 30.74  & 37.77  & 39.76  & 38.28  & 39.59  & 41.60  & 42.24  & 42.68  & 42.22  & 37.91  & 38.80  & 38.01  & 39.87  & 42.02  & 41.76  & 38.69  & 45.17  & 35.71  \\
%\cmidrule{3-21}          &       & 0.897  & 0.766  & 0.957  & 0.977  & 0.970  & 0.972  & 0.977  & 0.983  & 0.992  & 0.975  & 0.969  & 0.973  & 0.965  & 0.971  & 0.984  & 0.979  & 0.972  & 0.989  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{MCWNNM } & 37.38  & 29.54  & 37.02  & 38.54  & 38.26  & 39.89  & 41.47  & 42.07  & 44.22  & 42.48  & 39.46  & 38.78  & 39.87  & 40.18  & 41.33  & 41.74  & 40.71  & 45.38  & 35.84  \\
%\cmidrule{3-21}          &       & 0.929  & 0.888  & 0.950  & 0.967  & 0.965  & 0.970  & 0.977  & 0.979  & 0.988  & 0.976  & 0.961  & 0.971  & 0.957  & 0.963  & 0.976  & 0.975  & 0.973  & 0.990  & 0.952  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{TWSC } & 37.96  & /     & 37.90  & 39.66  & 38.62  & 40.62  & 41.65  & 42.52  & 44.94  & 42.26  & 38.71  & 38.81  & 38.77  & 40.12  & 41.71  & 42.23  & 40.65  & 45.49  & 35.40  \\
%\cmidrule{3-21}          &       & 0.942  & /     & 0.959  & 0.976  & 0.967  & 0.975  & 0.977  & 0.982  & 0.992  & 0.973  & 0.945  & 0.972  & 0.938  & 0.962  & 0.980  & 0.975  & 0.972  & 0.990  & 0.939  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{WTR1} & /     & /     & 37.80  & 37.32  & 38.20  & 38.19  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{3-21}          &       & /     & /     & 0.958  & 0.944  & 0.965  & 0.940  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{M-SVD} & 37.45  & 33.51  & 37.63  & 39.36  & 38.57  & 40.27  & 41.81  & 42.55  & 44.39  & 42.68  & 39.99  & 38.93  & 40.78  & 40.52  & 41.72  & 42.18  & 40.73  & 45.71  & 36.37  \\
%\cmidrule{3-21}          &       & 0.924  & 0.867  & 0.954  & 0.971  & 0.967  & 0.971  & 0.979  & 0.983  & 0.989  & 0.976  & 0.967  & 0.973  & 0.969  & 0.969  & 0.977  & 0.977  & 0.974  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{4DHOSVD} & 37.58  & 34.49  & 37.52  & 39.15  & 38.54  & 40.27  & 41.40  & 42.19  & 44.49  & 42.60  & 39.82  & 38.88  & 40.59  & 40.37  & 41.75  & 41.82  & 40.71  & 45.58  & 36.27  \\
%\cmidrule{3-21}          &       & 0.929  & 0.911  & 0.956  & 0.973  & 0.968  & 0.973  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.965  & 0.967  & 0.980  & 0.977  & 0.974  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D1} & 38.04  & 35.00  & 37.58  & 39.21  & 38.60  & 40.11  & 41.58  & 42.40  & 44.43  & 42.53  & 39.93  & 38.84  & 40.56  & 40.41  & 41.93  & 42.29  & 40.62  & 45.58  & 36.24  \\
%\cmidrule{3-21}          &       & 0.938  & 0.925  & 0.955  & 0.971  & 0.969  & 0.972  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.967  & 0.970  & 0.982  & 0.979  & 0.973  & 0.990  & 0.959  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D2} & 37.73  & 34.74  & 37.70  & 39.41  & 38.69  & 40.35  & 41.69  & 42.54  & 44.74  & 42.65  & 39.97  & 38.97  & 40.77  & 40.55  & 42.03  & 42.20  & 40.75  & 45.72  & 36.38  \\
%\cmidrule{3-21}          &       & 0.934  & 0.922  & 0.957  & 0.975  & 0.970  & 0.974  & 0.978  & 0.984  & 0.992  & 0.977  & 0.967  & 0.974  & 0.967  & 0.969  & 0.983  & 0.979  & 0.974  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D\_best} & /     & /     & 38.01  & 39.80  & 38.82  & 40.65  & 42.08  & 42.89  & 45.08  & 43.14  & 40.45  & 39.23  & 41.21  & 41.12  & 42.42  & 42.79  & 40.92  & 45.84  & 36.76  \\
%\cmidrule{3-21}          &       & /     & /     & 0.962  & 0.978  & 0.971  & 0.976  & 0.981  & 0.985  & 0.993  & 0.980  & 0.974  & 0.976  & 0.975  & 0.978  & 0.985  & 0.982  & 0.974  & 0.991  & 0.964  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CMSt-SVD} & 38.25  & 34.38  & 37.95  & 39.76  & 38.85  & 40.49  & 41.99  & 42.75  & 44.65  & 42.68  & 40.08  & 38.95  & 40.84  & 40.53  & 42.06  & 42.72  & 40.87  & 45.91  & 36.40  \\
%\cmidrule{3-21}          &       & 0.940  & 0.900  & 0.959  & 0.976  & 0.971  & 0.974  & 0.979  & 0.984  & 0.991  & 0.977  & 0.967  & 0.973  & 0.967  & 0.967  & 0.982  & 0.980  & 0.974  & 0.991  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{NLH-CC} & 38.85  & /     & 38.49  & 39.86  & 38.36  & 40.29  & 41.77  & 42.72  & 43.66  & 42.80  & 38.84  & 38.31  & 40.44  & 39.94  & 41.13  & 43.25  & NA    & 46.02  & 35.73  \\
%\cmidrule{3-21}          &       & 0.953  & /     & 0.965  & 0.976  & 0.965  & 0.971  & 0.979  & 0.984  & 0.986  & 0.978  & 0.959  & 0.968  & 0.964  & 0.963  & 0.976  & 0.981  & NA    & 0.991  & 0.955  \\
%    \midrule
%    \midrule
%    \multirow{368}[148]{*}{\shortstack[l]{DNN \\ methods}} & \multirow{2}[4]{*}{AINDNet} & 39.77  & 39.08  & 36.14  & \multicolumn{1}{c|}{37.19 } & 37.33  & 38.00  & 38.54  & 39.33  & 39.49  & 38.50  & 36.53  & 36.24  & 36.93  & 36.83  & 37.27  & 38.11  & 37.44  & 40.17  & 34.65  \\
%\cmidrule{3-21}          &       & 0.959  & 0.953  & 0.935  & 0.949  & 0.954  & 0.946  & 0.975  & 0.976  & 0.979  & 0.966  & 0.954  & 0.965  & 0.958  & 0.953  & 0.964  & 0.961  & 0.968  & 0.981  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{AP-BSN} & 37.29  & 35.97  & 35.44  & 36.76  & 36.99  & 38.26  & 40.23  & 41.29  & 42.72  & 41.40  & 37.87  & 37.62  & 37.47  & 38.29  & 40.83  & 40.86  & 39.55  & 43.73  & 34.37  \\
%\cmidrule{3-21}          &       & 0.932  & 0.925  & 0.936  & 0.956  & 0.956  & 0.965  & 0.973  & 0.979  & 0.986  & 0.970  & 0.949  & 0.966  & 0.939  & 0.960  & 0.977  & 0.973  & 0.969  & 0.983  & 0.937  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Blind2Unblind} & /     & /     & 36.51  & 38.18  & 38.25  & 39.03  & 40.71  & 41.72  & 43.11  & 41.17  & 39.35  & 38.27  & 39.39  & 39.04  & 40.88  & 40.90  & 39.76  & 43.78  & 35.75  \\
%\cmidrule{3-21}          &       & /     & /     & 0.935  & 0.958  & 0.968  & 0.962  & 0.974  & 0.981  & 0.990  & 0.970  & 0.967  & 0.971  & 0.962  & 0.958  & 0.976  & 0.970  & 0.971  & 0.986  & 0.956  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{BRDNet} & 33.80  & /     & 37.27  & 39.16  & 38.04  & 39.64  & 39.85  & 40.95  & 43.54  & 40.27  & 39.48  & 38.66  & 38.19  & 40.07  & 41.92  & 41.34  & 39.66  & 42.76  & 36.08  \\
%\cmidrule{3-21}          &       & 0.897  & /     & 0.953  & 0.974  & 0.960  & 0.969  & 0.965  & 0.974  & 0.989  & 0.958  & 0.958  & 0.973  & 0.943  & 0.969  & 0.981  & 0.972  & 0.965  & 0.979  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{C2N} & 37.28  & /     & 37.02  & /     & 37.69  & 38.86  & 41.12  & 41.95  & 42.61  & 41.33  & 38.73  & 38.15  & 38.95  & 38.67  & 40.50  & 40.78  & 40.05  & 44.64  & 35.53  \\
%\cmidrule{3-21}          &       & 0.924  & /     & 0.945  & /     & 0.958  & 0.960  & 0.976  & 0.980  & 0.980  & 0.966  & 0.954  & 0.965  & 0.956  & 0.945  & 0.977  & 0.964  & 0.970  & 0.987  & 0.952  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CBDNet} & 38.06  & 33.26  & 36.20  & 37.67  & 37.81  & 38.18  & 41.43  & 42.41  & 42.55  & 41.88  & 38.35  & 38.17  & 39.80  & 39.07  & 40.63  & 40.92  & 39.54  & 44.38  & 35.54  \\
%\cmidrule{3-21}          &       & 0.942  & 0.869  & 0.919  & 0.940  & 0.956  & 0.942  & 0.977  & 0.981  & 0.980  & 0.971  & 0.946  & 0.964  & 0.960  & 0.951  & 0.968  & 0.963  & 0.965  & 0.981  & 0.950  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CVF-SID} & 36.31  & 34.43  & 29.13  & 31.02  & 33.08  & 33.35  & 36.68  & 39.08  & 39.73  & 36.40  & 33.13  & 33.16  & 32.07  & 33.33  & 36.92  & 38.40  & 35.22  & 38.56  & 29.89  \\
%\cmidrule{3-21}          &       & 0.923  & 0.912  & 0.853  & 0.898  & 0.912  & 0.929  & 0.933  & 0.974  & 0.976  & 0.929  & 0.895  & 0.920  & 0.857  & 0.917  & 0.946  & 0.961  & 0.927  & 0.952  & 0.849  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CycleISP} & 39.57  & 39.42  & 35.40  & 36.87  & 37.61  & 37.70  & 41.26  & 41.84  & 42.64  & 41.59  & 38.47  & 38.01  & 38.79  & 38.67  & 40.61  & 40.03  & 39.86  & 44.75  & 35.54  \\
%\cmidrule{3-21}          &       & 0.955  & 0.956  & 0.916  & 0.939  & 0.955  & 0.936  & 0.977  & 0.977  & 0.978  & 0.969  & 0.952  & 0.966  & 0.961  & 0.952  & 0.970  & 0.953  & 0.968  & 0.987  & 0.949  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DANet} & 39.55  & 39.43  & 37.17  & 38.63  & 41.49  & 38.92  & 41.59  & 42.59  & 42.83  & 41.70  & 37.91  & 38.17  & 39.23  & 38.74  & 41.58  & 41.54  & 39.58  & 44.03  & 36.21  \\
%\cmidrule{3-21}          &       & 0.953  & 0.956  & 0.953  & 0.969  & 0.977  & 0.960  & 0.979  & 0.985  & 0.979  & 0.977  & 0.963  & 0.970  & 0.964  & 0.962  & 0.980  & 0.976  & 0.972  & 0.989  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DBF} & /     & /     & 38.48  & 40.59  & 38.87  & 40.09  & 41.56  & 42.87  & 44.85  & 42.36  & 39.98  & 38.86  & 40.17  & 40.26  & 42.12  & 43.17  & 40.67  & 44.75  & 36.45  \\
%\cmidrule{3-21}          &       & /     & /     & 0.960  & 0.981  & 0.970  & 0.970  & 0.979  & 0.984  & 0.992  & 0.975  & 0.967  & 0.972  & 0.966  & 0.966  & 0.982  & 0.982  & 0.973  & 0.987  & 0.963  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DCDicL} & /     & /     & 36.61  & /     & 37.45  & 38.12  & 37.77  & 38.24  & 38.39  & 38.62  & 35.87  & 36.07  & 35.83  & 36.25  & 39.84  & 39.38  & 37.04  & 40.24  & 34.72  \\
%\cmidrule{3-21}          &       & /     & /     & 0.945  & /     & 0.972  & 0.965  & 0.970  & 0.977  & 0.990  & 0.968  & 0.968  & 0.975  & 0.956  & 0.971  & 0.984  & 0.976  & 0.969  & 0.980  & 0.955  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DeamNet} & 39.63  & 39.35  & 36.63  & /     & 37.70  & 36.93  & 40.90  & 40.86  & 41.22  & 39.72  & 33.67  & 36.40  & 37.87  & 35.07  & 40.25  & 38.92  & 39.56  & 40.52  & 34.61  \\
%\cmidrule{3-21}          &       & 0.953  & 0.955  & 0.936  & /     & 0.958  & 0.944  & 0.977  & 0.978  & 0.979  & 0.967  & 0.953  & 0.964  & 0.961  & 0.948  & 0.966  & 0.957  & 0.969  & 0.980  & 0.952  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DIDN} & 39.64  & 39.78  & 36.06  & /     & 37.36  & 38.24  & 40.74  & 41.68  & 42.35  & 41.17  & 38.15  & 37.87  & 38.27  & 38.58  & 40.03  & 40.32  & 39.73  & 44.07  & 35.28  \\
%\cmidrule{3-21}          &       & 0.953  & 0.958  & 0.946  & /     & 0.953  & 0.950  & 0.975  & 0.977  & 0.975  & 0.966  & 0.951  & 0.965  & 0.954  & 0.950  & 0.963  & 0.959  & 0.966  & 0.985  & 0.949  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DnCNN} & 37.90  & 37.73  & 37.47  & 39.32  & 38.51  & 40.01  & 40.81  & 41.91  & 44.16  & 41.57  & 39.92  & 38.72  & 39.34  & 40.22  & 42.03  & 42.12  & 40.26  & 43.97  & 36.30  \\
%\cmidrule{3-21}          &       & 0.943  & 0.941  & 0.954  & 0.974  & 0.966  & 0.971  & 0.972  & 0.979  & 0.991  & 0.969  & 0.962  & 0.973  & 0.964  & 0.969  & 0.983  & 0.977  & 0.970  & 0.984  & 0.960  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DPIR} & /     & /     & 38.30  & 40.33  & 38.93  & 40.77  & 41.94  & 42.62  & 45.36  & 42.78  & 40.35  & 39.17  & 40.80  & 40.80  & 42.86  & 42.86  & 40.96  & 45.76  & 36.61  \\
%\cmidrule{3-21}          &       & /     & /     & 0.961  & 0.979  & 0.970  & 0.974  & 0.978  & 0.982  & 0.993  & 0.977  & 0.969  & 0.975  & 0.966  & 0.970  & 0.985  & 0.980  & 0.974  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DudeNet} & 33.18  & 27.55  & 36.03  & 37.44  & 39.92  & 38.18  & 39.94  & 41.13  & 42.97  & 41.06  & 38.63  & 37.83  & 39.09  & 38.58  & 40.73  & 40.63  & 39.71  & 43.34  & 35.44  \\
%\cmidrule{3-21}          &       & 0.810  & 0.645  & 0.933  & 0.953  & 0.973  & 0.955  & 0.972  & 0.977  & 0.988  & 0.971  & 0.962  & 0.969  & 0.962  & 0.961  & 0.976  & 0.969  & 0.972  & 0.985  & 0.955  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{FCCF} & 36.30  & 23.32  & 39.02  & 40.89  & 38.87  & 41.20  & 42.03  & 43.07  & 45.15  & 42.80  & 40.14  & 39.04  & 40.61  & 40.66  & 42.31  & 43.05  & 40.95  & 45.47  & 36.72  \\
%\cmidrule{3-21}          &       & 0.885  & 0.461  & 0.968  & 0.982  & 0.971  & 0.978  & 0.980  & 0.985  & 0.993  & 0.978  & 0.966  & 0.974  & 0.967  & 0.969  & 0.984  & 0.982  & 0.975  & 0.989  & 0.964  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{FFD-Net} & 37.61  & 38.27  & 37.67  & 39.73  & 38.76  & 40.28  & 41.67  & 42.55  & 44.77  & 42.44  & 40.05  & 38.96  & 40.60  & 40.50  & 42.43  & 42.44  & 40.75  & 45.71  & 36.47  \\
%\cmidrule{3-21}          &       & 0.942  & 0.948  & 0.956  & 0.977  & 0.970  & 0.973  & 0.977  & 0.982  & 0.992  & 0.976  & 0.967  & 0.974  & 0.964  & 0.971  & 0.984  & 0.979  & 0.973  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{IDR} & /     & /     & 34.26  & 36.18  & 36.28  & 36.44  & 39.33  & 40.31  & 40.94  & 39.74  & 37.38  & 37.39  & 38.30  & 38.15  & 39.68  & 38.22  & 38.01  & 43.15  & 34.64  \\
%\cmidrule{3-21}          &       & /     & /     & 0.877  & 0.923  & 0.925  & 0.910  & 0.955  & 0.962  & 0.961  & 0.935  & 0.927  & 0.957  & 0.938  & 0.944  & 0.951  & 0.913  & 0.941  & 0.978  & 0.929  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{InvDN} & 39.57  & 39.28  & 34.55  & 36.33  & 35.94  & 38.01  & 38.95  & 40.09  & 42.03  & 40.02  & 33.32  & 37.00  & 36.64  & 37.66  & 40.06  & 40.98  & 39.10  & 40.74  & 34.15  \\
%\cmidrule{3-21}          &       & 0.952  & 0.955  & 0.937  & 0.953  & 0.947  & 0.952  & 0.965  & 0.973  & 0.978  & 0.960  & 0.930  & 0.965  & 0.939  & 0.955  & 0.966  & 0.971  & 0.964  & 0.969  & 0.935  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{IRCNN} & 34.78  & 33.50  & 37.26  & 37.25  & 37.49  & 39.66  & 41.24  & 41.85  & 43.89  & 41.78  & 39.91  & 38.63  & 40.14  & 40.12  & 41.87  & 41.86  & 40.26  & 44.38  & 36.22  \\
%\cmidrule{3-21}          &       & 0.907  & 0.887  & 0.954  & 0.956  & 0.956  & 0.970  & 0.978  & 0.981  & 0.991  & 0.973  & 0.969  & 0.972  & 0.965  & 0.969  & 0.983  & 0.977  & 0.972  & 0.988  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{MIRNet} & 39.88  & 39.55  & 36.06  & 37.25  & 37.49  & 38.10  & 40.72  & 41.68  & 42.76  & 41.05  & 38.28  & 37.80  & 38.60  & 38.55  & 40.28  & 40.46  & 39.73  & 43.66  & 35.42  \\
%\cmidrule{3-21}          &       & 0.956  & 0.957  & 0.942  & 0.956  & 0.956  & 0.952  & 0.975  & 0.978  & 0.980  & 0.968  & 0.954  & 0.967  & 0.959  & 0.952  & 0.966  & 0.964  & 0.967  & 0.983  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{MPRNet} & 39.82  & 39.57  & 35.94  & /     & 37.50  & 38.04  & 40.59  & 41.30  & 42.59  & 41.23  & 38.35  & 37.92  & 38.95  & 38.62  & 40.21  & 40.20  & 39.77  & 44.05  & 35.49  \\
%\cmidrule{3-21}          &       & 0.954  & 0.958  & 0.935  & /     & 0.954  & 0.946  & 0.974  & 0.974  & 0.978  & 0.969  & 0.952  & 0.966  & 0.960  & 0.949  & 0.965  & 0.960  & 0.967  & 0.986  & 0.951  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{NAFNet} & 38.36  & 40.15  & 34.39  & /     & 36.38  & 37.88  & 40.12  & 40.23  & 40.66  & 40.01  & 36.13  & 35.87  & 36.66  & 36.79  & 36.53  & 39.93  & 39.32  & 40.45  & 34.82  \\
%\cmidrule{3-21}          &       & 0.943  & 0.960  & 0.923  & /     & 0.947  & 0.954  & 0.973  & 0.943  & 0.936  & 0.962  & 0.919  & 0.927  & 0.948  & 0.927  & 0.884  & 0.951  & 0.966  & 0.924  & 0.948  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{NBNet} & 39.89  & 39.64  & 35.89  & /     & 37.37  & 38.32  & 40.95  & 41.91  & 42.92  & 41.17  & 38.02  & 37.87  & 37.79  & 38.45  & 40.51  & 40.45  & 39.73  & 43.96  & 35.37  \\
%\cmidrule{3-21}          &       & 0.955  & 0.958  & 0.935  & /     & 0.957  & 0.955  & 0.977  & 0.980  & 0.982  & 0.971  & 0.955  & 0.967  & 0.956  & 0.955  & 0.972  & 0.967  & 0.969  & 0.984  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Neigh2Neigh} & /     & /     & 34.47  & 35.65  & 37.10  & 36.59  & 40.22  & 40.41  & 41.29  & 41.24  & 38.13  & 37.94  & 39.71  & 38.50  & 39.63  & 38.05  & 39.17  & 44.49  & 35.30  \\
%\cmidrule{3-21}          &       & /     & /     & 0.883  & 0.907  & 0.942  & 0.908  & 0.967  & 0.960  & 0.966  & 0.958  & 0.940  & 0.961  & 0.956  & 0.936  & 0.952  & 0.919  & 0.958  & 0.984  & 0.944  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{NLNet} & /     & /     & 37.56  & 39.32  & 38.58  & 40.17  & 41.43  & 42.18  & 44.53  & 42.19  & 39.96  & 38.89  & 40.06  & 40.61  & 42.14  & 42.16  & 40.63  & 44.87  & 36.34  \\
%\cmidrule{3-21}          &       & /     & /     & 0.955  & 0.974  & 0.968  & 0.973  & 0.976  & 0.981  & 0.991  & 0.974  & 0.969  & 0.973  & 0.964  & 0.971  & 0.983  & 0.978  & 0.973  & 0.988  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Noise2Noise} & /     & /     & 33.55  & 34.67  & 35.91  & 35.28  & 38.88  & 39.07  & 39.34  & 39.26  & 36.81  & 36.99  & 38.04  & 37.21  & 38.00  & 36.35  & 37.67  & 42.59  & 34.44  \\
%\cmidrule{3-21}          &       & /     & /     & 0.850  & 0.874  & 0.913  & 0.875  & 0.950  & 0.940  & 0.938  & 0.931  & 0.919  & 0.948  & 0.936  & 0.916  & 0.924  & 0.876  & 0.936  & 0.975  & 0.926  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{PD-Denoising} & 38.40  & 33.99  & 35.85  & 37.13  & 37.13  & 37.12  & 40.85  & 41.38  & 41.13  & 41.05  & 37.72  & 37.57  & 39.03  & 38.01  & 39.18  & 39.64  & 38.80  & 43.73  & 35.05  \\
%\cmidrule{3-21}          &       & 0.943  & 0.896  & 0.924  & 0.944  & 0.944  & 0.921  & 0.974  & 0.974  & 0.966  & 0.959  & 0.935  & 0.956  & 0.948  & 0.929  & 0.948  & 0.946  & 0.955  & 0.981  & 0.940  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{PNGAN} & 39.38  & 39.81  & 38.44  & /     & 39.57  & 40.51  & 41.79  & 43.13  & 44.73  & 42.55  & 39.84  & 38.78  & 40.63  & 40.20  & 41.85  & 43.15  & 40.87  & 45.32  & 36.40  \\
%\cmidrule{3-21}          &       & 0.953  & 0.959  & 0.963  & /     & 0.974  & 0.974  & 0.979  & 0.985  & 0.992  & 0.977  & 0.964  & 0.970  & 0.969  & 0.962  & 0.981  & 0.982  & 0.974  & 0.988  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{R2R} & /     & /     & 36.32  & 38.11  & 38.57  & 38.71  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{3-21}          &       & /     & /     & 0.937  & 0.961  & 0.970  & 0.958  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Restormer} & 40.03  & 39.79  & 36.33  & /     & 37.66  & 38.29  & 41.10  & 41.84  & 42.49  & 41.47  & 38.42  & 38.08  & 39.05  & 38.77  & 40.13  & 40.53  & 39.56  & 44.19  & 35.65  \\
%\cmidrule{3-21}          &       & 0.956  & 0.959  & 0.941  & /     & 0.956  & 0.948  & 0.977  & 0.979  & 0.976  & 0.968  & 0.952  & 0.966  & 0.960  & 0.949  & 0.963  & 0.962  & 0.963  & 0.986  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{RIDNet} & 39.26  & 38.70  & 36.84  & 38.11  & 38.57  & 38.60  & 41.09  & 42.15  & 42.39  & 41.59  & 38.88  & 38.21  & 38.67  & 39.02  & 40.91  & 41.01  & 40.07  & 44.40  & 35.76  \\
%\cmidrule{3-21}          &       & 0.953  & 0.950  & 0.941  & 0.961  & 0.970  & 0.956  & 0.977  & 0.980  & 0.989  & 0.975  & 0.962  & 0.970  & 0.963  & 0.959  & 0.978  & 0.977  & 0.972  & 0.987  & 0.957  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{SADNet} & 39.59  & /     & 37.76  & 38.11  & 39.22  & 38.90  & 40.82  & 42.02  & 44.25  & 41.85  & 39.53  & 38.33  & 39.83  & 39.69  & 39.81  & 41.64  & 40.70  & 44.61  & 36.36  \\
%\cmidrule{3-21}          &       & 0.952  & /     & 0.952  & 0.961  & 0.972  & 0.965  & 0.976  & 0.980  & 0.992  & 0.975  & 0.965  & 0.970  & 0.965  & 0.963  & 0.965  & 0.979  & 0.974  & 0.988  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Self2Self} & /     & /     & 36.26  & 38.23  & /     & 39.49  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{3-21}          &       & /     & /     & 0.947  & 0.969  & /     & 0.963  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Unet} & /     & /     & 36.95  & 38.96  & 38.05  & 39.62  & 40.40  & 41.36  & 43.58  & 41.12  & 39.35  & 38.25  & 38.94  & 39.95  & 41.32  & 41.70  & 39.51  & 43.17  & 36.09  \\
%\cmidrule{3-21}          &       & /     & /     & 0.943  & 0.971  & 0.962  & 0.967  & 0.968  & 0.977  & 0.989  & 0.968  & 0.963  & 0.971  & 0.959  & 0.968  & 0.979  & 0.974  & 0.966  & 0.981  & 0.958  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{VDNet} & /     & /     & 35.86  & /     & 37.58  & 38.43  & 40.97  & 42.37  & 43.08  & 41.19  & 38.23  & 37.95  & 37.88  & 38.60  & 40.81  & 41.21  & 39.93  & 44.27  & 35.49  \\
%\cmidrule{3-21}          &       & /     & /     & 0.945  & /     & 0.957  & 0.955  & 0.976  & 0.983  & 0.983  & 0.970  & 0.956  & 0.968  & 0.956  & 0.956  & 0.973  & 0.970  & 0.970  & 0.984  & 0.953  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{tab:addlabel}%
%\end{table*}%
%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Average PSNR, SSIM values on real-world color image datasets. `/' means the results are not available due to high computational burden or other issues. `C: CANON', `F: FUJIFILM', `H: HUAWEI', `I: IPHONE', 'N: NIKON', `O: OPPO', `S: SONY', `X: XIAOMI'.}
  \scalebox{0.586}{
  \renewcommand{\arraystretch}{0.118}
    \begin{tabular}{ccccccccccccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Methods/Models}} & \multirow{2}[4]{*}{DnD} & \multirow{2}[4]{*}{SIDD} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multirow{2}[4]{*}{HighISO} & \multicolumn{13}{c}{IOCI} \\
    \cmidrule{9-21}    \multicolumn{2}{c}{} &       &       &       &       &       &       & C-100D & C-600D & C-5DMark4 & F-X100T & H-Honor6X & H-Mate40Pro & I-5S & I-6S & I-13 & N-D5300 & O-R11s & S-A6500 & X-MI8 \\
    \midrule
    /     & \# Images & 1000  & 1280  & 15    & 60    & 100   & 100   & 55    & 25    & 83    & 71    & 30    & 126   & 36    & 67    & 174   & 56    & 39    & 36    & 50 \\
    \midrule
    \multirow{168}[56]{*}{\shortstack[c]{Traditional \\ denoisers}} & \multirow{2}[4]{*}{LSCD} & /     & /     & 36.20  & 37.69  & 37.97  & 38.64  & 40.65  & 41.45  & /     & /     & 39.22  & /     & 39.84  & 39.53  & /     & 40.83  & /     & 44.34  & 35.86  \\
\cmidrule{3-21}          &       & /     & /     & 0.942  & 0.963  & 0.964  & 0.962  & 0.973  & 0.979  & /     & /     & 0.963  & /     & 0.963  & 0.963  & /     & 0.973  & /     & 0.987  & 0.957  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{GID} & 34.32  & 27.16  & 37.17  & 38.41  & 38.37  & 39.63  & 40.86  & 41.60  & 44.11  & 42.31  & 39.52  & 38.66  & 40.12  & 40.16  & 41.50  & 41.09  & 40.50  & 44.96  & 36.11  \\
\cmidrule{3-21}          &       & 0.817  & 0.634  & 0.946  & 0.963  & 0.967  & 0.967  & 0.974  & 0.979  & 0.989  & 0.975  & 0.965  & 0.972  & 0.964  & 0.967  & 0.979  & 0.973  & 0.973  & 0.989  & 0.960  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Bitonic} & 37.85  & 36.67  & 35.22  & 35.98  & 36.64  & 37.37  & 39.38  & 39.63  & 40.76  & 41.05  & 37.71  & 37.41  & 38.98  & 38.04  & 39.09  & 39.22  & 38.87  & 43.25  & 34.92  \\
\cmidrule{3-21}          &       & 0.936  & 0.933  & 0.925  & 0.931  & 0.940  & 0.943  & 0.959  & 0.952  & 0.965  & 0.964  & 0.940  & 0.956  & 0.947  & 0.939  & 0.952  & 0.954  & 0.959  & 0.979  & 0.941  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{LLRT} & 35.45  & 30.74  & 37.77  & 39.76  & 38.28  & 39.59  & 41.60  & 42.24  & 42.68  & 42.22  & 37.91  & 38.80  & 38.01  & 39.87  & 42.02  & 41.76  & 38.69  & 45.17  & 35.71  \\
\cmidrule{3-21}          &       & 0.897  & 0.766  & 0.957  & 0.977  & 0.970  & 0.972  & 0.977  & 0.983  & 0.992  & 0.975  & 0.969  & 0.973  & 0.965  & 0.971  & 0.984  & 0.979  & 0.972  & 0.989  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{MCWNNM } & 37.38  & 29.54  & 37.02  & 38.54  & 38.26  & 39.89  & 41.47  & 42.07  & 44.22  & 42.48  & 39.46  & 38.78  & 39.87  & 40.18  & 41.33  & 41.74  & 40.71  & 45.38  & 35.84  \\
\cmidrule{3-21}          &       & 0.929  & 0.888  & 0.950  & 0.967  & 0.965  & 0.970  & 0.977  & 0.979  & 0.988  & 0.976  & 0.961  & 0.971  & 0.957  & 0.963  & 0.976  & 0.975  & 0.973  & 0.990  & 0.952  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{TWSC } & 37.96  & /     & 37.90  & 39.66  & 38.62  & 40.62  & 41.65  & 42.52  & 44.94  & 42.26  & 38.71  & 38.81  & 38.77  & 40.12  & 41.71  & 42.23  & 40.65  & 45.49  & 35.40  \\
\cmidrule{3-21}          &       & 0.942  & /     & 0.959  & 0.976  & 0.967  & 0.975  & 0.977  & 0.982  & 0.992  & 0.973  & 0.945  & 0.972  & 0.938  & 0.962  & 0.980  & 0.975  & 0.972  & 0.990  & 0.939  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{WTR1} & /     & /     & 37.80  & 37.32  & 38.20  & 38.19  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{3-21}          &       & /     & /     & 0.958  & 0.944  & 0.965  & 0.940  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{M-SVD} & 37.45  & 33.51  & 37.63  & 39.36  & 38.57  & 40.27  & 41.81  & 42.55  & 44.39  & 42.68  & 39.99  & 38.93  & 40.78  & 40.52  & 41.72  & 42.18  & 40.73  & 45.71  & 36.37  \\
\cmidrule{3-21}          &       & 0.924  & 0.867  & 0.954  & 0.971  & 0.967  & 0.971  & 0.979  & 0.983  & 0.989  & 0.976  & 0.967  & 0.973  & 0.969  & 0.969  & 0.977  & 0.977  & 0.974  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{4DHOSVD} & 37.58  & 34.49  & 37.52  & 39.15  & 38.54  & 40.27  & 41.40  & 42.19  & 44.49  & 42.60  & 39.82  & 38.88  & 40.59  & 40.37  & 41.75  & 41.82  & 40.71  & 45.58  & 36.27  \\
\cmidrule{3-21}          &       & 0.929  & 0.911  & 0.956  & 0.973  & 0.968  & 0.973  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.965  & 0.967  & 0.980  & 0.977  & 0.974  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D1} & 38.04  & 35.00  & 37.58  & 39.21  & 38.60  & 40.11  & 41.58  & 42.40  & 44.43  & 42.53  & 39.93  & 38.84  & 40.56  & 40.41  & 41.93  & 42.29  & 40.62  & 45.58  & 36.24  \\
\cmidrule{3-21}          &       & 0.938  & 0.925  & 0.955  & 0.971  & 0.969  & 0.972  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.967  & 0.970  & 0.982  & 0.979  & 0.973  & 0.990  & 0.959  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D2} & 37.73  & 34.74  & 37.70  & 39.41  & 38.69  & 40.35  & 41.69  & 42.54  & 44.74  & 42.65  & 39.97  & 38.97  & 40.77  & 40.55  & 42.03  & 42.20  & 40.75  & 45.72  & 36.38  \\
\cmidrule{3-21}          &       & 0.934  & 0.922  & 0.957  & 0.975  & 0.970  & 0.974  & 0.978  & 0.984  & 0.992  & 0.977  & 0.967  & 0.974  & 0.967  & 0.969  & 0.983  & 0.979  & 0.974  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D\_best} & /     & /     & 38.01  & 39.80  & 38.82  & 40.65  & 42.08  & 42.89  & 45.08  & 43.14  & 40.45  & 39.23  & 41.21  & 41.12  & 42.42  & 42.79  & 40.92  & 45.84  & 36.76  \\
\cmidrule{3-21}          &       & /     & /     & 0.962  & 0.978  & 0.971  & 0.976  & 0.981  & 0.985  & 0.993  & 0.980  & 0.974  & 0.976  & 0.975  & 0.978  & 0.985  & 0.982  & 0.974  & 0.991  & 0.964  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CMSt-SVD} & 38.25  & 34.38  & 37.95  & 39.76  & 38.85  & 40.49  & 41.99  & 42.75  & 44.65  & 42.68  & 40.08  & 38.95  & 40.84  & 40.53  & 42.06  & 42.72  & 40.87  & 45.91  & 36.40  \\
\cmidrule{3-21}          &       & 0.940  & 0.900  & 0.959  & 0.976  & 0.971  & 0.974  & 0.979  & 0.984  & 0.991  & 0.977  & 0.967  & 0.973  & 0.967  & 0.967  & 0.982  & 0.980  & 0.974  & 0.991  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{NLH-CC} & 38.85  & /     & 38.49  & 39.86  & 38.36  & 40.29  & 41.77  & 42.72  & 43.66  & 42.80  & 38.84  & 38.31  & 40.44  & 39.94  & 41.13  & 43.25  & /     & 46.02  & 35.73  \\
\cmidrule{3-21}          &       & 0.953  & /     & 0.965  & 0.976  & 0.965  & 0.971  & 0.979  & 0.984  & 0.986  & 0.978  & 0.959  & 0.968  & 0.964  & 0.963  & 0.976  & 0.981  & /     & 0.991  & 0.955  \\
    \midrule
    \midrule
    \multirow{368}[148]{*}{\shortstack[c]{DNN \\ methods}} & \multirow{2}[4]{*}{AINDNet} & 39.77  & 39.08  & 36.14  & 37.19  & 37.33  & 38.00  & 38.54  & 39.33  & 39.49  & 38.50  & 36.53  & 36.24  & 36.93  & 36.83  & 37.27  & 38.11  & 37.44  & 40.17  & 34.65  \\
\cmidrule{3-21}          &       & 0.959  & 0.953  & 0.935  & 0.949  & 0.954  & 0.946  & 0.975  & 0.976  & 0.979  & 0.966  & 0.954  & 0.965  & 0.958  & 0.953  & 0.964  & 0.961  & 0.968  & 0.981  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{AP-BSN} & 37.29  & 35.97  & 35.44  & 36.76  & 36.99  & 38.26  & 40.23  & 41.29  & 42.72  & 41.40  & 37.87  & 37.62  & 37.47  & 38.29  & 40.83  & 40.86  & 39.55  & 43.73  & 34.37  \\
\cmidrule{3-21}          &       & 0.932  & 0.925  & 0.936  & 0.956  & 0.956  & 0.965  & 0.973  & 0.979  & 0.986  & 0.970  & 0.949  & 0.966  & 0.939  & 0.960  & 0.977  & 0.973  & 0.969  & 0.983  & 0.937  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Blind2Unblind} & /     & /     & 36.51  & 38.18  & 38.25  & 39.03  & 40.71  & 41.72  & 43.11  & 41.17  & 39.35  & 38.27  & 39.39  & 39.04  & 40.88  & 40.90  & 39.76  & 43.78  & 35.75  \\
\cmidrule{3-21}          &       & /     & /     & 0.935  & 0.958  & 0.968  & 0.962  & 0.974  & 0.981  & 0.990  & 0.970  & 0.967  & 0.971  & 0.962  & 0.958  & 0.976  & 0.970  & 0.971  & 0.986  & 0.956  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{BRDNet} & 33.80  & /     & 37.27  & 39.16  & 38.04  & 39.64  & 39.85  & 40.95  & 43.54  & 40.27  & 39.48  & 38.66  & 38.19  & 40.07  & 41.92  & 41.34  & 39.66  & 42.76  & 36.08  \\
\cmidrule{3-21}          &       & 0.897  & /     & 0.953  & 0.974  & 0.960  & 0.969  & 0.965  & 0.974  & 0.989  & 0.958  & 0.958  & 0.973  & 0.943  & 0.969  & 0.981  & 0.972  & 0.965  & 0.979  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{C2N} & 37.28  & /     & 37.02  & /     & 37.69  & 38.86  & 41.12  & 41.95  & 42.61  & 41.33  & 38.73  & 38.15  & 38.95  & 38.67  & 40.50  & 40.78  & 40.05  & 44.64  & 35.53  \\
\cmidrule{3-21}          &       & 0.924  & /     & 0.945  & /     & 0.958  & 0.960  & 0.976  & 0.980  & 0.980  & 0.966  & 0.954  & 0.965  & 0.956  & 0.945  & 0.977  & 0.964  & 0.970  & 0.987  & 0.952  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CBDNet} & 38.06  & 33.26  & 36.20  & 37.67  & 37.81  & 38.18  & 41.43  & 42.41  & 42.55  & 41.88  & 38.35  & 38.17  & 39.80  & 39.07  & 40.63  & 40.92  & 39.54  & 44.38  & 35.54  \\
\cmidrule{3-21}          &       & 0.942  & 0.869  & 0.919  & 0.940  & 0.956  & 0.942  & 0.977  & 0.981  & 0.980  & 0.971  & 0.946  & 0.964  & 0.960  & 0.951  & 0.968  & 0.963  & 0.965  & 0.981  & 0.950  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CVF-SID} & 36.31  & 34.43  & 29.13  & 31.02  & 33.08  & 33.35  & 36.68  & 39.08  & 39.73  & 36.40  & 33.13  & 33.16  & 32.07  & 33.33  & 36.92  & 38.40  & 35.22  & 38.56  & 29.89  \\
\cmidrule{3-21}          &       & 0.923  & 0.912  & 0.853  & 0.898  & 0.912  & 0.929  & 0.933  & 0.974  & 0.976  & 0.929  & 0.895  & 0.920  & 0.857  & 0.917  & 0.946  & 0.961  & 0.927  & 0.952  & 0.849  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CycleISP} & 39.57  & 39.42  & 35.40  & 36.87  & 37.61  & 37.70  & 41.26  & 41.84  & 42.64  & 41.59  & 38.47  & 38.01  & 38.79  & 38.67  & 40.61  & 40.03  & 39.86  & 44.75  & 35.54  \\
\cmidrule{3-21}          &       & 0.955  & 0.956  & 0.916  & 0.939  & 0.955  & 0.936  & 0.977  & 0.977  & 0.978  & 0.969  & 0.952  & 0.966  & 0.961  & 0.952  & 0.970  & 0.953  & 0.968  & 0.987  & 0.949  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DANet} & 39.55  & 39.43  & 37.17  & 38.63  & 41.49  & 38.92  & 41.59  & 42.59  & 42.83  & 41.70  & 37.91  & 38.17  & 39.23  & 38.74  & 41.58  & 41.54  & 39.58  & 44.03  & 36.21  \\
\cmidrule{3-21}          &       & 0.953  & 0.956  & 0.953  & 0.969  & 0.977  & 0.960  & 0.979  & 0.985  & 0.979  & 0.977  & 0.963  & 0.970  & 0.964  & 0.962  & 0.980  & 0.976  & 0.972  & 0.989  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DBF} & /     & /     & 38.48  & 40.59  & 38.87  & 40.09  & 41.56  & 42.87  & 44.85  & 42.36  & 39.98  & 38.86  & 40.17  & 40.26  & 42.12  & 43.17  & 40.67  & 44.75  & 36.45  \\
\cmidrule{3-21}          &       & /     & /     & 0.960  & 0.981  & 0.970  & 0.970  & 0.979  & 0.984  & 0.992  & 0.975  & 0.967  & 0.972  & 0.966  & 0.966  & 0.982  & 0.982  & 0.973  & 0.987  & 0.963  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DCDicL} & /     & /     & 36.61  & /     & 37.45  & 38.12  & 37.77  & 38.24  & 38.39  & 38.62  & 35.87  & 36.07  & 35.83  & 36.25  & 39.84  & 39.38  & 37.04  & 40.24  & 34.72  \\
\cmidrule{3-21}          &       & /     & /     & 0.945  & /     & 0.972  & 0.965  & 0.970  & 0.977  & 0.990  & 0.968  & 0.968  & 0.975  & 0.956  & 0.971  & 0.984  & 0.976  & 0.969  & 0.980  & 0.955  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DeamNet} & 39.63  & 39.35  & 36.63  & /     & 37.70  & 36.93  & 40.90  & 40.86  & 41.22  & 39.72  & 33.67  & 36.40  & 37.87  & 35.07  & 40.25  & 38.92  & 39.56  & 40.52  & 34.61  \\
\cmidrule{3-21}          &       & 0.953  & 0.955  & 0.936  & /     & 0.958  & 0.944  & 0.977  & 0.978  & 0.979  & 0.967  & 0.953  & 0.964  & 0.961  & 0.948  & 0.966  & 0.957  & 0.969  & 0.980  & 0.952  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DIDN} & 39.64  & 39.78  & 36.06  & /     & 37.36  & 38.24  & 40.74  & 41.68  & 42.35  & 41.17  & 38.15  & 37.87  & 38.27  & 38.58  & 40.03  & 40.32  & 39.73  & 44.07  & 35.28  \\
\cmidrule{3-21}          &       & 0.953  & 0.958  & 0.946  & /     & 0.953  & 0.950  & 0.975  & 0.977  & 0.975  & 0.966  & 0.951  & 0.965  & 0.954  & 0.950  & 0.963  & 0.959  & 0.966  & 0.985  & 0.949  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DnCNN} & 37.90  & 37.73  & 37.47  & 39.32  & 38.51  & 40.01  & 40.81  & 41.91  & 44.16  & 41.57  & 39.92  & 38.72  & 39.34  & 40.22  & 42.03  & 42.12  & 40.26  & 43.97  & 36.30  \\
\cmidrule{3-21}          &       & 0.943  & 0.941  & 0.954  & 0.974  & 0.966  & 0.971  & 0.972  & 0.979  & 0.991  & 0.969  & 0.962  & 0.973  & 0.964  & 0.969  & 0.983  & 0.977  & 0.970  & 0.984  & 0.960  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DPIR} & /     & /     & 38.30  & 40.33  & 38.93  & 40.77  & 41.94  & 42.62  & 45.36  & 42.78  & 40.35  & 39.17  & 40.80  & 40.80  & 42.86  & 42.86  & 40.96  & 45.76  & 36.61  \\
\cmidrule{3-21}          &       & /     & /     & 0.961  & 0.979  & 0.970  & 0.974  & 0.978  & 0.982  & 0.993  & 0.977  & 0.969  & 0.975  & 0.966  & 0.970  & 0.985  & 0.980  & 0.974  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DudeNet} & 33.18  & 27.55  & 36.03  & 37.44  & 39.92  & 38.18  & 39.94  & 41.13  & 42.97  & 41.06  & 38.63  & 37.83  & 39.09  & 38.58  & 40.73  & 40.63  & 39.71  & 43.34  & 35.44  \\
\cmidrule{3-21}          &       & 0.810  & 0.645  & 0.933  & 0.953  & 0.973  & 0.955  & 0.972  & 0.977  & 0.988  & 0.971  & 0.962  & 0.969  & 0.962  & 0.961  & 0.976  & 0.969  & 0.972  & 0.985  & 0.955  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{FCCF} & 36.30  & 23.32  & 39.02  & 40.89  & 38.87  & 41.20  & 42.03  & 43.07  & 45.15  & 42.80  & 40.14  & 39.04  & 40.61  & 40.66  & 42.31  & 43.05  & 40.95  & 45.47  & 36.72  \\
\cmidrule{3-21}          &       & 0.885  & 0.461  & 0.968  & 0.982  & 0.971  & 0.978  & 0.980  & 0.985  & 0.993  & 0.978  & 0.966  & 0.974  & 0.967  & 0.969  & 0.984  & 0.982  & 0.975  & 0.989  & 0.964  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{FFD-Net} & 37.61  & 38.27  & 37.67  & 39.73  & 38.76  & 40.28  & 41.67  & 42.55  & 44.77  & 42.44  & 40.05  & 38.96  & 40.60  & 40.50  & 42.43  & 42.44  & 40.75  & 45.71  & 36.47  \\
\cmidrule{3-21}          &       & 0.942  & 0.948  & 0.956  & 0.977  & 0.970  & 0.973  & 0.977  & 0.982  & 0.992  & 0.976  & 0.967  & 0.974  & 0.964  & 0.971  & 0.984  & 0.979  & 0.973  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{IDR} & /     & /     & 34.26  & 36.18  & 36.28  & 36.44  & 39.33  & 40.31  & 40.94  & 39.74  & 37.38  & 37.39  & 38.30  & 38.15  & 39.68  & 38.22  & 38.01  & 43.15  & 34.64  \\
\cmidrule{3-21}          &       & /     & /     & 0.877  & 0.923  & 0.925  & 0.910  & 0.955  & 0.962  & 0.961  & 0.935  & 0.927  & 0.957  & 0.938  & 0.944  & 0.951  & 0.913  & 0.941  & 0.978  & 0.929  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{InvDN} & 39.57  & 39.28  & 34.55  & 36.33  & 35.94  & 38.01  & 38.95  & 40.09  & 42.03  & 40.02  & 33.32  & 37.00  & 36.64  & 37.66  & 40.06  & 40.98  & 39.10  & 40.74  & 34.15  \\
\cmidrule{3-21}          &       & 0.952  & 0.955  & 0.937  & 0.953  & 0.947  & 0.952  & 0.965  & 0.973  & 0.978  & 0.960  & 0.930  & 0.965  & 0.939  & 0.955  & 0.966  & 0.971  & 0.964  & 0.969  & 0.935  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{IRCNN} & 34.78  & 33.50  & 37.26  & 37.25  & 37.49  & 39.66  & 41.24  & 41.85  & 43.89  & 41.78  & 39.91  & 38.63  & 40.14  & 40.12  & 41.87  & 41.86  & 40.26  & 44.38  & 36.22  \\
\cmidrule{3-21}          &       & 0.907  & 0.887  & 0.954  & 0.956  & 0.956  & 0.970  & 0.978  & 0.981  & 0.991  & 0.973  & 0.969  & 0.972  & 0.965  & 0.969  & 0.983  & 0.977  & 0.972  & 0.988  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{MIRNet} & 39.88  & 39.55  & 36.06  & 37.25  & 37.49  & 38.10  & 40.72  & 41.68  & 42.76  & 41.05  & 38.28  & 37.80  & 38.60  & 38.55  & 40.28  & 40.46  & 39.73  & 43.66  & 35.42  \\
\cmidrule{3-21}          &       & 0.956  & 0.957  & 0.942  & 0.956  & 0.956  & 0.952  & 0.975  & 0.978  & 0.980  & 0.968  & 0.954  & 0.967  & 0.959  & 0.952  & 0.966  & 0.964  & 0.967  & 0.983  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{MPRNet} & 39.82  & 39.57  & 35.94  & /     & 37.50  & 38.04  & 40.59  & 41.30  & 42.59  & 41.23  & 38.35  & 37.92  & 38.95  & 38.62  & 40.21  & 40.20  & 39.77  & 44.05  & 35.49  \\
\cmidrule{3-21}          &       & 0.954  & 0.958  & 0.935  & /     & 0.954  & 0.946  & 0.974  & 0.974  & 0.978  & 0.969  & 0.952  & 0.966  & 0.960  & 0.949  & 0.965  & 0.960  & 0.967  & 0.986  & 0.951  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{NAFNet} & 38.36  & 40.15  & 34.39  & /     & 36.38  & 37.88  & 40.12  & 40.23  & 40.66  & 40.01  & 36.13  & 35.87  & 36.66  & 36.79  & 36.53  & 39.93  & 39.32  & 40.45  & 34.82  \\
\cmidrule{3-21}          &       & 0.943  & 0.960  & 0.923  & /     & 0.947  & 0.954  & 0.973  & 0.943  & 0.936  & 0.962  & 0.919  & 0.927  & 0.948  & 0.927  & 0.884  & 0.951  & 0.966  & 0.924  & 0.948  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{NBNet} & 39.89  & 39.64  & 35.89  & /     & 37.37  & 38.32  & 40.95  & 41.91  & 42.92  & 41.17  & 38.02  & 37.87  & 37.79  & 38.45  & 40.51  & 40.45  & 39.73  & 43.96  & 35.37  \\
\cmidrule{3-21}          &       & 0.955  & 0.958  & 0.935  & /     & 0.957  & 0.955  & 0.977  & 0.980  & 0.982  & 0.971  & 0.955  & 0.967  & 0.956  & 0.955  & 0.972  & 0.967  & 0.969  & 0.984  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Neigh2Neigh} & /     & /     & 34.47  & 35.65  & 37.10  & 36.59  & 40.22  & 40.41  & 41.29  & 41.24  & 38.13  & 37.94  & 39.71  & 38.50  & 39.63  & 38.05  & 39.17  & 44.49  & 35.30  \\
\cmidrule{3-21}          &       & /     & /     & 0.883  & 0.907  & 0.942  & 0.908  & 0.967  & 0.960  & 0.966  & 0.958  & 0.940  & 0.961  & 0.956  & 0.936  & 0.952  & 0.919  & 0.958  & 0.984  & 0.944  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{NLNet} & /     & /     & 37.56  & 39.32  & 38.58  & 40.17  & 41.43  & 42.18  & 44.53  & 42.19  & 39.96  & 38.89  & 40.06  & 40.61  & 42.14  & 42.16  & 40.63  & 44.87  & 36.34  \\
\cmidrule{3-21}          &       & /     & /     & 0.955  & 0.974  & 0.968  & 0.973  & 0.976  & 0.981  & 0.991  & 0.974  & 0.969  & 0.973  & 0.964  & 0.971  & 0.983  & 0.978  & 0.973  & 0.988  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Noise2Noise} & /     & /     & 33.55  & 34.67  & 35.91  & 35.28  & 38.88  & 39.07  & 39.34  & 39.26  & 36.81  & 36.99  & 38.04  & 37.21  & 38.00  & 36.35  & 37.67  & 42.59  & 34.44  \\
\cmidrule{3-21}          &       & /     & /     & 0.850  & 0.874  & 0.913  & 0.875  & 0.950  & 0.940  & 0.938  & 0.931  & 0.919  & 0.948  & 0.936  & 0.916  & 0.924  & 0.876  & 0.936  & 0.975  & 0.926  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{PD-Denoising} & 38.40  & 33.99  & 35.85  & 37.13  & 37.13  & 37.12  & 40.85  & 41.38  & 41.13  & 41.05  & 37.72  & 37.57  & 39.03  & 38.01  & 39.18  & 39.64  & 38.80  & 43.73  & 35.05  \\
\cmidrule{3-21}          &       & 0.943  & 0.896  & 0.924  & 0.944  & 0.944  & 0.921  & 0.974  & 0.974  & 0.966  & 0.959  & 0.935  & 0.956  & 0.948  & 0.929  & 0.948  & 0.946  & 0.955  & 0.981  & 0.940  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{PNGAN} & 39.38  & 39.81  & 38.44  & /     & 39.57  & 40.51  & 41.79  & 43.13  & 44.73  & 42.55  & 39.84  & 38.78  & 40.63  & 40.20  & 41.85  & 43.15  & 40.87  & 45.32  & 36.40  \\
\cmidrule{3-21}          &       & 0.953  & 0.959  & 0.963  & /     & 0.974  & 0.974  & 0.979  & 0.985  & 0.992  & 0.977  & 0.964  & 0.970  & 0.969  & 0.962  & 0.981  & 0.982  & 0.974  & 0.988  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{R2R} & /     & /     & 36.32  & 38.11  & 38.57  & 38.71  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{3-21}          &       & /     & /     & 0.937  & 0.961  & 0.970  & 0.958  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Restormer} & 40.03  & 39.79  & 36.33  & /     & 37.66  & 38.29  & 41.10  & 41.84  & 42.49  & 41.47  & 38.42  & 38.08  & 39.05  & 38.77  & 40.13  & 40.53  & 39.56  & 44.19  & 35.65  \\
\cmidrule{3-21}          &       & 0.956  & 0.959  & 0.941  & /     & 0.956  & 0.948  & 0.977  & 0.979  & 0.976  & 0.968  & 0.952  & 0.966  & 0.960  & 0.949  & 0.963  & 0.962  & 0.963  & 0.986  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{RIDNet} & 39.26  & 38.70  & 36.84  & 38.11  & 38.57  & 38.60  & 41.09  & 42.15  & 42.39  & 41.59  & 38.88  & 38.21  & 38.67  & 39.02  & 40.91  & 41.01  & 40.07  & 44.40  & 35.76  \\
\cmidrule{3-21}          &       & 0.953  & 0.950  & 0.941  & 0.961  & 0.970  & 0.956  & 0.977  & 0.980  & 0.989  & 0.975  & 0.962  & 0.970  & 0.963  & 0.959  & 0.978  & 0.977  & 0.972  & 0.987  & 0.957  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{SADNet} & 39.59  & /     & 37.76  & 38.11  & 39.22  & 38.90  & 40.82  & 42.02  & 44.25  & 41.85  & 39.53  & 38.33  & 39.83  & 39.69  & 39.81  & 41.64  & 40.70  & 44.61  & 36.36  \\
\cmidrule{3-21}          &       & 0.952  & /     & 0.952  & 0.961  & 0.972  & 0.965  & 0.976  & 0.980  & 0.992  & 0.975  & 0.965  & 0.970  & 0.965  & 0.963  & 0.965  & 0.979  & 0.974  & 0.988  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Self2Self} & /     & /     & 36.26  & 38.23  & /     & 39.49  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{3-21}          &       & /     & /     & 0.947  & 0.969  & /     & 0.963  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Unet} & /     & /     & 36.95  & 38.96  & 38.05  & 39.62  & 40.40  & 41.36  & 43.58  & 41.12  & 39.35  & 38.25  & 38.94  & 39.95  & 41.32  & 41.70  & 39.51  & 43.17  & 36.09  \\
\cmidrule{3-21}          &       & /     & /     & 0.943  & 0.971  & 0.962  & 0.967  & 0.968  & 0.977  & 0.989  & 0.968  & 0.963  & 0.971  & 0.959  & 0.968  & 0.979  & 0.974  & 0.966  & 0.981  & 0.958  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{VDNet} & /     & /     & 35.86  & /     & 37.58  & 38.43  & 40.97  & 42.37  & 43.08  & 41.19  & 38.23  & 37.95  & 37.88  & 38.60  & 40.81  & 41.21  & 39.93  & 44.27  & 35.49  \\
\cmidrule{3-21}          &       & /     & /     & 0.945  & /     & 0.957  & 0.955  & 0.976  & 0.983  & 0.983  & 0.970  & 0.956  & 0.968  & 0.956  & 0.956  & 0.973  & 0.970  & 0.970  & 0.984  & 0.953  \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_Results_Color_image_all}%
\end{table*}%


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_Results_MRI_all.tex <==
% Table generated by Excel2LaTeX from sheet 'Reported results combined'
%\begin{table*}[htbp]
%  \centering
%    \caption{Average PSNR/SSIM and computational time (s) of different methods on Brainweb and FastMRI data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
%    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%    \toprule
%    \multicolumn{1}{c}{Datasets} & $\sigma(\%)$ & 4DHOSVD & AONLM & BM4D1 & BM4D2 & ILR-HOSVD & OLMMSE & ROLMMSE & MStSVD & NLPCA & ODCT  & PRINLM & PRI-NLPCA \\
%    \midrule
%    \multirow{10}[20]{*}{Brainweb} & 1     & 43.86/0.993 & 41.87/0.991 & 43.18/0.992 & 43.43/0.992 & 44.55/0.994 & 42.37/0.991 & 42.39/0.991 & 43.99/0.993 & 44.13/0.994 & 43.25/0.992 & 43.33/0.993 & 44.28/0.994 \\
%\cmidrule{2-14}          & 3     & 37.49/0.976 & 36.52/0.971 & 36.59/0.971 & 37.21/0.975 & 38.22/0.981 & 35.99/0.968 & 35.98/0.969 & 37.46/0.975 & 37.74/0.977 & 36.43/0.970 & 36.87/0.975 & 38.12/0.981 \\
%\cmidrule{2-14}          & 5     & 34.64/0.959 & 33.78/0.947 & 33.71/0.950 & 34.56/0.959 & 35.46/0.966 & 33.37/0.949 & 33.36/0.949 & 34.65/0.958 & 33.84/0.940 & 33.57/0.949 & 33.97/0.955 & 35.29/0.967 \\
%\cmidrule{2-14}          & 7     & 32.85/0.941 & 31.91/0.921 & 31.80/0.926 & 32.84/0.943 & 33.62/0.951 & 31.58/0.925 & 31.61/0.928 & 32.83/0.940 & 31.87/0.912 & 31.66/0.927 & 32.01/0.934 & 33.36/0.951 \\
%\cmidrule{2-14}          & 9     & 31.49/0.922 & 30.47/0.894 & 30.35/0.901 & 31.54/0.928 & 32.31/0.938 & 30.16/0.898 & 30.23/0.904 & 31.31/0.924 & 31.15/0.908 & 30.23/0.905 & 30.49/0.911 & 31.86/0.934 \\
%\cmidrule{2-14}          & 11    & 30.36/0.903 & 29.29/0.865 & 29.15/0.873 & 30.49/0.912 & 31.17/0.922 & 28.93/0.868 & 29.09/0.880 & 30.22/0.906 & 29.98/0.883 & 29.08/0.882 & 29.28/0.888 & 30.66/0.916 \\
%\cmidrule{2-14}          & 13    & 29.40/0.883 & 28.26/0.836 & 28.14/0.844 & 29.59/0.895 & 30.22/0.909 & 27.82/0.834 & 28.08/0.856 & 29.29/0.888 & 28.97/0.855 & 28.11/0.861 & 28.24/0.864 & 29.65/0.898 \\
%\cmidrule{2-14}          & 15    & 28.56/0.862 & 27.35/0.807 & 27.26/0.814 & 28.81/0.879 & 29.42/0.894 & 26.82/0.799 & 27.26/0.835 & 28.48/0.870 & 28.06/0.826 & 27.27/0.841 & 27.36/0.841 & 28.76/0.879 \\
%\cmidrule{2-14}          & 17    & 27.79/0.842 & 26.50/0.775 & 26.46/0.785 & 28.10/0.862 & 27.87/0.845 & 25.91/0.762 & 26.54/0.815 & 27.74/0.853 & 27.27/0.798 & 26.52/0.819 & 26.59/0.817 & 27.97/0.860 \\
%\cmidrule{2-14}          & 19    & 27.09/0.822 & 25.74/0.744 & 25.73/0.755 & 27.44/0.845 & 27.26/0.828 & 25.05/0.725 & 25.86/0.797 & 27.07/0.835 & 26.56/0.772 & 25.83/0.799 & 25.92/0.797 & 27.25/0.841 \\
%    \midrule
%    \multirow{10}[20]{*}{FastMRI} & 1     & 29.50/0.936 & 39.36/0.956 & 42.07/0.977 & 42.53/0.979 & 42.30/0.977 & /     & /     & 42.09/0.977 & 29.69/0.941 & 40.96/0.968 & /     & / \\
%\cmidrule{2-14}          & 3     & 28.98/0.907 & 36.12/0.921 & 36.68/0.933 & 37.07/0.937 & 37.09/0.933 & /     & /     & 36.74/0.935 & 29.01/0.906 & 36.68/0.930 & /     & / \\
%\cmidrule{2-14}          & 5     & 29.57/0.887 & 34.01/0.884 & 34.57/0.901 & 35.12/0.911 & 35.34/0.911 & /     & /     & 34.61/0.906 & 29.14/0.866 & 34.62/0.899 & /     & / \\
%\cmidrule{2-14}          & 7     & 29.36/0.865 & 32.29/0.842 & 33.01/0.867 & 33.82/0.889 & 34.01/0.888 & /     & /     & 33.10/0.878 & 28.66/0.826 & 33.11/0.869 & /     & / \\
%\cmidrule{2-14}          & 9     & 29.07/0.840 & 30.79/0.793 & 31.61/0.829 & 32.71/0.866 & 33.04/0.868 & /     & /     & 31.92/0.854 & 28.76/0.819 & 31.81/0.836 & /     & / \\
%\cmidrule{2-14}          & 11    & 28.71/0.812 & 29.43/0.741 & 30.29/0.785 & 31.69/0.841 & 32.03/0.844 & /     & /     & 30.88/0.827 & 28.29/0.780 & 30.63/0.801 & /     & / \\
%\cmidrule{2-14}          & 13    & 28.24/0.779 & 28.18/0.683 & 29.05/0.737 & 30.72/0.814 & 31.19/0.822 & /     & /     & 29.92/0.799 & 27.74/0.738 & 29.55/0.764 & /     & / \\
%\cmidrule{2-14}          & 15    & 27.71/0.744 & 27.04/0.626 & 27.87/0.686 & 29.80/0.785 & 30.24/0.794 & /     & /     & 29.01/0.770 & 27.14/0.693 & 28.57/0.727 & /     & / \\
%\cmidrule{2-14}          & 17    & 27.11/0.708 & 26.01/0.571 & 26.77/0.634 & 28.92/0.755 & 29.48/0.769 & /     & /     & 28.15/0.741 & 26.49/0.649 & 27.7/0.693 & /     & / \\
%\cmidrule{2-14}          & 19    & 26.49/0.671 & 25.04/0.519 & 25.76/0.583 & 28.09/0.725 & 28.77/0.744 & /     & /     & 27.34/0.711 & 25.84/0.606 & 26.90/0.660 & /     & / \\
%    \midrule
%    Time (s) & /     & 614.1  & 426.7  & 57.1  & 171.2  & 1552.9  & >1h   & >1h   & 141.4  & 517.8  & 4.5   & 11.0  & 986.9  \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_Results_MRI_all}%
%\end{table*}%

%% Table generated by Excel2LaTeX from sheet 'Reported results combined'
%\begin{table*}[htbp]
%\scriptsize \tabcolsep5pt
%  \centering
%    \caption{Average PSNR/SSIM and computational time (s) of different methods on Brainweb and fastMRI data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
%    \scalebox{0.838}{
%    \begin{tabular}{cccccccccccccc}
%    \toprule
%    Datasets & $\sigma(\%)$ & 4DHOSVD & AONLM & BM4D1 & BM4D2 & ILR-HOSVD & OLMMSE & ROLMMSE & MStSVD & NLPCA & ODCT  & PRINLM & PRI-NLPCA \\
%    \midrule
%    \multirow{10}[20]{*}{Brainweb} & 1     & 43.86/0.993 & 41.87/0.991 & 43.18/0.992 & 43.43/0.992 & 44.55/0.994 & 42.37/0.991 & 42.39/0.991 & 43.99/0.993 & 44.13/0.994 & 43.25/0.992 & 43.33/0.993 & 44.28/0.994 \\
%\cmidrule{2-14}          & 3     & 37.49/0.976 & 36.52/0.971 & 36.59/0.971 & 37.21/0.975 & 38.22/0.981 & 35.99/0.968 & 35.98/0.969 & 37.46/0.975 & 37.74/0.977 & 36.43/0.970 & 36.87/0.975 & 38.12/0.981 \\
%\cmidrule{2-14}          & 5     & 34.64/0.959 & 33.78/0.947 & 33.71/0.950 & 34.56/0.959 & 35.46/0.966 & 33.37/0.949 & 33.36/0.949 & 34.65/0.958 & 33.84/0.940 & 33.57/0.949 & 33.97/0.955 & 35.29/0.967 \\
%\cmidrule{2-14}          & 7     & 32.85/0.941 & 31.91/0.921 & 31.80/0.926 & 32.84/0.943 & 33.62/0.951 & 31.58/0.925 & 31.61/0.928 & 32.83/0.940 & 31.87/0.912 & 31.66/0.927 & 32.01/0.934 & 33.36/0.951 \\
%\cmidrule{2-14}          & 9     & 31.49/0.922 & 30.47/0.894 & 30.35/0.901 & 31.54/0.928 & 32.31/0.938 & 30.16/0.898 & 30.23/0.904 & 31.31/0.924 & 31.15/0.908 & 30.23/0.905 & 30.49/0.911 & 31.86/0.934 \\
%\cmidrule{2-14}          & 11    & 30.36/0.903 & 29.29/0.865 & 29.15/0.873 & 30.49/0.912 & 31.17/0.922 & 28.93/0.868 & 29.09/0.880 & 30.22/0.906 & 29.98/0.883 & 29.08/0.882 & 29.28/0.888 & 30.66/0.916 \\
%\cmidrule{2-14}          & 13    & 29.40/0.883 & 28.26/0.836 & 28.14/0.844 & 29.59/0.895 & 30.22/0.909 & 27.82/0.834 & 28.08/0.856 & 29.29/0.888 & 28.97/0.855 & 28.11/0.861 & 28.24/0.864 & 29.65/0.898 \\
%\cmidrule{2-14}          & 15    & 28.56/0.862 & 27.35/0.807 & 27.26/0.814 & 28.81/0.879 & 29.42/0.894 & 26.82/0.799 & 27.26/0.835 & 28.48/0.870 & 28.06/0.826 & 27.27/0.841 & 27.36/0.841 & 28.76/0.879 \\
%\cmidrule{2-14}          & 17    & 27.79/0.842 & 26.50/0.775 & 26.46/0.785 & 28.10/0.862 & 27.87/0.845 & 25.91/0.762 & 26.54/0.815 & 27.74/0.853 & 27.27/0.798 & 26.52/0.819 & 26.59/0.817 & 27.97/0.860 \\
%\cmidrule{2-14}          & 19    & 27.09/0.822 & 25.74/0.744 & 25.73/0.755 & 27.44/0.845 & 27.26/0.828 & 25.05/0.725 & 25.86/0.797 & 27.07/0.835 & 26.56/0.772 & 25.83/0.799 & 25.92/0.797 & 27.25/0.841 \\
%    \midrule
%    \multirow{10}[20]{*}{fastMRI} & 1     & 29.50/0.936 & 39.36/0.956 & 42.07/0.977 & 42.53/0.979 & 42.30/0.977 & /     & /     & 42.09/0.977 & 29.69/0.941 & 40.96/0.968 & /     & / \\
%\cmidrule{2-14}          & 3     & 28.98/0.907 & 36.12/0.921 & 36.68/0.933 & 37.07/0.937 & 37.09/0.933 & /     & /     & 36.74/0.935 & 29.01/0.906 & 36.68/0.930 & /     & / \\
%\cmidrule{2-14}          & 5     & 29.57/0.887 & 34.01/0.884 & 34.57/0.901 & 35.12/0.911 & 35.34/0.911 & /     & /     & 34.61/0.906 & 29.14/0.866 & 34.62/0.899 & /     & / \\
%\cmidrule{2-14}          & 7     & 29.36/0.865 & 32.29/0.842 & 33.01/0.867 & 33.82/0.889 & 34.01/0.888 & /     & /     & 33.10/0.878 & 28.66/0.826 & 33.11/0.869 & /     & / \\
%\cmidrule{2-14}          & 9     & 29.07/0.840 & 30.79/0.793 & 31.61/0.829 & 32.71/0.866 & 33.04/0.868 & /     & /     & 31.92/0.854 & 28.76/0.819 & 31.81/0.836 & /     & / \\
%\cmidrule{2-14}          & 11    & 28.71/0.812 & 29.43/0.741 & 30.29/0.785 & 31.69/0.841 & 32.03/0.844 & /     & /     & 30.88/0.827 & 28.29/0.780 & 30.63/0.801 & /     & / \\
%\cmidrule{2-14}          & 13    & 28.24/0.779 & 28.18/0.683 & 29.05/0.737 & 30.72/0.814 & 31.19/0.822 & /     & /     & 29.92/0.799 & 27.74/0.738 & 29.55/0.764 & /     & / \\
%\cmidrule{2-14}          & 15    & 27.71/0.744 & 27.04/0.626 & 27.87/0.686 & 29.80/0.785 & 30.24/0.794 & /     & /     & 29.01/0.770 & 27.14/0.693 & 28.57/0.727 & /     & / \\
%\cmidrule{2-14}          & 17    & 27.11/0.708 & 26.01/0.571 & 26.77/0.634 & 28.92/0.755 & 29.48/0.769 & /     & /     & 28.15/0.741 & 26.49/0.649 & 27.7/0.693 & /     & / \\
%\cmidrule{2-14}          & 19    & 26.49/0.671 & 25.04/0.519 & 25.76/0.583 & 28.09/0.725 & 28.77/0.744 & /     & /     & 27.34/0.711 & 25.84/0.606 & 26.90/0.660 & /     & / \\
%    \midrule
%    Time (s) & /     & 614.1  & 426.7  & 57.1  & 171.2  & 1552.9  & $>$1h   & $>$1h   & 141.4  & 517.8  & 4.5   & 11.0  & 986.9  \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_Results_MRI_all}%
%  }
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Reported results combined'
% Table generated by Excel2LaTeX from sheet 'Reported results combined'
%\begin{table*}[htbp]
%  \centering
%    \caption{Average PSNR-SSIM and computational time (s) of different methods on Brainweb and FastMRI data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
%    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%    \toprule
%    \multicolumn{1}{c}{Datasets} & $\sigma(\%)$ & 4DHOSVD & AONLM & BM4D1 & BM4D2 & ILR-HOSVD & OLMMSE & ROLMMSE & MStSVD & NLPCA & ODCT  & PRINLM & PRI-NLPCA \\
%    \midrule
%    \multirow{10}[20]{*}{Brainweb} & 1     & 43.86-0.993 & 41.87-0.991 & 43.18-0.992 & 43.43-0.992 & 44.55-0.994 & 42.37-0.991 & 42.39-0.991 & 43.99-0.993 & 44.13-0.994 & 43.25-0.992 & 43.33-0.993 & 44.28-0.994 \\
%\cmidrule{2-14}          & 3     & 37.49-0.976 & 36.52-0.971 & 36.59-0.971 & 37.21-0.975 & 38.22-0.981 & 35.99-0.968 & 35.98-0.969 & 37.46-0.975 & 37.74-0.977 & 36.43-0.970 & 36.87-0.975 & 38.12-0.981 \\
%\cmidrule{2-14}          & 5     & 34.64-0.959 & 33.78-0.947 & 33.71-0.950 & 34.56-0.959 & 35.46-0.966 & 33.37-0.949 & 33.36-0.949 & 34.65-0.958 & 33.84-0.940 & 33.57-0.949 & 33.97-0.955 & 35.29-0.967 \\
%\cmidrule{2-14}          & 7     & 32.85-0.941 & 31.91-0.921 & 31.80-0.926 & 32.84-0.943 & 33.62-0.951 & 31.58-0.925 & 31.61-0.928 & 32.83-0.940 & 31.87-0.912 & 31.66-0.927 & 32.01-0.934 & 33.36-0.951 \\
%\cmidrule{2-14}          & 9     & 31.49-0.922 & 30.47-0.894 & 30.35-0.901 & 31.54-0.928 & 32.31-0.938 & 30.16-0.898 & 30.23-0.904 & 31.31-0.924 & 31.15-0.908 & 30.23-0.905 & 30.49-0.911 & 31.86-0.934 \\
%\cmidrule{2-14}          & 11    & 30.36-0.903 & 29.29-0.865 & 29.15-0.873 & 30.49-0.912 & 31.17-0.922 & 28.93-0.868 & 29.09-0.880 & 30.22-0.906 & 29.98-0.883 & 29.08-0.882 & 29.28-0.888 & 30.66-0.916 \\
%\cmidrule{2-14}          & 13    & 29.40-0.883 & 28.26-0.836 & 28.14-0.844 & 29.59-0.895 & 30.22-0.909 & 27.82-0.834 & 28.08-0.856 & 29.29-0.888 & 28.97-0.855 & 28.11-0.861 & 28.24-0.864 & 29.65-0.898 \\
%\cmidrule{2-14}          & 15    & 28.56-0.862 & 27.35-0.807 & 27.26-0.814 & 28.81-0.879 & 29.42-0.894 & 26.82-0.799 & 27.26-0.835 & 28.48-0.870 & 28.06-0.826 & 27.27-0.841 & 27.36-0.841 & 28.76-0.879 \\
%\cmidrule{2-14}          & 17    & 27.79-0.842 & 26.50-0.775 & 26.46-0.785 & 28.10-0.862 & 27.87-0.845 & 25.91-0.762 & 26.54-0.815 & 27.74-0.853 & 27.27-0.798 & 26.52-0.819 & 26.59-0.817 & 27.97-0.860 \\
%\cmidrule{2-14}          & 19    & 27.09-0.822 & 25.74-0.744 & 25.73-0.755 & 27.44-0.845 & 27.26-0.828 & 25.05-0.725 & 25.86-0.797 & 27.07-0.835 & 26.56-0.772 & 25.83-0.799 & 25.92-0.797 & 27.25-0.841 \\
%    \midrule
%    \multirow{10}[20]{*}{FastMRI} & 1     & 29.50-0.936 & 39.36-0.956 & 42.07-0.977 & 42.53-0.979 & 42.30-0.977 & -     & -     & 42.09-0.977 & 29.69-0.941 & 40.96-0.968 & -     & - \\
%\cmidrule{2-14}          & 3     & 28.98-0.907 & 36.12-0.921 & 36.68-0.933 & 37.07-0.937 & 37.09-0.933 & -     & -     & 36.74-0.935 & 29.01-0.906 & 36.68-0.930 & -     & - \\
%\cmidrule{2-14}          & 5     & 29.57-0.887 & 34.01-0.884 & 34.57-0.901 & 35.12-0.911 & 35.34-0.911 & -     & -     & 34.61-0.906 & 29.14-0.866 & 34.62-0.899 & -     & - \\
%\cmidrule{2-14}          & 7     & 29.36-0.865 & 32.29-0.842 & 33.01-0.867 & 33.82-0.889 & 34.01-0.888 & -     & -     & 33.10-0.878 & 28.66-0.826 & 33.11-0.869 & -     & - \\
%\cmidrule{2-14}          & 9     & 29.07-0.840 & 30.79-0.793 & 31.61-0.829 & 32.71-0.866 & 33.04-0.868 & -     & -     & 31.92-0.854 & 28.76-0.819 & 31.81-0.836 & -     & - \\
%\cmidrule{2-14}          & 11    & 28.71-0.812 & 29.43-0.741 & 30.29-0.785 & 31.69-0.841 & 32.03-0.844 & -     & -     & 30.88-0.827 & 28.29-0.780 & 30.63-0.801 & -     & - \\
%\cmidrule{2-14}          & 13    & 28.24-0.779 & 28.18-0.683 & 29.05-0.737 & 30.72-0.814 & 31.19-0.822 & -     & -     & 29.92-0.799 & 27.74-0.738 & 29.55-0.764 & -     & - \\
%\cmidrule{2-14}          & 15    & 27.71-0.744 & 27.04-0.626 & 27.87-0.686 & 29.80-0.785 & 30.24-0.794 & -     & -     & 29.01-0.770 & 27.14-0.693 & 28.57-0.727 & -     & - \\
%\cmidrule{2-14}          & 17    & 27.11-0.708 & 26.01-0.571 & 26.77-0.634 & 28.92-0.755 & 29.48-0.769 & -     & -     & 28.15-0.741 & 26.49-0.649 & 27.7-0.693 & -     & - \\
%\cmidrule{2-14}          & 19    & 26.49-0.671 & 25.04-0.519 & 25.76-0.583 & 28.09-0.725 & 28.77-0.744 & -     & -     & 27.34-0.711 & 25.84-0.606 & 26.90-0.660 & -     & - \\
%    \midrule
%    Time (s) & -     & 614.1  & 426.7  & 57.1  & 171.2  & 1552.9  & >1h   & >1h   & 141.4  & 517.8  & 4.5   & 11.0  & 986.9  \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_Results_MRI_all}%
%\end{table*}%

%% Table generated by Excel2LaTeX from sheet 'Reported results combined'
%\begin{table*}[htbp]
%\scriptsize \tabcolsep5pt
%  \centering
%    \caption{Average PSNR-SSIM and computational time (s) of different methods on Brainweb and fastMRI data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
%    \scalebox{0.838}{
%    \begin{tabular}{cccccccccccccc}
%    \toprule
%    Datasets & $\sigma(\%)$ & 4DHOSVD & AONLM & BM4D1 & BM4D2 & ILR-HOSVD & OLMMSE & ROLMMSE & MStSVD & NLPCA & ODCT  & PRINLM & PRI-NLPCA \\
%    \midrule
%    \multirow{10}[20]{*}{Brainweb} & 1     & 43.86-0.993 & 41.87-0.991 & 43.18-0.992 & 43.43-0.992 & 44.55-0.994 & 42.37-0.991 & 42.39-0.991 & 43.99-0.993 & 44.13-0.994 & 43.25-0.992 & 43.33-0.993 & 44.28-0.994 \\
%\cmidrule{2-14}          & 3     & 37.49-0.976 & 36.52-0.971 & 36.59-0.971 & 37.21-0.975 & 38.22-0.981 & 35.99-0.968 & 35.98-0.969 & 37.46-0.975 & 37.74-0.977 & 36.43-0.970 & 36.87-0.975 & 38.12-0.981 \\
%\cmidrule{2-14}          & 5     & 34.64-0.959 & 33.78-0.947 & 33.71-0.950 & 34.56-0.959 & 35.46-0.966 & 33.37-0.949 & 33.36-0.949 & 34.65-0.958 & 33.84-0.940 & 33.57-0.949 & 33.97-0.955 & 35.29-0.967 \\
%\cmidrule{2-14}          & 7     & 32.85-0.941 & 31.91-0.921 & 31.80-0.926 & 32.84-0.943 & 33.62-0.951 & 31.58-0.925 & 31.61-0.928 & 32.83-0.940 & 31.87-0.912 & 31.66-0.927 & 32.01-0.934 & 33.36-0.951 \\
%\cmidrule{2-14}          & 9     & 31.49-0.922 & 30.47-0.894 & 30.35-0.901 & 31.54-0.928 & 32.31-0.938 & 30.16-0.898 & 30.23-0.904 & 31.31-0.924 & 31.15-0.908 & 30.23-0.905 & 30.49-0.911 & 31.86-0.934 \\
%\cmidrule{2-14}          & 11    & 30.36-0.903 & 29.29-0.865 & 29.15-0.873 & 30.49-0.912 & 31.17-0.922 & 28.93-0.868 & 29.09-0.880 & 30.22-0.906 & 29.98-0.883 & 29.08-0.882 & 29.28-0.888 & 30.66-0.916 \\
%\cmidrule{2-14}          & 13    & 29.40-0.883 & 28.26-0.836 & 28.14-0.844 & 29.59-0.895 & 30.22-0.909 & 27.82-0.834 & 28.08-0.856 & 29.29-0.888 & 28.97-0.855 & 28.11-0.861 & 28.24-0.864 & 29.65-0.898 \\
%\cmidrule{2-14}          & 15    & 28.56-0.862 & 27.35-0.807 & 27.26-0.814 & 28.81-0.879 & 29.42-0.894 & 26.82-0.799 & 27.26-0.835 & 28.48-0.870 & 28.06-0.826 & 27.27-0.841 & 27.36-0.841 & 28.76-0.879 \\
%\cmidrule{2-14}          & 17    & 27.79-0.842 & 26.50-0.775 & 26.46-0.785 & 28.10-0.862 & 27.87-0.845 & 25.91-0.762 & 26.54-0.815 & 27.74-0.853 & 27.27-0.798 & 26.52-0.819 & 26.59-0.817 & 27.97-0.860 \\
%\cmidrule{2-14}          & 19    & 27.09-0.822 & 25.74-0.744 & 25.73-0.755 & 27.44-0.845 & 27.26-0.828 & 25.05-0.725 & 25.86-0.797 & 27.07-0.835 & 26.56-0.772 & 25.83-0.799 & 25.92-0.797 & 27.25-0.841 \\
%    \midrule
%    \multirow{10}[20]{*}{fastMRI} & 1     & 29.50-0.936 & 39.36-0.956 & 42.07-0.977 & 42.53-0.979 & 42.30-0.977 & -     & -     & 42.09-0.977 & 29.69-0.941 & 40.96-0.968 & -     & - \\
%\cmidrule{2-14}          & 3     & 28.98-0.907 & 36.12-0.921 & 36.68-0.933 & 37.07-0.937 & 37.09-0.933 & -     & -     & 36.74-0.935 & 29.01-0.906 & 36.68-0.930 & -     & - \\
%\cmidrule{2-14}          & 5     & 29.57-0.887 & 34.01-0.884 & 34.57-0.901 & 35.12-0.911 & 35.34-0.911 & -     & -     & 34.61-0.906 & 29.14-0.866 & 34.62-0.899 & -     & - \\
%\cmidrule{2-14}          & 7     & 29.36-0.865 & 32.29-0.842 & 33.01-0.867 & 33.82-0.889 & 34.01-0.888 & -     & -     & 33.10-0.878 & 28.66-0.826 & 33.11-0.869 & -     & - \\
%\cmidrule{2-14}          & 9     & 29.07-0.840 & 30.79-0.793 & 31.61-0.829 & 32.71-0.866 & 33.04-0.868 & -     & -     & 31.92-0.854 & 28.76-0.819 & 31.81-0.836 & -     & - \\
%\cmidrule{2-14}          & 11    & 28.71-0.812 & 29.43-0.741 & 30.29-0.785 & 31.69-0.841 & 32.03-0.844 & -     & -     & 30.88-0.827 & 28.29-0.780 & 30.63-0.801 & -     & - \\
%\cmidrule{2-14}          & 13    & 28.24-0.779 & 28.18-0.683 & 29.05-0.737 & 30.72-0.814 & 31.19-0.822 & -     & -     & 29.92-0.799 & 27.74-0.738 & 29.55-0.764 & -     & - \\
%\cmidrule{2-14}          & 15    & 27.71-0.744 & 27.04-0.626 & 27.87-0.686 & 29.80-0.785 & 30.24-0.794 & -     & -     & 29.01-0.770 & 27.14-0.693 & 28.57-0.727 & -     & - \\
%\cmidrule{2-14}          & 17    & 27.11-0.708 & 26.01-0.571 & 26.77-0.634 & 28.92-0.755 & 29.48-0.769 & -     & -     & 28.15-0.741 & 26.49-0.649 & 27.7-0.693 & -     & - \\
%\cmidrule{2-14}          & 19    & 26.49-0.671 & 25.04-0.519 & 25.76-0.583 & 28.09-0.725 & 28.77-0.744 & -     & -     & 27.34-0.711 & 25.84-0.606 & 26.90-0.660 & -     & - \\
%    \midrule
%    Time (s) & -     & 614.1  & 426.7  & 57.1  & 171.2  & 1552.9  & $>$1h   & $>$1h   & 141.4  & 517.8  & 4.5   & 11.0  & 986.9  \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_Results_MRI_all}%
%  }
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Reported results combined'
%\begin{table*}[htbp]
%\scriptsize \tabcolsep4.1pt
%  \centering
%    \caption{Average PSNR-SSIM and computational time (s) of different methods on Brainweb and fastMRI data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
%     \scalebox{0.838}{
%    \begin{tabular}{cccccccccccccc}
%    \toprule
%    \multirow{2}[1]{*}{Datasets} & \multirow{2}[1]{*}{Noise level} & 4DHOSVD & ANLM  & BM4D1 & BM4D2 & ILR-HOSVD & OLMMSE & ROLMMSE & MStSVD & NLPCA & ODCT  & PRINLM & PRI-NLPCA \\
%          &       & [ref] & [ref] & [ref] & [ref] & [ref] & [ref] & [ref] & [ref] & [ref] & [ref] & [ref] & [ref] \\
%    \toprule
%    \multirow{10}[20]{*}{Brainweb} & 1     & 43.86-0.993 & 41.87-0.991 & 43.18-0.992 & 43.43-0.992 & \textcolor{blue}{\textbf{44.55/0.994}} & 42.37-0.991 & 42.39-0.991 & 43.99-0.993 & 44.13-0.994 & 43.25-0.992 & 43.33-0.993 & 44.28-\textcolor{blue}{\textbf{0.994}} \\
%\cmidrule{2-14}          & 3     & 37.49-0.976 & 36.52-0.971 & 36.59-0.971 & 37.21-0.975 &  \textcolor{blue}{\textbf{38.22/0.981}} & 35.99-0.968 & 35.98-0.969 & 37.46-0.975 & 37.74-0.977 & 36.43-0.970 & 36.87-0.975 & 38.12-\textcolor{blue}{\textbf{0.981}} \\
%\cmidrule{2-14}          & 5     & 34.64-0.959 & 33.78-0.947 & 33.71-0.950 & 34.56-0.959 &  \textcolor{blue}{\textbf{35.46}}/0.966 & 33.37-0.949 & 33.36-0.949 & 34.65-0.958 & 33.84-0.940 & 33.57-0.949 & 33.97-0.955 & 35.29-\textcolor{blue}{\textbf{0.967}} \\
%\cmidrule{2-14}          & 7     & 32.85-0.941 & 31.91-0.921 & 31.80-0.926 & 32.84-0.943 &  \textcolor{blue}{\textbf{33.62-0.951}} & 31.58-0.925 & 31.61-0.928 & 32.83-0.940 & 31.87-0.912 & 31.66-0.927 & 32.01-0.934 & 33.36-\textcolor{blue}{\textbf{0.951}} \\
%\cmidrule{2-14}          & 9     & 31.49-0.922 & 30.47-0.894 & 30.35-0.901 & 31.54-0.928 &  \textcolor{blue}{\textbf{32.31-0.938}} & 30.16-0.898 & 30.23-0.904 & 31.31-0.924 & 31.15-0.908 & 30.23-0.905 & 30.49-0.911 & 31.86-0.934 \\
%\cmidrule{2-14}          & 11    & 30.36-0.903 & 29.29-0.865 & 29.15-0.873 & 30.49-0.912 &  \textcolor{blue}{\textbf{31.17-0.922}} & 28.93-0.868 & 29.09-0.880 & 30.22-0.906 & 29.98-0.883 & 29.08-0.882 & 29.28-0.888 & 30.66-0.916 \\
%\cmidrule{2-14}          & 13    & 29.40-0.883 & 28.26-0.836 & 28.14-0.844 & 29.59-0.895 &  \textcolor{blue}{\textbf{30.22-0.909}} & 27.82-0.834 & 28.08-0.856 & 29.29-0.888 & 28.97-0.855 & 28.11-0.861 & 28.24-0.864 & 29.65-0.898 \\
%\cmidrule{2-14}          & 15    & 28.56-0.862 & 27.35-0.807 & 27.26-0.814 & 28.81-0.879 &  \textcolor{blue}{\textbf{29.42-0.894}} & 26.82-0.799 & 27.26-0.835 & 28.48-0.870 & 28.06-0.826 & 27.27-0.841 & 27.36-0.841 & 28.76-0.879 \\
%\cmidrule{2-14}          & 17    & 27.79-0.842 & 26.50-0.775 & 26.46-0.785 &  \textcolor{blue}{\textbf{28.10-0.862}} & 27.87-0.845 & 25.91-0.762 & 26.54-0.815 & 27.74-0.853 & 27.27-0.798 & 26.52-0.819 & 26.59-0.817 & 27.97-0.860 \\
%\cmidrule{2-14}          & 19    & 27.09-0.822 & 25.74-0.744 & 25.73-0.755 &  \textcolor{blue}{\textbf{27.44-0.845}} & 27.26-0.828 & 25.05-0.725 & 25.86-0.797 & 27.07-0.835 & 26.56-0.772 & 25.83-0.799 & 25.92-0.797 & 27.25-0.841 \\
%    \midrule
%    \multirow{10}[20]{*}{fastMRI} & 1     & 41.50-0.975 & 39.36-0.956 & 42.07-0.977 &  \textcolor{blue}{\textbf{42.53-0.979}} & 42.30-0.977 & -     & -     & 42.09-0.977 & 41.69-0.976 & 40.96-0.968 & -     & - \\
%\cmidrule{2-14}          & 3     & 36.58-0.931 & 36.12-0.921 & 36.68-0.933 &  \textcolor{blue}{\textbf{37.07-0.937}} & 37.06-0.933 & -     & -     & 36.74-0.935 & 37.01-0.932 & 36.68-0.930 & -     & - \\
%\cmidrule{2-14}          & 5     & 34.13-0.901 & 34.01-0.884 & 34.57-0.901 & 35.12-\textcolor{blue}{\textbf{0.911}} &  \textcolor{blue}{\textbf{35.34-0.911}} & -     & -     & 34.61-0.906 & 34.15-0.902 & 34.62-0.899 & -     & - \\
%\cmidrule{2-14}          & 7     & 32.58-0.871 & 32.29-0.842 & 33.01-0.867 & 33.82- \textcolor{blue}{\textbf{0.889}} &  \textcolor{blue}{\textbf{34.01}}-0.888 & -     & -     & 33.10-0.878 & 32.08-0.866 & 33.11-0.869 & -     & - \\
%\cmidrule{2-14}          & 9     & 31.27-0.845 & 30.79-0.793 & 31.61-0.829 & 32.71-0.866 &  \textcolor{blue}{\textbf{33.04-0.868}} & -     & -     & 31.92-0.854 & 30.73-0.838 & 31.81-0.836 & -     & - \\
%\cmidrule{2-14}          & 11    & 30.01-0.814 & 29.43-0.741 & 30.29-0.785 & 31.69-0.841 &  \textcolor{blue}{\textbf{32.03-0.844}} & -     & -     & 30.88-0.827 & 29.31-0.804 & 30.63-0.801 & -     & - \\
%\cmidrule{2-14}          & 13    & 28.84-0.785 & 28.18-0.683 & 29.05-0.737 & 30.72-0.814 &  \textcolor{blue}{\textbf{31.19-0.822}} & -     & -     & 29.92-0.799 & 27.94-0.768 & 29.55-0.764 & -     & - \\
%\cmidrule{2-14}          & 15    & 27.91-0.754 & 27.04-0.626 & 27.87-0.686 & 29.80-0.785 &  \textcolor{blue}{\textbf{30.24-0.794}} & -     & -     & 29.01-0.770 & 27.14-0.711 & 28.57-0.727 & -     & - \\
%\cmidrule{2-14}          & 17    & 27.11-0.708 & 26.01-0.571 & 26.77-0.634 & 28.92-0.755 &  \textcolor{blue}{\textbf{29.48-0.769}} & -     & -     & 28.15-0.741 & 26.49-0.668 & 27.70-0.693 & -     & - \\
%\cmidrule{2-14}          & 19    & 26.49-0.671 & 25.04-0.519 & 25.76-0.583 & 28.09-0.725 &  \textcolor{blue}{\textbf{28.77-0.744}} & -     & -     & 27.34-0.711 & 25.84-0.606 & 26.90-0.660 & -     & - \\
%    \midrule
%    Time (s) & -     & 614.1  & 426.7  & 57.1  & 171.2  & 1552.9  & $>$1h   & $>$1h   & 141.4  & 517.8  &  \textcolor{blue}{\textbf{4.5}} & 11.0  & 986.9  \\
%    \bottomrule
%    \end{tabular}}
%  \label{Table_Results_MRI_all}%
%\end{table*}%

%% Table generated by Excel2LaTeX from sheet 'Reported results combined'
%\begin{table*}[htbp]
%\scriptsize \tabcolsep4.1pt
%  \centering
%    \caption{Average PSNR-SSIM and computational time (s) of different methods on Brainweb and fastMRI data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
%     \scalebox{0.818}{
%    \begin{tabular}{cccccccccccccc}
%    \toprule
%    \multirow{2}[1]{*}{Datasets} & \multirow{2}[1]{*}{Noise level} & 4DHOSVD & ANLM  & BM4D1 & BM4D2 & ILR-HOSVD & OLMMSE & ROLMMSE & MStSVD & NLPCA & ODCT  & PRINLM & PRI-NLPCA \\
%          &       & \cite{rajwade2012image} & \cite{manjon2010adaptive} &  \cite{maggioni2012nonlocal}  &  \cite{maggioni2012nonlocal}  & \cite{lv2019denoising} & \cite{aja2008noise} & \cite{aja2008noise} & \cite{kong2019color} &  \cite{manjon2015mri}  & \cite{manjon2012new} & \cite{manjon2012new} &  \cite{manjon2015mri}  \\
%    \toprule
%    \multirow{10}[20]{*}{Brainweb} & 1     & 43.86/0.993 & 41.87/0.991 & 43.18/0.992 & 43.43/0.992 & \textcolor{blue}{\textbf{44.55/0.994}} & 42.37/0.991 & 42.39/0.991 & 43.99/0.993 & 44.13/0.994 & 43.25/0.992 & 43.33/0.993 & 44.28/0.994 \\
%\cmidrule{2-14}          & 3     & 37.49/0.976 & 36.52/0.971 & 36.59/0.971 & 37.21/0.975 & \textcolor{blue}{\textbf{38.22/0.981}} & 35.99/0.968 & 35.98/0.969 & 37.46/0.975 & 37.74/0.977 & 36.43/0.970 & 36.87/0.975 & 38.12/0.981 \\
%\cmidrule{2-14}          & 5     & 34.64/0.959 & 33.78/0.947 & 33.71/0.950 & 34.56/0.959 & \textcolor{blue}{\textbf{35.46}}/0.966 & 33.37/0.949 & 33.36/0.949 & 34.65/0.958 & 33.84/0.940 & 33.57/0.949 & 33.97/0.955 & 35.29/\textcolor{blue}{\textbf{0.967}} \\
%\cmidrule{2-14}          & 7     & 32.85/0.941 & 31.91/0.921 & 31.80/0.926 & 32.84/0.943 & \textcolor{blue}{\textbf{33.62/0.951}} & 31.58/0.925 & 31.61/0.928 & 32.83/0.940 & 31.87/0.912 & 31.66/0.927 & 32.01/0.934 & 33.36/0.951 \\
%\cmidrule{2-14}          & 9     & 31.49/0.922 & 30.47/0.894 & 30.35/0.901 & 31.54/0.928 & \textcolor{blue}{\textbf{32.31/0.938}} & 30.16/0.898 & 30.23/0.904 & 31.31/0.924 & 31.15/0.908 & 30.23/0.905 & 30.49/0.911 & 31.86/0.934 \\
%\cmidrule{2-14}          & 11    & 30.36/0.903 & 29.29/0.865 & 29.15/0.873 & 30.49/0.912 & \textcolor{blue}{\textbf{31.17/0.922}} & 28.93/0.868 & 29.09/0.880 & 30.22/0.906 & 29.98/0.883 & 29.08/0.882 & 29.28/0.888 & 30.66/0.916 \\
%\cmidrule{2-14}          & 13    & 29.40/0.883 & 28.26/0.836 & 28.14/0.844 & 29.59/0.895 & \textcolor{blue}{\textbf{30.22/0.909}} & 27.82/0.834 & 28.08/0.856 & 29.29/0.888 & 28.97/0.855 & 28.11/0.861 & 28.24/0.864 & 29.65/0.898 \\
%\cmidrule{2-14}          & 15    & 28.56/0.862 & 27.35/0.807 & 27.26/0.814 & 28.81/0.879 & \textcolor{blue}{\textbf{29.42/0.894}} & 26.82/0.799 & 27.26/0.835 & 28.48/0.870 & 28.06/0.826 & 27.27/0.841 & 27.36/0.841 & 28.76/0.879 \\
%\cmidrule{2-14}          & 17    & 27.79/0.842 & 26.50/0.775 & 26.46/0.785 & \textcolor{blue}{\textbf{28.10/0.862}} & 27.87/0.845 & 25.91/0.762 & 26.54/0.815 & 27.74/0.853 & 27.27/0.798 & 26.52/0.819 & 26.59/0.817 & 27.97/0.860 \\
%\cmidrule{2-14}          & 19    & 27.09/0.822 & 25.74/0.744 & 25.73/0.755 & \textcolor{blue}{\textbf{27.44/0.845}} & 27.26/0.828 & 25.05/0.725 & 25.86/0.797 & 27.07/0.835 & 26.56/0.772 & 25.83/0.799 & 25.92/0.797 & 27.25/0.841 \\
%    \midrule
%    \multirow{10}[20]{*}{fastMRI} & 1     & 41.50/0.975 & 39.36/0.956 & 42.07/0.977 & \textcolor{blue}{\textbf{42.53/0.979}} & 42.30/0.977 & -     & -     & 42.09/0.977 & 41.69/0.976 & 40.96/0.968 & -     & - \\
%\cmidrule{2-14}          & 3     & 36.58/0.931 & 36.12/0.921 & 36.68/0.933 & 37.07/\textcolor{blue}{\textbf{0.937}} & \textcolor{blue}{\textbf{37.09}}/0.933 & -     & -     & 36.74/0.935 & 37.01/0.932 & 36.68/0.930 & -     & - \\
%\cmidrule{2-14}          & 5     & 34.13/0.901 & 34.01/0.884 & 34.57/0.901 & 35.12/0.911 & \textcolor{blue}{\textbf{35.34/0.911}} & -     & -     & 34.61/0.906 & 34.15/0.902 & 34.62/0.899 & -     & - \\
%\cmidrule{2-14}          & 7     & 32.58/0.871 & 32.29/0.842 & 33.01/0.867 & 33.82/0.889 & 34.01/0.888 & -     & -     & 33.10/0.878 & 32.08/0.866 & 33.11/0.869 & -     & - \\
%\cmidrule{2-14}          & 9     & 31.27/0.845 & 30.79/0.793 & 31.61/0.829 & 32.71/0.866 & \textcolor{blue}{\textbf{33.04/0.868}} & -     & -     & 31.92/0.854 & 30.73/0.838 & 31.81/0.836 & -     & - \\
%\cmidrule{2-14}          & 11    & 30.01/0.814 & 29.43/0.741 & 30.29/0.785 & 31.69/0.841 & \textcolor{blue}{\textbf{32.03/0.844}} & -     & -     & 30.88/0.827 & 29.31/0.804 & 30.63/0.801 & -     & - \\
%\cmidrule{2-14}          & 13    & 28.84/0.785 & 28.18/0.683 & 29.05/0.737 & 30.72/0.814 & \textcolor{blue}{\textbf{31.19/0.822}} & -     & -     & 29.92/0.799 & 27.94/0.768 & 29.55/0.764 & -     & - \\
%\cmidrule{2-14}          & 15    & 27.91/0.754 & 27.04/0.626 & 27.87/0.686 & 29.80/0.785 & \textcolor{blue}{\textbf{30.24/0.794}} & -     & -     & 29.01/0.770 & 27.12/0.711 & 28.57/0.727 & -     & - \\
%\cmidrule{2-14}          & 17    & 27.11/0.708 & 26.01/0.571 & 26.77/0.634 & 28.92/0.755 & \textcolor{blue}{\textbf{29.48/0.769}} & -     & -     & 28.15/0.741 & 26.49/0.668 & 27.70/0.693 & -     & - \\
%\cmidrule{2-14}          & 19    & 26.49/0.671 & 25.04/0.519 & 25.76/0.583 & 28.09/0.725 & \textcolor{blue}{\textbf{28.77/0.744}} & -     & -     & 27.34/0.711 & 25.84/0.606 & 26.90/0.660 & -     & - \\
%    \midrule
%    Time (s) &  -    & 614.1  & 426.7  & 57.1  & 171.2  & 1552.9  & $>1h$   & $>1h$   & 141.4  & 517.8  & \textcolor{blue}{\textbf{4.5}} & 11.0  & 986.9  \\
%    \bottomrule
%    \end{tabular}}%
%  \label{Table_Results_MRI_all}%
%\end{table*}%



% Table generated by Excel2LaTeX from sheet 'Reported results combined'
\begin{table*}[htbp]
\scriptsize \tabcolsep4.1pt
  \centering
    \caption{Average PSNR-SSIM and computational time (s) of different methods on Brainweb and fastMRI data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
     \scalebox{0.828}{
    \begin{tabular}{cccccccccccccc}
    \toprule
    \multirow{2}[1]{*}{Datasets} & \multirow{2}[1]{*}{Noise level} & 4DHOSVD & ANLM  & BM4D1 & BM4D2 & ILR-HOSVD & OLMMSE & ROLMMSE & MStSVD & NLPCA & ODCT  & PRINLM & PRI-NLPCA \\
          &       & \cite{rajwade2012image} & \cite{manjon2010adaptive} &  \cite{maggioni2012nonlocal}  &  \cite{maggioni2012nonlocal}  & \cite{lv2019denoising} & \cite{aja2008noise} & \cite{aja2008noise} & \cite{kong2019color} &  \cite{manjon2015mri}  & \cite{manjon2012new} & \cite{manjon2012new} &  \cite{manjon2015mri}  \\
    \toprule
    \multirow{10}[20]{*}{Brainweb} & 1     & 43.86/0.993 & 41.87/0.991 & 43.18/0.992 & 43.43/0.992 & {\textbf{44.55/0.994}} & 42.37/0.991 & 42.39/0.991 & 43.99/0.993 & 44.13/0.994 & 43.25/0.992 & 43.33/0.993 & 44.28/0.994 \\
\cmidrule{2-14}          & 3     & 37.49/0.976 & 36.52/0.971 & 36.59/0.971 & 37.21/0.975 & {\textbf{38.22/0.981}} & 35.99/0.968 & 35.98/0.969 & 37.46/0.975 & 37.74/0.977 & 36.43/0.970 & 36.87/0.975 & 38.12/0.981 \\
\cmidrule{2-14}          & 5     & 34.64/0.959 & 33.78/0.947 & 33.71/0.950 & 34.56/0.959 & {\textbf{35.46}}/0.966 & 33.37/0.949 & 33.36/0.949 & 34.65/0.958 & 33.84/0.940 & 33.57/0.949 & 33.97/0.955 & 35.29/{\textbf{0.967}} \\
\cmidrule{2-14}          & 7     & 32.85/0.941 & 31.91/0.921 & 31.80/0.926 & 32.84/0.943 & {\textbf{33.62/0.951}} & 31.58/0.925 & 31.61/0.928 & 32.83/0.940 & 31.87/0.912 & 31.66/0.927 & 32.01/0.934 & 33.36/0.951 \\
\cmidrule{2-14}          & 9     & 31.49/0.922 & 30.47/0.894 & 30.35/0.901 & 31.54/0.928 & {\textbf{32.31/0.938}} & 30.16/0.898 & 30.23/0.904 & 31.31/0.924 & 31.15/0.908 & 30.23/0.905 & 30.49/0.911 & 31.86/0.934 \\
\cmidrule{2-14}          & 11    & 30.36/0.903 & 29.29/0.865 & 29.15/0.873 & 30.49/0.912 & {\textbf{31.17/0.922}} & 28.93/0.868 & 29.09/0.880 & 30.22/0.906 & 29.98/0.883 & 29.08/0.882 & 29.28/0.888 & 30.66/0.916 \\
\cmidrule{2-14}          & 13    & 29.40/0.883 & 28.26/0.836 & 28.14/0.844 & 29.59/0.895 & {\textbf{30.22/0.909}} & 27.82/0.834 & 28.08/0.856 & 29.29/0.888 & 28.97/0.855 & 28.11/0.861 & 28.24/0.864 & 29.65/0.898 \\
\cmidrule{2-14}          & 15    & 28.56/0.862 & 27.35/0.807 & 27.26/0.814 & 28.81/0.879 & {\textbf{29.42/0.894}} & 26.82/0.799 & 27.26/0.835 & 28.48/0.870 & 28.06/0.826 & 27.27/0.841 & 27.36/0.841 & 28.76/0.879 \\
\cmidrule{2-14}          & 17    & 27.79/0.842 & 26.50/0.775 & 26.46/0.785 & {\textbf{28.10/0.862}} & 27.87/0.845 & 25.91/0.762 & 26.54/0.815 & 27.74/0.853 & 27.27/0.798 & 26.52/0.819 & 26.59/0.817 & 27.97/0.860 \\
\cmidrule{2-14}          & 19    & 27.09/0.822 & 25.74/0.744 & 25.73/0.755 & {\textbf{27.44/0.845}} & 27.26/0.828 & 25.05/0.725 & 25.86/0.797 & 27.07/0.835 & 26.56/0.772 & 25.83/0.799 & 25.92/0.797 & 27.25/0.841 \\
    \midrule
    \multirow{10}[20]{*}{fastMRI} & 1     & 41.50/0.975 & 39.36/0.956 & 42.07/0.977 & {\textbf{42.53/0.979}} & 42.30/0.977 & -     & -     & 42.09/0.977 & 41.69/0.976 & 40.96/0.968 & -     & - \\
\cmidrule{2-14}          & 3     & 36.58/0.931 & 36.12/0.921 & 36.68/0.933 & 37.07/{\textbf{0.937}} & {\textbf{37.09}}/0.933 & -     & -     & 36.74/0.935 & 37.01/0.932 & 36.68/0.930 & -     & - \\
\cmidrule{2-14}          & 5     & 34.13/0.901 & 34.01/0.884 & 34.57/0.901 & 35.12/0.911 & {\textbf{35.34/0.911}} & -     & -     & 34.61/0.906 & 34.15/0.902 & 34.62/0.899 & -     & - \\
\cmidrule{2-14}          & 7     & 32.58/0.871 & 32.29/0.842 & 33.01/0.867 & 33.82/0.889 & \textbf{34.01/0.888} & -     & -     & 33.10/0.878 & 32.08/0.866 & 33.11/0.869 & -     & - \\
\cmidrule{2-14}          & 9     & 31.27/0.845 & 30.79/0.793 & 31.61/0.829 & 32.71/0.866 & {\textbf{33.04/0.868}} & -     & -     & 31.92/0.854 & 30.73/0.838 & 31.81/0.836 & -     & - \\
\cmidrule{2-14}          & 11    & 30.01/0.814 & 29.43/0.741 & 30.29/0.785 & 31.69/0.841 & {\textbf{32.03/0.844}} & -     & -     & 30.88/0.827 & 29.31/0.804 & 30.63/0.801 & -     & - \\
\cmidrule{2-14}          & 13    & 28.84/0.785 & 28.18/0.683 & 29.05/0.737 & 30.72/0.814 & {\textbf{31.19/0.822}} & -     & -     & 29.92/0.799 & 27.94/0.768 & 29.55/0.764 & -     & - \\
\cmidrule{2-14}          & 15    & 27.91/0.754 & 27.04/0.626 & 27.87/0.686 & 29.80/0.785 & {\textbf{30.24/0.794}} & -     & -     & 29.01/0.770 & 27.12/0.711 & 28.57/0.727 & -     & - \\
\cmidrule{2-14}          & 17    & 27.11/0.708 & 26.01/0.571 & 26.77/0.634 & 28.92/0.755 & {\textbf{29.48/0.769}} & -     & -     & 28.15/0.741 & 26.49/0.668 & 27.70/0.693 & -     & - \\
\cmidrule{2-14}          & 19    & 26.49/0.671 & 25.04/0.519 & 25.76/0.583 & 28.09/0.725 & {\textbf{28.77/0.744}} & -     & -     & 27.34/0.711 & 25.84/0.606 & 26.90/0.660 & -     & - \\
    \midrule
    Time (s) &  -    & 614.1  & 426.7  & 57.1  & 171.2  & 1552.9  & $>1$h   & $>1$h   & 141.4  & 517.8  & {\textbf{4.5}} & 11.0  & 986.9  \\
    \bottomrule
    \end{tabular}}%
  \label{Table_Results_MRI_all}%
\end{table*}%




==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_Results_MSI-HSI_all.tex <==
%% Table generated by Excel2LaTeX from sheet 'All-in-one'
%\begin{table*}[htbp]
%\tiny \tabcolsep2.08pt
%  \centering
%  \caption{Comparison of quantitative results on CAVE (with i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$) and Real-HSI datasets. The average denoising time (minutes) is calculated based on the CAVE dataset when $\sigma = 100$.}
%  \scalebox{0.806}{
%    \begin{tabular}{cccccccccccccccccccccccccccccc}
%    \toprule
%    \multirow{3}[4]{*}{Datasets} & \multirow{3}[4]{*}{$\sigma$} & \multirow{3}[4]{*}{Metrics} & \multicolumn{20}{c}{Traditonal denoisers}                                                                                                                     & \multicolumn{1}{c|}{} & \multicolumn{6}{c}{DNN methods} \\
%\cmidrule{4-30}          &       &       & 4DHOSVD & ANLM  & BM4D1 & BM4D2 & FastHyDe & ISTReg & LLRGTV & LLRT  & LRMR  & LRTA  & LTDL  & LRTDGS & MSt-SVD & MTSNMF & NGMeet & OLRT  & PARAFAC & RTA-LSM & SDS   & SSTV  & \multicolumn{1}{c|}{TDL} & GRN   & HSI-DeNet & MAN   & QRNN3D & sDeCNN & SST \\
%          &       &       & \cite{rajwade2012image} & \cite{manjon2010adaptive}  & \cite{maggioni2012nonlocal} & \cite{maggioni2012nonlocal} & \cite{zhuang2018fast} & \cite{xie2016multispectral} & \cite{He2018LLRGTV} & \cite{chang2017hyper} & \cite{zhang2013hyperspectral} & \cite{renard2008denoising} & \cite{gong2020low} & \cite{chen2019hyperspectral} & \cite{kong2017new} & \cite{ye2014multitask} & \cite{he2019non} & \cite{chang2020hyperspectral} & \cite{liu2012denoising} & \cite{dong2018robust} & \cite{lam2012denoising} & \cite{zeng2021hyperspectral} & \multicolumn{1}{c}{\cite{peng2014decomposable}} & \cite{cao2021deep} & \cite{chang2018hsi} & \cite{lai2023mixed} & \cite{wei20203} & \cite{maffei2019single} & \cite{li2022spatial} \\
%    \midrule
%    \multirow{19}[32]{*}{CAVE} & \multirow{4}[8]{*}{10} & PSNR  & 45.43  & 41.52  & 43.04  & 44.61  & 42.87  & 45.14  & 39.62  & 46.60  & 39.47  & 41.36  & 45.90  & 35.99  & 45.20  & 43.04  & 46.59  & \textcolor{blue}{\textbf{47.07}} & 35.43  & 46.43  & 39.69  & 38.91  & 44.39  & 30.98  & 37.01  & 43.31  & 40.36  & 41.40  & 39.75  \\
%\cmidrule{3-30}          &       & SSIM  & 0.9812  & 0.9576  & 0.9700  & 0.9784  & 0.9763  & 0.9792  & 0.9274  & 0.9868  & 0.9125  & 0.9499  & 0.9855  & 0.8976  & 0.9814  & 0.9706  & \textcolor{blue}{\textbf{0.9880}} & 0.9877  & 0.8762  & 0.9857  & 0.9483  & 0.9153  & 0.9797  & 0.8622  & 0.8936  & 0.9804  & 0.9672  & 0.9624  & 0.9730  \\
%\cmidrule{3-30}          &       & SAM   & 0.1084  & 0.2183  & 0.1844  & 0.1289  & 0.1398  & 0.1311  & 0.2676  & 0.0842  & 0.3282  & 0.1718  & 0.0923  & 0.1764  & 0.1064  & 0.1342  & 0.0853  & \textcolor{blue}{\textbf{0.0840}} & 0.2407  & 0.0926  & 0.2159  & 0.2669  & 0.1055  & 0.4971  & 0.3236  & 0.1273  & 0.1926  & 0.1524  & 0.1632  \\
%\cmidrule{3-30}          &       & EGRAS & 30.83  & 47.79  & 40.07  & 33.32  & 42.90  & 31.71  & 63.65  & 26.75  & 63.52  & 49.53  & 29.06  & 103.69  & 32.05  & 40.29  & 27.26  & \textcolor{blue}{\textbf{25.53}} & 108.34  & 27.15  & 61.88  & 65.86  & 34.39  & 209.61  & 85.92  & 44.09  & 65.31  & 52.04  & 66.63  \\
%\cmidrule{2-30}          & \multirow{4}[8]{*}{30} & PSNR  & 39.78  & 34.70  & 37.05  & 38.80  & 37.22  & 40.37  & 32.26  & 41.49  & 31.43  & 36.06  & 41.21  & 35.12  & 40.23  & 37.02  & 41.60  & \textcolor{blue}{\textbf{41.79}} & 33.46  & 41.32  & 32.07  & 31.35  & 39.06  & 30.94  & 30.83  & 40.06  & 38.48  & 37.58  & 37.82  \\
%\cmidrule{3-30}          &       & SSIM  & 0.9336  & 0.8068  & 0.9236  & 0.9283  & 0.9151  & 0.9462  & 0.7150  & 0.9681  & 0.6517  & 0.8775  & 0.9656  & 0.8795  & 0.9530  & 0.8758  & \textcolor{blue}{\textbf{0.9693}} & 0.9680  & 0.8255  & 0.9598  & 0.6723  & 0.6078  & 0.9493  & 0.8605  & 0.6467  & 0.9620  & 0.9496  & 0.9247  & 0.9564  \\
%\cmidrule{3-30}          &       & SAM   & 0.2272  & 0.4302  & 0.2898  & 0.2579  & 0.3123  & 0.2254  & 0.5538  & 0.1221  & 0.5899  & 0.2446  & 0.1299  & 0.2104  & 0.1737  & 0.2267  & 0.1238  & \textcolor{blue}{\textbf{0.1180}} & 0.3362  & 0.1556  & 0.4959  & 0.5190  & 0.1496  & 0.4970  & 0.5105  & 0.1835  & 0.2320  & 0.1959  & 0.2144  \\
%\cmidrule{3-30}          &       & EGRAS & 59.12  & 103.96  & 83.28  & 65.23  & 81.44  & 54.82  & 141.67  & 48.50  & 154.15  & 90.50  & 49.68  & 109.98  & 56.26  & 79.30  & 48.15  & \textcolor{blue}{\textbf{46.65}} & 126.99  & 49.42  & 143.67  & 155.14  & 63.24  & 209.90  & 177.76  & 61.45  & 76.21  & 78.28  & 80.25  \\
%\cmidrule{2-30}          & \multirow{4}[8]{*}{50} & PSNR  & 36.82  & 30.76  & 34.51  & 35.90  & 34.56  & 37.88  & 28.53  & 38.65  & 27.44  & 33.52  & 38.62  & 33.84  & 37.73  & 33.50  & 38.87  & \textcolor{blue}{\textbf{39.13}} & 31.25  & 38.60  & 26.09  & 25.48  & 36.44  & 30.82  & -     & 38.11  & 37.02  & 35.49  & 36.43  \\
%\cmidrule{3-30}          &       & SSIM  & 0.8722  & 0.6064  & 0.8823  & 0.8685  & 0.8471  & 0.9168  & 0.5368  & 0.9482  & 0.4410  & 0.8201  & 0.9464  & 0.8470  & 0.9285  & 0.7585  & \textcolor{blue}{\textbf{0.9507}} & 0.9481  & 0.7307  & 0.9301  & 0.3529  & 0.3019  & 0.9171  & 0.8564  & -     & 0.9444  & 0.9314  & 0.8947  & 0.9408  \\
%\cmidrule{3-30}          &       & SAM   & 0.3385  & 0.5801  & 0.3540  & 0.3557  & 0.4395  & 0.2737  & 0.7113  & 0.1551  & 0.7273  & 0.2897  & 0.1630  & 0.2674  & 0.2231  & 0.2956  & 0.1617  & \textcolor{blue}{\textbf{0.1436}} & 0.4541  & 0.2199  & 0.7170  & 0.7473  & 0.2007  & 0.4966  & -     & 0.2309  & 0.2741  & 0.2141  & 0.2524  \\
%\cmidrule{3-30}          &       & EGRAS & 83.36  & 164.17  & 110.14  & 91.19  & 108.74  & 73.32  & 211.99  & 67.56  & 241.87  & 121.15  & 66.73  & 122.70  & 75.03  & 118.36  & 65.72  & \textcolor{blue}{\textbf{63.41}} & 158.53  & 67.27  & 290.93  & 306.21  & 85.24  & 210.86  & -     & 76.14  & 87.15  & 98.54  & 92.86  \\
%\cmidrule{2-30}          & \multirow{4}[8]{*}{100} & PSNR  & 32.66  & 24.92  & 31.21  & 31.84  & 30.62  & 31.85  & 23.36  & \textcolor{blue}{\textbf{35.39}} & 21.91  & 30.06  & 34.86  & 30.34  & 34.20  & 28.04  & 34.98  & 35.18  & 26.77  & 34.66  & 18.48  & 16.75  & 32.89  & 29.45  & -     & 35.35  & 30.33  & 32.51  & 33.96  \\
%\cmidrule{3-30}          &       & SSIM  & 0.7307  & 0.2828  & 0.7854  & 0.7197  & 0.6717  & 0.8176  & 0.2859  & \textcolor{blue}{\textbf{0.9154}} & 0.1962  & 0.7138  & 0.9002  & 0.6852  & 0.8800  & 0.4988  & 0.9073  & 0.8944  & 0.4481  & 0.8418  & 0.1067  & 0.0720  & 0.8283  & 0.7814  & -     & 0.9053  & 0.7128  & 0.8309  & 0.9016  \\
%\cmidrule{3-30}          &       & SAM   & 0.5600  & 0.7968  & 0.4638  & 0.5160  & 0.6097  & 0.3605  & 0.9229  & \textcolor{blue}{\textbf{0.1962}} & 0.9175  & 0.3649  & 0.2349  & 0.4707  & 0.3142  & 0.4180  & 0.2504  & 0.2100  & 0.6942  & 0.3714  & 0.9868  & 1.0569  & 0.3138  & 0.4991  & -     & 0.3161  & 0.5161  & 0.2748  & 0.3225  \\
%\cmidrule{3-30}          &       & EGRAS & 134.34  & 324.49  & 158.47  & 144.91  & 168.92  & 148.29  & 376.10  & \textcolor{blue}{\textbf{99.37}} & 456.12  & 180.03  & 102.61  & 174.87  & 115.24  & 221.84  & 101.86  & 99.93  & 260.85  & 105.99  & 718.40  & 834.58  & 128.22  & 225.29  & -     & 103.68  & 172.68  & 136.17  & 120.41  \\
%    \midrule
%    \multirow{4}[8]{*}{Real-HSI} & \multirow{4}[8]{*}{-} & PSNR  & 25.86  & -     & 25.84  & 25.88  & 23.99  & 25.91  & 24.63  & 25.90  & 24.81  & 24.27  & 25.80  & 25.12  & 25.86  & 25.51  & 25.87  & \textcolor{blue}{\textbf{25.94}} & 25.08  & -     & 25.58  & 25.31  & 25.33  & 24.91  & 25.63  & 25.82  & 25.82  & 25.70  & - \\
%\cmidrule{3-30}          &       & SSIM  & 0.8664  & -     & 0.8574  & 0.8653  & 0.5484  & 0.8688  & 0.7344  & 0.8610  & 0.7753  & 0.5876  & 0.8413  & 0.8181  & 0.8665  & 0.7819  & 0.8659  & \textcolor{blue}{\textbf{0.8695}} & 0.7668  & -     & 0.8126  & 0.7923  & 0.7634  & 0.8006  & 0.8534  & 0.8694  & 0.8691  & 0.8597  & - \\
%\cmidrule{3-30}          &       & SAM   & 0.0632  & -     & 0.0698  & 0.0660  & 0.2275  & 0.0551  & 0.1057  & 0.0604  & 0.1542  & 0.2198  & 0.0742  & 0.0669  & 0.0635  & 0.1020  & \textcolor{blue}{\textbf{0.0509}} & 0.0538  & 0.1084  & -     & 0.0891  & 0.0816  & 0.1232  & 0.1635  & 0.0921  & 0.0596  & 0.0638  & 0.0928  & - \\
%\cmidrule{3-30}          &       & EGRAS & 222.73  & -     & 224.51  & 222.67  & 252.24  & 222.18  & 243.68  & 224.05  & 246.39  & 248.57  & 223.32  & 234.02  & 222.64  & 226.58  & 222.69  & \textcolor{blue}{\textbf{221.94}} & 233.43  & -     & 226.23  & 229.18  & 229.32  & 248.41  & 232.73  & 224.41  & 225.32  & 227.88  & - \\
%    \midrule
%    Time  & -     & minutes & 2.5   & 1.7   & 1.5   & 4.1   & \textcolor{blue}{\textbf{0.1}} & 41.9  & 2.9   & 16.5  & 4.9   & \textcolor{blue}{\textbf{0.1}} & 35.0  & 0.6   & 2.8   & 0.5   & 4.1   & 24.3  & 1.5   & 12.5  & \textcolor{blue}{\textbf{0.1}} & 3.0   & 0.9   & \textcolor{blue}{\textbf{0.1}} & 0.8   & 0.2   & \textcolor{blue}{\textbf{0.1}} & 0.7   & \textcolor{blue}{\textbf{0.1}} \\
%    \bottomrule
%    \end{tabular}}%
%  \label{Table_Results_MSI-HSI_all}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'All-in-one'
\begin{table*}[htbp]
\tiny \tabcolsep2.08pt
  \centering
  \caption{Comparison of quantitative results on CAVE (with i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$) and Real-HSI datasets. The average denoising time (minutes) is calculated based on the CAVE dataset when $\sigma = 100$.}
  \scalebox{0.806}{
    \begin{tabular}{cccccccccccccccccccccccccccccc}
    \toprule
    \multirow{3}[4]{*}{Datasets} & \multirow{3}[4]{*}{$\sigma$} & \multirow{3}[4]{*}{Metrics} & \multicolumn{20}{c}{Traditonal denoisers}                                                                                                                     & \multicolumn{1}{c|}{} & \multicolumn{6}{c}{DNN methods} \\
\cmidrule{4-30}          &       &       & 4DHOSVD & ANLM  & BM4D1 & BM4D2 & FastHyDe & ISTReg & LLRGTV & LLRT  & LRMR  & LRTA  & LTDL  & LRTDGS & MSt-SVD & MTSNMF & NGMeet & OLRT  & PARAFAC & RTA-LSM & SDS   & SSTV  & \multicolumn{1}{c|}{TDL} & GRN   & HSI-DeNet & MAN   & QRNN3D & sDeCNN & SST \\
          &       &       & \cite{rajwade2012image} & \cite{manjon2010adaptive}  & \cite{maggioni2012nonlocal} & \cite{maggioni2012nonlocal} & \cite{zhuang2018fast} & \cite{xie2016multispectral} & \cite{He2018LLRGTV} & \cite{chang2017hyper} & \cite{zhang2013hyperspectral} & \cite{renard2008denoising} & \cite{gong2020low} & \cite{chen2019hyperspectral} & \cite{kong2017new} & \cite{ye2014multitask} & \cite{he2019non} & \cite{chang2020hyperspectral} & \cite{liu2012denoising} & \cite{dong2018robust} & \cite{lam2012denoising} & \cite{zeng2021hyperspectral} & \multicolumn{1}{c}{\cite{peng2014decomposable}} & \cite{cao2021deep} & \cite{chang2018hsi} & \cite{lai2023mixed} & \cite{wei20203} & \cite{maffei2019single} & \cite{li2022spatial} \\
    \midrule
    \multirow{19}[32]{*}{CAVE} & \multirow{4}[8]{*}{10} & PSNR  & 45.43  & 41.52  & 43.04  & 44.61  & 42.87  & 45.14  & 39.62  & 46.60  & 39.47  & 41.36  & 45.90  & 35.99  & 45.20  & 43.04  & 46.59  & {\textbf{47.07}} & 35.43  & 46.43  & 39.69  & 38.91  & 44.39  & 30.98  & 37.01  & 43.31  & 40.36  & 41.40  & 39.75  \\
\cmidrule{3-30}          &       & SSIM  & 0.9812  & 0.9576  & 0.9700  & 0.9784  & 0.9763  & 0.9792  & 0.9274  & 0.9868  & 0.9125  & 0.9499  & 0.9855  & 0.8976  & 0.9814  & 0.9706  & {\textbf{0.9880}} & 0.9877  & 0.8762  & 0.9857  & 0.9483  & 0.9153  & 0.9797  & 0.8622  & 0.8936  & 0.9804  & 0.9672  & 0.9624  & 0.9730  \\
\cmidrule{3-30}          &       & SAM   & 0.1084  & 0.2183  & 0.1844  & 0.1289  & 0.1398  & 0.1311  & 0.2676  & 0.0842  & 0.3282  & 0.1718  & 0.0923  & 0.1764  & 0.1064  & 0.1342  & 0.0853  & {\textbf{0.0840}} & 0.2407  & 0.0926  & 0.2159  & 0.2669  & 0.1055  & 0.4971  & 0.3236  & 0.1273  & 0.1926  & 0.1524  & 0.1632  \\
\cmidrule{3-30}          &       & EGRAS & 30.83  & 47.79  & 40.07  & 33.32  & 42.90  & 31.71  & 63.65  & 26.75  & 63.52  & 49.53  & 29.06  & 103.69  & 32.05  & 40.29  & 27.26  & {\textbf{25.53}} & 108.34  & 27.15  & 61.88  & 65.86  & 34.39  & 209.61  & 85.92  & 44.09  & 65.31  & 52.04  & 66.63  \\
\cmidrule{2-30}          & \multirow{4}[8]{*}{30} & PSNR  & 39.78  & 34.70  & 37.05  & 38.80  & 37.22  & 40.37  & 32.26  & 41.49  & 31.43  & 36.06  & 41.21  & 35.12  & 40.23  & 37.02  & 41.60  & {\textbf{41.79}} & 33.46  & 41.32  & 32.07  & 31.35  & 39.06  & 30.94  & 30.83  & 40.06  & 38.48  & 37.58  & 37.82  \\
\cmidrule{3-30}          &       & SSIM  & 0.9336  & 0.8068  & 0.9236  & 0.9283  & 0.9151  & 0.9462  & 0.7150  & 0.9681  & 0.6517  & 0.8775  & 0.9656  & 0.8795  & 0.9530  & 0.8758  & {\textbf{0.9693}} & 0.9680  & 0.8255  & 0.9598  & 0.6723  & 0.6078  & 0.9493  & 0.8605  & 0.6467  & 0.9620  & 0.9496  & 0.9247  & 0.9564  \\
\cmidrule{3-30}          &       & SAM   & 0.2272  & 0.4302  & 0.2898  & 0.2579  & 0.3123  & 0.2254  & 0.5538  & 0.1221  & 0.5899  & 0.2446  & 0.1299  & 0.2104  & 0.1737  & 0.2267  & 0.1238  & {\textbf{0.1180}} & 0.3362  & 0.1556  & 0.4959  & 0.5190  & 0.1496  & 0.4970  & 0.5105  & 0.1835  & 0.2320  & 0.1959  & 0.2144  \\
\cmidrule{3-30}          &       & EGRAS & 59.12  & 103.96  & 83.28  & 65.23  & 81.44  & 54.82  & 141.67  & 48.50  & 154.15  & 90.50  & 49.68  & 109.98  & 56.26  & 79.30  & 48.15  & {\textbf{46.65}} & 126.99  & 49.42  & 143.67  & 155.14  & 63.24  & 209.90  & 177.76  & 61.45  & 76.21  & 78.28  & 80.25  \\
\cmidrule{2-30}          & \multirow{4}[8]{*}{50} & PSNR  & 36.82  & 30.76  & 34.51  & 35.90  & 34.56  & 37.88  & 28.53  & 38.65  & 27.44  & 33.52  & 38.62  & 33.84  & 37.73  & 33.50  & 38.87  & {\textbf{39.13}} & 31.25  & 38.60  & 26.09  & 25.48  & 36.44  & 30.82  & -     & 38.11  & 37.02  & 35.49  & 36.43  \\
\cmidrule{3-30}          &       & SSIM  & 0.8722  & 0.6064  & 0.8823  & 0.8685  & 0.8471  & 0.9168  & 0.5368  & 0.9482  & 0.4410  & 0.8201  & 0.9464  & 0.8470  & 0.9285  & 0.7585  & {\textbf{0.9507}} & 0.9481  & 0.7307  & 0.9301  & 0.3529  & 0.3019  & 0.9171  & 0.8564  & -     & 0.9444  & 0.9314  & 0.8947  & 0.9408  \\
\cmidrule{3-30}          &       & SAM   & 0.3385  & 0.5801  & 0.3540  & 0.3557  & 0.4395  & 0.2737  & 0.7113  & 0.1551  & 0.7273  & 0.2897  & 0.1630  & 0.2674  & 0.2231  & 0.2956  & 0.1617  & {\textbf{0.1436}} & 0.4541  & 0.2199  & 0.7170  & 0.7473  & 0.2007  & 0.4966  & -     & 0.2309  & 0.2741  & 0.2141  & 0.2524  \\
\cmidrule{3-30}          &       & EGRAS & 83.36  & 164.17  & 110.14  & 91.19  & 108.74  & 73.32  & 211.99  & 67.56  & 241.87  & 121.15  & 66.73  & 122.70  & 75.03  & 118.36  & 65.72  & {\textbf{63.41}} & 158.53  & 67.27  & 290.93  & 306.21  & 85.24  & 210.86  & -     & 76.14  & 87.15  & 98.54  & 92.86  \\
\cmidrule{2-30}          & \multirow{4}[8]{*}{100} & PSNR  & 32.66  & 24.92  & 31.21  & 31.84  & 30.62  & 31.85  & 23.36  & {\textbf{35.39}} & 21.91  & 30.06  & 34.86  & 30.34  & 34.20  & 28.04  & 34.98  & 35.18  & 26.77  & 34.66  & 18.48  & 16.75  & 32.89  & 29.45  & -     & 35.35  & 30.33  & 32.51  & 33.96  \\
\cmidrule{3-30}          &       & SSIM  & 0.7307  & 0.2828  & 0.7854  & 0.7197  & 0.6717  & 0.8176  & 0.2859  & {\textbf{0.9154}} & 0.1962  & 0.7138  & 0.9002  & 0.6852  & 0.8800  & 0.4988  & 0.9073  & 0.8944  & 0.4481  & 0.8418  & 0.1067  & 0.0720  & 0.8283  & 0.7814  & -     & 0.9053  & 0.7128  & 0.8309  & 0.9016  \\
\cmidrule{3-30}          &       & SAM   & 0.5600  & 0.7968  & 0.4638  & 0.5160  & 0.6097  & 0.3605  & 0.9229  & {\textbf{0.1962}} & 0.9175  & 0.3649  & 0.2349  & 0.4707  & 0.3142  & 0.4180  & 0.2504  & 0.2100  & 0.6942  & 0.3714  & 0.9868  & 1.0569  & 0.3138  & 0.4991  & -     & 0.3161  & 0.5161  & 0.2748  & 0.3225  \\
\cmidrule{3-30}          &       & EGRAS & 134.34  & 324.49  & 158.47  & 144.91  & 168.92  & 148.29  & 376.10  & {\textbf{99.37}} & 456.12  & 180.03  & 102.61  & 174.87  & 115.24  & 221.84  & 101.86  & 99.93  & 260.85  & 105.99  & 718.40  & 834.58  & 128.22  & 225.29  & -     & 103.68  & 172.68  & 136.17  & 120.41  \\
    \midrule
    \multirow{4}[8]{*}{Real-HSI} & \multirow{4}[8]{*}{-} & PSNR  & 25.86  & -     & 25.84  & 25.88  & 23.99  & 25.91  & 24.63  & 25.90  & 24.81  & 24.27  & 25.80  & 25.12  & 25.86  & 25.51  & 25.87  & {\textbf{25.94}} & 25.08  & -     & 25.58  & 25.31  & 25.33  & 24.91  & 25.63  & 25.82  & 25.82  & 25.70  & - \\
\cmidrule{3-30}          &       & SSIM  & 0.8664  & -     & 0.8574  & 0.8653  & 0.5484  & 0.8688  & 0.7344  & 0.8610  & 0.7753  & 0.5876  & 0.8413  & 0.8181  & 0.8665  & 0.7819  & 0.8659  & {\textbf{0.8695}} & 0.7668  & -     & 0.8126  & 0.7923  & 0.7634  & 0.8006  & 0.8534  & 0.8694  & 0.8691  & 0.8597  & - \\
\cmidrule{3-30}          &       & SAM   & 0.0632  & -     & 0.0698  & 0.0660  & 0.2275  & 0.0551  & 0.1057  & 0.0604  & 0.1542  & 0.2198  & 0.0742  & 0.0669  & 0.0635  & 0.1020  & {\textbf{0.0509}} & 0.0538  & 0.1084  & -     & 0.0891  & 0.0816  & 0.1232  & 0.1635  & 0.0921  & 0.0596  & 0.0638  & 0.0928  & - \\
\cmidrule{3-30}          &       & EGRAS & 222.73  & -     & 224.51  & 222.67  & 252.24  & 222.18  & 243.68  & 224.05  & 246.39  & 248.57  & 223.32  & 234.02  & 222.64  & 226.58  & 222.69  & {\textbf{221.94}} & 233.43  & -     & 226.23  & 229.18  & 229.32  & 248.41  & 232.73  & 224.41  & 225.32  & 227.88  & - \\
    \midrule
    Time  & -     & minutes & 2.5   & 1.7   & 1.5   & 4.1   & {\textbf{0.1}} & 41.9  & 2.9   & 16.5  & 4.9   & {\textbf{0.1}} & 35.0  & 0.6   & 2.8   & 0.5   & 4.1   & 24.3  & 1.5   & 12.5  & {\textbf{0.1}} & 3.0   & 0.9   & {\textbf{0.1}} & 0.8   & 0.2   & {\textbf{0.1}} & 0.7   & {\textbf{0.1}} \\
    \bottomrule
    \end{tabular}}%
  \label{Table_Results_MSI-HSI_all}%
\end{table*}%

%% Table generated by Excel2LaTeX from sheet 'All-in-one'
%\begin{table*}[htbp]
%\tiny \tabcolsep2.08pt
%  \centering
%  \caption{Comparison of quantitative results on CAVE (with i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$) and Real-HSI datasets. The average denoising time (minutes) is calculated based on the CAVE dataset when $\sigma = 100$.}
%  \scalebox{0.826}{
%    \begin{tabular}{ccccccccccccccccccccccccccccc}
%    \toprule
%    \multirow{3}[4]{*}{Datasets} & \multirow{3}[4]{*}{$\sigma$} & \multirow{3}[4]{*}{Metrics} & \multicolumn{20}{c}{Traditonal denoisers}                                                                                                                     & \multicolumn{1}{c|}{} & \multicolumn{5}{c}{DNN methods} \\
%\cmidrule{4-29}          &       &       & 4DHOSVD & ANLM  & BM4D1 & BM4D2 & FastHyDe & ISTReg & LLRGTV & LLRT  & LRMR  & LRTA  & LTDL  & LRTDGS & MSt-SVD & MTSNMF & NGMeet & OLRT  & PARAFAC & RTA-LSM & SDS   & SSTV  & \multicolumn{1}{c}{TDL} & GRN   & HSI-DeNet & QRNN3D & sDeCNN & SST \\
%           &       &       & \cite{rajwade2012image} & \cite{manjon2010adaptive}  & \cite{maggioni2012nonlocal} & \cite{maggioni2012nonlocal} & \cite{zhuang2018fast} & \cite{xie2016multispectral} & \cite{He2018LLRGTV} & \cite{chang2017hyper} & \cite{zhang2013hyperspectral} & \cite{renard2008denoising} & \cite{gong2020low} & \cite{chen2019hyperspectral} & \cite{kong2017new} & \cite{ye2014multitask} & \cite{he2019non} & \cite{chang2020hyperspectral} & \cite{liu2012denoising} & \cite{dong2018robust} & \cite{lam2012denoising} & \cite{zeng2021hyperspectral} & \multicolumn{1}{c}{\cite{peng2014decomposable}} & \cite{cao2021deep} & \cite{chang2018hsi} & \cite{wei20203} & \cite{maffei2019single} & \cite{li2022spatial} \\
%    \midrule
%    \multirow{16}[32]{*}{CAVE} & \multirow{4}[8]{*}{10} & PSNR  & 45.43  & 41.52  & 43.04  & 44.61  & 42.87  & 45.14  & 39.62  & 46.60  & 39.47  & 41.36  & 45.90  & 35.99  & 45.20  & 43.04  & 46.59  & \textcolor{blue}{\textbf{47.07}} & 35.43  & 46.43  & 39.69  & 38.91  & 44.39  & 30.98  & 37.01  & 40.36  & 41.40  & 39.75  \\
%\cmidrule{3-29}          &       & SSIM  & 0.9812  & 0.9576  & 0.9700  & 0.9784  & 0.9763  & 0.9792  & 0.9274  & 0.9868  & 0.9125  & 0.9499  & 0.9855  & 0.8976  & 0.9814  & 0.9706  & \textcolor{blue}{\textbf{0.9880}} & 0.9877  & 0.8762  & 0.9857  & 0.9483  & 0.9153  & 0.9797  & 0.8622  & 0.8936  & 0.9672  & 0.9624  & 0.9730  \\
%\cmidrule{3-29}          &       & SAM   & 0.1084  & 0.2183  & 0.1844  & 0.1289  & 0.1398  & 0.1311  & 0.2676  & 0.0842  & 0.3282  & 0.1718  & 0.0923  & 0.1764  & 0.1064  & 0.1342  & 0.0853  & \textcolor{blue}{\textbf{0.0840}} & 0.2407  & 0.0926  & 0.2159  & 0.2669  & 0.1055  & 0.4971  & 0.3236  & 0.1926  & 0.1524  & 0.1632  \\
%\cmidrule{3-29}          &       & EGRAS & 30.83  & 47.79  & 40.07  & 33.32  & 42.90  & 31.71  & 63.65  & 26.75  & 63.52  & 49.53  & 29.06  & 103.69  & 32.05  & 40.29  & 27.26  & \textcolor{blue}{\textbf{25.53}} & 108.34  & 27.15  & 61.88  & 65.86  & 34.39  & 209.61  & 85.92  & 65.31  & 52.04  & 66.63  \\
%\cmidrule{2-29}          & \multirow{4}[8]{*}{30} & PSNR  & 39.78  & 34.70  & 37.05  & 38.80  & 37.22  & 40.37  & 32.26  & 41.49  & 31.43  & 36.06  & 41.21  & 35.12  & 40.23  & 37.02  & 41.60  & \textcolor{blue}{\textbf{41.79}} & 33.46  & 41.32  & 32.07  & 31.35  & 39.06  & 30.94  & 30.83  & 38.48  & 37.58  & 37.82  \\
%\cmidrule{3-29}          &       & SSIM  & 0.9336  & 0.8068  & 0.9236  & 0.9283  & 0.9151  & 0.9462  & 0.7150  & 0.9681  & 0.6517  & 0.8775  & 0.9656  & 0.8795  & 0.9530  & 0.8758  & \textcolor{blue}{\textbf{0.9693}} & 0.9680  & 0.8255  & 0.9598  & 0.6723  & 0.6078  & 0.9493  & 0.8605  & 0.6467  & 0.9496  & 0.9247  & 0.9564  \\
%\cmidrule{3-29}          &       & SAM   & 0.2272  & 0.4302  & 0.2898  & 0.2579  & 0.3123  & 0.2254  & 0.5538  & 0.1221  & 0.5899  & 0.2446  & 0.1299  & 0.2104  & 0.1737  & 0.2267  & 0.1238  & \textcolor{blue}{\textbf{0.1180}} & 0.3362  & 0.1556  & 0.4959  & 0.5190  & 0.1496  & 0.4970  & 0.5105  & 0.2320  & 0.1959  & 0.2143  \\
%\cmidrule{3-29}          &       & EGRAS & 59.12  & 103.96  & 83.28  & 65.23  & 81.44  & 54.82  & 141.67  & 48.50  & 154.15  & 90.50  & 49.68  & 109.98  & 56.26  & 79.30  & 48.15  & \textcolor{blue}{\textbf{46.65}} & 126.99  & 49.42  & 143.67  & 155.14  & 63.24  & 209.90  & 177.76  & 76.21  & 78.28  & 80.26  \\
%\cmidrule{2-29}          & \multirow{4}[8]{*}{50} & PSNR  & 36.82  & 30.76  & 34.51  & 35.90  & 34.56  & 37.88  & 28.53  & 38.65  & 27.44  & 33.52  & 38.62  & 33.84  & 37.73  & 33.50  & 38.87  & \textcolor{blue}{\textbf{39.13}} & 31.25  & 38.60  & 26.09  & 25.48  & 36.44  & 30.82  & -     & 37.02  & 35.49  & 36.43  \\
%\cmidrule{3-29}          &       & SSIM  & 0.8722  & 0.6064  & 0.8823  & 0.8685  & 0.8471  & 0.9168  & 0.5368  & 0.9482  & 0.4410  & 0.8201  & 0.9464  & 0.8470  & 0.9285  & 0.7585  & \textcolor{blue}{\textbf{0.9507}} & 0.9481  & 0.7307  & 0.9301  & 0.3529  & 0.3019  & 0.9171  & 0.8564  & -     & 0.9314  & 0.8947  &  0.9408  \\
%\cmidrule{3-29}          &       & SAM   & 0.3385  & 0.5801  & 0.3540  & 0.3557  & 0.4395  & 0.2737  & 0.7113  & 0.1551  & 0.7273  & 0.2897  & 0.1630  & 0.2674  & 0.2231  & 0.2956  & 0.1617  & \textcolor{blue}{\textbf{0.1436}} & 0.4541  & 0.2199  & 0.7170  & 0.7473  & 0.2007  & 0.4966  & -     & 0.2741  & 0.2141  & 0.2524  \\
%\cmidrule{3-29}          &       & EGRAS & 83.36  & 164.17  & 110.14  & 91.19  & 108.74  & 73.32  & 211.99  & 67.56  & 241.87  & 121.15  & 66.73  & 122.70  & 75.03  & 118.36  & 65.72  & \textcolor{blue}{\textbf{63.41}} & 158.53  & 67.27  & 290.93  & 306.21  & 85.24  & 210.86  & -     & 87.15  & 98.54  & 92.86  \\
%\cmidrule{2-29}          & \multirow{4}[8]{*}{100} & PSNR  & 32.66  & 24.92  & 31.21  & 31.84  & 30.62  & 31.85  & 23.36  & \textcolor{blue}{\textbf{35.39}} & 21.91  & 30.06  & 34.86  & 30.34  & 34.20  & 28.04  & 34.98  & 35.18  & 26.77  & 34.66  & 18.48  & 16.75  & 32.89  & 29.45  & -     & 30.33  & 32.51  & 33.96 \\
%\cmidrule{3-29}          &       & SSIM  & 0.7307  & 0.2828  & 0.7854  & 0.7197  & 0.6717  & 0.8176  & 0.2859  & \textcolor{blue}{\textbf{0.9154}} & 0.1962  & 0.7138  & 0.9002  & 0.6852  & 0.8800  & 0.4988  & 0.9073  & 0.8944  & 0.4481  & 0.8418  & 0.1067  & 0.0720  & 0.8283  & 0.7814  & -     & 0.7128  & 0.8309  & 0.9016  \\
%\cmidrule{3-29}          &       & SAM   & 0.5600  & 0.7968  & 0.4638  & 0.5160  & 0.6097  & 0.3605  & 0.9229  & \textcolor{blue}{\textbf{0.1962}} & 0.9175  & 0.3649  & 0.2349  & 0.4707  & 0.3142  & 0.4180  & 0.2504  & 0.2100  & 0.6942  & 0.3714  & 0.9868  & 1.0569  & 0.3138  & 0.4991  & -     & 0.5161  & 0.2748  & 0.3225  \\
%\cmidrule{3-29}          &       & EGRAS & 134.34  & 324.49  & 158.47  & 144.91  & 168.92  & 148.29  & 376.10  & \textcolor{blue}{\textbf{99.37}} & 456.12  & 180.03  & 102.61  & 174.87  & 115.24  & 221.84  & 101.86  & 99.93  & 260.85  & 105.99  & 718.40  & 834.58  & 128.22  & 225.29  & -     & 172.68  & 136.17  & 120.40  \\
%    \midrule
%    \multirow{4}[8]{*}{Real-HSI} & \multirow{4}[8]{*}{-} & PSNR  & 25.86  & -     & 25.84  & 25.88  & 23.99  & 25.91  & 24.63  & 25.90  & 24.81  & 24.27  & 25.80  & 25.12  & 25.86  & 25.51  & 25.87  & \textcolor{blue}{\textbf{25.94}} & 25.08  & -     & 25.58  & 25.31  & 25.33  & 24.91  & 25.63  & 25.82  & 25.70  & - \\
%\cmidrule{3-29}          &       & SSIM  & 0.8664  & -     & 0.8574  & 0.8653  & 0.5484  & 0.8688  & 0.7344  & 0.8610  & 0.7753  & 0.5876  & 0.8413  & 0.8181  & 0.8665  & 0.7819  & 0.8659  & \textcolor{blue}{\textbf{0.8695}} & 0.7668  & -     & 0.8126  & 0.7923  & 0.7634  & 0.8006  & 0.8534  & 0.8691  & 0.8597  & - \\
%\cmidrule{3-29}          &       & SAM   & 0.0632  & -     & 0.0698  & 0.0660  & 0.2275  & 0.0551  & 0.1057  & 0.0604  & 0.1542  & 0.2198  & 0.0742  & 0.0669  & 0.0635  & 0.1020  & \textcolor{blue}{\textbf{0.0509}} & 0.0538  & 0.1084  & -     & 0.0891  & 0.0816  & 0.1232  & 0.1635  & 0.0921  & 0.0638  & 0.0928  & - \\
%\cmidrule{3-29}          &       & EGRAS & 222.73  & -     & 224.51  & 222.67  & 252.24  & 222.18  & 243.68  & 224.05  & 246.39  & 248.57  & 223.32  & 234.02  & 222.64  & 226.58  & 222.69  & \textcolor{blue}{\textbf{221.94}} & 233.43  & -     & 226.23  & 229.18  & 229.32  & 248.41  & 232.73  & 225.32  & 227.88  & - \\
%    \midrule
%    Time (m)  & -     & - & 2.5   & 1.7   & 1.5   & 4.1   & \textcolor{blue}{\textbf{0.1}} & 41.9  & 2.9   & 16.5  & 4.9   & \textcolor{blue}{\textbf{0.1}} & 35.0  & 0.6   & 2.8   & 0.5   & 4.1   & 24.3  & 1.5   & 12.5  & \textcolor{blue}{\textbf{0.1}} & 3.0   & 0.9   & \textcolor{blue}{\textbf{0.1}} & 0.8   & \textcolor{blue}{\textbf{0.1}} & 0.7   &  \textcolor{blue}{\textbf{0.1}}  \\
%    \bottomrule
%    \end{tabular}}%
%  \label{Table_Results_MSI-HSI_all}%
%\end{table*}%



% Table generated by Excel2LaTeX from sheet 'All-in-one'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Comparison of quantitative results and computational time (minutes) on CAVE and Real-HSI datasets.}
%  \scalebox{0.636}{
%    \begin{tabular}{ccccccccccccccccccccccccccc}
%    \toprule
%\cmidrule{24-27}    \multirow{2}[4]{*}{Datasets} & \multirow{2}[4]{*}{$\sigma$} & \multirow{2}[4]{*}{Metrics} & \multicolumn{20}{c|}{Traditonal denoisers}                                                                                                                    & \multicolumn{4}{c}{DNN methods} \\
%\cmidrule{4-27}          &       &       & 4DHOSVD & ANLM  & BM4D1 & BM4D2 & FastHyDe & ISTReg & LLRGTV & LLRT  & LRMR  & LRTA  & LTDL  & LRTDGS & MStSVD & MTSNMF & NGMeet & OLRT  & PARAFAC & RTA-LSM & SDS   & \multicolumn{1}{c|}{SSTV} & GRN   & HSI-DeNet & QRNN3D & sDeCNN \\
%    \midrule
%    \multirow{16}[32]{*}{CAVE} & \multirow{4}[8]{*}{10} & PSNR  & 45.43  & 41.52  & 43.04  & 44.61  & 42.87  & 45.14  & 39.62  & 46.60  & 39.47  & 41.36  & 45.90  & 35.99  & 45.20  & 43.04  & 46.59  & /     & 35.43  & 46.43  & 39.69  & 38.91  & 30.98  & 37.01  & 40.36  & 41.40  \\
%\cmidrule{3-27}          &       & SSIM  & 0.981  & 0.958  & 0.970  & 0.978  & 0.976  & 0.979  & 0.927  & 0.987  & 0.912  & 0.950  & 0.986  & 0.898  & 0.981  & 0.971  & 0.988  & /     & 0.876  & 0.986  & 0.948  & 0.915  & 0.862  & 0.894  & 0.967  & 0.962  \\
%\cmidrule{3-27}          &       & SAM   & 0.108  & 0.218  & 0.184  & 0.129  & 0.140  & 0.131  & 0.268  & 0.084  & 0.328  & 0.172  & 0.092  & 0.176  & 0.106  & 0.134  & 0.085  & /     & 0.241  & 0.093  & 0.216  & 0.267  & 0.497  & 0.324  & 0.193  & 0.152  \\
%\cmidrule{3-27}          &       & EGRAS & 30.8  & 47.8  & 40.1  & 33.3  & 42.9  & 31.7  & 63.7  & 26.8  & 63.5  & 49.5  & 29.1  & 103.7  & 32.0  & 40.3  & 27.3  & /     & 108.3  & 27.1  & 61.9  & 65.9  & 209.6  & 85.9  & 65.3  & 52.0  \\
%\cmidrule{2-27}          & \multirow{4}[8]{*}{30} & PSNR  & 39.78  & 34.70  & 37.05  & 38.80  & 37.22  & 40.37  & 32.26  & 41.49  & 31.43  & 36.06  & 41.21  & 35.12  & 40.23  & 37.02  & 41.60  & /     & 33.46  & 41.32  & 32.07  & 31.35  & 30.94  & 30.83  & 38.48  & 37.58  \\
%\cmidrule{3-27}          &       & SSIM  & 0.934  & 0.807  & 0.924  & 0.928  & 0.915  & 0.946  & 0.715  & 0.968  & 0.652  & 0.878  & 0.966  & 0.879  & 0.953  & 0.876  & 0.969  & /     & 0.826  & 0.960  & 0.672  & 0.608  & 0.861  & 0.647  & 0.950  & 0.925  \\
%\cmidrule{3-27}          &       & SAM   & 0.227  & 0.430  & 0.290  & 0.258  & 0.312  & 0.225  & 0.554  & 0.122  & 0.590  & 0.245  & 0.130  & 0.210  & 0.174  & 0.227  & 0.124  & /     & 0.336  & 0.156  & 0.496  & 0.519  & 0.497  & 0.511  & 0.232  & 0.196  \\
%\cmidrule{3-27}          &       & EGRAS & 59.1  & 104.0  & 83.3  & 65.2  & 81.4  & 54.8  & 141.7  & 48.5  & 154.2  & 90.5  & 49.7  & 110.0  & 56.3  & 79.3  & 48.1  & /     & 127.0  & 49.4  & 143.7  & 155.1  & 209.9  & 177.8  & 76.2  & 78.3  \\
%\cmidrule{2-27}          & \multirow{4}[8]{*}{50} & PSNR  & 36.82  & 30.76  & 34.51  & 35.90  & 34.56  & 37.88  & 28.53  & 38.65  & 27.44  & 33.52  & 38.62  & 33.84  & 37.73  & 33.50  & 38.87  & /     & 31.25  & 38.60  & 26.09  & 25.48  & 30.82  & 23.00  & 37.02  & 35.49  \\
%\cmidrule{3-27}          &       & SSIM  & 0.872  & 0.606  & 0.882  & 0.869  & 0.847  & 0.917  & 0.537  & 0.948  & 0.441  & 0.820  & 0.946  & 0.847  & 0.928  & 0.759  & 0.951  & /     & 0.731  & 0.930  & 0.353  & 0.302  & 0.856  & 0.240  & 0.931  & 0.895  \\
%\cmidrule{3-27}          &       & SAM   & 0.339  & 0.580  & 0.354  & 0.356  & 0.439  & 0.274  & 0.711  & 0.155  & 0.727  & 0.290  & 0.163  & 0.267  & 0.223  & 0.296  & 0.162  & /     & 0.454  & 0.220  & 0.717  & 0.747  & 0.497  & 0.701  & 0.274  & 0.214  \\
%\cmidrule{3-27}          &       & EGRAS & 83.4  & 164.2  & 110.1  & 91.2  & 108.7  & 73.3  & 212.0  & 67.6  & 241.9  & 121.1  & 66.7  & 122.7  & 75.0  & 118.4  & 65.7  & /     & 158.5  & 67.3  & 290.9  & 306.2  & 210.9  & 465.5  & 87.1  & 98.5  \\
%\cmidrule{2-27}          & \multirow{4}[8]{*}{100} & PSNR  & 32.66  & 24.92  & 31.21  & 31.84  & 30.62  & 31.85  & 23.36  & 35.39  & 21.91  & 30.06  & 34.86  & 30.34  & 34.20  & 28.04  & 34.98  & /     & 26.77  & 34.66  & 18.48  & 16.75  & 29.45  & 13.12  & 30.33  & 32.51  \\
%\cmidrule{3-27}          &       & SSIM  & 0.731  & 0.283  & 0.785  & 0.720  & 0.672  & 0.818  & 0.286  & 0.915  & 0.196  & 0.714  & 0.900  & 0.685  & 0.880  & 0.499  & 0.907  & /     & 0.448  & 0.842  & 0.107  & 0.072  & 0.781  & 0.039  & 0.713  & 0.831  \\
%\cmidrule{3-27}          &       & SAM   & 0.560  & 0.797  & 0.464  & 0.516  & 0.610  & 0.360  & 0.923  & 0.196  & 0.917  & 0.365  & 0.235  & 0.471  & 0.314  & 0.418  & 0.250  & /     & 0.694  & 0.371  & 0.987  & 1.057  & 0.499  & 0.896  & 0.516  & 0.275  \\
%\cmidrule{3-27}          &       & EGRAS & 134.3  & 324.5  & 158.5  & 144.9  & 168.9  & 148.3  & 376.1  & 99.4  & 456.1  & 180.0  & 102.6  & 174.9  & 115.2  & 221.8  & 101.9  & /     & 260.9  & 106.0  & 718.4  & 834.6  & 225.3  & 1301.7  & 172.7  & 136.2  \\
%    \midrule
%    \multirow{4}[8]{*}{Real-HSI} & \multirow{4}[8]{*}{/} & PSNR  & 25.86  & /     & 25.84  & 25.88  & 23.99  & 25.91  & 24.63  & 25.90  & 24.81  & 24.27  & 25.80  & 25.12  & 25.86  & 25.51  & 25.87  & 25.94  & 25.08  & /     & 25.58  & 25.31  & 24.91  & 25.63  & 25.82  & 25.70  \\
%\cmidrule{3-27}          &       & SSIM  & 0.866  & /     & 0.857  & 0.865  & 0.548  & 0.869  & 0.734  & 0.861  & 0.775  & 0.588  & 0.841  & 0.818  & 0.867  & 0.782  & 0.866  & 0.870  & 0.767  & /     & 0.813  & 0.792  & 0.801  & 0.853  & 0.869  & 0.860  \\
%\cmidrule{3-27}          &       & SAM   & 0.063  & /     & 0.070  & 0.066  & 0.228  & 0.055  & 0.106  & 0.060  & 0.154  & 0.220  & 0.074  & 0.067  & 0.063  & 0.102  & 0.051  & 0.054  & 0.108  & /     & 0.089  & 0.082  & 0.164  & 0.092  & 0.064  & 0.093  \\
%\cmidrule{3-27}          &       & EGRAS & 222.7  & /     & 224.5  & 222.7  & 252.2  & 222.2  & 243.7  & 224.1  & 246.4  & 248.6  & 223.3  & 234.0  & 222.6  & 226.6  & 222.7  & 221.9  & 233.4  & /     & 226.2  & 229.2  & 248.4  & 232.7  & 225.3  & 227.9  \\
%    \midrule
%    Time (m) & /     & /     & 2.5   & 1.7   & 1.5   & 4.1   & 0.1   & 41.9  & 2.9   & 16.5  & 4.9   & 0.1   & 35.0  & 0.6   & 2.8   & 0.5   & 4.1   & 0.0   & 1.5   & 12.5  & 0.1   & 3.0   & 0.1   & 0.8   & 0.1   & 0.7  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_Results_MSI-HSI_all}
%\end{table*}%




==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_color_all.tex <==
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Average PSNR, SSIM values and computational time of compared methods on CC15, Xu-100 and Kong-Image datasets. The average computational time is based on images of size $512 \times 512$. The best results are black bolded.}
%  \scalebox{0.83}{
%    \begin{tabular}{cccccccccccccccc}
%    \toprule
%    \multirow{2}[4]{*}{Method} & Dataset & CC15  & CC60  & Xu-100 & CANON 100D & CANON 600D & HUAWEI Honor6X & IPHONE 5S & IPHONE 6S & SONY A6500 & XIAOMI MI8 & OPPO R11s & FUJIFILM X100T & \multirow{2}[4]{*}{Implementation} & \multirow{2}[4]{*}{Time (s)} \\
%\cmidrule{2-14}          & \multicolumn{1}{l}{\# Images} & 15    & 60    & 100   & 55    & 25    & 30    & 36    & 67    & 36    & 50    & 39    & 71    &       &  \\
%    \midrule
%    \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{Noisy} & 33.41  & 34.51  & 35.97  & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{/} \\
%          &       & 0.8476  & 0.8712  & 0.9125  & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251  & 0.9356  & 0.9307  &       &  \\
%    \midrule
%    \multirow{28}[28]{*}{\shortstack[l]{DNN \\ methods}} & \multirow{2}[2]{*}{DnCNN} & 37.47  & 39.32  & 38.51  & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{3.28} \\
%          &       & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{FFD-Net} & 37.67  & 39.73  & 38.56  & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{1.99} \\
%          &       & 0.9563  & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBDNet} & 36.36  & 37.46  & 36.93  & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{3.58} \\
%          &       & 0.9294  & 0.9482  & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DBF} & 38.38  & 40.59  & 38.87  & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.32} \\
%          &       & 0.9644  & 0.9811  & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DIDN} & 36.04  & \multirow{2}[2]{*}{N/A} & 37.32  & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9456  &       & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{FCCF} & \textbf{39.04} & \textbf{40.89} & 38.85  & 41.91  & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.66} & \textbf{40.93} & \textbf{42.78} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{36.36} \\
%          &       & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & 0.9794  & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640} & \textbf{0.9747} & \textbf{0.9782} &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{NLNet} & 37.56  & 39.32  & 38.58  & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{49.98} \\
%          &       & 0.9554  & 0.9744  & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{Unet} & 36.95  & 38.96  & 38.05  & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{5.69} \\
%          &       & 0.9425  & 0.9708  & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{VDNet} & 35.86  & \multirow{2}[2]{*}{N/A} & 37.58  & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.21} \\
%          &       & 0.9454  &       & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{AINDNet} & 35.88  & 36.98  & 37.22  & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.29} \\
%          &       & 0.9113  & 0.9708  & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CycleISP} & 35.40  & 36.87  & 37.61  & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.38} \\
%          &       & 0.9158  & 0.9393  & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{RIDNet} & 36.83  & 38.11  & 38.57  & 41.08  & 42.18  & 38.88  & 38.69  & 39.02  & 44.40  & 35.75  & 40.08  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.06} \\
%          &       & 0.9406  & 0.9609  & 0.9702  & 0.9770  & 0.9801  & 0.9621  & 0.9627  & 0.9588  & 0.9873  & 0.9570  & 0.9719  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{SADNet} & 37.80  & \multirow{2}[2]{*}{N/A} & \textbf{39.30} & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.33} \\
%          &       & 0.9521  &       & \textbf{0.9725} & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DPIR} & 38.30  & 40.33  & 38.93  & \textbf{41.94} & 42.62  & \textbf{40.35} & \textbf{40.80} & \textbf{40.80} & 45.76  & 36.61  & \textbf{40.96} & \textbf{42.78} & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9608  & 0.9791  & 0.9700  & 0.9779  & 0.9819  & \textbf{0.9694} & 0.9661  & \textbf{0.9700} & 0.9895  & 0.9607  & 0.9741  & 0.9770  &       &  \\
%    \midrule
%    \midrule
%    \multirow{24}[24]{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{2}[2]{*}{LCSD} & 36.20  & 37.69  & 37.97  & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.45} \\
%          &       & 0.9339  & 0.9626  & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{LLRT} & 37.36  & 38.51  & 38.51  & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{>1000} \\
%          &       & 0.9559  & 0.9636  & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{GID} & 37.02  & 38.41  & 38.37  & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{38.88} \\
%          &       & 0.9459  & 0.9633  & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{MCWNNM} & 37.72  & 39.03  & 38.51  & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{228.16} \\
%          &       & 0.9568  & 0.9698  & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{NLH\_CC} & 38.49  & 39.86  & 38.36  & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & \textbf{46.00} & 35.73  & 40.69  & \textbf{42.80 } & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{51.86} \\
%          &       & 0.9647  & 0.9759  & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905} & 0.9552  & 0.9740  & 0.9776  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{TWSC} & 37.90  & 39.66  & 38.62  & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{368.68} \\
%          &       & 0.9592  & 0.9759  & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{M-SVD} & 37.62  & 39.27  & 38.56  & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{75.88} \\
%          &       & 0.9542  & 0.9705  & 0.9671  & 0.9788  & 0.9823  & 0.9671  & \textbf{0.9680} & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{4DHOSVD1} & 37.51  & 39.15  & 38.51  & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{86.69} \\
%          &       & 0.9559  & 0.9729  & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CMSt-SVD} & 37.95  & 39.75  & 38.82  & \textbf{41.99} & 42.75  & 40.08  & \textbf{40.84} & 40.53  & 45.89  & 36.40  & 40.85  & 42.68  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.18} \\
%          &       & 0.9588  & 0.9756  & 0.9694  & \textbf{0.9794} & 0.9840  & 0.9674  & 0.9668  & 0.9674  & 0.9903  & 0.9616  & 0.9743  & 0.9770  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D1} & 37.56  & 39.21  & 38.52  & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{0.95} \\
%          &       & 0.9562  & 0.9729  & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D2} & 37.70  & 39.41  & 38.69  & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{4.38} \\
%          &       & 0.9572  & 0.9740  & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D\_best} & 37.95  & 39.68  & 38.81  & \textbf{42.08 } & 42.89  & \textbf{40.48} & \textbf{41.25} & \textbf{41.16} & 45.81  & \textbf{36.66} & \textbf{40.89} & \textbf{43.14} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{4.38} \\
%          &       & 0.9621  & 0.9775  & 0.9712  & \textbf{0.9808} & 0.9851  & \textbf{0.9741} & \textbf{0.9758} & \textbf{0.9783} & 0.9904  & \textbf{0.9640} & 0.9742  & \textbf{0.9805} &       &  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_color_all}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet2'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Average PSNR, SSIM values and computational time (second) on four realistic color image datasets. The average time is calculated based on the PolyU dataset, and 'N/A' means the models can not handle certain size of images. The best results (excluding CBM3D\_best) are black bolded.}
%    \scalebox{0.806}{
%    \renewcommand{\arraystretch}{0.399}
%    \begin{tabular}{cccccccccccccccc}
%    \toprule
%    \multirow{3}[6]{*}{Method} & \multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multicolumn{9}{c}{IOCI}                                        & \multirow{3}[6]{*}{Implementation} & \multirow{3}[6]{*}{Time (s)} \\
%\cmidrule{6-14}          &       &       &       &       & CANON 100D & CANON 600D & HUAWEI Honor6X & IPHONE 5S & IPHONE 6S & SONY A6500 & XIAOMI MI8 & OPPO R11s & FUJIFILM X100T &       &  \\
%\cmidrule{2-14}          & \multicolumn{1}{l}{\# Images} & 15    & 60    & 100   & 55    & 25    & 30    & 36    & 67    & 36    & 50    & 39    & 71    &       &  \\
%    \midrule
%    \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{Noisy} & 33.41  & 34.51  & 35.97  & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{/} \\
%          &       & 0.8476  & 0.8712  & 0.9125  & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251  & 0.9356  & 0.9307  &       &  \\
%    \midrule
%    \multirow{32}[32]{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{2}[2]{*}{LCSD} & 36.20  & 37.69  & 37.97  & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.45} \\
%          &       & 0.9339  & 0.9626  & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{LLRT} & 37.36  & 38.51  & 38.51  & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{$>$1000} \\
%          &       & 0.9559  & 0.9636  & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{GID} & 37.02  & 38.41  & 38.37  & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{38.88} \\
%          &       & 0.9459  & 0.9633  & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{MCWNNM} & 37.72  & 39.03  & 38.51  & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{228.16} \\
%          &       & 0.9568  & 0.9698  & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{NLH} & 38.49  & 39.86  & 38.36  & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & 46.00  & 35.73  & 40.69  & 42.80  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{51.86} \\
%          &       & 0.9647  & 0.9759  & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & 0.9905  & 0.9552  & 0.9740  & 0.9776  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{TWSC} & 37.90  & 39.66  & 38.62  & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{368.68} \\
%          &       & 0.9592  & 0.9759  & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{M-SVD} & 37.62  & 39.27  & 38.56  & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{75.88} \\
%          &       & 0.9542  & 0.9705  & 0.9671  & 0.9788  & 0.9823  & 0.9671  & 0.9680  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{4DHOSVD} & 37.51  & 39.15  & 38.51  & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{80.69} \\
%          &       & 0.9559  & 0.9729  & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CMSt-SVD} & 37.95  & 39.75  & 38.82  & \textbf{41.99} & 42.75  & 40.08  & \textbf{40.84} & 40.53  & \textbf{45.89} & 36.40  & \textbf{40.85} & 42.68  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.18} \\
%          &       & 0.9588  & 0.9756  & 0.9694  & \textbf{0.9794} & 0.9840  & 0.9674  & 0.9668  & 0.9674  & \textbf{0.9903} & 0.9616  & 0.9743  & 0.9770  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D1} & 37.56  & 39.21  & 38.52  & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{0.95} \\
%          &       & 0.9562  & 0.9729  & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D2} & 37.70  & 39.41  & 38.69  & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{4.38} \\
%          &       & 0.9572  & 0.9740  & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D\_best} & 37.95  & 39.68  & 38.81  & \textbf{42.08} & 42.89  & \textbf{40.48} & \textbf{41.25} & \textbf{41.16} & \textbf{45.81} & \textbf{36.66} & \textbf{40.89} & \textbf{43.14} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{/} \\
%          &       & 0.9621  & 0.9775  & 0.9712  & \textbf{0.9808} & 0.9851  & \textbf{0.9741} & \textbf{0.9758} & \textbf{0.9783} & \textbf{0.9904} & \textbf{0.9640} & 0.9742  & \textbf{0.9805} &       &  \\
%    \midrule
%    \midrule
%    \multirow{52}[52]{*}{\shortstack[l]{DNN \\ methods}} & \multirow{2}[2]{*}{DnCNN} & 37.47  & 39.32  & 38.51  & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{3.28} \\
%          &       & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{FFDNet} & 37.68  & 39.73  & 38.56  & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{1.99} \\
%          &       & 0.9563  & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBDNet} & 36.36  & 37.46  & 36.93  & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{3.58} \\
%          &       & 0.9294  & 0.9482  & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DBF} & 38.38  & 40.59  & 38.87  & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.32} \\
%          &       & 0.9644  & 0.9811  & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DIDN} & 36.04  & \multirow{2}[2]{*}{N/A} & 37.32  & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9456  &       & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{FCCF} & \textbf{39.04} & \textbf{40.89} & 38.85  & \textbf{41.91} & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.66 } & \textbf{40.93} & \textbf{42.78} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{36.36} \\
%          &       & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & \textbf{0.9794} & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640} & \textbf{0.9747} & \textbf{0.9782} &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{NLNet} & 37.56  & 39.32  & 38.58  & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{49.98} \\
%          &       & 0.9554  & 0.9744  & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{UDnet} & 36.95  & 38.96  & 38.05  & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{5.69} \\
%          &       & 0.9425  & 0.9708  & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{VDNet} & 35.86  & \multirow{2}[2]{*}{N/A} & 37.58  & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.21} \\
%          &       & 0.9454  &       & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{AINDNet} & 35.88  & 36.98  & 37.22  & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.29} \\
%          &       & 0.9113  & 0.9708  & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CycleISP} & 35.40  & 36.87  & 37.61  & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.38} \\
%          &       & 0.9158  & 0.9393  & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{RIDNet} & 36.83  & 38.11  & 38.57  & 41.08  & 42.18  & 38.88  & 38.69  & 39.02  & 44.40  & 35.75  & 40.08  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.06} \\
%          &       & 0.9406  & 0.9609  & 0.9702  & 0.9770  & 0.9801  & 0.9621  & 0.9627  & 0.9588  & 0.9873  & 0.9570  & 0.9719  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{SADNet} & 37.80  & \multirow{2}[2]{*}{N/A} & 39.30 & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.33} \\
%          &       & 0.9521  &       & 0.9725 & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DANet} & 37.17  & 38.63  & \textbf{41.76}  & 41.59  & 42.47  & 38.46  & 39.39  & 38.80  & 44.71  & 36.21  & 39.92  & 41.44  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.12} \\
%          &       & 0.9528  & 0.9694  & \textbf{0.9771}  & 0.9788  & 0.9833  & 0.9545  & 0.9661  & 0.9527  & 0.9874  & 0.9608  & 0.9673  & 0.9693  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{Self2Self} & 36.26 & 37.88 &	37.50 &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A}
% & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{$>$2000} \\
%          &       & 0.9466 & 0.9672 & 0.9801 &  &	 &  &  &  &  &  &  &  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{MIRNet} & 36.06 & 37.25 &	37.49 &	40.72 & 41.68 &	38.28 &	38.60 &	38.55 &	43.66 &	35.42 &	39.73 &	41.05
% & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9416 & 0.9556 & 0.9556 & 0.9747 &	0.9777 & 0.9539 & 0.9591 & 0.9522 & 0.9834 & 0.9525 & 0.9670 & 0.9679 &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DRUNet} & 38.30  & 40.33  & 38.93  & \textbf{41.94} & 42.62  & \textbf{40.35} & 40.80  & \textbf{40.80} & 45.76  & 36.61  & \textbf{40.96} & \textbf{42.78} & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9608  & 0.9791  & 0.9700  & 0.9779  & 0.9819  & \textbf{0.9694} & 0.9661  & \textbf{0.9700} & 0.9895  & 0.9607  & 0.9741  & 0.9770  &       &  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_color_all}%
%\end{table*}%


\begin{table*}[htbp]
\tiny
  \centering
  \caption{Average PSNR, SSIM values and computational time (second) on four realistic color image datasets. The average time is calculated based on the PolyU dataset, and 'N/A' means the models can not handle certain size of images. The best results (excluding CBM3D\_best) are black bolded.}
    \scalebox{0.808}{
    \renewcommand{\arraystretch}{0.66}
    \begin{tabular}{cccccccccccccccc}
    \toprule
    \multirow{3}[6]{*}{Method} & \multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multicolumn{9}{c}{IOCI}                                        & \multirow{3}[6]{*}{Implementation} & \multirow{3}[6]{*}{Time (s)} \\
\cmidrule{6-14}          &       &       &       &       & CANON 100D & CANON 600D & HUAWEI Honor6X & IPHONE 5S & IPHONE 6S & SONY A6500 & XIAOMI MI8 & OPPO R11s & FUJIFILM X100T &       &  \\
\cmidrule{2-14}          & \multicolumn{1}{l}{\# Images} & 15    & 60    & 100   & 55    & 25    & 30    & 36    & 67    & 36    & 50    & 39    & 71    &       &  \\
    \midrule
    \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{Noisy} & 33.41  & 34.51  & 35.97  & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{/} \\
          &       & 0.8476  & 0.8712  & 0.9125  & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251  & 0.9356  & 0.9307  &       &  \\
    \midrule
    \multirow{28}[28]{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{2}[2]{*}{LCSD} & 36.20  & 37.69  & 37.97  & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.45} \\
          &       & 0.9339  & 0.9626  & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{LLRT} & 37.36  & 38.51  & 38.51  & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{$>$1000} \\
          &       & 0.9559  & 0.9636  & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{GID} & 37.02  & 38.41  & 38.37  & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{38.88} \\
          &       & 0.9459  & 0.9633  & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{MCWNNM} & 37.72  & 39.03  & 38.51  & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{228.16} \\
          &       & 0.9568  & 0.9698  & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{NLH} & 38.49  & 39.86  & 38.36  & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & \textbf{46.00}  & 35.73  & 40.69  & 42.80  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{51.86} \\
          &       & 0.9647  & 0.9759  & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905}  & 0.9552  & 0.9740  & 0.9776  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{TWSC} & 37.90  & 39.66  & 38.62  & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{368.68} \\
          &       & 0.9592  & 0.9759  & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{M-SVD} & 37.62  & 39.27  & 38.56  & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{75.88} \\
          &       & 0.9542  & 0.9705  & 0.9671  & 0.9788  & 0.9823  & 0.9671  & \textbf{0.9680}  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{4DHOSVD} & 37.51  & 39.15  & 38.51  & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{80.69} \\
          &       & 0.9559  & 0.9729  & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CMSt-SVD} & 37.95  & 39.75  & 38.82  & \textbf{41.99} & 42.75  & 40.08  & \textbf{40.84} & 40.53  & 45.89 & 36.40  & 40.85 & 42.68  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.18} \\
          &       & 0.9588  & 0.9756  & 0.9694  & \textbf{0.9794} & 0.9840  & 0.9674  & 0.9668  & 0.9674  & 0.9903 & 0.9616  & 0.9743  & 0.9770  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D1} & 37.56  & 39.21  & 38.52  & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{0.95} \\
          &       & 0.9562  & 0.9729  & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D2} & 37.70  & 39.41  & 38.69  & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{4.38} \\
          &       & 0.9572  & 0.9740  & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D\_best} & 37.95  & 39.68  & 38.81  & {42.08} & 42.89  & {40.48} & {41.25} & {41.16} & {45.81} & {36.66} & {40.89} & {43.14} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{/} \\
          &       & 0.9621  & 0.9775  & 0.9712  & {0.9808} & 0.9851  & {0.9741} & {0.9758} & {0.9783} & {0.9904} & {0.9640} & 0.9742  & {0.9805} &       &  \\
    \midrule
    \midrule
    \multirow{43}[43]{*}{\shortstack[l]{DNN \\ methods}} & \multirow{2}[2]{*}{DnCNN} & 37.47  & 39.32  & 38.51  & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{3.28} \\
          &       & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{FFDNet} & 37.68  & 39.73  & 38.56  & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{1.99} \\
          &       & 0.9563  & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & \textbf{0.9707}  & 0.9901  & 0.9607  & 0.9733  & 0.9759  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CBDNet} & 36.36  & 37.46  & 36.93  & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{3.58} \\
          &       & 0.9294  & 0.9482  & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{DBF} & 38.38  & 40.59  & 38.87  & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.32} \\
          &       & 0.9644  & 0.9811  & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{DIDN} & 36.04  & \multirow{2}[2]{*}{N/A} & 37.32  & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
          &       & 0.9456  &       & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{FCCF} & \textbf{39.04} & \textbf{40.89} & 38.85  & \textbf{41.91} & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.66 } & \textbf{40.93} & \textbf{42.78} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{36.36} \\
          &       & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & \textbf{0.9794} & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9888  & \textbf{0.9640} & \textbf{0.9747} & \textbf{0.9782} &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{NLNet} & 37.56  & 39.32  & 38.58  & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{49.98} \\
          &       & 0.9554  & 0.9744  & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & \textbf{0.9709}  & 0.9875  & 0.9617  & 0.9729  & 0.9739  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{UDnet} & 36.95  & 38.96  & 38.05  & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{5.69} \\
          &       & 0.9425  & 0.9708  & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{VDNet} & 35.86  & \multirow{2}[2]{*}{N/A} & 37.58  & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.21} \\
          &       & 0.9454  &       & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{AINDNet} & 35.88  & 36.98  & 37.22  & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.18  & 34.49  & 37.20  & 38.50  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.29} \\
          &       & 0.9113  & 0.9305  & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CycleISP} & 35.40  & 36.87  & 37.61  & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.38} \\
          &       & 0.9158  & 0.9393  & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{RIDNet} & 36.83  & 38.11  & 38.57  & 41.08  & 42.18  & 38.88  & 38.69  & 39.02  & 44.40  & 35.75  & 40.08  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.06} \\
          &       & 0.9406  & 0.9609  & 0.9702  & 0.9770  & 0.9801  & 0.9621  & 0.9627  & 0.9588  & 0.9873  & 0.9570  & 0.9719  & 0.9750  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{SADNet} & 37.80  & \multirow{2}[2]{*}{N/A} & 39.30 & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.33} \\
          &       & 0.9521  &       & 0.9725 & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{DANet} & 37.17  & 38.63  & \textbf{41.76}  & 41.59  & 42.47  & 38.46  & 39.39  & 38.80  & 44.71  & 36.21  & 39.92  & 41.44  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.12} \\
          &       & 0.9528  & 0.9694  & \textbf{0.9771}  & 0.9788  & 0.9833  & 0.9545  & 0.9661  & 0.9527  & 0.9874  & 0.9608  & 0.9673  & 0.9693  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{Self2Self} & 36.26 & 37.88 &	37.66 &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A}
 & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{$>$2000} \\
          &       & 0.9466 & 0.9672 & 0.9563 &  &	 &  &  &  &  &  &  &  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{MIRNet} & 36.06 & 37.25 &	37.49 &	40.72 & 41.68 &	38.28 &	38.60 &	38.55 &	43.66 &	35.42 &	39.73 &	41.05
 & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
          &       & 0.9416 & 0.9556 & 0.9556 & 0.9747 &	0.9777 & 0.9539 & 0.9591 & 0.9522 & 0.9834 & 0.9525 & 0.9670 & 0.9679 &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{DRUNet} & 38.30  & 40.33  & 38.93  & \textbf{41.94} & 42.62  & \textbf{40.35} & \textbf{40.80}  & \textbf{40.80} & 45.76  & 36.61  & \textbf{40.96} & \textbf{42.78} & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
          &       & 0.9608  & 0.9791  & 0.9700  & 0.9779  & 0.9819  & \textbf{0.9694} & 0.9661  & 0.9700 & 0.9895  & 0.9607  & 0.9741  & 0.9770  &       &  \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_color_all}%
\end{table*}%




==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_color_all_psnr.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%\renewcommand{\arraystretch}{0.9}
%\tiny
%  \centering
%  \caption{Average PSNR and computational time of compared methods on CC15, Xu-100 and Kong-Image datasets. The average computational time is based on images of size $512 \times 512$.}
%  \scalebox{0.96}{
%    \begin{tabular}{cccccccccccccccc}
%    \toprule
%    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset}                                                                  & \multirow{2}[4]{*}{Implementation} & \multirow{2}[4]{*}{Time (s)} \\
%\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI &       &  \\
%    \midrule
%    \multicolumn{2}{c}{Noisy} & 33.41 & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & MATLAB + MEX & 1.99  \\
%    \midrule
%    \multirow{12}[24]{*}{Deep Network} & FFDNet & 37.67  & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & MATLAB + MEX & 3.58  \\
%\cmidrule{2-16}          & CBDNet & 36.36  & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & Python + GPU & 0.32  \\
%\cmidrule{2-16}          & DeepBoosting & 38.38  & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & Python + GPU & 0.18  \\
%\cmidrule{2-16}          & DIDN  & 36.04  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & Python + GPU & 0.98  \\
%\cmidrule{2-16}          & FCCF  & 39.04  & 40.89  & 38.85 & 41.91  & 43.07  & 40.11  & 40.39  & 40.65  & 45.38  & 36.67  & 40.93  & 42.78  & MATLAB + MEX & 49.98  \\
%\cmidrule{2-16}          & NLNet & 37.56  & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & MATLAB + MEX & 5.69  \\
%\cmidrule{2-16}          & Unet  & 36.95  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & Python + GPU & 0.21  \\
%\cmidrule{2-16}          & VDNet & 35.86  & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & Python + GPU & 1.29  \\
%\cmidrule{2-16}          & AINDNet & 35.88  & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & Python + GPU & 0.98  \\
%\cmidrule{2-16}          & CycleISP & 35.40  & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & Python + GPU & 0.38  \\
%\cmidrule{2-16}          & SADNet & 37.80  & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & Python + GPU & 0.33  \\
%\cmidrule{2-16}          & DnCNN & 37.47  & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & MATLAB + MEX & 3.28  \\
%    \midrule
%    \midrule
%    \multirow{12}[24]{*}{Gaussian} & LCSD  & 36.20  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & MATLAB + MEX & 6.45  \\
%\cmidrule{2-16}          & LLRT  & 37.36  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & Pure MATLAB & $>$1000 \\
%\cmidrule{2-16}          & GID   & 37.02  & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & Pure MATLAB  & 38.88  \\
%\cmidrule{2-16}          & MCWNNM & 37.72  & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & Pure MATLAB & 228.16  \\
%\cmidrule{2-16}          & NLH\_CC & 38.49  & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & 46.00  & 35.73  & 40.69  & 42.80  & MATLAB + MEX & 51.86  \\
%\cmidrule{2-16}          & TWSC  & 37.90  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & Pure MATLAB & 368.68  \\
%\cmidrule{2-16}          & CBM3D1 & 37.56  & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & MATLAB + MEX & 0.95  \\
%\cmidrule{2-16}          & CBM3D2 & 37.70  & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & MATLAB + MEX & 4.38  \\
%\cmidrule{2-16}          & M-SVD & 37.62  & 39.27 & 38.56 & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & Pure MATLAB & 4.38  \\
%\cmidrule{2-16}          & CBM3D\_best & 37.95  & 39.68 & 38.81 & 42.08 & 42.89 & 40.48 & 41.25 & 41.16 & 45.81 & 36.66  & 40.89  & 43.14  & Pure MATLAB & 75.88  \\
%\cmidrule{2-16}          & 4DHOSVD1 & 37.51  & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & Pure MATLAB & 86.69  \\
%\cmidrule{2-16}          & CMSt-SVD & 37.95  & 39.75 & 38.82 & 41.99  & 42.75  & 40.08  & 40.84  & 40.53  & 45.89  & 36.40  & 40.85  & 42.68  & MATLAB + MEX & 6.18  \\
%    \bottomrule
%    \end{tabular}}%
%  \label{Table_color_all_psnr}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Average PSNR values and computational time of compared methods on CC15, Xu-100 and Kong-Image datasets. The average computational time is based on images of size $512 \times 512$. The best results are black bolded.}
    \scalebox{0.96}{
    \renewcommand{\arraystretch}{0.69}
    \begin{tabular}{cccccccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset}                                                                  & \multirow{2}[4]{*}{Implementation} & \multirow{2}[4]{*}{Time (s)} \\
\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO& FUJIFILM &       &  \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 33.41 & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & MATLAB + MEX & 1.99  \\
    \midrule
    \multirow{12}[24]{*}{\shortstack[l]{Deep \\ Network}} & FFDNet & 37.67  & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & MATLAB + MEX & 3.58  \\
\cmidrule{2-16}          & CBDNet & 36.36  & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & Python + GPU & 0.32  \\
\cmidrule{2-16}          & DeepBoosting & 38.38  & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & Python + GPU & 0.18  \\
\cmidrule{2-16}          & DIDN  & 36.04  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & Python + GPU & 0.98  \\
\cmidrule{2-16}          & FCCF  & \textbf{39.04} & \textbf{40.89} & \textbf{38.85} & \textbf{41.91} & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.67} & \textbf{40.93} & 42.78  & MATLAB + MEX & 49.98  \\
\cmidrule{2-16}          & NLNet & 37.56  & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & MATLAB + MEX & 5.69  \\
\cmidrule{2-16}          & Unet  & 36.95  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & Python + GPU & 0.21  \\
\cmidrule{2-16}          & VDNet & 35.86  & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & Python + GPU & 1.29  \\
\cmidrule{2-16}          & AINDNet & 35.88  & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & Python + GPU & 0.98  \\
\cmidrule{2-16}          & CycleISP & 35.40  & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & Python + GPU & 0.38  \\
\cmidrule{2-16}          & SADNet & 37.80  & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & Python + GPU & 0.33  \\
\cmidrule{2-16}          & DnCNN & 37.47  & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & MATLAB + MEX & 3.28  \\
    \midrule
    \midrule
    \multirow{12}[24]{*}{\shortstack[l]{Traditional \\ Denoiser}} & LSCD  & 36.20  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & MATLAB + MEX & 6.45  \\
\cmidrule{2-16}          & LLRT  & 37.36  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & Pure MATLAB & $>$1000 \\
\cmidrule{2-16}          & GID   & 37.02  & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & Pure MATLAB & 38.88  \\
\cmidrule{2-16}          & MCWNNM & 37.72  & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & Pure MATLAB & 228.16  \\
\cmidrule{2-16}          & NLH\_CC & 38.49  & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & \textbf{46.00 } & 35.73  & 40.69  & 42.80  & MATLAB + MEX & 51.86  \\
\cmidrule{2-16}          & TWSC  & 37.90  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & Pure MATLAB & 368.68  \\
\cmidrule{2-16}          & CBM3D1 & 37.56  & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & MATLAB + MEX & 0.95  \\
\cmidrule{2-16}          & CBM3D2 & 37.70  & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & MATLAB + MEX & 4.38  \\
\cmidrule{2-16}          & M-SVD & 37.62  & 39.27 & 38.56 & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & Pure MATLAB & 4.38  \\
\cmidrule{2-16}          & CBM3D\_best & 37.95  & 39.68 & \textbf{38.81} & \textbf{42.08} & 42.89 & \textbf{40.48} & \textbf{41.25} & \textbf{41.16} & \textbf{45.81} & \textbf{36.66} & \textbf{40.89} & \textbf{43.14} & MATLAB + mex & 75.88  \\
\cmidrule{2-16}          & 4DHOSVD1 & 37.51  & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & Pure MATLAB & 86.69  \\
\cmidrule{2-16}          & CMSt-SVD & 37.95  & 39.75 & \textbf{38.82} & \textbf{41.99} & 42.75  & 40.08  & 40.84  & 40.53  & \textbf{45.89} & 36.40  & \textbf{40.85} & 42.68  & MATLAB + MEX & 6.18  \\
    \bottomrule
    \end{tabular}}%
  \label{Table_color_all_psnr}%
\end{table*}%



==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_color_all_ssim.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Add caption}
%    \begin{tabular}{c|ccccccccccccc}
%    \multicolumn{2}{c}{\multirow{2}[3]{*}{Method}} & \multicolumn{12}{c}{Dataset} \\
%\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI \\
%    \midrule
%    \multicolumn{2}{c}{Noisy} & 0.8476 & 0.8712 & 0.9125 & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251 & 0.9356  & 0.9307  \\
%    \midrule
%    \multirow{12}[24]{*}{Deep Network} & FFD-Net & 0.9563 & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  \\
%\cmidrule{2-14}          & CBDNet & 0.9294 & 0.9482 & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  \\
%\cmidrule{2-14}          & DeepBoosting & 0.9644 & 0.9811 & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  \\
%\cmidrule{2-14}          & DIDN  & 0.9456 & N/A   & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  \\
%\cmidrule{2-14}          & FCCF  & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & 0.9794  & \textbf{0.9852 } & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640 } & \textbf{0.9747 } & 0.9782  \\
%\cmidrule{2-14}          & NLNet & 0.9554 & 0.9744 & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  \\
%\cmidrule{2-14}          & Unet  & 0.9425 & 0.9708 & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  \\
%\cmidrule{2-14}          & VDNet & 0.9454 & N/A   & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  \\
%\cmidrule{2-14}          & AINDNet & 0.9113 & 0.9708 & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  \\
%\cmidrule{2-14}          & CycleISP & 0.9158 & 0.9393 & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  \\
%\cmidrule{2-14}          & SADNet & 0.9521 & N/A   & 0.9725  & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  \\
%\cmidrule{2-14}          & DnCNN & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  \\
%    \midrule
%    \midrule
%    \multirow{12}[24]{*}{Gaussian Denoiser} & LCSD  & 0.9339 & 0.9626 & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  \\
%\cmidrule{2-14}          & LLRT  & 0.9559 & 0.9636 & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  \\
%\cmidrule{2-14}          & GID   & 0.9459 & 0.9633 & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  \\
%\cmidrule{2-14}          & MCWNNM & 0.9568 & 0.9698 & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  \\
%\cmidrule{2-14}          & NLH\_CC & 0.9647 & 0.9759 & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905 } & 0.9552  & 0.9740  & 0.9776  \\
%\cmidrule{2-14}          & TWSC  & 0.9592 & 0.9759 & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  \\
%\cmidrule{2-14}          & CBM3D1 & 0.9562 & 0.9729 & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  \\
%\cmidrule{2-14}          & CBM3D2 & 0.9572 & 0.974 & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  \\
%\cmidrule{2-14}          & M-SVD & 0.9542 & 0.9705 & 0.9671  & 0.9788  & 0.9823  & 0.9671  & 0.9680  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  \\
%\cmidrule{2-14}          & CBM3D\_best & 0.9621 & 0.9775 & \textbf{0.9712 } & \textbf{0.9808 } & \textbf{0.9851 } & \textbf{0.9741 } & \textbf{0.9758 } & \textbf{0.9783 } & \textbf{0.9904 } & \textbf{0.9640 } & 0.9742  & \textbf{0.9805 } \\
%\cmidrule{2-14}          & 4DHOSVD1 & 0.9559 & 0.9729 & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  \\
%\cmidrule{2-14}          & CMSt-SVD & 0.9588 & 0.9756 & 0.9694  & 0.9794  & 0.9840  & 0.9674  & 0.9668  & 0.9674  & \textbf{0.9903 } & 0.9616  & \textbf{0.9743 } & 0.9770  \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_color_all_ssim}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
\tiny
  \centering
    \caption{Average SSIM values of compared methods on CC15, Xu-100 and Kong-Image datasets. The best results are black bolded.}
    \renewcommand{\arraystretch}{0.69}
    \begin{tabular}{cccccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset} \\
\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 0.8476 & 0.8712 & 0.9125 & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251 & 0.9356  & 0.9307  \\
    \midrule
    \multirow{12}[24]{*}{Deep Network} & FFDNet & 0.9563 & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  \\
\cmidrule{2-14}          & CBDNet & 0.9294 & 0.9482 & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  \\
\cmidrule{2-14}          & DeepBoosting & 0.9644 & 0.9811 & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  \\
\cmidrule{2-14}          & DIDN  & 0.9456 & N/A   & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  \\
\cmidrule{2-14}          & FCCF  & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & 0.9794  & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640} & \textbf{0.9747} & 0.9782  \\
\cmidrule{2-14}          & NLNet & 0.9554 & 0.9744 & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  \\
\cmidrule{2-14}          & Unet  & 0.9425 & 0.9708 & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  \\
\cmidrule{2-14}          & VDNet & 0.9454 & N/A   & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  \\
\cmidrule{2-14}          & AINDNet & 0.9113 & 0.9708 & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  \\
\cmidrule{2-14}          & CycleISP & 0.9158 & 0.9393 & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  \\
\cmidrule{2-14}          & SADNet & 0.9521 & N/A   & 0.9725  & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  \\
\cmidrule{2-14}          & DnCNN & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  \\
    \midrule
    \midrule
    \multirow{12}[24]{*}{Gaussian Denoiser} & LSCD  & 0.9339 & 0.9626 & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  \\
\cmidrule{2-14}          & LLRT  & 0.9559 & 0.9636 & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  \\
\cmidrule{2-14}          & GID   & 0.9459 & 0.9633 & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  \\
\cmidrule{2-14}          & MCWNNM & 0.9568 & 0.9698 & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  \\
\cmidrule{2-14}          & NLH\_CC & 0.9647 & 0.9759 & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905} & 0.9552  & 0.9740  & 0.9776  \\
\cmidrule{2-14}          & TWSC  & 0.9592 & 0.9759 & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  \\
\cmidrule{2-14}          & CBM3D1 & 0.9562 & 0.9729 & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  \\
\cmidrule{2-14}          & CBM3D2 & 0.9572 & 0.974 & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  \\
\cmidrule{2-14}          & M-SVD & 0.9542 & 0.9705 & 0.9671  & 0.9788  & 0.9823  & 0.9671  & 0.9680  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  \\
\cmidrule{2-14}          & CBM3D\_best & 0.9621 & 0.9775 & \textbf{0.9712} & \textbf{0.9808} & \textbf{0.9851} & \textbf{0.9741} & \textbf{0.9758} & \textbf{0.9783} & \textbf{0.9904} & \textbf{0.9640} & 0.9742  & \textbf{0.9805} \\
\cmidrule{2-14}          & 4DHOSVD1 & 0.9559 & 0.9729 & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  \\
\cmidrule{2-14}          & CMSt-SVD & 0.9588 & 0.9756 & 0.9694  & 0.9794  & 0.9840  & 0.9674  & 0.9668  & 0.9674  & \textbf{0.9903} & 0.9616  & \textbf{0.9743} & 0.9770  \\
    \bottomrule
    \end{tabular}%
  \label{Table_color_all_ssim}%
\end{table*}%


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_color_video_rating.tex <==
%\begin{table}[htbp]
%\vspace{-0.1cm}
%\scriptsize
%  \centering
%  \caption{Human rating results of sequences generated by different methods based on our IOCV dataset. The top two results are bolded.}
%  \scalebox{0.88}{
%  \renewcommand{\arraystretch}{0.89}
%    \begin{tabular}{ccccccc}
%    \multicolumn{7}{c}{Ratings} \\
%    \midrule
%    \# Image & Mean  & Noisy & CVMSt-SVD & VBM4D1 & FastDVDNet & VNLNet \\
%    \midrule
%    1     & \textcolor{blue}{\textbf{9}} & 0     & 1     & 2     & \textcolor{blue}{\textbf{5}} & 3 \\
%    \midrule
%    2     & \textcolor{blue}{\textbf{8}} & 1     & 0     & 4     & \textcolor{blue}{\textbf{7}} & 6 \\
%    \midrule
%    3     & \textcolor{blue}{\textbf{10}} & 0     & 0     & \textcolor{blue}{\textbf{8}} & 3     & 5 \\
%    \midrule
%    4     & \textcolor{blue}{\textbf{8}} & 0     & 0     & 4     & 7     & \textcolor{blue}{\textbf{8}} \\
%    \midrule
%    5     & \textcolor{blue}{\textbf{10}} & 0     & 0     & 4     & 4     & \textcolor{blue}{\textbf{7}} \\
%    \midrule
%    6     & \textcolor{blue}{\textbf{10}} & 0     & 0     & 5     & 6     & \textcolor{blue}{\textbf{7}} \\
%    \midrule
%    7     & \textcolor{blue}{\textbf{10}} & 0     & 0     & 5     & \textcolor{blue}{\textbf{8}} & 5 \\
%    \midrule
%    8     & \textcolor{blue}{\textbf{10}} & 2     & 2     & \textcolor{blue}{\textbf{8}} & 5     & 6 \\
%    \midrule
%    9     & \textcolor{blue}{\textbf{9}} & 0     & 2     & 4     & 2     & \textcolor{blue}{\textbf{7}} \\
%    \midrule
%    10    & 4     & 4     & 4     & 4     & \textcolor{blue}{\textbf{5}}     & \textcolor{blue}{\textbf{8}} \\
%    \midrule
%    Average & \textcolor{blue}{\textbf{8.80}} & 0.70  & 0.90  & 4.80  & 5.20  & \textcolor{blue}{\textbf{6.20}} \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_color_video_rating}%
%\end{table}%


\begin{table}[htbp]
\vspace{-0.1cm}
\scriptsize
  \centering
  \caption{Human rating results of sequences generated by different methods based on our IOCV dataset. The top two results are bolded.}
  \scalebox{0.89}{
  \renewcommand{\arraystretch}{0.909}
    \begin{tabular}{ccccccc}
    \multicolumn{7}{c}{Ratings} \\
    \midrule
    \# Image & Mean  & Noisy & CVMSt-SVD & VBM4D1 & FastDVDNet & VNLNet \\
    \midrule
    1     & {\textbf{9}} & 0     & 1     & 2     & {\textbf{5}} & 3 \\
    \midrule
    2     & {\textbf{8}} & 1     & 0     & 4     & {\textbf{7}} & 6 \\
    \midrule
    3     & {\textbf{10}} & 0     & 0     & {\textbf{8}} & 3     & 5 \\
    \midrule
    4     & {\textbf{8}} & 0     & 0     & 4     & 7     & {\textbf{8}} \\
    \midrule
    5     & {\textbf{10}} & 0     & 0     & 4     & 4     & {\textbf{7}} \\
    \midrule
    6     & {\textbf{10}} & 0     & 0     & 5     & 6     & {\textbf{7}} \\
    \midrule
    7     & {\textbf{10}} & 0     & 0     & 5     & {\textbf{8}} & 5 \\
    \midrule
    8     & {\textbf{10}} & 2     & 2     & {\textbf{8}} & 5     & 6 \\
    \midrule
    9     & {\textbf{9}} & 0     & 2     & 4     & 2     & {\textbf{7}} \\
    \midrule
    10    & 4     & 4     & 4     & 4     & {\textbf{5}}     & {\textbf{8}} \\
    \midrule
    Average & {\textbf{8.80}} & 0.70  & 0.90  & 4.80  & 5.20  & {\textbf{6.20}} \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_color_video_rating}%
\end{table}%





==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_dataset_description.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table}[htbp]
%\tiny
%  \centering
%  \caption{Detailed information of popular multi-dimensional image denoising datasets for synthetic and real-world experiments.}
%    \begin{tabular}{ccccccc}
%    \toprule
%    Type  & Name  & Experiments & GT    & \# Cameras & Image size & \# Images \\
%    \midrule
%    \multirow{8}[16]{*}{Color image} & Kodak & Synthetic & A     & /     & 768 x 512x3 & 24 \\
%\cmidrule{2-7}          & RENOIR & Real-world & A     & 3     & 3684 x 2760x3 & 120 \\
%\cmidrule{2-7}          & CC15  & Real-world & A     & 3     & 512 x 512x3 & 15 \\
%\cmidrule{2-7}          & CC60  & Real-world & A     & 3     & 512 x 512 x 3 & 60 \\
%\cmidrule{2-7}          & Xu-100 & Real-world & A     & 5     & 512 x 512 x 3 & 100 \\
%\cmidrule{2-7}          & DND   & Real-world & NA    & 4     & 512 x 512 x 3 & 1000 \\
%\cmidrule{2-7}          & SIDD  & Real-world & NA    & 5     & 256 x 256 x 3 & 1280 \\
%\cmidrule{2-7}          & Kong-Image & Real-world & A     & 9     & 1024 x 1024 x 3 & 409 \\
%    \midrule
%    \multirow{4}[8]{*}{Color video} & Set8  & Synthetic & A     & /     & 960x 540x 3 x F & 4 \\
%\cmidrule{2-7}          & DAVIS & Synthetic & A     & /     & 854 ?480 x 3 x F & 30 \\
%\cmidrule{2-7}          & CRVD  & Real-world & A     & 1     & 1920 x 1080 x F & 61 \\
%\cmidrule{2-7}          & Kong-Video & Real-world & A     & 2     & 512 x 512 x 3 x F & 39 \\
%    \midrule
%    \multirow{3}[6]{*}{MSI} & CAVE  & Synthetic & A     & 1     & 512 x 512 x 31 & 32 \\
%\cmidrule{2-7}          & ICVL  & Real-world & NA    & 1     & 1392 x 1300 x 31 & 201 \\
%\cmidrule{2-7}          & HHD   & Real-world & NA    & 1     & 1392 x 1040 x 31 & 77 \\
%    \midrule
%    \multirow{2}[4]{*}{MRI} & BrainWeb & Synthetic & A     & /     & 181 x 217 x 181 & 3 \\
%\cmidrule{2-7}          & OAS1  & Real-world & NA    & /     & 256 x 256 x 128 & 2 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_dataset_description}%
%\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table}[htbp]
%\tiny
%  \centering
%  \caption{Information of popular multi-dimensional image denoising datasets for synthetic and real-world experiments. 'GT': ground-truth, 'A': Available, 'N/A': Not-Available, 'F': number of frames.}
%  \scalebox{0.88}{
%   \renewcommand{\arraystretch}{0.69}
%    \begin{tabular}{ccccccc}
%    \toprule
%    Type  & Name  & Experiments & GT    & \# Cameras & Image size & \# Images \\
%    \midrule
%    \multirow{8}[26]{*}{Color image} & Kodak \cite{Kodak} & Synthetic & A     & /     & 768 $\times$ 512 $\times$ 3 & 24 \\
%\cmidrule{2-7}          & RENOIR \cite{anaya2018renoir} & Real-world & A     & 3     & 3684 $\times$  2760 $\times$ 3 & 120 \\
%\cmidrule{2-7}          & Nam-CC15 \cite{nam2016holistic} & Real-world & A     & 3     & 512 $\times$  512 $\times$ 3 & 15 \\
%\cmidrule{2-7}          & Nam-CC60 \cite{nam2016holistic} & Real-world & A     & 3     & 500 $\times$  500 $\times$  3 & 60 \\
%\cmidrule{2-7}          & PolyU \cite{xu2018real}& Real-world & A     & 5     & 512 $\times$  512 $\times$  3 & 100 \\
%\cmidrule{2-7}          & DND   \cite{plotz2017benchmarking} & Real-world & N/A    & 4     & 512 $\times$  512 $\times$  3 & 1000 \\
%\cmidrule{2-7}          & SIDD  \cite{abdelhamed2018high}& Real-world & A    & 5     & 256 $\times$  256 $\times$  3 & 1280 \\
%\cmidrule{2-7}          & High-ISO \cite{yue2019high}  & Real-world & A    & 2     & 512 $\times$  512 $\times$  3 & 90 \\
%\cmidrule{2-7}          & Our IOCI & Real-world & A     & 9     & 1024 $\times$  1024 $\times$  3 & 409 \\
%    \midrule
%    \multirow{4}[12]{*}{Color video} & Set8 \cite{Set8} & Synthetic & A     & /     & 960 $\times$ 540 $\times$ 3 $\times$ F & 4 \\
%\cmidrule{2-7}          & DAVIS \cite{Perazzi2016} & Synthetic & A     & /     & 854 $\times$ 480 $\times$ 3 $\times$ F & 30 \\
%\cmidrule{2-7}          & CRVD \cite{yue2020supervised} & Real-world & A     & 1     & 1920 $\times$ 1080 $\times$ 3 $\times$ F & 61 \\
%\cmidrule{2-7}          & Our IOCV & Real-world & A     & 4     & 512 $\times$  512 $\times$  3 $\times$  F & 39 \\
%    \midrule
%    \multirow{3}[8]{*}{MSI} & CAVE \cite{CAVE_0293}  & Synthetic & A     & 1     & 512 $\times$ 512 $\times$ 31 & 32 \\
%\cmidrule{2-7}          & ICVL \cite{arad_and_ben_shahar_2016_ECCV} & Synthetic & A    & 1     & 1392 $\times$ 1300 $\times$  31 & 201 \\
%\cmidrule{2-7}          & HHD \cite{chakrabarti2011statistics}  & Real-world & N/A    & 1     & 1392 $\times$ 1040 $\times$ 31 & 77 \\
%    \midrule
%    \multirow{2}[4]{*}{MRI} & BrainWeb \cite{cocosco1997brainweb} & Synthetic & A     & /     & 181 $\times$ 217 $\times$ 181 & 3 \\
%\cmidrule{2-7}          & OASIS \cite{marcus2007open}  & Real-world & N/A    & /     & 256 $\times$ 256 $\times$ 128 & 2 \\
%    \bottomrule
%    \end{tabular}
%    }%
%  \label{Table_dataset_description}%
%\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\tiny
  \centering
  \caption{Popular datasets for synthetic and real-world experiments. 'GT': ground-truth, '$\surd$': Available, '-': Not available, 'F': number of frames.}
  \scalebox{0.93}{
    \begin{tabular}{cccccc}
    \toprule
    Applications & Name  & Experiments & GT    & Data size & \# Data \\
    \midrule
    \multicolumn{1}{c}{\multirow{10}[29]{*}{Grayscale/Color Image}} & Standard set \cite{dabov2007image} & Synthetic & $\surd$     & 512 $\times$ 512 / 256$\times$256 & 11 \\
\cmidrule{2-6}          & BSD \cite{MartinFTM01} & Synthetic & $\surd$     & 481 $\times$ 321 $\times$ 3 & 500 \\
\cmidrule{2-6}          & Kodak \cite{Kodak} & Synthetic & $\surd$     & 512 $\times$ 512 $\times$ 3 & 24 \\
\cmidrule{2-6}          & RENOIR \cite{anaya2018renoir} & Real-world & $\surd$     & 3684 $\times$ 2760 $\times$ 3 & 120 \\
\cmidrule{2-6}          & Nam-CC15 \cite{nam2016holistic} & Real-world & $\surd$     & 512 $\times$ 512 $\times$ 3 & 15 \\
\cmidrule{2-6}          & Nam-CC60 \cite{nam2016holistic} & Real-world & $\surd$     & 500 $\times$ 500 $\times$ 3 & 60 \\
\cmidrule{2-6}          & PolyU \cite{xu2018real} & Real-world & $\surd$     & 512 $\times$ 512 $\times$ 3 & 100 \\
\cmidrule{2-6}          & DnD \cite{plotz2017benchmarking} & Real-world & -   & 512 $\times$ 512 $\times$ 3 & 1000 \\
\cmidrule{2-6}          & SIDD \cite{abdelhamed2018high} & Real-world & -   & 256 $\times$ 256 $\times$ 3 & 1280 \\
\cmidrule{2-6}          & HighISO \cite{yue2019high} & Real-world & $\surd$     & 512 $\times$ 512 $\times$ 3 & 100 \\
\cmidrule{2-6}          & Our IOCI & Real-world & $\surd$     & 1024 $\times$ 1024 $\times$ 3 & 848 \\
    \midrule
    \multirow{6}[9]{*}{Video} & Set8 \cite{Set8} & Synthetic & $\surd$     & 960 $\times$ 540 $\times$ 3 $\times$ F & 8 \\
\cmidrule{2-6}          & DAVIS \cite{Perazzi2016} & Synthetic & $\surd$     & 854 $\times$ 480 $\times$ 3 $\times$ F & 30 \\
\cmidrule{2-6}          & CRVD \cite{yue2020supervised} & Real-world & $\surd$     & 1920 $\times$ 1080 $\times$ 3 $\times$ F & 61 \\
\cmidrule{2-6}          & PVDD \cite{xu2022pvdd} & Real-world & -    & - & 200 \\
\cmidrule{2-6}          & Our IOCV & Real-world & $\surd$     & 512 $\times$ 512 $\times$ 3 $\times$ F & 39 \\
    \midrule
    \multirow{6}[12]{*}{MSI/HSI} & CAVE \cite{CAVE_0293} & Synthetic & $\surd$     & 512 $\times$ 512 $\times$ 31 & 32 \\
\cmidrule{2-6}          & ICVL \cite{arad_and_ben_shahar_2016_ECCV} & Synthetic & $\surd$     & 1392 $\times$ 1300 $\times$ 31 & 201 \\
\cmidrule{2-6}          & Indian Pines \cite{PURR1947} & Synthetic & $\surd$     & 145 $\times$ 145 $\times$ 224 & 1 \\
\cmidrule{2-6}          & Urban \cite{PURR1947} & Real-world & -   & 307 $\times$ 307 $\times$ 210 & 1 \\
\cmidrule{2-6}          & HHD \cite{chakrabarti2011statistics} & Real-world & -   & 1392 $\times$ 1040 $\times$ 31 & 77 \\
\cmidrule{2-6}          & Real-HSI \cite{zhang2021hyperspectral} & Real-world & $\surd$     & 696 $\times$ 520 $\times$ 34 & 59 \\
    \midrule
    \multirow{3}[6]{*}{MRI} & BrainWeb \cite{cocosco1997brainweb} & Synthetic & $\surd$     & 181 $\times$ 217 $\times$ 181 & 3 \\
\cmidrule{2-6}          & fastMRI \cite{zbontar2018fastmri} & Synthetic & $\surd$     & 320 $\times$ 320 $\times$ 40 & 50 \\
\cmidrule{2-6}          & OASIS \cite{marcus2007open} & Real-world & -   & 256 $\times$ 256 $\times$ 128 & 2 \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_dataset_description}%
\end{table}%



==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_msi_psnr_ssim.tex <==
%% Table generated by Excel2LaTeX from sheet 'Origin'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Quantitative results comparison under i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$ on CAVE dataset.}
%    \begin{tabular}{cccccccccccccccccc}
%    \toprule
%    \multirow{2}[4]{*}{Methods} & \multicolumn{4}{c}{$\sigma$ = 10} & \multicolumn{4}{c}{$\sigma$ = 30} & \multicolumn{4}{c}{$\sigma$ = 50} & \multicolumn{4}{c}{$\sigma$ = 100} & \multirow{2}[4]{*}{Time (m)} \\
%\cmidrule{2-17}          & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   &  \\
%    \midrule
%    Noisy & 28.13  & 0.4371 & 236.40  & 0.7199 & 18.59  & 0.1069 & 676.01  & 1.0085 & 14.15 & 0.0475  & 1126.7 & 1.1461 & 8.13  & 0.0136  & 2253.4 & 1.3074  & / \\
%    \midrule
%    PARAFAC & 35.39  & 0.8759 & 108.78  & 0.2363 & 33.65  & 0.8294 & 125.13  & 0.3291 & 31.52 & 0.7393  & 154.19 & 0.4351 & 27.13  & 0.4637  & 250.68 & 0.6681  & 3.9 \\
%    \midrule
%    LRTA  & 41.36  & 0.9499 & 49.53  & 0.1718 & 36.06  & 0.8775 & 90.50  & 0.2446 & 33.52 & 0.8201  & 121.15 & 0.2897 & 30.06  & 0.7138  & 180.03 & 0.3649  & \textbf{0.5} \\
%    \midrule
%    LRMR  & 39.27  & 0.9094 & 64.81  & 0.3343 & 31.36  & 0.6451 & 157.65  & 0.6021 & 26.67 & 0.4000  & 264.28 & 0.7534 & 26.67  & 0.1850  & 469.26 & 0.9306  & / \\
%    \midrule
%    LLRGTV & 38.96  & 0.9384 & 71.54  & 0.2292 & 33.56  & 0.7862 & 122.45  & 0.4756 & 30.33 & 0.6375  & 172.22 & 0.6386 & 25.62  & 0.3917  & 288.78 & 0.8593  & 3.8 \\
%    \midrule
%    4DHOSVD1 & 45.43  & 0.9811 & 30.83  & 0.1084 & 39.78  & 0.9336 & 59.12  & 0.2272 & 36.82 & 0.8722  & 83.36 & 0.3385 & 32.66  & 0.7307  & 134.34 & 0.5599  & 4.9 \\
%    \midrule
%    BM4D1 & 42.76  & 0.9716  & 42.19  & 0.1585  & 37.13  & 0.9235  & 82.33  & 0.2910  & 34.55  & 0.8803  & 109.43  & 0.3591  & 31.17  & 0.7763  & 158.83  & 0.4751  & 2.1 \\
%    \midrule
%    BM4D2 & 44.61  & 0.9784 & 33.32  & 0.1289 & 38.80  & 0.9283 & 65.23  & 0.2579 & 35.90  & 0.8685  & 91.19 & 0.3557 & 31.84  & 0.7197  & 144.91 & 0.5160  & 8.8 \\
%    \midrule
%    TDL   & 44.41  & 0.9797 & 34.32  & 0.1048 & 39.07  & 0.9493 & 63.18  & 0.1493 & 36.46 & 0.9171  & 85.24 & 0.2008 & 32.92  & 0.8284  & 128.15 & 0.3132  & 0.9 \\
%    \midrule
%    ISTReg & 45.77  & 0.9802 & 30.53  & 0.1086 & 40.51  & 0.9488 & 53.05  & 0.1374 & 37.75 & 0.9271  & 70.16 & 0.1619 & 33.01  & 0.8648  & 120.77 & 0.2376  & / \\
%    \midrule
%    FastHyDe & 42.87  & 0.9763 & 42.90  & 0.1398 & 37.22  & 0.9151 & 81.44  & 0.3123 & 34.56 & 0.8471  & 108.75 & 0.4395 & 30.62  & 0.6717  & 168.92 & 0.6096  & 0.8 \\
%    \midrule
%    HSI-DeCNN & 41.40  & 0.9624 & 52.04  & 0.1523 & 37.57  & 0.9247  & 78.28 & 0.1959  & 35.49  & 0.8947  & 98.54 & 0.2141  & 32.51  & 0.8309  & 136.16 & 0.2748  & 56.8 \\
%    \midrule
%    LLRT  & \textbf{46.60} & \textbf{0.9868} & \textbf{26.75} & \textbf{0.0842} & \textbf{41.49} & \textbf{0.9681} & \textbf{48.50} & \textbf{0.1221} & \textbf{38.65} & \textbf{0.9482} & 67.56 & \textbf{0.1551} & \textbf{35.39} & \textbf{0.9154} & \textbf{99.37} & \textbf{0.1962} & 43.8 \\
%    \midrule
%    MSt-SVD & 45.20  & 0.9814 & 32.05  & 0.1064 & 40.23  & 0.9530  & 56.26  & 0.1737 & 37.73 & 0.9285  & 75.03 & 0.2231 & 34.20  & 0.8800  & 115.24 & 0.3142  & 1.5 \\
%    \midrule
%    LTDL  & 45.90  & 0.9859  & 29.06  & 0.0925 & 41.20  & 0.9644  & 49.73  & 0.1301 & \textbf{38.63 } & 0.9459  & \textbf{66.68 } & 0.1650  & 34.87  & 0.9015  & 103.65  & 0.2353  & 60.2 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_msi_psnr_ssim}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Origin'
\begin{table*}[ht]
\tiny
  \centering
  \caption{Comparison of quantitative results and computational time (minutes) under i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$ on CAVE dataset.}
  \renewcommand{\arraystretch}{0.918}
    \begin{tabular}{cccccccccccccccccc}
    \toprule
    \multirow{2}[4]{*}{Methods} & \multicolumn{4}{c}{$\sigma$ = 10} & \multicolumn{4}{c}{$\sigma$ = 30} & \multicolumn{4}{c}{$\sigma$ = 50} & \multicolumn{4}{c}{$\sigma$ = 100} & \multirow{2}[4]{*}{Time (m)} \\
\cmidrule{2-17}          & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   &  \\
    \midrule
    Noisy & 28.13  & 0.4371 & 236.40  & 0.7199 & 18.59  & 0.1069 & 676.01  & 1.0085 & 14.15 & 0.0475  & 1126.7 & 1.1461 & 8.13  & 0.0136  & 2253.4 & 1.3074  & / \\
    \midrule
    PARAFAC & 35.39  & 0.8759 & 108.78  & 0.2363 & 33.65  & 0.8294 & 125.13  & 0.3291 & 31.52 & 0.7393  & 154.19 & 0.4351 & 27.13  & 0.4637  & 250.68 & 0.6681  & 3.9 \\
    \midrule
    LRTA  & 41.36  & 0.9499 & 49.53  & 0.1718 & 36.06  & 0.8775 & 90.50  & 0.2446 & 33.52 & 0.8201  & 121.15 & 0.2897 & 30.06  & 0.7138  & 180.03 & 0.3649  & \textbf{0.5} \\
    \midrule
    LRMR  & 39.27  & 0.9094 & 64.81  & 0.3343 & 31.36  & 0.6451 & 157.65  & 0.6021 & 26.67 & 0.4000  & 264.28 & 0.7534 & 26.67  & 0.1850  & 469.26 & 0.9306  & 4.1 \\
    \midrule
    LLRGTV & 38.96  & 0.9384 & 71.54  & 0.2292 & 33.56  & 0.7862 & 122.45  & 0.4756 & 30.33 & 0.6375  & 172.22 & 0.6386 & 25.62  & 0.3917  & 288.78 & 0.8593  & 3.8 \\
    \midrule
    4DHOSVD1 & 45.43  & 0.9811 & 30.83  & 0.1084 & 39.78  & 0.9336 & 59.12  & 0.2272 & 36.82 & 0.8722  & 83.36 & 0.3385 & 32.66  & 0.7307  & 134.34 & 0.5599  & 4.9 \\
    \midrule
    BM4D1 & 42.76  & 0.9716  & 42.19  & 0.1585  & 37.13  & 0.9235  & 82.33  & 0.2910  & 34.55  & 0.8803  & 109.43  & 0.3591  & 31.17  & 0.7763  & 158.83  & 0.4751  & 2.1 \\
    \midrule
    BM4D2 & 44.61  & 0.9784 & 33.32  & 0.1289 & 38.80  & 0.9283 & 65.23  & 0.2579 & 35.90 & 0.8685  & 91.19 & 0.3557 & 31.84  & 0.7197  & 144.91 & 0.5160  & 8.8 \\
    \midrule
    TDL   & 44.41  & 0.9797 & 34.32  & 0.1048 & 39.07  & 0.9493 & 63.18  & 0.1493 & 36.46 & 0.9171  & 85.24 & 0.2008 & 32.92  & 0.8284  & 128.15 & 0.3132  & 0.9 \\
    \midrule
    ITSReg & 45.77  & 0.9802 & 30.53  & 0.1086 & 40.51  & 0.9488 & 53.05  & 0.1374 & 37.75 & 0.9271  & 70.16 & 0.1619 & 33.01  & 0.8648  & 120.77 & 0.2376  & 5.2 \\
    \midrule
    FastHyDe & 42.87  & 0.9763 & 42.90  & 0.1398 & 37.22  & 0.9151 & 81.44  & 0.3123 & 34.56 & 0.8471  & 108.75 & 0.4395 & 30.62  & 0.6717  & 168.92 & 0.6096  & 0.8 \\
    \midrule
    HSI-SDeCNN & 41.40  & 0.9624 & 52.04  & 0.1523 & 37.57  & 0.9247  & 78.28 & 0.1959  & 35.49  & 0.8947  & 98.54 & 0.2141  & 32.51  & 0.8309  & 136.16 & 0.2748  & 0.98 \\
    \midrule
    QRNN3D & 40.36  & 0.9672  & 65.31  & 0.1926  & 38.48  & 0.9496  & 76.21  & 0.2320  & 37.02  & 0.9314  & 87.15  & 0.2741  & 30.33  & 0.7128  & 172.68  & 0.5161  & 0.01  \\
    \midrule
    LLRT  & \textbf{46.60} & 0.9868 & \textbf{26.75} & \textbf{0.0842} & 41.49  & 0.9681 & 48.50 & \textbf{0.1221} & 38.65 & 0.9482  & 67.56 & \textbf{0.1551} & \textbf{35.39} & \textbf{0.9154} & \textbf{99.37} & \textbf{0.1962} & 43.8 \\
    \midrule
    MSt-SVD & 45.20  & 0.9814 & 32.05  & 0.1064 & 40.23  & 0.9530  & 56.26  & 0.1737 & 37.73 & 0.9285  & 75.03 & 0.2231 & 34.20  & 0.8800  & 115.24 & 0.3142  & 1.5 \\
    \midrule
    NGMeet & \textbf{46.58} & \textbf{0.9881} & 27.27  & 0.0853 & \textbf{41.60} & \textbf{0.9692} & \textbf{48.14} & 0.1238 & \textbf{38.88} & \textbf{0.9507} & \textbf{65.64} & 0.1616  & 34.97  & 0.9072  & 101.98 & 0.2506  & 4.6 \\
    \midrule
    LTDL  & 45.90  & 0.9859  & 29.06  & 0.0925 & 41.20  & 0.9644  & 49.73  & 0.1301 & 38.63  & 0.9459  & 66.68  & 0.1650  & 34.87  & 0.9015  & 103.65  & 0.2353  & 60.2 \\
    \bottomrule
    \end{tabular}%
  \label{Table_msi_psnr_ssim}%
\end{table*}%



==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_number_cameras_comparsion.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Changes of the proposed IOCI dataset for real-world image denoising.}
  \scalebox{0.95}{
    \begin{tabular}{cccc}
    \toprule
    Version & Number of camera devices & Number of scenes & Number of images \\
    \midrule
    Previous (TPAMI-2020-11-1630) & 9     & 106   & 289 \\
    \midrule
    Current manuscript & \textbf{13} & \textbf{169} & \textbf{409} \\
    \bottomrule
    \end{tabular}}%
  \label{Table_number_cameras_comparsion}%
\end{table}%


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_number_methods_comparison.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Difference in the number of methods and datasets between previous and current versions.}
    \begin{tabular}{ccc}
    \toprule
    Version & Number of compared methods/models & Number of datasets \\
    \midrule
    Previous (TPAMI-2020-11-1630) & 58    & 8 \\
    \midrule
    Current manuscript & \textbf{96}    & \textbf{18} \\
    \bottomrule
    \end{tabular}%
  \label{Table_number_methods_comparison}%
\end{table}%


==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_supp_SIDD_validation_test.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet2'
%\begin{table*}[htbp]
%  \centering
%  \caption{Add caption}
%    \begin{tabular}{cccccccccccccccccccccc}
%    \toprule
%    \multirow{2}[4]{*}{PSNR} & \multicolumn{6}{c}{\textcolor[rgb]{ 1,  0,  0}{\textbf{Traditional Methods}}} & \multicolumn{15}{c}{\textcolor[rgb]{ 0,  .439,  .753}{\textbf{Deep learning methods}}} \\
%\cmidrule{2-22}          & Bitonic & CBM3D1 & CBM3D2 & CMS-TSVD & NLH\_CC & AINDNet & CBDNet & CycleISP & DANet & DeamNet & DIDN  & InvDN & MIRNet & MPRNet & NAFNet & NBNet & PD-Denoising & PNGAN & Restormer & RIDNet & VDIR \\
%    \midrule
%    Validation &       & 35.07  & 34.80  & 34.26  &       & 39.08  & 38.35  & 39.52  & 39.54  & 39.47  & 40.04  & 39.32  & 39.68  & 39.71  & 40.21  & 39.76  & 33.99  & 40.07  & 39.93  & 38.78  & 39.37  \\
%    \midrule
%    Test  &       & 35.00  & 34.74  & 34.38  &       & 39.08  & 33.26  & 39.35  & 39.78  & 39.35  & 39.78  & 39.28  & 39.55  & 39.57  & 40.15  & 39.64  & 33.99  & 39.81  & 39.79  & 38.70  & 39.26 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_supp_SIDD_validation_test}%
%\end{table*}%
%

%% Table generated by Excel2LaTeX from sheet 'Sheet2'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Add caption}
%  \scalebox{0.83}{
%    \begin{tabular}{ccccccccccccccccccccc}
%    \toprule
%    \multirow{2}[4]{*}{PSNR} & \multicolumn{4}{c}{Traditional denoisers} & \multicolumn{16}{c}{DNN methods} \\
%\cmidrule{2-21}          & Bitonic & CBM3D2 & CMSt-SVD & NLH\_CC & AINDNet & CBDNet & CycleISP & DANet & DeamNet & DIDN  & InvDN & MIRNet & MPRNet & NAFNet & NBNet & PD-Denoising & PNGAN & Restormer & RIDNet & VDIR \\
%    \midrule
%    Validation &       & 34.80  & 34.26  &       & 39.08  & 38.35  & 39.52  & 39.54  & 39.47  & 40.04  & 39.32  & 39.68  & 39.71  & 40.21  & 39.76  & 33.99  & 40.07  & 39.93  & 38.78  & 39.37  \\
%    \midrule
%    Test  &       & 34.74  & 34.38  &       & 39.08  & 33.26  & 39.35  & 39.78  & 39.35  & 39.78  & 39.28  & 39.55  & 39.57  & 40.15  & 39.64  & 33.99  & 39.81  & 39.79  & 38.70  & 39.26 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_supp_SIDD_validation_test}}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Average PSNR value of compared methods on the validation and test data of the SIDD datasets.}
  \scalebox{0.908}{
    \begin{tabular}{ccccccccccccccccccc}
    \toprule
    \multirow{2}[4]{*}{PSNR} & \multicolumn{4}{c|}{Traditional denoisers} & \multicolumn{14}{c}{DNN methods} \\
\cmidrule{2-19}          & Bitonic & CBM3D2 & CMSt-SVD & NLHCC & AINDNet & CycleISP & DANet & DeamNet & DIDN  & InvDN & MIRNet & MPRNet & NAFNet & NBNet & PNGAN & Restormer & RIDNet & VDIR \\
    \midrule
    Validation & 36.46  & 34.80  & 34.26  & 35.18  & 39.06  & 39.52  & 39.54  & 39.47  & 40.04  & 39.32  & 39.68  & 39.71  & 40.21  & 39.76  & 40.07  & 39.93  & 38.78  & 39.37  \\
    \midrule
    Test  & 36.68  & 34.74  & 34.38  & 35.31  & 39.08  & 39.35  & 39.78  & 39.35  & 39.78  & 39.28  & 39.55  & 39.57  & 40.15  & 39.64  & 39.81  & 40.02  & 38.70  & 39.26 \\
    \midrule
    Difference & 0.22  & 0.06  & 0.12  & 0.13  & 0.02  & 0.17  & 0.24  & 0.12  & 0.26  & 0.04  & 0.13  & 0.14  & 0.06  & 0.12  & 0.26  & 0.14  & 0.08  & 0.11  \\
    \bottomrule
    \end{tabular}%
  \label{Table_supp_SIDD_validation_test}}%
\end{table*}%





==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_traditional_method.tex <==
%\begin{table*}[htbp]
%\scriptsize
%\centering
%\caption{Related traditional denoisers for multi-dimensional image data with different noise modeling techniques and applications. 'CI': color image, 'CV': color video, 'MSI': multispectral imaging, 'HSI': hyperspectral imaging, 'MRI': magnetic resonance imaging.}
%\scalebox{0.869}{
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%\textbf{Category}                      & \textbf{Representation}           & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                     \\
%\hline
%\multirow{41}{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{26}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color,othman2006noise}           & AWGN                        & CI, MSI, HSI      & Adaptive wavelet thresholding methods    \\
%\cline{3-6}
%                              &                          & DCT \cite{yaroslavsky1996local, foi2007pointwise}           & AWGN                        & CI                & Image denoising with discrete cosine transform (DCT)   \\
%\cline{3-6}
%                              &                          & NLM \cite{buades2005review, dai2013multichannel}           & AWGN                        & CI                & nonlocal means (NLM) algorithm with Gaussian kernels                           \\
%\cline{3-6}
%                              &                          & K-SVD \cite{elad2006image, mairal2007sparse, fu2015adaptive}           & AWGN                        & CI, MSI               & Over-complete dictionary learning and sparse coding                \\
%\cline{3-6}
%                              &                          & TCVD \cite{liu2010high}         & AWGN                        & CV                & Combination of robust optical flow with NLM                   \\
%\cline{3-6}
%                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                        & CI, MRI           & Applications of SVD transform                             \\
%\cline{3-6}
%                              &                          & EPLL \cite{zoran2011learning, hurault2018epll}           & AWGN                        & CI                & A Bayesian method for whole image restoration                          \\
%\cline{3-6}
%                              &                          & LRMR \cite{zhang2013hyperspectral}         & AWGN                        & MRI               & A low-rank matrix decomposition model                         \\
%\cline{3-6}
%                              &                          & GID \cite{xu2018external}          & AWGN                        & CI                & External data guided and internal prior learning              \\
%\cline{3-6}
%                              &                          & SPTWO \cite{buades2016patch}         & AWGN                        & CV                & NLPCA with optical flow estimation                            \\
%\cline{3-6}
%                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                        & CI, MSI, HSI      & Spectral component decomposition with line feature        \\
%%\cline{3-6}
%%                              &                          & Global-Search \cite{ehret2017global} & AWGN                        & CV                & Efficient approximate global patch search                     \\
%\cline{3-6}
%                              &                          & MCWNNM \cite{gu2014weighted, xu2017multi}        & AWGN                        & CI                & Extension of WNNM to color images                             \\
%\cline{3-6}
%                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                        & CI              & A trilateral weighted sparse coding scheme                   \\
%\cline{3-6}
%                              &                          & VNLB \cite{arias2018video}         & AWGN                        & CV                & A patch-based Bayesian model for video denoising                   \\
%\cline{3-6}
%                              &                          & NLH \cite{hou2020nlh}      & AWGN                        & CI                & Nonlocal pixel similarity with Haar transform                 \\
%\cline{3-6}
%                              &                          & AMF \cite{chan2005salt}          & Impulsive                   & CI                & Impulsive noise removal by adaptive median filter             \\
%%\cline{3-6}
%%                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                   & CI                & Impulsive noise removal by iterative adaptive fuzzy filter    \\
%\cline{3-6}
%                              &                          & NoiseClinic \cite{lebrun2015multiscale}         & AWGN and Realistic                   & CI                & A multiscale blind Bayes denoising algorithm    \\
%\cline{3-6}
%                              &                          & LSM-NLR \cite{huang2017mixed}      & AWGN, Poisson and Impulsive & CV                & Low-rank with laplacian scale mixture modeling                \\
%\cline{3-6}
%                              &                          & FastHyde \cite{zhuang2018fast}     & AWGN and Poisson            & MSI, HSI          & Low-rank and sparse representation                            \\
%\cline{3-6}
%                              &                          & NMoG \cite{chen2017denoising}         & AWGN, Stripe and Impulsive  & MSI, HSI          & Low-rank matrix model with non i.i.d Gaussian noise           \\
%\cline{3-6}
%                              &                          & ODCT \cite{manjon2012new}          & AWGN and Rician             & MRI               & A 3D DCT implementation                                       \\
%\cline{3-6}
%                              &                          & ONLM \cite{coupe2008optimized}         & AWGN and Rician             & MRI               & An optimized blockwise NLM Filter                             \\
%\cline{3-6}
%                              &                          & ANLM \cite{manjon2010adaptive}       & AWGN and Rician             & MRI               & Adaptive NLM with spatially varying noise levels              \\
%\cline{3-6}
%                              &                          & RLMMSE \cite{aja2008noise}       & Rician                      & MRI               & A novel linear minimum mean square error estimator    \\
%\cline{3-6}
%                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician             & MRI               & A rotationally invariant version of the NLM filter            \\
%\cline{3-6}
%                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician             & MRI               & A two stage filter based on NLPCA and PRI-NLM                 \\
%\cline{2-6}
%                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                        & CI, CV                & BM3D with oppenent and YUV color mode transforms              \\
%%\cline{3-6}
%%                              &                          & CVBM3D \cite{dabov2007video}        & AWGN                        & CV                & Extention of CBM3D to color videos                            \\
%\cline{3-6}
%                              &                          & LRTA \cite{renard2008denoising}         & AWGN                        & MSI, HSI          & A low Tucker rank tensor decomposition  model                 \\
%\cline{3-6}
%                              &                          & PARAFAC \cite{liu2012denoising}       & AWGN                        & MSI               & A rank-one candecomp/parafac (CP) model                             \\
%\cline{3-6}
%                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                        & MSI, HSI, MRI     & Extention of BM3D to MSI and MRI using 3D patch               \\
%\cline{3-6}
%                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                        & CV                & Extention of BM3D to color videos using 3D patch              \\
%\cline{3-6}
%                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising, zhang2017denoise}      & AWGN                        & CI, MSI, HSI, MRI & Applications of 4DHOSVD transform                             \\
%\cline{3-6}
%                              &                          & TDL \cite{peng2014decomposable}           & AWGN                        & MSI, HSI          & A Tucker based tensor dictionary learning algorithm           \\
%\cline{3-6}
%                              &                          & KTSVD \cite{Zhang2015KTSVD}         & AWGN                        & MSI, HSI          & A t-SVD based tensor dictionary learning algorithm            \\
%\cline{3-6}
%                              &                          & LRTV \cite{he2015total}         & AWGN                        & MSI, HSI          & Low-rank model with total variation (TV) regularization            \\
%\cline{3-6}
%                              &                          & ITSReg \cite{xie2016multispectral}        & AWGN                        & MSI, HSI          & Intrinsic Tensor Sparsity Regularization                      \\
%\cline{3-6}
%                              &                          & LLRT \cite{chang2017hyper}        & AWGN                        & CI, MSI          & low-rank tensor with hyper-laplacian regularization                      \\
%\cline{3-6}
%                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                        & MSI, HSI          & Low Tucker rank decomposition with total variation            \\
%\cline{3-6}
%                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                        & CI                & A weighted rank-one CP decomposition model                    \\
%\cline{3-6}
%                              &                          & ILR-HOSVD \cite{lv2019denoising}    & AWGN                        & MRI               & A recursive low Tucker rank model with rank estimation        \\
%\cline{3-6}
%                              &                          & MSt-SVD \cite{kong2017new, kong2019color}       & AWGN                        & CI, MRI, MSI, HSI & An efficient one-step t-SVD implementation  \\
%\cline{3-6}
%                              &                          & NGMeet \cite{he2019non}       & AWGN                        & MSI, HSI          & Low-rank tensor model with iterative regularization           \\
%\cline{3-6}
%                              &                          & LTDL \cite{gong2020low}         & AWGN                        & MSI, HSI          & A low-rank tensor dictionary learning method                  \\
%\cline{3-6}
%                              &                          & NLTA-LSM \cite{dong2015low}      & AWGN and Poisson            & MSI, HSI, MRI     & Low Tucker rank with laplacian scale mixture modeling         \\
%\hline
%\end{tabular}
%}
%\label{Table_traditional_method}
%\end{table*}


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Representative traditional denoisers with different noise modeling techniques and representation.}
  \scalebox{0.859}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Category & Representation & Methods & year  & Noise modeling & Key words \\
    \hline
    \multirow{56}{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{16}[56]{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color}  & 1995  & AWGN  & Adaptive wavelet thresholding methods \\
\cline{3-6}          &       & DCT \cite{yaroslavsky1996local, foi2007pointwise} & 1999  & AWGN  & Image denoising with discrete cosine transform (DCT) \\
\cline{3-6}          &       & NLM \cite{buades2005review, dai2013multichannel} & 2005  & AWGN  & nonlocal means (NLM) algorithm with Gaussian kernels \\
\cline{3-6}          &       & AMF \cite{chan2005salt} & 2005  & Impulse & Impulsive noise removal by adaptive median filter \\
\cline{3-6}          &       & K-SVD \cite{elad2006image} & 2006  & AWGN  & Over-complete dictionary learning and sparse coding \\
\cline{3-6}          &       & ONLM \cite{coupe2008optimized} & 2008  & AWGN and Rician & An optimized blockwise NLM Filter \\
\cline{3-6}          &       & ROLMMSE \cite{aja2008noise} & 2010  & Rician & A novel linear minimum mean square error estimator \\
\cline{3-6}          &       & AONLM \cite{manjon2010adaptive} & 2010  & AWGN and Rician & Adaptive NLM with spatially varying noise levels \\
\cline{3-6}          &       & TCVD \cite{liu2010high} & 2010  & AWGN  & Combination of robust optical flow with NLM \\
\cline{3-6}          &       & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d} & 2010  & AWGN  & Applications of SVD transform \\
\cline{3-6}          &       & EPLL \cite{zoran2011learning} & 2011  & AWGN  & A Bayesian method for whole image restoration \\
\cline{3-6}          &       & PRI-NLM \cite{manjon2012new} & 2012  & AWGN and Rician & A rotationally invariant version of the NLM filter \\
\cline{3-6}          &       & ODCT \cite{manjon2012new} & 2012  & AWGN and Rician & A 3D DCT implementation \\
%\cline{3-6}          &       & IAFF \cite{ahmed2013removal} & 2013  & Impulsive & Impulsive noise removal by iterative adaptive fuzzy filter \\
\cline{3-6}          &       & LRMR \cite{zhang2013hyperspectral} & 2013  & AWGN  & A low-rank matrix decomposition model \\
\cline{3-6}          &       & MCWNNM \cite{gu2014weighted, xu2017multi} & 2014  & AWGN  & Extension of WNNM to color images \\
\cline{3-6}          &       & PRI-NLPCA \cite{manjon2015mri} & 2015  & AWGN and Rician & A two stage filter based on NLPCA and PRI-NLM \\
\cline{3-6}          &       & NoiseClinic \cite{lebrun2015multiscale} & 2015  & AWGN and Realistic & A multiscale blind Bayes denoising algorithm \\
\cline{3-6}          &       & SPTWO \cite{buades2016patch} & 2016  & AWGN  & NLPCA with optical flow estimation \\
\cline{3-6}          &       & LSCD \cite{rizkinia2016local} & 2016  & AWGN  & Spectral component decomposition with line feature \\
\cline{3-6}          &       & Global-Search \cite{ehret2017global} & 2017  & AWGN  & Efficient approximate global patch search \\
\cline{3-6}          &       & LSM-NLR \cite{huang2017mixed} & 2017  & AWGN, Poisson and Impulse & Low-rank with laplacian scale mixture modeling \\
\cline{3-6}          &       & NMoG \cite{chen2017denoising} & 2017  & AWGN, Stripe and Impulse & Low-rank matrix model with non i.i.d Gaussian noise \\
\cline{3-6}          &       & FastHyde \cite{zhuang2018fast} & 2018  & AWGN and Poisson & Low-rank and sparse representation \\
\cline{3-6}          &       & TWSC \cite{xu2018trilateral} & 2018  & AWGN  & A trilateral weighted sparse coding scheme \\
\cline{3-6}          &       & VNLB \cite{arias2018video} & 2018  & AWGN  & A patch-based Bayesian model for video denoising \\
\cline{3-6}          &       & GID \cite{xu2018external} & 2018  & AWGN  & External data guided and internal prior learning \\
\cline{3-6}          &       & NLH \cite{hou2020nlh} & 2020  & AWGN  & Nonlocal pixel similarity with Haar transform \\
\cline{3-6}          &       & Bitonic \cite{treece2022real} & 2022  & AWGN and Realistic  & A non-learning bitonic filter with locally adaptive masks \\
\cline{2-6}          & \multirow{12}[38]{*}{Tensor} & CBM3D \cite{dabov2007color} & 2007  & AWGN  & BM3D with oppenent and YUV color mode transforms \\
%\cline{3-6}          &       & CVBM3D \cite{dabov2007video} & 2007  & AWGN  & Extention of CBM3D to color videos \\
\cline{3-6}          &       & LRTA \cite{renard2008denoising} & 2008  & AWGN  & A low Tucker rank tensor decomposition  model \\
\cline{3-6}          &       & PARAFAC \cite{liu2012denoising} & 2012  & AWGN  & A rank-one candecomp/parafac (CP) model \\
\cline{3-6}          &       & BM4D \cite{maggioni2012nonlocal} & 2012  & AWGN  & An extention of BM3D to MSI and MRI using 3D patch \\
%\cline{3-6}          &       & VBM4D \cite{maggioni2012video} & 2012  & AWGN  & An extention of BM3D to color videos using 3D patch \\
\cline{3-6}          &       & 4DHOSVD \cite{rajwade2012image, zhang2015denoising, zhang2017denoise} & 2012  & AWGN  & Applications of 4DHOSVD transform \\
\cline{3-6}          &       & TDL \cite{peng2014decomposable} & 2014  & AWGN  & A Tucker based tensor dictionary learning algorithm \\
\cline{3-6}          &       & KTSVD \cite{Zhang2015KTSVD} & 2015  & AWGN  & A t-SVD based tensor dictionary learning algorithm \\
\cline{3-6}          &       & LRTV \cite{he2015total} & 2015  & AWGN  & Low-rank model with total variation (TV) regularization \\
\cline{3-6}          &       & NLTA-LSM \cite{dong2015low} & 2015  & AWGN and Poisson & Low Tucker rank with laplacian scale mixture modeling \\
\cline{3-6}          &       & ITSReg \cite{xie2016multispectral} & 2016  & AWGN  & Intrinsic Tensor Sparsity Regularization \\
\cline{3-6}          &       & LLRT \cite{chang2017hyper} & 2017  & AWGN  & low-rank tensor with hyper-laplacian regularization \\
\cline{3-6}          &       & MSt-SVD \cite{kong2017new, kong2019color} & 2017  & AWGN  & An efficient one-step t-SVD implementation \\
\cline{3-6}          &       & LLRGTV \cite{He2018LLRGTV} & 2018  & AWGN  & Low Tucker rank decomposition with total variation \\
\cline{3-6}          &       & WTR1 \cite{wu2018weighted} & 2019  & AWGN  & A weighted rank-one CP decomposition model \\
\cline{3-6}          &       & ILR-HOSVD \cite{lv2019denoising} & 2019  & AWGN  & A recursive low Tucker rank model with rank estimation \\
\cline{3-6}          &       & NGMeet \cite{he2019non} & 2019  & AWGN  & Low-rank tensor model with iterative regularization \\
\cline{3-6}          &       & LTDL \cite{gong2020low} & 2020  & AWGN  & A low-rank tensor dictionary learning method \\
\cline{3-6}          &       & OLRT \cite{chang2020hyperspectral} & 2020  & AWGN and Stripe  & A low-rank tensor model with sparse error component \\
\cline{3-6}          &       & GLF \cite{zhuang2021hyperspectral} & 2021  & AWGN  & A low-rank tensor model with global and local factorization \\
\cline{3-6}          &       & HLTA \cite{xie2022novel} & 2022  & AWGN, Stripe and Impulse  & A low-rank tensor model for denoising and completion \\
\cline{3-6}          &       & TRSTR \cite{zhang2023hyperspectral} & 2023  & AWGN, Stripe and Impulse  & A low-rank tensor-ring decomposition model \\
    \hline
    \end{tabular}}%
  \label{Table_traditional_method}%
\end{table*}%





==> A Comparison of Image Denoising Methods_submitted_to_arxiv_2023_05_09/Table_video_psnr_ssim.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet4'
%\begin{table}[htbp]
%\scriptsize
%  \centering
%  \caption{Add caption}
%  \scalebox{0.92}{
%    \begin{tabular}{ccccccc}
%    \toprule
%    \multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{Metric} & \multicolumn{5}{c}{Method} \\
%\cmidrule{3-7}          &       & Noisy & Fastdvdnet & Vnlnet & CVMStSVD & VBM4D \\
%    \midrule
%    \multirow{2}[4]{*}{HUAWEI\_BC} & PSNR  & 38.11  & 41.26  & 41.35  & 40.80  & 41.19  \\
%\cmidrule{2-7}          & SSIM  & 0.9593  & 0.9857  & 0.9868  & 0.9834  & 0.9830  \\
%    \midrule
%    \multirow{2}[4]{*}{HUAWEI\_FC} & PSNR  & 35.58  & 38.03  & 38.79  & 38.71  & 38.76  \\
%\cmidrule{2-7}          & SSIM  & 0.9413  & 0.9776  & 0.9809  & 0.9780  & 0.9785  \\
%    \midrule
%    \multirow{2}[4]{*}{OPPO\_BC} & PSNR  & 32.06  & 33.05  & 33.56  & 33.44  & 33.26  \\
%\cmidrule{2-7}          & SSIM  & 0.9071  & 0.9476  & 0.9544  & 0.9508  & 0.9456  \\
%    \midrule
%    \multirow{2}[4]{*}{OPPO\_FC} & PSNR  & 36.90  & 39.06  & 40.11  & 39.66  & 39.56  \\
%\cmidrule{2-7}          & SSIM  & 0.9447  & 0.9751  & 0.9823  & 0.9791  & 0.9785  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_video_psnr_ssim}%
%\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet4'
%\begin{table}[htbp]
%\scriptsize
%  \centering
%  \caption{PSNR and SSIM values of compared methods on real-world color video dataset. Average time per frame is also included. The best results are bolded. 'FC' and 'BC' represent front camera and back camera, respectively.}
%  \scalebox{0.88}{
%  \renewcommand{\arraystretch}{0.99}
%    \begin{tabular}{cccccc}
%    \toprule
%    \multirow{2}[4]{*}{Dataset} & \multicolumn{5}{c}{Method} \\
%\cmidrule{2-6}          & Noisy & FastDVDNet & VNLNet & CVMSt-SVD & VBM4D1 \\
%    \midrule
%    \multirow{2}[4]{*}{HUAWEI\_BC} & 38.11  & \textbf{41.26} & \textbf{41.35} & 40.80  & 41.19  \\
%\cmidrule{2-6}          & 0.9593  & 0.9857  & \textbf{0.9868} & 0.9834  & 0.9830  \\
%    \midrule
%    \multirow{2}[4]{*}{HUAWEI\_FC} & 35.58  & 38.03  & \textbf{38.79} & \textbf{38.71} & \textbf{38.76} \\
%\cmidrule{2-6}          & 0.9413  & 0.9776  & \textbf{0.9809} & 0.9780  & 0.9785  \\
%    \midrule
%    \multirow{2}[4]{*}{OPPO\_BC} & 32.06  & 33.05  & \textbf{33.56} & \textbf{33.44} & 33.26  \\
%\cmidrule{2-6}          & 0.9071  & 0.9476  & \textbf{0.9544} & 0.9508  & 0.9456  \\
%    \midrule
%    \multirow{2}[4]{*}{OPPO\_FC} & 36.90  & 39.06  & \textbf{40.11} & 39.66  & 39.56  \\
%\cmidrule{2-6}          & 0.9447  & 0.9751  & \textbf{0.9823} & 0.9791  & 0.9785  \\
%    \midrule
%    Implementation & /     & GPU   & GPU   & MEX   & MEX \\
%    \midrule
%    Time/Frame (s) & /     & \textbf{0.08}  & 0.66  & 1.86  & 1.09 \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_video_psnr_ssim}%
%\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[htbp]
\scriptsize
  \centering
  \caption{PSNR and SSIM values of compared methods on real-world color video dataset. Average time per frame is also included. The best results are bolded. 'FC' and 'BC' represent front camera and back camera, respectively.}
  \scalebox{0.89}{
  \renewcommand{\arraystretch}{0.99}
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}[4]{*}{Dataset} & \multicolumn{5}{c}{Method} \\
\cmidrule{2-6}          & Noisy & CVMSt-SVD & VBM4D1 & FastDVDNet & VNLNet \\
    \midrule
    \multirow{2}[4]{*}{HUAWEI\_BC} & 38.11  & 40.80  & 41.19  & \textbf{41.26} & \textbf{41.35} \\
\cmidrule{2-6}          & 0.9593  & 0.9834  & 0.9830  & 0.9857  & \textbf{0.9868} \\
    \midrule
    \multirow{2}[4]{*}{HUAWEI\_FC} & 35.58  & \textbf{38.71} & \textbf{38.76} & 38.03  & \textbf{38.79} \\
\cmidrule{2-6}          & 0.9413  & 0.9780  & 0.9785  & 0.9776  & \textbf{0.9809} \\
    \midrule
    \multirow{2}[4]{*}{OPPO\_BC} & 32.06  & \textbf{33.44} & 33.26  & 33.05  & \textbf{33.56} \\
\cmidrule{2-6}          & 0.9071  & 0.9508  & 0.9456  & 0.9476  & \textbf{0.9544} \\
    \midrule
    \multirow{2}[4]{*}{OPPO\_FC} & 36.90  & 39.66  & 39.56  & 39.06  & \textbf{40.11} \\
\cmidrule{2-6}          & 0.9447  & 0.9791  & 0.9785  & 0.9751  & \textbf{0.9823} \\
    \midrule
    Implementation & /     & MEX   & MEX   & GPU   & GPU \\
    \midrule
    Time/Frame (s) & /     & 1.86  & 1.29  & \textbf{0.08}  & 0.66 \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_video_psnr_ssim}%
\end{table}%



==> FIg_compare_MRI_NLSVD_HOSVD.tex <==
%\begin{figure}[htbp]
%\graphicspath{{Figs/combine_real_MRI_in_Supplementary/}}
%\centering
%%\subfigure[MRI\_0092]{
%%\label{Fig4}
%%\includegraphics[width=0.78in]{MRI_0092_Noisy_slice48_combine_marked}}
%\subfigure[SVD]{
%\label{Fig4}
%\includegraphics[MRI_0092_NLPCA_slice48_combined}}
%\subfigure[HOSVD]{
%\label{Fig4}
%\includegraphics[width=0.78in]{MRI_0092_HOSVD_slice48_combined}}
%
%
%\caption{Comparison of SVD and HOSVD transforms for real MRI denoising.}
%
%\label{Fig_compare_MRI_NLSVD_HOSVD}
%\end{figure}

\begin{figure}[htbp]
\graphicspath{{Figs/combine_real_MRI_in_Supplementary/}}
\centering
\subfigure[MRI\_0092]{
\label{Fig4}
\includegraphics[width=1.08in]{MRI_0092_Noisy_slice48_combine_marked}}
\subfigure[SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{MRI_0092_NLPCA_slice48_combined}}
\subfigure[HOSVD]{
\label{Fig4}
\includegraphics[width=1.08in]{MRI_0092_HOSVD_slice48_combined}}


\caption{Comparison of SVD and HOSVD for real MRI denoising.}
\label{Fig_compare_MRI_NLSVD_HOSVD}
\end{figure}


==> Fig_CBM3D_noise_level_influence.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_discussion/}}
\centering
\subfigure[PSNR]{
\label{Fig4}
\includegraphics[width=1.65in]{CBM3D1_PSNR_change_new2}}
\subfigure[SSIM]{
\label{Fig4}
\includegraphics[width=1.699in]{CBM3D1_SSIM_change_new}}


\caption{PSNR and SSIM change of CBM3D1 with noise level $\sigma \in [10, 30]$ on five real-world color image datasets.}
\label{Fig_CBM3D_noise_level_influence}
\end{figure}


==> Fig_CC15.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_CC15/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_Origin}}
\subfigure[Noisy (33.26)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_Noisy}}
\subfigure[NI (38.78)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_NI_mark}}
\subfigure[DeNoiseAI (36.63)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_Topaz_marked}}
\subfigure[DBF (41.42)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_DeepBoosting}}
\subfigure[DRUNet (40.85)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_DRUNet}}\\

\subfigure[FFDNet (40.15)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_FFDNet}}
\subfigure[FCCF (41.21)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_FCCF}}
\subfigure[CBM3D2 (39.59)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_CBM3D2}}
\subfigure[CMSt-SVD (39.98)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_MS-TSVD}}
\subfigure[TWSC (40.27)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_TWSC}}
\subfigure[NLH (40.21)]{
\label{Fig4}
\includegraphics[width=1.1in]{d800_iso3200_1_real_NLH}}


\caption{Visual evaluations of compared methods (PSNR) on CC15 dataset.}
\label{Fig_CC15}
\end{figure*}


==> Fig_CRVD.tex <==
\begin{figure}[htbp]
\graphicspath{{C:/Users/KZM11/Desktop/Figs_Video/result_images_sample/selected_for_comparison/Combined/CRVD/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}\\
\subfigure[DVDNet]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=0.808in]{ISO6400_scene3_Clean_frame7_combined}}

\caption{Visual evaluation of compared methods (PSNR) on our IOCI's IPHONE 5S dataset.}
\label{Fig_CRVD}
\end{figure}


==> Fig_HUAWEI-Mate40Pro_IPHONE13_compare.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[HUAWEI Mate40Pro]{
\label{Fig4}
\includegraphics[width=1.28in]{Huawei_Mate40Pro_IMG15_6_noisy_combined}}
\subfigure[IPHONE 13]{
\label{Fig4}
\includegraphics[width=1.28in]{IPHONE13_IMG39_9_noisy_combined}}

\caption{Images captured by two popular smartphone cameras of the same objects in the dark environment.}
\label{Fig_HUAWEI-Mate40Pro_IPHONE13_compare}
\end{figure}


==> Fig_HUAWEI-Mate40Pro_dark_environment_demo.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_images_Supp_proposed_dataset/}}
\centering
\subfigure[Trees]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo1}}
\subfigure[Streetlight]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo2}}
\subfigure[Grass]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo3}}

\caption{Images captured by HUAWEI Mate40Pro in dark environments.}
\label{Fig_HUAWEI-Mate40Pro_dark_environment_demo}
\end{figure}


==> Fig_HUAWEI-Mate40Pro_different_environment_demo.tex <==
%\begin{figure}[htbp]
%\graphicspath{{C:/Users/KZM11/Desktop/Fig_images_Supp_proposed_dataset/Combined/}}
%\centering
%\subfigure[Morning]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_sufficient-light_combined_marked}}
%\subfigure[Afternoon]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_low-light_combined}}
%\subfigure[Midnight]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_dark_combined}}
%
%\caption{Images of HUAWEI Mate40Pro under different lighting conditions.}
%\label{Fig_HUAWEI-Mate40Pro_different_environment_demo}
%\end{figure}


\begin{figure}[htbp]
\graphicspath{{Figs/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[Morning]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_sufficient-light_combined_marked}}
\subfigure[Afternoon]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_low-light_combined}}
\subfigure[Midnight]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_dark_combined}}

\caption{Images of IPHONE13 under different lighting conditions.}
\label{Fig_HUAWEI-Mate40Pro_different_environment_demo}
\end{figure}


==> Fig_HUAWEI-Mate40Pro_noise_pattern_compare.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[Cups]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG4_2_noisy_combined}}
\subfigure[Streetlight]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG13_3_noisy_combined}}
\subfigure[Building A]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG30_6_noisy_combined}}
\subfigure[Building B]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG28_1_noisy_combined}}

\caption{Images captured by HUAWEI Mate40Pro of different scenes.}
\label{Fig_HUAWEI-Mate40Pro_noise_pattern_compare}
\end{figure}


==> Fig_IOCV_new.tex <==
%\begin{figure*}[htbp]
%\graphicspath{{Figs/combined_IOCV/}}
%\centering
%\subfigure[Mean]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Clean_sclice1_combined}}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Noisy_sclice1_combined}}
%\subfigure[CVMSt-SVD]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_CVMStSVD_combined}}
%\subfigure[VBM4D2]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_VBM4D2_combined}}
%\subfigure[DVDNet]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_DVDNet_sig15_combined}}
%\subfigure[FastDVDNet]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_fastdvdnet_sig10_combined}}\\
%
%\subfigure[FloRNN]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_FloRNN_sig40_combined}}
%\subfigure[MAP-VDNet]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_MAP-VDNet_sig15_combined}}
%\subfigure[RFR]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_RFR_sig25_combined}}
%\subfigure[UDVD]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_UDVD_sig30_combined}}
%\subfigure[ViDeNN]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_ViDeNN_ckpt_videnn_combined}}
%\subfigure[VNLNet]{
%\label{Fig4}
%\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_vnlnet_sig20_combined}}
%
%
%\caption{Visual evaluation of video denoising on the IOCV dataset. The camera device is OPPO R11s.}
%\label{Fig_IOCV_new}
%\end{figure*}
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_IOCV/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Clean_sclice1_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Noisy_sclice1_combined}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_CVMStSVD_combined}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_VBM4D2_combined}}
\subfigure[DVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_DVDNet_sig15_combined}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_fastdvdnet_sig10_combined}}\\

\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_FloRNN_sig40_combined}}
\subfigure[MAP-VDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_MAP-VDNet_sig15_combined}}
\subfigure[RVRT]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_RVRT_sig20_combined}}
\subfigure[UDVD]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_UDVD_sig30_combined}}
\subfigure[ViDeNN]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_ViDeNN_ckpt_videnn_combined}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_vnlnet_sig20_combined}}


\caption{Visual evaluation of video denoising on the IOCV dataset. The camera device is OPPO R11s.}
\label{Fig_IOCV_new}
\end{figure*}


==> Fig_SIDD_validate_test_similar.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Figs_Supp_Experiments_Image_dataset/}}
\centering
\subfigure[Validation]{
\label{Fig4}
\includegraphics[width=1.28in]{SIDD_Validate_noisysRGB_19_23_sigma_0}}
\subfigure[Test]{
\label{Fig4}
\includegraphics[width=1.28in]{SIDD_Benchmark_noisysRGB_19_2_sigma_0}}

\caption{Sample images from the validation and test sets of SIDD.}
\label{Fig_SIDD_validate_test_similar}
\end{figure}


==> Fig_Set8.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_Set8/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.828in]{Clean_Motorbike_slice18_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.828in]{Noisy_Motorbike_slice18_sig40_combined}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.828in]{18_CVMStSVD_sig40_combined}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=0.828in]{18_VBM4D2_sig40_combined}}
\subfigure[DVDNet]{
\label{Fig4}
\includegraphics[width=0.828in]{18_DVDNet_sig40_combined}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=0.828in]{18_FastDVDNet_sig40_combined}}
\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=0.828in]{18_FloRNN_sig40_combined}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=0.828in]{18_vnlnet_sig40_combined}}

\caption{Visual evaluation of compared methods on the Set8 dataset.}
\label{Fig_Set8}
\end{figure*}


==> Fig_Xu_100.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_Xu_100/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_Origin}}
\subfigure[Noisy (36.68)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_Noisy}}
\subfigure[NI (36.78)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_NI}}
\subfigure[DeNoiseAI (36.01)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_Topaz}}
\subfigure[DBF (36.62)]{
\label{Fig4}
\includegraphics[width=1.1in]{Figs/combined_Xu_100/NikonD800_4-5_160_1800_classroom_5_real_DeepBoosting_mark.png}}
\subfigure[DRUNet (37.57)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_DRUNet}}\\
\subfigure[FFDNet (36.95)]{
\label{Fig4}
\includegraphics[width=1.1in]{Figs/combined_Xu_100/NikonD800_4-5_160_1800_classroom_5_real_FFDNet.png}}
\subfigure[FCCF (37.48)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_FCCF}}
\subfigure[CBM3D2 (37.81)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_CBM3D2}}
\subfigure[CMSt-SVD (37.80)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_MS-TSVD}}
\subfigure[TWSC (37.16)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_TWSC}}
\subfigure[NLH (37.14)]{
\label{Fig4}
\includegraphics[width=1.1in]{NikonD800_4-5_160_1800_classroom_5_real_NLH}}


\caption{Visual evaluation of compared methods (PSNR) on PolyU dataset.}
\label{Fig_Xu_100}
\end{figure*}


==> Fig_choose_N_noisy_for_mean_image.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Figs_Supp_Experiments_Image_dataset/}}
\centering
\subfigure[Relative error]{
\label{Fig4}
\includegraphics[width=1.696in]{Fig_Compare_mean_GT_img_relative_error}}
\subfigure[SSIM]{
\label{Fig4}
\includegraphics[width=1.696in]{Fig_Compare_mean_GT_img_SSIM}}

\caption{Relative error and SSIM of different mean images compared to the ground-truth. The camera device is IPHONE 13.}
\label{Fig_choose_N_noisy_for_mean_image}
\end{figure}


==> Fig_color_video.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/combined_real_video/combine/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.08in]{Clean}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{CVMStSVD}}\\
\subfigure[VBM4D1]{
\label{Fig4}
\includegraphics[width=1.08in]{VBM4D1}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{Fastdvdnet}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=1.08in]{Vnlnet}}\\


\caption{Visual evaluation of video denoising on the IOCV dataset.}
\label{Fig_color_video}
\end{figure}


==> Fig_discussion_visual_enhancement.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_discussion/}}
\centering
\subfigure[Noisy (RENOIR)]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy_demo_combine_marked}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{denoised_demo_combine}}
\subfigure[CMSt-SVD\_R]{
\label{Fig4}
\includegraphics[width=1.08in]{resized_demo_combine}}

\subfigure[Noisy (DND)]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy_demo2_combine_marked}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{denoised_demo2_combine}}
\subfigure[CMSt-SVD\_R]{
\label{Fig4}
\includegraphics[width=1.08in]{resized_demo2_combine}}


\caption{Visual evaluation of CMSt-SVD with and without the image resizing strategy on RENOIR (first row) and DND (second row) datasets.}
\label{Fig_discussion_visual_enhancement}
\end{figure}


==> Fig_fastMRI.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_fastMRI/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.81in]{Clean_img_9_slice_26_combined}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.81in]{Noisy_img_9_slice_26_combined}}
\subfigure[4DHOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{4DHOSVD1_img_9_slice_26_combined}}
\subfigure[AONLM]{
\label{Fig4}
\includegraphics[width=0.81in]{AONLM_img_9_slice_26_combined}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.81in]{BM4D2_img_9_slice_26_combined}}
\subfigure[ILR-HOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{ILRHOSVD_img_9_slice_26_combined}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.81in]{MStSVD_img_9_slice_26_combined}}
\subfigure[ODCT]{
\label{Fig4}
\includegraphics[width=0.81in]{ODCT_img_9_slice_26_combined}}


\caption{Visual evaluation of compared methods on the fastMRI dataset with noise level $\sigma$ = 19\%.}
\label{Fig_fastMRI}
\end{figure*}


==> Fig_my_dataset_SONYA6500.tex <==
%\begin{figure*}[htbp]
%\graphicspath{{Figs/combined_my_dataset_SonyA6500/}}
%\centering
%\subfigure[Mean]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_clean_combined_marked}}
%\subfigure[Noisy]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_combined}}
%\subfigure[4DHOSVD]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_4DHOSVD_combined}}
%\subfigure[mSVD]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_mSVD_combined}}
%\subfigure[Bitonic]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_bitonic_combined}}
%\subfigure[CBM3D2]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_CBM3D2_combined}} \\
%
%\subfigure[CMSt-SVD]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_CMSt-SVD_combined}}
%\subfigure[MCWNNM]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_MCWNNM_combined}}
%\subfigure[NLHCC]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_NLHCC_combined}}
%\subfigure[TWSC]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_TWSC_combined}}
%\subfigure[DIDN]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_DIDN_combined}}
%\subfigure[DRUNet]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_DPIR_combined}}\\
%
%\subfigure[FCCF]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_FCCF_combined}}
%\subfigure[FFDNet]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_FFDNet_combined}}
%\subfigure[NAFNet]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_NAFNet_combined}}
%\subfigure[PNGAN]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_PNGAN_combined}}
%\subfigure[Restormer]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_Restormer_combined}}
%\subfigure[VDIR]{
%\label{Fig4}
%\includegraphics[width=1.1in]{SONY_A6500_IMG16_3_noisy_VDIR_combined}}
%
%
%\caption{Visual evaluation of compared methods on the IOCI dataset. The camera device is SONYA6500.}
%\label{Fig_my_dataset_SONYA6500}
%\end{figure*}


\begin{figure*}[htbp]
\graphicspath{{Figs/combined_my_dataset_SonyA6500/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_clean_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_combined}}
\subfigure[Bitonic]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_bitonic_combined}}
\subfigure[CBM3D2]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_CBM3D2_combined}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_CMSt-SVD_combined}}
\subfigure[MCWNNM]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_MCWNNM_combined}}
\subfigure[4DHOSVD]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_4DHOSVD_combined}}
\subfigure[mSVD]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_mSVD_combined}}
\subfigure[NLHCC]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_NLHCC_combined}}\\

\subfigure[TWSC]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_TWSC_combined}}
\subfigure[DIDN]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_DIDN_combined}}
\subfigure[DRUNet]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_DPIR_combined}}
\subfigure[FCCF]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_FCCF_combined}}
\subfigure[FFDNet]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_FFDNet_combined}}
\subfigure[NAFNet]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_NAFNet_combined}}
\subfigure[PNGAN]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_PNGAN_combined}}
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_Restormer_combined}}
\subfigure[VDIR]{
\label{Fig4}
\includegraphics[width=0.726in]{SONY_A6500_IMG16_3_noisy_VDIR_combined}}


\caption{Visual evaluation of compared methods on the IOCI dataset. The camera device is SONYA6500.}
\label{Fig_my_dataset_SONYA6500}
\end{figure*} 



==> Fig_my_own.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_my_own/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_Origin}}
\subfigure[Noisy (41.23)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_Noisy}}
\subfigure[NI (42.89)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_NI}}
\subfigure[DeNoiseAI (41.06)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_Topaz_marked}}
\subfigure[DBF (42.66)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_DeepBoosting}}
\subfigure[DRUNet (44.47)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_DRUNet}}\\
\subfigure[FFDNet (44.77)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_FFDNet}}
\subfigure[FCCF (43.40)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_FCCF}}
\subfigure[CBM3D2 (44.54)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_CBM3D2}}
\subfigure[CMSt-SVD (44.81)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_MS-TSVD}}
\subfigure[TWSC (42.60)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_TWSC}}
\subfigure[NLH (44.47)]{
\label{Fig4}
\includegraphics[width=1.1in]{IPHONE_5s_IMG18_7_noisy_NLH}}


\caption{Visual evaluation of compared methods (PSNR) on our IOCI's IPHONE 5S dataset.}
\label{Fig_my_own}
\end{figure*}


==> Fig_oversmooth.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_appendix/}}
\centering
\subfigure[Origin]{
\label{Fig4}
\includegraphics[width=1.10in]{Origin}}
\subfigure[T-HOSVD]{
\label{Fig4}
\includegraphics[width=1.10in]{Over_smooth}}
\subfigure[Origin - T-HOSVD]{
\label{Fig4}
\includegraphics[width=1.10in]{Difference}}


\caption{Illustration of over-smooth effects produced by truncated HOSVD (T-HOSVD) when all the patches in a group are the same.}
\label{Fig_oversmooth}
\end{figure}


==> Fig_pre_train.tex <==
\begin{figure}[htbp]
%\setlength{\abovecaptionskip}{0.cm}
%\setlength{\belowcaptionskip}{-0.8cm}

\graphicspath{{Figs/Fig_discussion/}}

%\centering
%\includegraphics[width=2.36in]{PSNR_diff}
\centering
\subfigure[PSNR]{
\label{Fig4}
\includegraphics[width=1.69in]{PSNR_pre_train}}
\subfigure[SSIM]{
\label{Fig4}
\includegraphics[width=1.69in]{SSIM_pre_train}}

\caption{PSNR and SSIM values of DANet on the PolyU test set w.r.t different training epochs.}

\label{Fig_pre_train}
\end{figure}


==> Fig_timeline.tex <==
\begin{figure*}[htbp]
%\setlength{\abovecaptionskip}{0.cm}
%\setlength{\belowcaptionskip}{-0.8cm}

\graphicspath{{Figs/Fig_frameworks/}}

\centering
\includegraphics[width=6.999in]{time_line}


\caption{Timeline of representative multi-dimensional image denoising methods and datasets.}

\label{Fig_timeline}
\end{figure*}


==> Figs_IOCV.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/combined_IOCV/}}
\centering
\subfigure[Mean]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Clean_sclice1_combined}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_Noisy_sclice1_combined}}
\subfigure[CVMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_CVMStSVD_combined}}
\subfigure[VBM4D2]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_VBM4D2_combined}}
\subfigure[DVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_DVDNet_sig15_combined}}
\subfigure[FastDVDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_fastdvdnet_sig10_combined}}\\

\subfigure[FloRNN]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_FloRNN_sig40_combined}}
\subfigure[MAP-VDNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_MAP-VDNet_sig15_combined}}
\subfigure[RFR]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_RFR_sig25_combined}}
\subfigure[UDVD]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_UDVD_sig30_combined}}
\subfigure[ViDeNN]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_ViDeNN_ckpt_videnn_combined}}
\subfigure[VNLNet]{
\label{Fig4}
\includegraphics[width=1.08in]{OPPO_R11s_BC_S_80_INDOOR_V2_1_noisy_sclice1_vnlnet_sig20_combined}}


\caption{Visual evaluation of video denoising on the IOCV dataset. The camera device is OPPO R11s.}
\label{Fig_IOCV_new}
\end{figure}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Table_CC15.tex <==
%% Table generated by Excel2LaTeX from sheet 'Results_all'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Psnr results and average computational time(s) of compared methods on CC15 dataset. The best results are bolded and the second best are underlined.}
%    \begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|c|c|}
%    \toprule
%    \multicolumn{2}{|c|}{Methods} & \multicolumn{3}{c|}{CANON 5D ISO = 3200} & \multicolumn{3}{c|}{CANON D600 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 1600} & \multicolumn{3}{c|}{NIKON D800 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 6400} & Average & Time(s) \\
%    \midrule
%    \multicolumn{2}{|c|}{Noisy} & 37.00  & 33.88  & 33.83  & 33.28  & 33.77  & 34.93  & 35.47  & 35.71  & 34.81  & 33.26  & 32.89  & 32.91  & 29.63  & 29.97  & 29.87  & 33.41  & / \\
%    \midrule
%    \multirow{15}[30]{*}{Deep Learning} & TNRD  & 39.51  & 36.47  & 36.45  & 34.79  & 36.37  & 39.49  & 38.11  & 40.52  & 38.17  & 37.69  & 35.90  & 38.21  & 32.81  & 32.33  & 32.29  & 36.61  & 0.63  \\
%\cmidrule{2-19}          & MLP   & 39.01  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & 1.28  \\
%\cmidrule{2-19}          & FFD-Net & 39.40  & 37.02  & 36.53  & 34.97  & 36.73  & 41.02  & 38.66  & 41.53  & 38.80  & 40.15  & 37.61  & 41.18  & 34.13  & 33.66  & 33.69  & 37.67  & 1.99  \\
%\cmidrule{2-19}          & CBDNet & 38.63  & 36.18  & 36.10  & 34.83  & 35.69  & 38.32  & 38.44  & 39.98  & 37.29  & 37.78  & 37.15  & 37.39  & 32.58  & 33.01  & 32.01  & 36.36  & 3.58  \\
%\cmidrule{2-19}          & DeepBoosting & 39.74  & 37.23  & 36.87  & 35.39  & 36.98  & 41.08  & 39.72  & 42.02  & 39.68  & 41.42  & 38.76  & 42.34  & 35.78  & 34.48  & 34.27  & 38.38  & 0.32  \\
%\cmidrule{2-19}          & DIDN  & 35.45  & 36.16  & 35.10  & 34.34  & 35.25  & 37.88  & 38.52  & 36.82  & 39.50  & 38.62  & 37.61  & 38.15  & 32.16  & 32.46  & 32.56  & 36.04  & 0.18  \\
%\cmidrule{2-19}          & FCCF  & 41.41  & 37.63  & 37.49  & 36.94  & 39.07  & 42.71  & 39.88  & 42.37  & 40.03  & 41.21  & 38.73  & 41.67  & 36.22  & 35.10  & 35.09  & \textbf{39.04} & 36.36  \\
%\cmidrule{2-19}          & NLNet & 40.57  & 37.05  & 36.86  & 35.26  & 36.80  & 40.47  & 39.03  & 41.53  & 39.19  & 39.37  & 37.13  & 39.83  & 33.68  & 33.33  & 33.26  & 37.56  & 49.98  \\
%\cmidrule{2-19}          & Unet  & 39.72  & 36.75  & 36.54  & 35.28  & 36.53  & 40.47  & 39.09  & 41.13  & 39.33  & 38.50  & 36.89  & 38.75  & 31.69  & 31.88  & 31.74  & 36.95  & 5.69  \\
%\cmidrule{2-19}          & VDNet & 35.68  & 35.32  & 34.93  & 33.73  & 34.92  & 37.55  & 38.27  & 37.23  & 38.56  & 38.19  & 37.69  & 38.54  & 32.45  & 32.26  & 32.65  & 35.86  & 0.21  \\
%\cmidrule{2-19}          & AINDNet & 37.57  & 36.10  & 36.04  & 34.91  & 35.90  & 37.81  & 38.22  & 38.73  & 37.00  & 36.68  & 36.85  & 35.70  & 31.86  & 32.96  & 31.93  & 35.88  & 1.29  \\
%\cmidrule{2-19}          & Noise2Noise & 36.93  & 33.79  & 33.78  & 32.99  & 33.46  & 34.71  & 35.57  & 35.83  & 34.91  & 33.20  & 33.02  & 32.98  & 29.62  & 29.94  & 29.81  & 33.37  & 0.98  \\
%\cmidrule{2-19}          & CycleISP & 36.83  & 35.38  & 35.75  & 34.36  & 35.42  & 37.82  & 38.19  & 39.26  & 37.56  & 35.79  & 35.37  & 35.35  & 31.17  & 31.42  & 31.32  & 35.40  & 0.38  \\
%\cmidrule{2-19}          & SADNet & 38.40  & 37.51  & 36.35  & 35.98  & 37.26  & 41.00  & 39.65  & 41.23  & 39.59  & 39.67  & 37.94  & 41.35  & 33.65  & 34.08  & 33.27  & 37.80  & 0.33  \\
%\cmidrule{2-19}          & DnCNN & 39.51  & 36.92  & 36.54  & 35.02  & 36.46  & 40.59  & 38.94  & 41.33  & 39.05  & 39.57  & 37.43  & 40.18  & 33.56  & 33.53  & 33.41  & 37.47  & 3.28  \\
%    \midrule
%    \midrule
%    \multirow{13}[26]{*}{Traditional Gaussian} & LCSD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 6.45  \\
%\cmidrule{2-19}          & LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & $>$1000 \\
%\cmidrule{2-19}          & WTR1  & 41.09  & 36.92  & 36.25  & 34.68  & 36.48  & 40.52  & 38.26  & 41.40  & 38.61  & 39.98  & 37.70  & 41.36  & 35.16  & 34.22  & 34.43  & 37.80  & $>$1000 \\
%\cmidrule{2-19}          & GID   & 40.82  & 37.19  & 36.92  & 35.32  & 36.62  & 38.68  & 38.88  & 40.66  & 39.20  & 37.92  & 36.62  & 37.64  & 33.01  & 32.93  & 32.96  & 37.02  & 38.88  \\
%\cmidrule{2-19}          & MCWNNM & 41.21  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & 37.72  & 228.16  \\
%\cmidrule{2-19}          & NLH\_CC & 41.57  & 37.39  & 36.68  & 35.51  & 37.21  & 41.34  & 39.67  & 42.66  & 40.04  & 40.21  & 37.30  & 42.02  & 36.19  & 34.70  & 34.83  & 38.49  & 51.86  \\
%\cmidrule{2-19}          & TWSC  & 40.55  & 35.92  & 35.15  & 35.36  & 37.09  & 41.13  & 39.36  & 41.91  & 38.81  & 40.27  & 37.22  & 42.09  & 35.53  & 34.15  & 33.93  & 37.90  & 368.68  \\
%\cmidrule{2-19}          & CBM3D1 & 40.23  & 37.02  & 36.18  & 34.78  & 36.61  & 40.44  & 38.58  & 41.34  & 39.15  & 39.57  & 37.35  & 39.79  & 34.59  & 33.84  & 33.94  & 37.56  & 0.95  \\
%\cmidrule{2-19}          & CBM3D2 & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & 37.70  & 4.38  \\
%\cmidrule{2-19}          & CBM3D\_best & 40.96  & 37.31  & 37.15  & 35.38  & 36.81  & 40.45  & 39.25  & 41.65  & 39.59  & 39.86  & 37.54  & 40.38  & 34.85  & 33.92  & 34.16  & 37.95  & 4.38  \\
%\cmidrule{2-19}          & M-SVD & 41.43  & 37.17  & 36.84  & 35.20  & 36.97  & 40.23  & 38.90  & 41.75  & 39.60  & 39.33  & 37.26  & 38.70  & 34.52  & 33.53  & 33.74  & 37.68  & 75.88  \\
%\cmidrule{2-19}          & 4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 86.69  \\
%\cmidrule{2-19}          & CMSt-SVD & 40.79  & 37.37  & 37.01  & 35.29  & 36.95  & 40.93  & 39.21  & 41.98  & 39.54  & 39.98  & 37.65  & 40.05  & 34.50  & 33.93  & 34.01  & 37.95  & 6.18  \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:addlabel}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Results_all'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Psnr results and average computational time(s) of compared methods on CC15 dataset. The best results are bolded and the second best are underlined.}
    \begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|c|c|}
    \toprule
    \multicolumn{2}{|c|}{Methods} & \multicolumn{3}{c|}{CANON 5D ISO = 3200} & \multicolumn{3}{c|}{CANON D600 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 1600} & \multicolumn{3}{c|}{NIKON D800 ISO = 3200} & \multicolumn{3}{c|}{NIKON D800 ISO = 6400} & Average & Time(s) \\
    \midrule
    \multicolumn{2}{|c|}{Noisy} & 37.00  & 33.88  & 33.83  & 33.28  & 33.77  & 34.93  & 35.47  & 35.71  & 34.81  & 33.26  & 32.89  & 32.91  & 29.63  & 29.97  & 29.87  & 33.41  & / \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{15}[30]{*}{Deep Learning models}} & TNRD  & 39.51  & 36.47  & 36.45  & 34.79  & 36.37  & 39.49  & 38.11  & 40.52  & 38.17  & 37.69  & 35.90  & 38.21  & 32.81  & 32.33  & 32.29  & 36.61  & 0.63  \\
\cmidrule{2-19}          & MLP   & 39.01  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & 1.28  \\
\cmidrule{2-19}          & FFDNet & 39.40  & 37.02  & 36.53  & 34.97  & 36.73  & 41.02  & 38.66  & 41.53  & 38.80  & 40.15  & 37.61  & 41.18  & 34.13  & 33.66  & 33.69  & 37.67  & 1.99  \\
\cmidrule{2-19}          & CBDNet & 38.63  & 36.18  & 36.10  & 34.83  & 35.69  & 38.32  & 38.44  & 39.98  & 37.29  & 37.78  & 37.15  & 37.39  & 32.58  & 33.01  & 32.01  & 36.36  & 3.58  \\
\cmidrule{2-19}          & DeepBoosting & 39.74  & 37.23  & 36.87  & 35.39  & 36.98  & 41.08  & 39.72  & 42.02  & 39.68  & 41.42  & 38.76  & 42.34  & 35.78  & 34.48  & 34.27  & 38.38  & 0.32  \\
\cmidrule{2-19}          & DIDN  & 35.45  & 36.16  & 35.10  & 34.34  & 35.25  & 37.88  & 38.52  & 36.82  & 39.50  & 38.62  & 37.61  & 38.15  & 32.16  & 32.46  & 32.56  & 36.04  & 0.18  \\
\cmidrule{2-19}          & FCCF  & 41.41  & 37.63  & 37.49  & 36.94  & 39.07  & 42.71  & 39.88  & 42.37  & 40.03  & 41.21  & 38.73  & 41.67  & 36.22  & 35.10  & 35.09  & \textbf{39.04} & 36.36  \\
\cmidrule{2-19}          & NLNet & 40.57  & 37.05  & 36.86  & 35.26  & 36.80  & 40.47  & 39.03  & 41.53  & 39.19  & 39.37  & 37.13  & 39.83  & 33.68  & 33.33  & 33.26  & 37.56  & 49.98  \\
\cmidrule{2-19}          & Unet  & 39.72  & 36.75  & 36.54  & 35.28  & 36.53  & 40.47  & 39.09  & 41.13  & 39.33  & 38.50  & 36.89  & 38.75  & 31.69  & 31.88  & 31.74  & 36.95  & 5.69  \\
\cmidrule{2-19}          & VDNet & 35.68  & 35.32  & 34.93  & 33.73  & 34.92  & 37.55  & 38.27  & 37.23  & 38.56  & 38.19  & 37.69  & 38.54  & 32.45  & 32.26  & 32.65  & 35.86  & 0.21  \\
\cmidrule{2-19}          & AINDNet & 37.57  & 36.10  & 36.04  & 34.91  & 35.90  & 37.81  & 38.22  & 38.73  & 37.00  & 36.68  & 36.85  & 35.70  & 31.86  & 32.96  & 31.93  & 35.88  & 1.29  \\
\cmidrule{2-19}          & Noise2Noise & 36.93  & 33.79  & 33.78  & 32.99  & 33.46  & 34.71  & 35.57  & 35.83  & 34.91  & 33.20  & 33.02  & 32.98  & 29.62  & 29.94  & 29.81  & 33.37  & 0.98  \\
\cmidrule{2-19}          & CycleISP & 36.83  & 35.38  & 35.75  & 34.36  & 35.42  & 37.82  & 38.19  & 39.26  & 37.56  & 35.79  & 35.37  & 35.35  & 31.17  & 31.42  & 31.32  & 35.40  & 0.38  \\
\cmidrule{2-19}          & SADNet & 38.40  & 37.51  & 36.35  & 35.98  & 37.26  & 41.00  & 39.65  & 41.23  & 39.59  & 39.67  & 37.94  & 41.35  & 33.65  & 34.08  & 33.27  & 37.80  & 0.33  \\
\cmidrule{2-19}          & DnCNN & 39.51  & 36.92  & 36.54  & 35.02  & 36.46  & 40.59  & 38.94  & 41.33  & 39.05  & 39.57  & 37.43  & 40.18  & 33.56  & 33.53  & 33.41  & 37.47  & 3.28  \\
    \midrule
    \midrule
    \multicolumn{1}{|c|}{\multirow{13}[26]{*}{Traditional Gaussian Denoiser}} & LCSD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 6.45  \\
\cmidrule{2-19}          & LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & $>$1000 \\
\cmidrule{2-19}          & WTR1  & 41.09  & 36.92  & 36.25  & 34.68  & 36.48  & 40.52  & 38.26  & 41.40  & 38.61  & 39.98  & 37.70  & 41.36  & 35.16  & 34.22  & 34.43  & 37.80  & $>$2000 \\
\cmidrule{2-19}          & GID   & 40.82  & 37.19  & 36.92  & 35.32  & 36.62  & 38.68  & 38.88  & 40.66  & 39.20  & 37.92  & 36.62  & 37.64  & 33.01  & 32.93  & 32.96  & 37.02  & 38.88  \\
\cmidrule{2-19}          & MCWNNM & 41.21  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & 37.72  & 228.16  \\
\cmidrule{2-19}          & NLH\_CC & 41.57  & 37.39  & 36.68  & 35.51  & 37.21  & 41.34  & 39.67  & 42.66  & 40.04  & 40.21  & 37.30  & 42.02  & 36.19  & 34.70  & 34.83  & 38.49  & 51.86  \\
\cmidrule{2-19}          & TWSC  & 40.55  & 35.92  & 35.15  & 35.36  & 37.09  & 41.13  & 39.36  & 41.91  & 38.81  & 40.27  & 37.22  & 42.09  & 35.53  & 34.15  & 33.93  & 37.90  & 368.68  \\
\cmidrule{2-19}          & CBM3D1 & 40.23  & 37.02  & 36.18  & 34.78  & 36.61  & 40.44  & 38.58  & 41.34  & 39.15  & 39.57  & 37.35  & 39.79  & 34.59  & 33.84  & 33.94  & 37.56  & 0.95  \\
\cmidrule{2-19}          & CBM3D2 & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & 37.70  & 4.38  \\
\cmidrule{2-19}          & CBM3D\_best & 40.96  & 37.31  & 37.15  & 35.38  & 36.81  & 40.45  & 39.25  & 41.65  & 39.59  & 39.86  & 37.54  & 40.38  & 34.85  & 33.92  & 34.16  & 37.95  & 4.38  \\
\cmidrule{2-19}          & M-SVD & 41.43  & 37.17  & 36.84  & 35.20  & 36.97  & 40.23  & 38.90  & 41.75  & 39.60  & 39.33  & 37.26  & 38.70  & 34.52  & 33.53  & 33.74  & 37.68  & 75.88  \\
\cmidrule{2-19}          & 4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 86.69  \\
\cmidrule{2-19}          & CMSt-SVD & 40.79  & 37.37  & 37.01  & 35.29  & 36.95  & 40.93  & 39.21  & 41.98  & 39.54  & 39.98  & 37.65  & 40.05  & 34.50  & 33.93  & 34.01  & 37.95  & 6.18  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> Table_Color_other_datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'Results_all'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Psnr results of compared methods on CC60, Xu-100 and Kong-Image dataset. The three best results are bolded.}
    \begin{tabular}{c|cccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{11}{c}{Dataset} \\
\cmidrule{3-13}    \multicolumn{2}{c}{} & CC60  & Xu-100 & CANON 100D & CANON 600D & HUAWEI & IPHONE 5S & IPHONE 6S & SONY & XIAOMI & OPPO & FUJIFILM \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  \\
    \midrule
    \multirow{12}[24]{*}{Deep Learning Models} & FFD-Net & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  \\
\cmidrule{2-13}          & CBDNet & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  \\
\cmidrule{2-13}          & DeepBoosting & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  \\
\cmidrule{2-13}          & DIDN  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  \\
\cmidrule{2-13}          & FCCF  & 40.89  & 38.85 & 41.91  & 43.07  & 40.11  & 40.39  & 40.65  & 45.38  & 36.67  & 40.93  & 42.78  \\
\cmidrule{2-13}          & NLNet & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  \\
\cmidrule{2-13}          & Unet  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  \\
\cmidrule{2-13}          & VDNet & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  \\
\cmidrule{2-13}          & AINDNet & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  \\
\cmidrule{2-13}          & CycleISP & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  \\
\cmidrule{2-13}          & SADNet & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  \\
\cmidrule{2-13}          & DnCNN & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  \\
    \midrule
    \midrule
    \multicolumn{1}{c|}{\multirow{11}[22]{*}{Traditional Gaussian Denoisers}} & LCSD  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  \\
\cmidrule{2-13}          & LLRT  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  \\
\cmidrule{2-13}          & GID   & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  \\
\cmidrule{2-13}          & MCWNNM & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  \\
\cmidrule{2-13}          & NLH\_CC & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & 46.00  & 35.73  & 40.69  & 42.80  \\
\cmidrule{2-13}          & TWSC  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  \\
\cmidrule{2-13}          & CBM3D1 & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  \\
\cmidrule{2-13}          & CBM3D2 & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  \\
\cmidrule{2-13}          & CBM3D\_best & 39.68 & 38.81 & 42.08 & 42.89 & 40.48 & 41.25 & 41.16 & 45.81 & 36.66  & 40.89  & 43.14  \\
\cmidrule{2-13}          & 4DHOSVD1 & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  \\
\cmidrule{2-13}          & CMSt-SVD & 39.75 & 38.82 & 41.99  & 42.75  & 40.08  & 40.84  & 40.53  & 45.89  & 36.40  & 40.85  & 42.68  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> Table_ICVL.tex <==
%\begin{table}[htbp]
%  \centering
%  \caption{Average PSNR/SSIM of representative denoising methods under i.i.d Gaussian noise $\sigma \in \{10,20,40\}$ with ICVL dataset.}
%    \begin{tabular}{cccc}
%    \toprule
%    Methods & $\sigma = 10$    & $\sigma = 20$    & $\sigma = 40$ \\
%    \midrule
%    MSt-SVD & 46.58/0.9868 & 42.98/0.9746 & 39.32/0.9525 \\
%    \midrule
%    QRNN3D & 47.37/0.9908 & 45.08/0.9842 & 42.38/0.9731 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_ICVL}%
%\end{table}%


% Table generated by Excel2LaTeX from sheet 'ICVL'
\begin{table}[htbp]
\scriptsize
  \centering
  \caption{Average PSNR/SSIM and computational time (minutes) of MSt-SVD and QRNN3D under i.i.d Gaussian noise $\sigma \in \{10,20,40\}$ on the first 20 MSI data of ICVL dataset.}
    \begin{tabular}{ccccc}
    \toprule
    Methods & $\sigma = 10$    & $\sigma = 20$    & $\sigma = 40$    & Time (m) \\
    \midrule
    MSt-SVD & 46.58/0.9868 & 42.98/0.9746 & 39.32/0.9525 & 10.1 \\
    \midrule
    QRNN3D & \textbf{47.37/0.9908} & \textbf{45.08/0.9842} & \textbf{42.38/0.9731} & \textbf{0.16} \\
    \bottomrule
    \end{tabular}%
  \label{Table_ICVL}%
\end{table}%


==> Table_MRI.tex <==
% Table generated by Excel2LaTeX from sheet 'All'
%\begin{table*}[htbp]
%\scriptsize
%  \centering
%  \caption{Average PSNR (left value in each cell), SSIM and computational time (s) of different methods with T1w, T2w, and PDw data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
%  \renewcommand{\arraystretch}{0.98}
%  \scalebox{0.83}{
%    \begin{tabular}{ccccccccccccc}
%    \toprule
%    $\sigma$ ($\%$) & Noisy & AONLM & ODCT  & ONLM  & PRINLM & BM4D1 & BM4D2 & NLPCA & PRI-NLPCA & ILR-HOSVD & 4DHOSVD & MSt-SVD \\
%    \midrule
%    1    & 40.0/0.971 & 41.9/0.991 & 43.3/0.992 & 41.7/0.991 & 43.3/0.993 & 43.2/0.992 & 43.4/0.992 & 44.1/0.994 & 44.3/0.994 & \textbf{44.4/0.994} & 43.9/0.993 & 44.0/0.993 \\
%    \midrule
%    3     & 30.5/0.822 & 36.5/0.971 & 36.4/0.970 & 36.4/0.969 & 36.9/0.975 & 36.6/0.972 & 37.2/0.975 & 37.7/0.977 & \textbf{38.1/0.981} & 38.0/0.978 & 37.5/0.976 & 37.5/0.975 \\
%    \midrule
%    5     & 26.1/0.676 & 33.8/0.947 & 33.6/0.949 & 33.3/0.940 & 34.0/0.955 & 33.7/0.950 & 34.6/0.959 & 33.8/0.940 & \textbf{35.3/0.967} & 35.2/0.963 & 34.6/0.959 & 34.6/0.958 \\
%    \midrule
%    7     & 23.2/0.564 & 31.9/0.921 & 31.7/0.927 & 31.2/0.911 & 32.0/0.934 & 31.8/0.926 & 32.8/0.943 & 31.9/0.912 & \textbf{33.4/0.951} & 33.4/0.948 & 32.9/0.941 & 32.8/0.940 \\
%    \midrule
%    9     & 21.0/0.479 & 30.5/0.894 & 30.2/0.905 & 29.4/0.880 & 30.5/0.911 & 30.3/0.899 & 31.5/0.928 & 31.2/0.908 & \textbf{31.9/0.934} & \textbf{32.0/0.933} & 31.5/0.922 & 31.3/0.924 \\
%    \midrule
%    11    & 19.3/0.414 & 29.3/0.865 & 29.1/0.883 & 27.8/0.847 & 29.3/0.888 & 29.2/0.873 & 30.5/0.912 & 30.0/0.883 & 30.7/0.916 & \textbf{30.9/0.917} & 30.4/0.903 & 30.2/0.906 \\
%    \midrule
%    13    & 17.8/0.361 & 28.3/0.836 & 28.1/0.861 & 26.3/0.811 & 28.2/0.864 & 28.1/0.844 & 29.6/0.895 & 29.0/0.855 & 29.6/0.898 & \textbf{29.9/0.902} & 29.4/0.883 & 29.3/0.888 \\
%    \midrule
%    15    & 16.6/0.319 & 27.4/0.807 & 27.3/0.840 & 24.9/0.771 & 27.4/0.841 & 27.3/0.814 & 28.8/0.879 & 28.1/0.826 & 28.8/0.879 & \textbf{29.1/0.886} & 28.6/0.863 & 28.5/0.871 \\
%    \midrule
%    17    & 15.5/0.284 & 26.5/0.775 & 26.5/0.820 & 23.4/0.729 & 26.6/0.817 & 26.5/0.785 & \textbf{28.1/0.862} & 27.3/0.798 & 28.0/0.860 & 27.7/0.838 & 27.8/0.842 & 27.7/0.853 \\
%    \midrule
%    19    & 14.6/0.254 & 25.7/0.744 & 25.8/0.799 & 22.0/0.684 & 25.9/0.797 & 25.7/0.755 & \textbf{27.4/0.845} & 26.6/0.772 & 27.3/0.841 & 27.0/0.819 & 27.1/0.822 & 27.1/0.835 \\
%    \midrule
%    Implementation & /     & Mex   & Mex   & Mex   & Mex   & Mex   & Mex   & MATLAB & MEX   & MATLAB & MATLAB & MEX \\
%    \midrule
%    Time (s) & /     & 868.1 & \textbf{10.5}  & 139.9 & 18.6  & 69.9  & 211.3 & 638.8 & 868.9 & 1896.3 & 706.9 & 99.6 \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_MRI}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'All'
\begin{table*}[htbp]
\scriptsize
  \centering
  \caption{Average PSNR/SSIM and computational time (s) of different methods with T1w, T2w, and PDw data corrupted by Rician noise. The standard deviations $\sigma$ of the noise is expressed as percentage relative to the maximum intensity value of the noise-free data \cite{maggioni2012nonlocal}.}
  \renewcommand{\arraystretch}{0.99}
  \scalebox{0.839}{
    \begin{tabular}{ccccccccccccc}
    \toprule
    $\sigma (\%)$ & Noisy & ONLM  & AONLM & ODCT  & PRINLM & BM4D1 & BM4D2 & NLPCA & PRI-NLPCA & ILR-HOSVD & 4DHOSVD & MSt-SVD \\
    \midrule
    1     & 40.0/0.971 & 41.7/0.991 & 41.9/0.991 & 43.3/0.992 & 43.3/0.993 & 43.2/0.992 & 43.4/0.992 & 44.1/0.994 & 44.3/0.994 & \textbf{44.4/0.994} & 43.9/0.993 & 44.0/0.993 \\
    \midrule
    3     & 30.5/0.822 & 36.4/0.969 & 36.5/0.971 & 36.4/0.970 & 36.9/0.975 & 36.6/0.972 & 37.2/0.975 & 37.7/0.977 & \textbf{38.1/0.981} & 38.0/0.978 & 37.5/0.976 & 37.5/0.975 \\
    \midrule
    5     & 26.1/0.676 & 33.3/0.940 & 33.8/0.947 & 33.6/0.949 & 34.0/0.955 & 33.7/0.950 & 34.6/0.959 & 33.8/0.940 & \textbf{35.3/0.967} & 35.2/0.963 & 34.6/0.959 & 34.6/0.958 \\
    \midrule
    7     & 23.2/0.564 & 31.2/0.911 & 31.9/0.921 & 31.7/0.927 & 32.0/0.934 & 31.8/0.926 & 32.8/0.943 & 31.9/0.912 & \textbf{33.4/0.951} & 33.4/0.948 & 32.9/0.941 & 32.8/0.940 \\
    \midrule
    9     & 21.0/0.479 & 29.4/0.880 & 30.5/0.894 & 30.2/0.905 & 30.5/0.911 & 30.3/0.899 & 31.5/0.928 & 31.2/0.908 & \textbf{31.9/0.934} & \textbf{32.0/0.933} & 31.5/0.922 & 31.3/0.924 \\
    \midrule
    11    & 19.3/0.414 & 27.8/0.847 & 29.3/0.865 & 29.1/0.883 & 29.3/0.888 & 29.2/0.873 & 30.5/0.912 & 30.0/0.883 & 30.7/0.916 & \textbf{30.9/0.917} & 30.4/0.903 & 30.2/0.906 \\
    \midrule
    13    & 17.8/0.361 & 26.3/0.811 & 28.3/0.836 & 28.1/0.861 & 28.2/0.864 & 28.1/0.844 & 29.6/0.895 & 29.0/0.855 & 29.6/0.898 & \textbf{29.9/0.902} & 29.4/0.883 & 29.3/0.888 \\
    \midrule
    15    & 16.6/0.319 & 24.9/0.771 & 27.4/0.807 & 27.3/0.840 & 27.4/0.841 & 27.3/0.814 & 28.8/0.879 & 28.1/0.826 & 28.8/0.879 & \textbf{29.1/0.886} & 28.6/0.863 & 28.5/0.871 \\
    \midrule
    17    & 15.5/0.284 & 23.4/0.729 & 26.5/0.775 & 26.5/0.820 & 26.6/0.817 & 26.5/0.785 & \textbf{28.1/0.862} & 27.3/0.798 & 28.0/0.860 & 27.7/0.838 & 27.8/0.842 & 27.7/0.853 \\
    \midrule
    19    & 14.6/0.254 & 22.0/0.684 & 25.7/0.744 & 25.8/0.799 & 25.9/0.797 & 25.7/0.755 & \textbf{27.4/0.845} & 26.6/0.772 & 27.3/0.841 & 27.0/0.819 & 27.1/0.822 & 27.1/0.835 \\
    \midrule
    Implementation & /     & Mex   & Mex   & Mex   & Mex   & Mex   & Mex   & MATLAB & MEX   & MATLAB & MATLAB & MEX \\
    \midrule
    Time (s) & /     & 139.9 & 868.1 & \textbf{10.5} & 18.6  & 69.9  & 211.3 & 638.8 & 868.9 & 1896.3 & 706.9 & 99.6 \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_MRI}%
\end{table*}%



==> Table_Method_all.tex <==
%\begin{table*}
%\scriptsize
%\centering
%\caption{aa}
%\scalebox{0.88}{
%\renewcommand{\arraystretch}{1.02}
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%Category                      & Representation           & Methods       & Noise Modeling Experiments      & Applications     & Key Words                                                     \\
%\hline
%\multirow{41}{*}{Traditional} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color, othman2006noise}           & AWGN                            & CI, MSI          & Adaptive wavelet thresholding with thresholding techniques    \\
%\cline{3-6}
%                              &                          & NLM \cite{buades2005review, dai2013multichannel}          & AWGN                            & CI               & NLM algorithm with Gaussian kernels                           \\
%\cline{3-6}
%                              &                          & WSM \cite{coupe20083d}          & AWGN                            & MRI              & 3D wavelet subbands mixing for image denoising                \\
%\cline{3-6}
%                              &                          & TCVD \cite{liu2010high}         & AWGN                            & CV               & Integration of robust optical flow into NLM                   \\
%\cline{3-6}
%                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                            & CI, MRI          & Applications of SVD decomposition                             \\
%\cline{3-6}
%                              &                          & LRMR \cite{zhang2013hyperspectral}          & AWGN                            & MRI              & A low-rank matrix decomposition model                         \\
%\cline{3-6}
%                              &                          & GID \cite{xu2018external}          & AWGN                            & CI               & External data guided and internal prior learning              \\
%\cline{3-6}
%                              &                          & SPTWO \cite{buades2016patch}        & AWGN                            & CV               & NLPCA with optical flow estimation                            \\
%\cline{3-6}
%                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                            & CI, MSI          & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                            & CV               & Efficient approximate global patch search                     \\
%\cline{3-6}
%                              &                          & MCWNNM \cite{xu2017multi}       & AWGN                            & CI               & Extension of WNNM to color images                             \\
%\cline{3-6}
%                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                            & CV               & ~A trilateral weighted sparse coding scheme                   \\
%\cline{3-6}
%                              &                          & NLH\_CC \cite{hou2020nlh}      & AWGN                            & CI               & Nonlocal pixel similarity with Haar transform                 \\
%\cline{3-6}
%                              &                          & AMF \cite{chan2005salt}          & Impulsive                       & CI               & Impulsive noise removal by adaptive median filter             \\
%\cline{3-6}
%                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                       & CI               & Impulsive noise removal by iterative adaptive fuzzy filter    \\
%\cline{3-6}
%                              &                          & LSM-NLR \cite{huang2017mixed}      & Gaussian, Poisson and Impulsive & CV               & Low-rank with laplacian scale mixture modeling                \\
%\cline{3-6}
%                              &                          & FastHyde \cite{zhuang2018fast}     & Gaussian and Poisson        & MSI              & Low-rank and sparse representation                            \\
%\cline{3-6}
%                              &                          & NMoG \cite{chen2017denoising}         & Gaussian, Stripe and Impulsive  & MSI              & Low-rank matrix model with non i.i.d Gaussian noise           \\
%\cline{3-6}
%                              &                          & ODCT \cite{manjon2012new}         & AWGN and Rician                 & MRI              & A 3D DCT implementation                                       \\
%\cline{3-6}
%                              &                          & OBNLM \cite{coupe2008optimized}        & AWGN and Rician                 & MRI              & An optimized blockwise NLM Filter                             \\
%\cline{3-6}
%                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician                 & MRI              & Adaptive NLM with spatially varying noise levels              \\
%\cline{3-6}
%                              &                          & RLMMSE \cite{aja2008noise}       & Rician                          & MRI              & A novel linear minimum mean square error (LMMSE) estimator    \\
%\cline{3-6}
%                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician                 & MRI              & A rotationally invariant version of the NLM filter            \\
%\cline{3-6}
%                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician                 & MRI              & A two stage filter based on NLPCA and PRI-NLM                 \\
%\cline{2-6}
%                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                            & CI               & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}       & AWGN                            & CV               & Extention of CBM3D to color videos                            \\
%\cline{3-6}
%                              &                          & LRTA \cite{renard2008denoising}         & AWGN                            & MSI              & A low Tucker rank tensor decomposition  model                 \\
%\cline{3-6}
%                              &                          & PARAFAC \cite{liu2012denoising}      & AWGN                            & MSI              & A rank-one CP decomposition model                             \\
%\cline{3-6}
%                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                            & CV               & Extention of BM3D to color videos using 3D patch              \\
%\cline{3-6}
%                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                            & MSI, MRI         & Extention of BM4D to MSI and MRI using 3D patch               \\
%\cline{3-6}
%                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising}      & AWGN                            & CI, MSI, MRI     & Applications of 4DHOSVD transform                             \\
%\cline{3-6}
%                              &                          & TDL \cite{peng2014decomposable}           & AWGN                            & MSI              & A Tucker based tensor dictionary learning algorithm           \\
%\cline{3-6}
%                              &                          & KTSVD \cite{Zhang2015KTSVD}        & AWGN                            & MSI              & A t-SVD based tensor dictionary learning algorithm            \\
%\cline{3-6}
%                              &                          & ITSReg \cite{xie2016multispectral}       & AWGN                            & MSI              & Intrinsic Tensor Sparsity Regularization                      \\
%\cline{3-6}
%                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                            & MSI              & Low Tucker rank decomposition with total variation            \\
%\cline{3-6}
%                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                            & CI               & A weighted rank-one CP decomposition model                    \\
%\cline{3-6}
%                              &                          & HOSVDR\_S \cite{lv2019denoising}    & AWGN                            & MRI              & A recursive low Tucker rank model with rank estimation        \\
%\cline{3-6}
%                              &                          & MSt-SVD \cite{kong2017new, kong2019color}      & AWGN                            & CI, CV, MRI, MSI & An efficient one-stage multi-diemsional t-SVD implementation  \\
%\cline{3-6}
%                              &                          & NGMeet \cite{he2019non}        & AWGN                            & MSI              & Low-rank tensor model with iterative regularization           \\
%\cline{3-6}
%                              &                          & LTDL \cite{gong2020low}         & AWGN                            & MSI              & A low-rank tensor dictionary learning method                  \\
%\cline{3-6}
%                              &                          & NLTA-LSM \cite{dong2015low}     & Gaussian and Poisson         & MSI, MRI         & Low Tucker rank with laplacian scale mixture modeling         \\
%\hline
%\end{tabular}
%}
%\end{table*}

% \usepackage{multirow}

\begin{table*}[htbp]
\scriptsize
\centering
\caption{Related multi-dimensional image denoising methods with different noise modeling techniques and applications. 'CI': color image, 'CV': color video, 'MSI': multispectral imaging, 'MRI': magnetic resonance imaging.}
\scalebox{0.84}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Category}                      & \textbf{Representation}           & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                     \\
\hline
\multirow{41}{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color,othman2006noise}           & AWGN                        & CI, MSI, HSI      & Adaptive wavelet thresholding with thresholding techniques    \\
\cline{3-6}
                              &                          & DCT \cite{yaroslavsky1996local, foi2007pointwise}           & AWGN                        & CI                & high-quality denoising with discrete cosine transform (DCT)   \\
\cline{3-6}
                              &                          & NLM \cite{buades2005review, dai2013multichannel}           & AWGN                        & CI                & NLM algorithm with Gaussian kernels                           \\
\cline{3-6}
                              &                          & WSM \cite{coupe20083d}           & AWGN                        & MRI               & 3D wavelet subbands mixing for image denoising                \\
\cline{3-6}
                              &                          & K-SVD \cite{mairal2007sparse, fu2015adaptive}           & AWGN                        & CI, MSI               & 3D wavelet over-complete dictionary learning and sparse coding                \\
\cline{3-6}
                              &                          & TCVD \cite{liu2010high}         & AWGN                        & CV                & Integration of robust optical flow into NLM                   \\
\cline{3-6}
                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                        & CI, MRI           & Applications of SVD decomposition                             \\
\cline{3-6}
                              &                          & EPLL \cite{zoran2011learning, hurault2018epll}           & AWGN                        & CI                & A Bayesian patch-based method for whole image restoration                          \\
\cline{3-6}
                              &                          & LRMR \cite{zhang2013hyperspectral}         & AWGN                        & MRI               & A low-rank matrix decomposition model                         \\
\cline{3-6}
                              &                          & GID \cite{xu2018external}          & AWGN                        & CI                & External data guided and internal prior learning              \\
\cline{3-6}
                              &                          & SPTWO \cite{buades2016patch}         & AWGN                        & CV                & NLPCA with optical flow estimation                            \\
\cline{3-6}
                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                        & CI, MSI, HSI      & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                        & CV                & Efficient approximate global patch search                     \\
\cline{3-6}
                              &                          & MCWNNM \cite{xu2017multi}        & AWGN                        & CI                & Extension of WNNM to color images                             \\
\cline{3-6}
                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                        & CI              & A trilateral weighted sparse coding scheme                   \\
\cline{3-6}
                              &                          & VNLB \cite{arias2018video}         & AWGN                        & CV                & A patch-based Bayesian model for video denoising                   \\
\cline{3-6}
                              &                          & NLH \cite{hou2020nlh}      & AWGN                        & CI                & Nonlocal pixel similarity with Haar transform                 \\
\cline{3-6}
                              &                          & AMF \cite{chan2005salt}          & Impulsive                   & CI                & Impulsive noise removal by adaptive median filter             \\
\cline{3-6}
                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                   & CI                & Impulsive noise removal by iterative adaptive fuzzy filter    \\
\cline{3-6}
                              &                          & NoiseClinic \cite{lebrun2015multiscale}         & AWGN and Realistic                   & CI                & A multiscale blind Bayes denoising algorithm    \\
\cline{3-6}
                              &                          & LSM-NLR \cite{huang2017mixed}      & AWGN, Poisson and Impulsive & CV                & Low-rank with laplacian scale mixture modeling                \\
\cline{3-6}
                              &                          & FastHyde \cite{zhuang2018fast}     & AWGN and Poisson            & MSI, HSI          & Low-rank and sparse representation                            \\
\cline{3-6}
                              &                          & NMoG \cite{chen2017denoising}         & AWGN, Stripe and Impulsive  & MSI, HSI          & Low-rank matrix model with non i.i.d Gaussian noise           \\
\cline{3-6}
                              &                          & ODCT \cite{manjon2012new}          & AWGN and Rician             & MRI               & A 3D DCT implementation                                       \\
\cline{3-6}
                              &                          & OBNLM \cite{coupe2008optimized}         & AWGN and Rician             & MRI               & An optimized blockwise NLM Filter                             \\
\cline{3-6}
                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician             & MRI               & Adaptive NLM with spatially varying noise levels              \\
\cline{3-6}
                              &                          & RLMMSE \cite{aja2008noise}       & Rician                      & MRI               & A novel linear minimum mean square error (LMMSE) estimator    \\
\cline{3-6}
                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician             & MRI               & A rotationally invariant version of the NLM filter            \\
\cline{3-6}
                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician             & MRI               & A two stage filter based on NLPCA and PRI-NLM                 \\
\cline{2-6}
                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                        & CI, CV                & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}        & AWGN                        & CV                & Extention of CBM3D to color videos                            \\
\cline{3-6}
                              &                          & LRTA \cite{renard2008denoising}         & AWGN                        & MSI, HSI          & A low Tucker rank tensor decomposition  model                 \\
\cline{3-6}
                              &                          & PARAFAC \cite{liu2012denoising}       & AWGN                        & MSI               & A rank-one CP decomposition model                             \\
\cline{3-6}
                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                        & CV                & Extention of BM3D to color videos using 3D patch              \\
\cline{3-6}
                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                        & MSI, HSI, MRI     & Extention of BM4D to MSI and MRI using 3D patch               \\
\cline{3-6}
                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising, zhang2017denoise}      & AWGN                        & CI, MSI, HSI, MRI & Applications of 4DHOSVD transform                             \\
\cline{3-6}
                              &                          & TDL \cite{peng2014decomposable}           & AWGN                        & MSI, HSI          & A Tucker based tensor dictionary learning algorithm           \\
\cline{3-6}
                              &                          & KTSVD \cite{Zhang2015KTSVD}         & AWGN                        & MSI, HSI          & A t-SVD based tensor dictionary learning algorithm            \\
\cline{3-6}
                              &                          & LRTV \cite{he2015total}         & AWGN                        & MSI, HSI          & Low-rank model with total variation (TV) regularization            \\
\cline{3-6}
                              &                          & ITSReg \cite{xie2016multispectral}        & AWGN                        & MSI, HSI          & Intrinsic Tensor Sparsity Regularization                      \\
\cline{3-6}
                              &                          & LLRT \cite{chang2017hyper}        & AWGN                        & CI, MSI          & low-rank tensor with hyper-laplacian regularization                      \\
\cline{3-6}
                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                        & MSI, HSI          & Low Tucker rank decomposition with total variation            \\
\cline{3-6}
                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                        & CI                & A weighted rank-one CP decomposition model                    \\
\cline{3-6}
                              &                          & ILR-HOSVD \cite{lv2019denoising}    & AWGN                        & MRI               & A recursive low Tucker rank model with rank estimation        \\
\cline{3-6}
                              &                          & MSt-SVD \cite{kong2017new, kong2019color}       & AWGN                        & CI, MRI, MSI, HSI & An efficient one-stage t-SVD implementation  \\
\cline{3-6}
                              &                          & NGMeet \cite{he2019non}       & AWGN                        & MSI, HSI          & Low-rank tensor model with iterative regularization           \\
\cline{3-6}
                              &                          & LTDL \cite{gong2020low}         & AWGN                        & MSI, HSI          & A low-rank tensor dictionary learning method                  \\
\cline{3-6}
                              &                          & NLTA-LSM \cite{dong2015low}      & AWGN and Poisson            & MSI, HSI, MRI     & Low Tucker rank with laplacian scale mixture modeling         \\
\hline
\textbf{Category}                      & \textbf{Network  Architectures}   & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                  \\
\hline
\multirow{32}{*}{\shortstack[l]{DNN \\ methods}}         & \multirow{22}{*}{CNN}    & DnCNN \cite{zhang2017beyond, jiang2018denoising}       & AWGN                        & CI, MRI           & Residual learning and batch normalization                     \\
\cline{3-6}
                              &                          & NLNet \cite{lefkimmiatis2017non}         & AWGN                        & CI                & A nonlocal CNN model                                          \\
\cline{3-6}
                              &                          & UDNet \cite{Lefkimmiatis_2018_CVPR}        & AWGN                        & CI                & A robust and flexible CNN model                               \\
\cline{3-6}
                              &                          & FFDNet \cite{zhang2018ffdnet}       & AWGN                        & CI                & A flexible model with tunable input noise levels              \\
\cline{3-6}
                              &                          & HSID-CNN \cite{yuan2018hyperspectral}      & AWGN                        & MSI, HSI          & A 2D and 3D combined CNN model                                \\
\cline{3-6}
                              &                          & HSI-SDeCNN \cite{maffei2019single}    & AWGN                        & MSI, HSI          & A single CNN model with spatial and spectral information      \\
\cline{3-6}
                              &                          & VNLNet \cite{davy2018non}       & AWGN                        & CV                & The first nonlocal CNN model for video                        \\
\cline{3-6}
                              &                          & ViDeNN \cite{claus2019videnn}       & AWGN                        & CV                & Combination of spatial and temporal filtering with CNN        \\
\cline{3-6}
                              &                          & SADNet \cite{chang2020spatial}        & AWGN                        & CI                & A novel spatial-adaptive CNN model                            \\
\cline{3-6}
                              &                          & FastDVDNet \cite{Tassano_2020_CVPR}   & AWGN                        & CV                & A real-time method without flow estimation                    \\
\cline{3-6}
                              &                          & LIDIA \cite{Vaksman_2020_CVPR_Workshops}        & AWGN                        & CI                & A lightweight denoiser with instance adaptation               \\
\cline{3-6}
                              &                          & DRUNet \cite{zhang2020plug}     & AWGN                   & CI                & A plug-and-play method with deep denoiser prior     \\
\cline{3-6}
                              &                          & HSI-DeNet \cite{chang2018hsi}    & AWGN and Strip              & MSI, HSI          & A CNN method with mixed noise modeling                        \\
\cline{3-6}
                              &                          & Noise2noise \cite{lehtinen2018noise2noise}       & AWGN and Poisson                     & CI              & A CNN model trained only with noisy data.                         \\
\cline{3-6}
                              &                          & VDNet \cite{yue2019variational}        & AWGN and Realistic          & CI                & A variational inference method with noise estimation          \\
\cline{3-6}
                              &                          & CBDNet \cite{guo2019toward}       & Realistic                   & CI                & a convolutional blind denoising network                       \\
\cline{3-6}
                              &                          & PRI-PB-CNN \cite{manjon2018mri}   & AWGN an Rician              & MRI               & Combination of sliding window scheme and 3D CNN               \\
\cline{3-6}
                              &                          & DIDN \cite{yu2019deep}         & AWGN and Realistic          & CI                & A deep iterative down-up CNN model                            \\
\cline{3-6}
                              &                          & DRDN \cite{song2019dynamic}         & Realistic                   & CI                & A dynamic residual dense network model                        \\
\cline{3-6}
                              &                          & FCCF \cite{yue2019high}         & AWGN and Realistic          & CI                & Fusion of collaborative filtering and CNN                     \\
\cline{3-6}
                              &                          & DBF \cite{chen2019real}          & AWGN and Realistic          & CI                & Integration of CNN into a boosting algorithm                    \\
\cline{3-6}
                              &                          & RIDNet \cite{anwar2019real}       & AWGN and Realistic          & CI                & A single stage model with feature attention                   \\
\cline{3-6}
                              &                          & AINDNet \cite{Kim_2020_CVPR}      & AWGN and Realistic          & CI                & Transfer learning with adaptive instance normalization        \\
\cline{3-6}
                              &                          & QRNN3D \cite{wei20203}          & AWGN and Stripe                   & MSI, HSI                & A deep recurrent neural network model with 3D convolution           \\
\cline{3-6}
                              &                          & CycleISP \cite{zamir2020cycleisp}     & Realistic                   & CI                & A camera pipeline model in forward and reverse directions     \\
\cline{3-6}
                              &                          & MIRNet \cite{Zamir2020MIRNet}        & Realistic                   & CI                & A multi-scale model with parallel convolution streams                   \\
\cline{2-6}
                              & \multirow{10}{*}{Others} & MLP \cite{burger2012image}          & AWGN                        & CI                & A multilayer perceptron model                                 \\
\cline{3-6}
                              &                          & TNRD \cite{chen2016trainable}         & AWGN                        & CI                & A trainable nonlinear difussion model                         \\
\cline{3-6}
                              &                          & SCGAN \cite{yan2019unsupervised}        & AWGN                        & CI                & Unsupervised modeling with self-consistent GAN                \\
\cline{3-6}
                              &                          & ADRN \cite{zhao2020adrn}          & AWGN                   & MSI, HSI                & A deep residual network model with channel attention scheme            \\
%\cline{3-6}
%                              &                          & LLRefineNet \cite{jiang2018deep}  & AWGN and Impulsive          & CI                & Encoder-decoder network with skip connections                 \\
\cline{3-6}
                              &                          & GCBD \cite{Chen_2018_CVPR}         & AWGN and Realistic          & CI                & A GAN-based blind denoiser                               \\
\cline{3-6}
                              &                          & DnGAN \cite{yeh2018image}        & AWGN and Blur               & CI                & GAN with  maximum a posteriori (MAP) framework                \\
\cline{3-6}
                              &                          & RED-WGAN \cite{ran2019denoising}     & AWGN and Rician             & MRI               & A residual encoder decoder Wasserstein GAN model              \\
\cline{3-6}
                              &                          & ADGAN \cite{Lin_2019_CVPR_Workshops}        & Realistic                   & CI                & Attentive GAN with noise domain adaptation                    \\
\cline{3-6}
                              &                          & MIFCN \cite{abbasi2019three}        & Realistic                   & MRI               & A fully convolutional network model                           \\
\cline{3-6}
                              &                          & SGN \cite{gu2019self}          & Realistic                   & CI                & A self-guided network with top-down architecture              \\
\cline{3-6}
                              &                          & DANet \cite{yue2020dual}        & Realistic                   & CI                & A Bayesian framework for noise removal and generation.                    \\
\hline
\end{tabular}
}
\label{Table_Method_all}
\end{table*}



==> Table_Method_all_new.tex <==
\begin{table*}[htbp]
\scriptsize
\centering
\caption{Related multi-dimensional image denoising methods with different noise modeling techniques and applications. 'CI': color image, 'CV': color video, 'MSI': multispectral imaging, 'HSI': hyperspectral imaging, 'MRI': magnetic resonance imaging.}
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Category}                      & \textbf{Representation}           & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                     \\
\hline
\multirow{41}{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{24}{*}{Matrix} & AWT \cite{donoho1995noising, huang2005color,othman2006noise}           & AWGN                        & CI, MSI, HSI      & Adaptive wavelet thresholding with thresholding techniques    \\
\cline{3-6}
                              &                          & DCT \cite{yaroslavsky1996local, foi2007pointwise}           & AWGN                        & CI                & high-quality denoising with discrete cosine transform (DCT)   \\
\cline{3-6}
                              &                          & NLM \cite{buades2005review, dai2013multichannel}           & AWGN                        & CI                & NLM algorithm with Gaussian kernels                           \\
\cline{3-6}
                              &                          & K-SVD \cite{mairal2007sparse, fu2015adaptive}           & AWGN                        & CI, MSI               & 3D wavelet over-complete dictionary learning and sparse coding                \\
\cline{3-6}
                              &                          & TCVD \cite{liu2010high}         & AWGN                        & CV                & Combination of robust optical flow with NLM                   \\
\cline{3-6}
                              &                          & NLPCA \cite{zhang2010two, dong2012nonlocal, phophalia20173d}        & AWGN                        & CI, MRI           & Applications of SVD decomposition                             \\
\cline{3-6}
                              &                          & EPLL \cite{zoran2011learning, hurault2018epll}           & AWGN                        & CI                & A Bayesian patch-based method for whole image restoration                          \\
\cline{3-6}
                              &                          & LRMR \cite{zhang2013hyperspectral}         & AWGN                        & MRI               & A low-rank matrix decomposition model                         \\
\cline{3-6}
                              &                          & GID \cite{xu2018external}          & AWGN                        & CI                & External data guided and internal prior learning              \\
\cline{3-6}
                              &                          & SPTWO \cite{buades2016patch}         & AWGN                        & CV                & NLPCA with optical flow estimation                            \\
\cline{3-6}
                              &                          & LSCD \cite{rizkinia2016local}         & AWGN                        & CI, MSI, HSI      & Spectral component decomposition based on line feature        \\
%\cline{3-6}
%                              &                          & Global-Search \cite{ehret2017global} & AWGN                        & CV                & Efficient approximate global patch search                     \\
\cline{3-6}
                              &                          & MCWNNM \cite{xu2017multi}        & AWGN                        & CI                & Extension of WNNM to color images                             \\
\cline{3-6}
                              &                          & TWSC \cite{xu2018trilateral}         & AWGN                        & CI              & A trilateral weighted sparse coding scheme                   \\
\cline{3-6}
                              &                          & VNLB \cite{arias2018video}         & AWGN                        & CV                & A patch-based Bayesian model for video denoising                   \\
\cline{3-6}
                              &                          & NLH \cite{hou2020nlh}      & AWGN                        & CI                & Nonlocal pixel similarity with Haar transform                 \\
\cline{3-6}
                              &                          & AMF \cite{chan2005salt}          & Impulsive                   & CI                & Impulsive noise removal by adaptive median filter             \\
%\cline{3-6}
%                              &                          & IAFF \cite{ahmed2013removal}         & Impulsive                   & CI                & Impulsive noise removal by iterative adaptive fuzzy filter    \\
\cline{3-6}
                              &                          & NoiseClinic \cite{lebrun2015multiscale}         & AWGN and Realistic                   & CI                & A multiscale blind Bayes denoising algorithm    \\
\cline{3-6}
                              &                          & LSM-NLR \cite{huang2017mixed}      & AWGN, Poisson and Impulsive & CV                & Low-rank with laplacian scale mixture modeling                \\
\cline{3-6}
                              &                          & FastHyde \cite{zhuang2018fast}     & AWGN and Poisson            & MSI, HSI          & Low-rank and sparse representation                            \\
\cline{3-6}
                              &                          & NMoG \cite{chen2017denoising}         & AWGN, Stripe and Impulsive  & MSI, HSI          & Low-rank matrix model with non i.i.d Gaussian noise           \\
\cline{3-6}
                              &                          & ODCT \cite{manjon2012new}          & AWGN and Rician             & MRI               & A 3D DCT implementation                                       \\
\cline{3-6}
                              &                          & OBNLM \cite{coupe2008optimized}         & AWGN and Rician             & MRI               & An optimized blockwise NLM Filter                             \\
\cline{3-6}
                              &                          & AOBNLM \cite{manjon2010adaptive}       & AWGN and Rician             & MRI               & Adaptive NLM with spatially varying noise levels              \\
\cline{3-6}
                              &                          & RLMMSE \cite{aja2008noise}       & Rician                      & MRI               & A novel linear minimum mean square error (LMMSE) estimator    \\
\cline{3-6}
                              &                          & PRI-NLM \cite{manjon2012new}      & AWGN and Rician             & MRI               & A rotationally invariant version of the NLM filter            \\
\cline{3-6}
                              &                          & PRI-NLPCA \cite{manjon2015mri}    & AWGN and Rician             & MRI               & A two stage filter based on NLPCA and PRI-NLM                 \\
\cline{2-6}
                              & \multirow{17}{*}{Tensor} & CBM3D \cite{dabov2007color}        & AWGN                        & CI, CV                & BM3D with oppenent and YUV color mode transforms              \\
%\cline{3-6}
%                              &                          & CVBM3D \cite{dabov2007video}        & AWGN                        & CV                & Extention of CBM3D to color videos                            \\
\cline{3-6}
                              &                          & LRTA \cite{renard2008denoising}         & AWGN                        & MSI, HSI          & A low Tucker rank tensor decomposition  model                 \\
\cline{3-6}
                              &                          & PARAFAC \cite{liu2012denoising}       & AWGN                        & MSI               & A rank-one CP decomposition model                             \\
\cline{3-6}
                              &                          & VBM4D \cite{maggioni2012video}        & AWGN                        & CV                & Extention of BM3D to color videos using 3D patch              \\
\cline{3-6}
                              &                          & BM4D \cite{maggioni2012nonlocal}         & AWGN                        & MSI, HSI, MRI     & Extention of BM4D to MSI and MRI using 3D patch               \\
\cline{3-6}
                              &                          & 4DHOSVD \cite{rajwade2012image, zhang2015denoising, zhang2017denoise}      & AWGN                        & CI, MSI, HSI, MRI & Applications of 4DHOSVD transform                             \\
\cline{3-6}
                              &                          & TDL \cite{peng2014decomposable}           & AWGN                        & MSI, HSI          & A Tucker based tensor dictionary learning algorithm           \\
\cline{3-6}
                              &                          & KTSVD \cite{Zhang2015KTSVD}         & AWGN                        & MSI, HSI          & A t-SVD based tensor dictionary learning algorithm            \\
\cline{3-6}
                              &                          & LRTV \cite{he2015total}         & AWGN                        & MSI, HSI          & Low-rank model with total variation (TV) regularization            \\
\cline{3-6}
                              &                          & ITSReg \cite{xie2016multispectral}        & AWGN                        & MSI, HSI          & Intrinsic Tensor Sparsity Regularization                      \\
\cline{3-6}
                              &                          & LLRT \cite{chang2017hyper}        & AWGN                        & CI, MSI          & low-rank tensor with hyper-laplacian regularization                      \\
\cline{3-6}
                              &                          & LLRGTV \cite{He2018LLRGTV}       & AWGN                        & MSI, HSI          & Low Tucker rank decomposition with total variation            \\
\cline{3-6}
                              &                          & WTR1 \cite{wu2018weighted}         & AWGN                        & CI                & A weighted rank-one CP decomposition model                    \\
\cline{3-6}
                              &                          & ILR-HOSVD \cite{lv2019denoising}    & AWGN                        & MRI               & A recursive low Tucker rank model with rank estimation        \\
\cline{3-6}
                              &                          & MSt-SVD \cite{kong2017new, kong2019color}       & AWGN                        & CI, MRI, MSI, HSI & An efficient one-stage t-SVD implementation  \\
\cline{3-6}
                              &                          & NGMeet \cite{he2019non}       & AWGN                        & MSI, HSI          & Low-rank tensor model with iterative regularization           \\
\cline{3-6}
                              &                          & LTDL \cite{gong2020low}         & AWGN                        & MSI, HSI          & A low-rank tensor dictionary learning method                  \\
\cline{3-6}
                              &                          & NLTA-LSM \cite{dong2015low}      & AWGN and Poisson            & MSI, HSI, MRI     & Low Tucker rank with laplacian scale mixture modeling         \\
\hline
\textbf{Category}                      & \textbf{Network  Architectures}   & \textbf{Methods}       & \textbf{Noise Modeling}  & \textbf{Applications}      & \textbf{Key Words}                                                  \\
\hline
\multirow{32}{*}{\shortstack[l]{DNN \\ methods}}         & \multirow{29}{*}{CNN/NN}   & MLP \cite{burger2012image}          & AWGN                        & CI                & A multilayer perceptron model                                 \\

\cline{3-6}
                              &                          & TNRD \cite{chen2016trainable}         & AWGN                        & CI                & A trainable nonlinear difussion model                         \\
\cline{3-6}
                              &                          & DnCNN \cite{zhang2017beyond, jiang2018denoising}          & AWGN                        & CI, MRI                 & CNN with Residual learning and batch normalization                       \\
\cline{3-6}
                              &                          & NLNet \cite{lefkimmiatis2017non}         & AWGN                        & CI                & A nonlocal CNN model                                          \\
\cline{3-6}
                              &                          & UDNet \cite{Lefkimmiatis_2018_CVPR}        & AWGN                        & CI                & A robust and flexible CNN model                               \\
\cline{3-6}
                              &                          & FFDNet \cite{zhang2018ffdnet}       & AWGN                        & CI                & A flexible model with tunable input noise levels              \\
\cline{3-6}
                              &                          & HSID-CNN \cite{yuan2018hyperspectral}      & AWGN                        & MSI, HSI          & A 2D and 3D combined CNN model                                \\
\cline{3-6}
                              &                          & HSI-SDeCNN \cite{maffei2019single}    & AWGN                        & MSI, HSI          & A single CNN model with spatial and spectral information      \\
\cline{3-6}
                              &                          & VNLNet \cite{davy2018non}       & AWGN                        & CV                & The first nonlocal CNN model for video                        \\
\cline{3-6}
                              &                          & ViDeNN \cite{claus2019videnn}       & AWGN                        & CV                & Combination of spatial and temporal filtering with CNN        \\
\cline{3-6}
                              &                          & SADNet \cite{chang2020spatial}        & AWGN                        & CI                & A novel spatial-adaptive CNN model                            \\
\cline{3-6}
                              &                          & FastDVDNet \cite{Tassano_2020_CVPR}   & AWGN                        & CV                & A real-time method without flow estimation                    \\
\cline{3-6}
                              &                          & LIDIA \cite{Vaksman_2020_CVPR_Workshops}        & AWGN                        & CI                & A lightweight denoiser with instance adaptation               \\
\cline{3-6}
                              &                          & DRUNet \cite{zhang2020plug}     & AWGN                   & CI                & A plug-and-play method with deep denoiser prior     \\
\cline{3-6}
                              &                          & ADRN \cite{zhao2020adrn}          & AWGN                   & MSI, HSI                & A deep residual network model with channel attention scheme            \\
\cline{3-6}
                              &                          & HSI-DeNet \cite{chang2018hsi}    & AWGN and Strip              & MSI, HSI          & A CNN method with mixed noise modeling                        \\
\cline{3-6}
                              &                          & Noise2noise \cite{lehtinen2018noise2noise}       & AWGN and Poisson                     & CI              & A CNN model trained only with noisy data.                         \\
\cline{3-6}
                              &                          & VDNet \cite{yue2019variational}        & AWGN and Realistic          & CI                & A variational inference method with noise estimation          \\
\cline{3-6}
                              &                          & CBDNet \cite{guo2019toward}       & Realistic                   & CI                & a convolutional blind denoising network                       \\
\cline{3-6}
                              &                          & PRI-PB-CNN \cite{manjon2018mri}   & AWGN an Rician              & MRI               & Combination of sliding window scheme and 3D CNN               \\
\cline{3-6}
                              &                          & MIFCN \cite{abbasi2019three}        & Realistic                   & MRI               & A fully convolutional network model                           \\
\cline{3-6}
                              &                          & DIDN \cite{yu2019deep}         & AWGN and Realistic          & CI                & A deep iterative down-up CNN model                            \\
\cline{3-6}
                              &                          & DRDN \cite{song2019dynamic}         & Realistic                   & CI                & A dynamic residual dense network model                        \\
\cline{3-6}
                              &                          & FCCF \cite{yue2019high}         & AWGN and Realistic          & CI                & Fusion of collaborative filtering and CNN                     \\
\cline{3-6}
                              &                          & DBF \cite{chen2019real}          & AWGN and Realistic          & CI                & Integration of CNN into a boosting algorithm                    \\
\cline{3-6}
                              &                          & RIDNet \cite{anwar2019real}       & AWGN and Realistic          & CI                & A single stage model with feature attention                   \\
\cline{3-6}
                              &                          & AINDNet \cite{Kim_2020_CVPR}      & AWGN and Realistic          & CI                & Transfer learning with adaptive instance normalization        \\
\cline{3-6}
                              &                          & QRNN3D \cite{wei20203}          & AWGN and Stripe                   & MSI, HSI                & A deep recurrent neural network model with 3D convolution           \\
\cline{3-6}
                              &                          & CycleISP \cite{zamir2020cycleisp}     & Realistic                   & CI                & A camera pipeline model in forward and reverse directions     \\
\cline{3-6}
                              &                          & MIRNet \cite{Zamir2020MIRNet}        & Realistic                   & CI                & A multi-scale model with parallel convolution streams                   \\
\cline{2-6}
                              & \multirow{8}{*}{CNN + GAN} & GCBD \cite{Chen_2018_CVPR}         & AWGN and Realistic          & CI                & A GAN-based blind denoiser                               \\
\cline{3-6}
                              &                          & SCGAN \cite{yan2019unsupervised}        & AWGN                        & CI                & Unsupervised modeling with self-consistent GAN                \\
\cline{3-6}
                              &                          & DnGAN \cite{yeh2018image}        & AWGN and Blur               & CI                & GAN with  maximum a posteriori (MAP) framework                \\
\cline{3-6}
                              &                          & RED-WGAN \cite{ran2019denoising}     & AWGN and Rician             & MRI               & A residual encoder decoder Wasserstein GAN model              \\
\cline{3-6}
                              &                          & ADGAN \cite{Lin_2019_CVPR_Workshops}        & Realistic                   & CI                & Attentive GAN with noise domain adaptation                    \\
\cline{3-6}
                              &                          & SGN \cite{gu2019self}          & Realistic                   & CI                & A self-guided network with top-down architecture              \\
\cline{3-6}
                              &                          & DANet \cite{yue2020dual}        & Realistic                   & CI                & A Bayesian framework for noise removal and generation.                    \\
\hline
\end{tabular}
}
\label{Table_Method_all}
\end{table*}



==> Table_Results_Color_Video_all.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Average PSNR and SSIM values of compared methods on four video datasets (sRGB space). The average computational time (s) is calculated based on the Set8 dataset with noise level $\sigma = 50$. `-' means the results are not available due to high computational cost or other issues.}
%  \renewcommand{\arraystretch}{0.668}
%  \scalebox{0.918}{
%    \begin{tabular}{ccccccccccccccccc}
%    \toprule
%    \multirow{3}[4]{*}{Dataset} & \multirow{3}[4]{*}{$\sigma$} & \multicolumn{6}{c|}{Traditional denoisers}   & \multicolumn{9}{c}{DNN methods} \\
%    \cmidrule{3-17}          &       & CVMSt-SVD & RTA-LSM & VBM4D1 & VBM4D2 & VIDOSAT & DVDNet & FastDVDNet & FloRNN & MAP-VDNet & MMNet & RVRT  & RFR   & UDVD  & ViDeNN & VNLNet \\
%              &     &  \cite{kong2019color}   &   \cite{dong2018robust}  &     \cite{maggioni2012video}   &   \cite{maggioni2012video}    &    \cite{wen2018vidosat}   &  \cite{tassano2019dvdnet}   &  \cite{Tassano_2020_CVPR}   &  \cite{li2022unidirectional}     &  \cite{sun2021deep}     &    \cite{chen2021multiframe}   &  \cite{liang2022recurrent} &  \cite{lee2021restore}   &    \cite{sheth2021unsupervised}   &  \cite{claus2019videnn}    &  \cite{davy2019non}  \\
%    \midrule
%    \multirow{10}[20]{*}{Set8} & \multirow{2}[4]{*}{10} & 36.25  & 36.36  & 35.69  & 35.96  & 34.75  & 36.04  & 36.38  & 37.55  & -     & 37.28  & \textcolor{blue}{\textbf{37.58}} & -  & 32.30  & 34.80  & 37.28  \\
%\cmidrule{3-17}          &       & 0.9453  & 0.9474  & 0.9342  & 0.9405  & 0.9244  & 0.9487  & 0.9513  & 0.9617  & -     & 0.9595  & \textcolor{blue}{\textbf{0.9626}} & - & 0.9081  & 0.9114  & 0.9584  \\
%\cmidrule{2-17}          & \multirow{2}[4]{*}{20} & 32.50  & 32.87  & 31.56  & 32.10  & 31.12  & 33.42  & 33.35  & 34.65  & -     & 34.11  & \textcolor{blue}{\textbf{34.85}} & 30.95  & 32.24  & 28.34  & 34.02  \\
%\cmidrule{3-17}          &       & 0.8891  & 0.8977  & 0.8485  & 0.8731  & 0.8571  & 0.9151  & 0.9159  & 0.9347  & -     & 0.9270  & \textcolor{blue}{\textbf{0.9383}} & 0.8321  & 0.8937  & 0.7619  & 0.9243  \\
%\cmidrule{2-17}          & \multirow{2}[4]{*}{30} & 30.38  & 30.84  & 29.20  & 29.90  & -     & 31.70  & 31.59  & 32.94  & -     & 32.27  & \textcolor{blue}{\textbf{33.31}} & 30.18  & 31.02  & 23.07  & - \\
%\cmidrule{3-17}          &       & 0.8369  & 0.8542  & 0.7626  & 0.8081  & -     & 0.8825  & 0.8848  & 0.9100  & -     & 0.8973  & \textcolor{blue}{\textbf{0.9173}} & 0.8299  & 0.8653  & 0.5719  & - \\
%\cmidrule{2-17}          & \multirow{2}[4]{*}{40} & 28.92  & 29.41  & 27.56  & 28.37  & 27.67  & 30.45  & 30.36  & 31.71  & -     & 30.98  & \textcolor{blue}{\textbf{32.21}} & 28.89  & 29.46  & 18.89  & 30.72  \\
%\cmidrule{3-17}          &       & 0.7871  & 0.8170  & 0.6820  & 0.7482  & 0.7526  & 0.8528  & 0.8569  & 0.8869  & -     & 0.8702  & \textcolor{blue}{\textbf{0.8981}} & 0.7891  & 0.8221  & 0.4070  & 0.8596  \\
%\cmidrule{2-17}          & \multirow{2}[4]{*}{50} & 27.80  & 28.34  & 26.29  & 27.20  & -     & 29.45  & 29.42  & 30.75  & 26.48  & 29.99  & \textcolor{blue}{\textbf{31.32}} & 26.57  & 27.89  & 15.42  & - \\
%\cmidrule{3-17}          &       & 0.7392  & 0.7860  & 0.6086  & 0.6935  & -     & 0.8264  & 0.8317  & 0.8653  & 0.7220  & 0.8452  & \textcolor{blue}{\textbf{0.8800}} & 0.6461  & 0.7654  & 0.2379  & - \\
%    \midrule
%    \multirow{10}[20]{*}{DAVIS} & \multirow{2}[4]{*}{10} & 38.49  & -     & 37.57  & 37.97  & -     & 37.70  & 38.33  & 38.92  & -     & 38.25  & \textcolor{blue}{\textbf{39.07}} & -  & 33.65  & 35.90  & 38.68  \\
%\cmidrule{3-17}          &       & 0.9611  & -     & 0.9475  & 0.9555  & -     & 0.9600  & 0.9631  & 0.9680  & -     & 0.9639  & \textcolor{blue}{\textbf{0.9691}} & -  & 0.9204  & 0.9253  & 0.9653  \\
%\cmidrule{2-17}          & \multirow{2}[4]{*}{20} & 34.73  & -     & 33.33  & 34.03  & -     & 35.34  & 35.52  & 36.43  & -     & 35.63  & \textcolor{blue}{\textbf{36.69}} & 33.09  & 33.95  & 30.20  & 35.84  \\
%\cmidrule{3-17}          &       & 0.9147  & -     & 0.8709  & 0.9000  & -     & 0.9361  & 0.9364  & 0.9493  & -     & 0.9384  & \textcolor{blue}{\textbf{0.9520}} & 0.8765  & 0.9154  & 0.8124  & 0.9398  \\
%\cmidrule{2-17}          & \multirow{2}[4]{*}{30} & 32.53  & -     & 30.82  & 31.71  & -     & 33.84  & 33.88  & 35.06  & -     & 34.06  & \textcolor{blue}{\textbf{35.47}} & 31.93  & 32.85  & 24.75  & - \\
%\cmidrule{3-17}          &       & 0.8665  & -     & 0.7866  & 0.8415  & -     & 0.9140  & 0.9134  & 0.9341  & -     & 0.9166  & \textcolor{blue}{\textbf{0.9394}} & 0.8564  & 0.8918  & 0.6586  & - \\
%\cmidrule{2-17}          & \multirow{2}[4]{*}{40} & 30.96  & -     & 29.02  & 30.06  & -     & 32.70  & 32.71  &       & -     & 32.93  & \textcolor{blue}{\textbf{34.58}} & 30.22  & 31.29  & 20.60  & 33.01  \\
%\cmidrule{3-17}          &       & 0.8182  & -     & 0.7036  & 0.7838  & -     & 0.8931  & 0.8926  &       & -     & 0.8969  & \textcolor{blue}{\textbf{0.9280}} & 0.7997  & 0.8545  & 0.5121  & 0.8959  \\
%\cmidrule{2-17}          & \multirow{2}[4]{*}{50} & 29.72  & -     & 27.61  & 28.78  & -     & 31.76  & 31.79  & 33.18  & 28.35  & 32.04  & \textcolor{blue}{\textbf{33.85}} & 27.22  & 29.65  & 17.01  & - \\
%\cmidrule{3-17}          &       & 0.7701  & -     & 0.6270  & 0.7287  & -     & 0.8730  & 0.8735  & 0.9054  & 0.7911  & 0.8788  & \textcolor{blue}{\textbf{0.9170}} & 0.6350  & 0.8033  & 0.3429  & - \\
%    \midrule
%    \multirow{2}[4]{*}{CRVD} & \multirow{2}[4]{*}{-} & 36.66  & -     & 34.67  & 34.14  & 34.16  & 34.50  & 35.84  & 36.66  & 23.16  & 31.01  & \textcolor{blue}{\textbf{36.94}} & 31.30  & -     & 32.31  & 36.11  \\
%\cmidrule{3-17}          &       & 0.9463  & -     & 0.9224  & 0.9079  & 0.9384  & 0.9493  & 0.9306  &  \textcolor{blue}{\textbf{0.9605}} & 0.7327  & 0.7551  & 0.9559  & 0.7785  & -     & 0.8449  & 0.9449  \\
%    \midrule
%    \multirow{2}[4]{*}{IOCV} & \multirow{2}[4]{*}{-} & 38.22  & -     & 38.65  & \textcolor{blue}{\textbf{38.76}} & -     & 38.53  & 37.57  & 38.64  & 35.52  & 21.33  & 38.50  & 31.46  & 35.02  & 36.13  & \textcolor{blue}{\textbf{38.76}} \\
%\cmidrule{3-17}          &       & 0.9736  & -     & 0.9763  & \textcolor{blue}{\textbf{0.9765}} & -     & 0.9754  & 0.9699  & 0.9743  & 0.9313  & 0.4962  & 0.9672  & 0.8346  & 0.9660  & 0.9506  & \textcolor{blue}{\textbf{0.9765}} \\
%    \midrule
%    Implementation & -     & MEX & MATLAB &  MEX &  MEX & C++   & Python & Python & Python & Python & Python & Python & Python & Python & Python & Python
% \\
%    \midrule
%    Time (s) & -     & 888.0  & $>1$h  & 920.9  & 2076.0  & 4313.7  & 818.8  & \textcolor{blue}{\textbf{6.6}} & 53.9  & 77.2  & 30.1  & 93.3  & 37.8  & 163.4  & 19.0  & 217.1  \\
%    \bottomrule
%    \end{tabular}}%
%  \label{Table_Results_Color_video_all}%
%\end{table*}%


\begin{table*}[htbp]
\tiny
  \centering
  \caption{Average PSNR and SSIM values of compared methods on four video datasets (sRGB space). The average computational time (s) is calculated based on the Set8 dataset with noise level $\sigma = 50$. `-' means the results are not available due to high computational cost or other issues.}
  \renewcommand{\arraystretch}{0.668}
  \scalebox{0.938}{
    \begin{tabular}{ccccccccccccccccc}
    \toprule
    \multirow{3}[4]{*}{Dataset} & \multirow{3}[4]{*}{$\sigma$} & \multicolumn{6}{c|}{Traditional denoisers}   & \multicolumn{9}{c}{DNN methods} \\
    \cmidrule{3-17}          &       & CVMSt-SVD & RTA-LSM & VBM4D1 & VBM4D2 & VIDOSAT & DVDNet & FastDVDNet & FloRNN & MAP-VDNet & MMNet & RVRT  & RFR   & UDVD  & ViDeNN & VNLNet \\
              &     &  \cite{kong2019color}   &   \cite{dong2018robust}  &     \cite{maggioni2012video}   &   \cite{maggioni2012video}    &    \cite{wen2018vidosat}   &  \cite{tassano2019dvdnet}   &  \cite{Tassano_2020_CVPR}   &  \cite{li2022unidirectional}     &  \cite{sun2021deep}     &    \cite{chen2021multiframe}   &  \cite{liang2022recurrent} &  \cite{lee2021restore}   &    \cite{sheth2021unsupervised}   &  \cite{claus2019videnn}    &  \cite{davy2019non}  \\
    \midrule
    \multirow{10}[20]{*}{Set8} & \multirow{2}[4]{*}{10} & 36.25  & 36.36  & 35.69  & 35.96  & 34.75  & 36.04  & 36.38  & 37.55  & -     & 37.28  & {\textbf{37.58}} & -  & 32.30  & 34.80  & 37.28  \\
\cmidrule{3-17}          &       & 0.9453  & 0.9474  & 0.9342  & 0.9405  & 0.9244  & 0.9487  & 0.9513  & 0.9617  & -     & 0.9595  & {\textbf{0.9626}} & - & 0.9081  & 0.9114  & 0.9584  \\
\cmidrule{2-17}          & \multirow{2}[4]{*}{20} & 32.50  & 32.87  & 31.56  & 32.10  & 31.12  & 33.42  & 33.35  & 34.65  & -     & 34.11  & {\textbf{34.85}} & 30.95  & 32.24  & 28.34  & 34.02  \\
\cmidrule{3-17}          &       & 0.8891  & 0.8977  & 0.8485  & 0.8731  & 0.8571  & 0.9151  & 0.9159  & 0.9347  & -     & 0.9270  & {\textbf{0.9383}} & 0.8321  & 0.8937  & 0.7619  & 0.9243  \\
\cmidrule{2-17}          & \multirow{2}[4]{*}{30} & 30.38  & 30.84  & 29.20  & 29.90  & -     & 31.70  & 31.59  & 32.94  & -     & 32.27  & {\textbf{33.31}} & 30.18  & 31.02  & 23.07  & - \\
\cmidrule{3-17}          &       & 0.8369  & 0.8542  & 0.7626  & 0.8081  & -     & 0.8825  & 0.8848  & 0.9100  & -     & 0.8973  & {\textbf{0.9173}} & 0.8299  & 0.8653  & 0.5719  & - \\
\cmidrule{2-17}          & \multirow{2}[4]{*}{40} & 28.92  & 29.41  & 27.56  & 28.37  & 27.67  & 30.45  & 30.36  & 31.71  & -     & 30.98  & {\textbf{32.21}} & 28.89  & 29.46  & 18.89  & 30.72  \\
\cmidrule{3-17}          &       & 0.7871  & 0.8170  & 0.6820  & 0.7482  & 0.7526  & 0.8528  & 0.8569  & 0.8869  & -     & 0.8702  & {\textbf{0.8981}} & 0.7891  & 0.8221  & 0.4070  & 0.8596  \\
\cmidrule{2-17}          & \multirow{2}[4]{*}{50} & 27.80  & 28.34  & 26.29  & 27.20  & -     & 29.45  & 29.42  & 30.75  & 26.48  & 29.99  & {\textbf{31.32}} & 26.57  & 27.89  & 15.42  & - \\
\cmidrule{3-17}          &       & 0.7392  & 0.7860  & 0.6086  & 0.6935  & -     & 0.8264  & 0.8317  & 0.8653  & 0.7220  & 0.8452  & {\textbf{0.8800}} & 0.6461  & 0.7654  & 0.2379  & - \\
    \midrule
    \multirow{10}[20]{*}{DAVIS} & \multirow{2}[4]{*}{10} & 38.49  & -     & 37.57  & 37.97  & -     & 37.70  & 38.33  & 38.92  & -     & 38.25  & {\textbf{39.07}} & -  & 33.65  & 35.90  & 38.68  \\
\cmidrule{3-17}          &       & 0.9611  & -     & 0.9475  & 0.9555  & -     & 0.9600  & 0.9631  & 0.9680  & -     & 0.9639  & {\textbf{0.9691}} & -  & 0.9204  & 0.9253  & 0.9653  \\
\cmidrule{2-17}          & \multirow{2}[4]{*}{20} & 34.73  & -     & 33.33  & 34.03  & -     & 35.34  & 35.52  & 36.43  & -     & 35.63  & {\textbf{36.69}} & 33.09  & 33.95  & 30.20  & 35.84  \\
\cmidrule{3-17}          &       & 0.9147  & -     & 0.8709  & 0.9000  & -     & 0.9361  & 0.9364  & 0.9493  & -     & 0.9384  & {\textbf{0.9520}} & 0.8765  & 0.9154  & 0.8124  & 0.9398  \\
\cmidrule{2-17}          & \multirow{2}[4]{*}{30} & 32.53  & -     & 30.82  & 31.71  & -     & 33.84  & 33.88  & 35.06  & -     & 34.06  & {\textbf{35.47}} & 31.93  & 32.85  & 24.75  & - \\
\cmidrule{3-17}          &       & 0.8665  & -     & 0.7866  & 0.8415  & -     & 0.9140  & 0.9134  & 0.9341  & -     & 0.9166  & {\textbf{0.9394}} & 0.8564  & 0.8918  & 0.6586  & - \\
\cmidrule{2-17}          & \multirow{2}[4]{*}{40} & 30.96  & -     & 29.02  & 30.06  & -     & 32.70  & 32.71  &       & -     & 32.93  & {\textbf{34.58}} & 30.22  & 31.29  & 20.60  & 33.01  \\
\cmidrule{3-17}          &       & 0.8182  & -     & 0.7036  & 0.7838  & -     & 0.8931  & 0.8926  &       & -     & 0.8969  & {\textbf{0.9280}} & 0.7997  & 0.8545  & 0.5121  & 0.8959  \\
\cmidrule{2-17}          & \multirow{2}[4]{*}{50} & 29.72  & -     & 27.61  & 28.78  & -     & 31.76  & 31.79  & 33.18  & 28.35  & 32.04  & {\textbf{33.85}} & 27.22  & 29.65  & 17.01  & - \\
\cmidrule{3-17}          &       & 0.7701  & -     & 0.6270  & 0.7287  & -     & 0.8730  & 0.8735  & 0.9054  & 0.7911  & 0.8788  & {\textbf{0.9170}} & 0.6350  & 0.8033  & 0.3429  & - \\
    \midrule
    \multirow{2}[4]{*}{CRVD} & \multirow{2}[4]{*}{-} & 36.66  & -     & 34.66  & 34.14  & 34.16  & 34.50  & 35.84  & 36.66  & -  & -  & {\textbf{36.94}} & 31.30  & -     & 32.31  & 36.11  \\
\cmidrule{3-17}          &       & 0.9463  & -     & 0.9224  & 0.9079  & 0.9384  & 0.9493  & 0.9306  &  {\textbf{0.9605}} & -  & -  & 0.9559  & 0.7785  & -     & 0.8449  & 0.9449  \\
    \midrule
    \multirow{2}[4]{*}{IOCV} & \multirow{2}[4]{*}{-} & 38.22  & -     & 38.65  & {\textbf{38.76}} & -     & 38.53  & 37.57  & 38.64  & 35.52  & -  & 38.50  & 31.46  & 35.02  & 36.13  & {\textbf{38.76}} \\
\cmidrule{3-17}          &       & 0.9736  & -     & 0.9763  & {\textbf{0.9765}} & -     & 0.9754  & 0.9699  & 0.9743  & 0.9313  & -  & 0.9672  & 0.8346  & 0.9660  & 0.9506  & {\textbf{0.9765}} \\
    \midrule
    Implementation & -     & MEX & MATLAB &  MEX &  MEX & C++   & Python & Python & Python & Python & Python & Python & Python & Python & Python & Python
 \\
    \midrule
    Time (s) & -     & 888.0  & $>1$h  & 920.9  & 2076.0  & 4313.7  & 818.8  & {\textbf{6.6}} & 53.9  & 77.2  & 30.1  & 93.3  & 37.8  & 163.4  & 19.0  & 217.1  \\
    \bottomrule
    \end{tabular}}%
  \label{Table_Results_Color_video_all}%
\end{table*}%




==> Table_Results_Color_image_all_detailed.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%  \centering
%  \caption{Add caption}
%  \scalebox{0.59}{
%  \renewcommand{\arraystretch}{0.118}
%    \begin{tabular}{ccccccccccccccccccccc}
%    \toprule
%    \multicolumn{2}{c}{\multirow{2}[4]{*}{Methods/Models}} & \multirow{2}[4]{*}{DnD} & \multirow{2}[4]{*}{SIDD} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multirow{2}[4]{*}{HighISO} & \multicolumn{13}{c}{IOCI} \\
%    \cmidrule{9-21}    \multicolumn{2}{c}{} &       &       &       &       &       &       & C-100D & C-600D & C-5DMark4 & F-X100T & H-Honor6X & H-Mate40Pro & I-5S & I-6S & I-13 & N-D5300 & O-R11s & S-A6500 & X-MI8 \\
%    \midrule
%    /     & \# Images & 1000  & 1280  & 15    & 60    & 100   & 100   & 55    & 25    & 83    & 71    & 30    & 126   & 36    & 67    & 174   & 56    & 39    & 36    & 50 \\
%    \midrule
%    \multirow{128}[56]{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{2}[4]{*}{LSCD} & /     & /     & 36.20  & 37.69  & 37.97  & 38.64  & 40.65  & 41.45  & /     & /     & 39.22  & /     & 39.84  & 39.53  & /     & 40.83  & /     & 44.34  & 35.86  \\
%\cmidrule{3-21}          &       & /     & /     & 0.942  & 0.963  & 0.964  & 0.962  & 0.973  & 0.979  & /     & /     & 0.963  & /     & 0.963  & 0.963  & /     & 0.973  & /     & 0.987  & 0.957  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{GID} & 34.32  & 27.16  & 37.17  & 38.41  & 38.37  & 39.63  & 40.86  & 41.60  & 44.11  & 42.31  & 39.52  & 38.66  & 40.12  & 40.16  & 41.50  & 41.09  & 40.50  & 44.96  & 36.11  \\
%\cmidrule{3-21}          &       & 0.817  & 0.634  & 0.946  & 0.963  & 0.967  & 0.967  & 0.974  & 0.979  & 0.989  & 0.975  & 0.965  & 0.972  & 0.964  & 0.967  & 0.979  & 0.973  & 0.973  & 0.989  & 0.960  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Bitonic} & 37.85  & 36.67  & 35.22  & 35.98  & 36.64  & 37.37  & 39.38  & 39.63  & 40.76  & 41.05  & 37.71  & 37.41  & 38.98  & 38.04  & 39.09  & 39.22  & 38.87  & 43.25  & 34.92  \\
%\cmidrule{3-21}          &       & 0.936  & 0.933  & 0.925  & 0.931  & 0.940  & 0.943  & 0.959  & 0.952  & 0.965  & 0.964  & 0.940  & 0.956  & 0.947  & 0.939  & 0.952  & 0.954  & 0.959  & 0.979  & 0.941  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{LLRT} & 35.45  & 30.74  & 37.77  & 39.76  & 38.28  & 39.59  & 41.60  & 42.24  & 42.68  & 42.22  & 37.91  & 38.80  & 38.01  & 39.87  & 42.02  & 41.76  & 38.69  & 45.17  & 35.71  \\
%\cmidrule{3-21}          &       & 0.897  & 0.766  & 0.957  & 0.977  & 0.970  & 0.972  & 0.977  & 0.983  & 0.992  & 0.975  & 0.969  & 0.973  & 0.965  & 0.971  & 0.984  & 0.979  & 0.972  & 0.989  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{MCWNNM } & 37.38  & 29.54  & 37.02  & 38.54  & 38.26  & 39.89  & 41.47  & 42.07  & 44.22  & 42.48  & 39.46  & 38.78  & 39.87  & 40.18  & 41.33  & 41.74  & 40.71  & 45.38  & 35.84  \\
%\cmidrule{3-21}          &       & 0.929  & 0.888  & 0.950  & 0.967  & 0.965  & 0.970  & 0.977  & 0.979  & 0.988  & 0.976  & 0.961  & 0.971  & 0.957  & 0.963  & 0.976  & 0.975  & 0.973  & 0.990  & 0.952  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{TWSC } & 37.96  & /     & 37.90  & 39.66  & 38.62  & 40.62  & 41.65  & 42.52  & 44.94  & 42.26  & 38.71  & 38.81  & 38.77  & 40.12  & 41.71  & 42.23  & 40.65  & 45.49  & 35.40  \\
%\cmidrule{3-21}          &       & 0.942  & /     & 0.959  & 0.976  & 0.967  & 0.975  & 0.977  & 0.982  & 0.992  & 0.973  & 0.945  & 0.972  & 0.938  & 0.962  & 0.980  & 0.975  & 0.972  & 0.990  & 0.939  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{WTR1} & /     & /     & 37.80  & 37.32  & 38.20  & 38.19  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{3-21}          &       & /     & /     & 0.958  & 0.944  & 0.965  & 0.940  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{M-SVD} & 37.45  & 33.51  & 37.63  & 39.36  & 38.57  & 40.27  & 41.81  & 42.55  & 44.39  & 42.68  & 39.99  & 38.93  & 40.78  & 40.52  & 41.72  & 42.18  & 40.73  & 45.71  & 36.37  \\
%\cmidrule{3-21}          &       & 0.924  & 0.867  & 0.954  & 0.971  & 0.967  & 0.971  & 0.979  & 0.983  & 0.989  & 0.976  & 0.967  & 0.973  & 0.969  & 0.969  & 0.977  & 0.977  & 0.974  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{4DHOSVD} & 37.58  & 34.49  & 37.52  & 39.15  & 38.54  & 40.27  & 41.40  & 42.19  & 44.49  & 42.60  & 39.82  & 38.88  & 40.59  & 40.37  & 41.75  & 41.82  & 40.71  & 45.58  & 36.27  \\
%\cmidrule{3-21}          &       & 0.929  & 0.911  & 0.956  & 0.973  & 0.968  & 0.973  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.965  & 0.967  & 0.980  & 0.977  & 0.974  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D1} & 38.04  & 35.00  & 37.58  & 39.21  & 38.60  & 40.11  & 41.58  & 42.40  & 44.43  & 42.53  & 39.93  & 38.84  & 40.56  & 40.41  & 41.93  & 42.29  & 40.62  & 45.58  & 36.24  \\
%\cmidrule{3-21}          &       & 0.938  & 0.925  & 0.955  & 0.971  & 0.969  & 0.972  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.967  & 0.970  & 0.982  & 0.979  & 0.973  & 0.990  & 0.959  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D2} & 37.73  & 34.74  & 37.70  & 39.41  & 38.69  & 40.35  & 41.69  & 42.54  & 44.74  & 42.65  & 39.97  & 38.97  & 40.77  & 40.55  & 42.03  & 42.20  & 40.75  & 45.72  & 36.38  \\
%\cmidrule{3-21}          &       & 0.934  & 0.922  & 0.957  & 0.975  & 0.970  & 0.974  & 0.978  & 0.984  & 0.992  & 0.977  & 0.967  & 0.974  & 0.967  & 0.969  & 0.983  & 0.979  & 0.974  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D\_best} & /     & /     & 38.01  & 39.80  & 38.82  & 40.65  & 42.08  & 42.89  & 45.08  & 43.14  & 40.45  & 39.23  & 41.21  & 41.12  & 42.42  & 42.79  & 40.92  & 45.84  & 36.76  \\
%\cmidrule{3-21}          &       & /     & /     & 0.962  & 0.978  & 0.971  & 0.976  & 0.981  & 0.985  & 0.993  & 0.980  & 0.974  & 0.976  & 0.975  & 0.978  & 0.985  & 0.982  & 0.974  & 0.991  & 0.964  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CMSt-SVD} & 38.25  & 34.38  & 37.95  & 39.76  & 38.85  & 40.49  & 41.99  & 42.75  & 44.65  & 42.68  & 40.08  & 38.95  & 40.84  & 40.53  & 42.06  & 42.72  & 40.87  & 45.91  & 36.40  \\
%\cmidrule{3-21}          &       & 0.940  & 0.900  & 0.959  & 0.976  & 0.971  & 0.974  & 0.979  & 0.984  & 0.991  & 0.977  & 0.967  & 0.973  & 0.967  & 0.967  & 0.982  & 0.980  & 0.974  & 0.991  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{NLH-CC} & 38.85  & /     & 38.49  & 39.86  & 38.36  & 40.29  & 41.77  & 42.72  & 43.66  & 42.80  & 38.84  & 38.31  & 40.44  & 39.94  & 41.13  & 43.25  & NA    & 46.02  & 35.73  \\
%\cmidrule{3-21}          &       & 0.953  & /     & 0.965  & 0.976  & 0.965  & 0.971  & 0.979  & 0.984  & 0.986  & 0.978  & 0.959  & 0.968  & 0.964  & 0.963  & 0.976  & 0.981  & NA    & 0.991  & 0.955  \\
%    \midrule
%    \midrule
%    \multirow{368}[148]{*}{\shortstack[l]{DNN \\ methods}} & \multirow{2}[4]{*}{AINDNet} & 39.77  & 39.08  & 36.14  & \multicolumn{1}{c|}{37.19 } & 37.33  & 38.00  & 38.54  & 39.33  & 39.49  & 38.50  & 36.53  & 36.24  & 36.93  & 36.83  & 37.27  & 38.11  & 37.44  & 40.17  & 34.65  \\
%\cmidrule{3-21}          &       & 0.959  & 0.953  & 0.935  & 0.949  & 0.954  & 0.946  & 0.975  & 0.976  & 0.979  & 0.966  & 0.954  & 0.965  & 0.958  & 0.953  & 0.964  & 0.961  & 0.968  & 0.981  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{AP-BSN} & 37.29  & 35.97  & 35.44  & 36.76  & 36.99  & 38.26  & 40.23  & 41.29  & 42.72  & 41.40  & 37.87  & 37.62  & 37.47  & 38.29  & 40.83  & 40.86  & 39.55  & 43.73  & 34.37  \\
%\cmidrule{3-21}          &       & 0.932  & 0.925  & 0.936  & 0.956  & 0.956  & 0.965  & 0.973  & 0.979  & 0.986  & 0.970  & 0.949  & 0.966  & 0.939  & 0.960  & 0.977  & 0.973  & 0.969  & 0.983  & 0.937  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Blind2Unblind} & /     & /     & 36.51  & 38.18  & 38.25  & 39.03  & 40.71  & 41.72  & 43.11  & 41.17  & 39.35  & 38.27  & 39.39  & 39.04  & 40.88  & 40.90  & 39.76  & 43.78  & 35.75  \\
%\cmidrule{3-21}          &       & /     & /     & 0.935  & 0.958  & 0.968  & 0.962  & 0.974  & 0.981  & 0.990  & 0.970  & 0.967  & 0.971  & 0.962  & 0.958  & 0.976  & 0.970  & 0.971  & 0.986  & 0.956  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{BRDNet} & 33.80  & /     & 37.27  & 39.16  & 38.04  & 39.64  & 39.85  & 40.95  & 43.54  & 40.27  & 39.48  & 38.66  & 38.19  & 40.07  & 41.92  & 41.34  & 39.66  & 42.76  & 36.08  \\
%\cmidrule{3-21}          &       & 0.897  & /     & 0.953  & 0.974  & 0.960  & 0.969  & 0.965  & 0.974  & 0.989  & 0.958  & 0.958  & 0.973  & 0.943  & 0.969  & 0.981  & 0.972  & 0.965  & 0.979  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{C2N} & 37.28  & /     & 37.02  & /     & 37.69  & 38.86  & 41.12  & 41.95  & 42.61  & 41.33  & 38.73  & 38.15  & 38.95  & 38.67  & 40.50  & 40.78  & 40.05  & 44.64  & 35.53  \\
%\cmidrule{3-21}          &       & 0.924  & /     & 0.945  & /     & 0.958  & 0.960  & 0.976  & 0.980  & 0.980  & 0.966  & 0.954  & 0.965  & 0.956  & 0.945  & 0.977  & 0.964  & 0.970  & 0.987  & 0.952  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CBDNet} & 38.06  & 33.26  & 36.20  & 37.67  & 37.81  & 38.18  & 41.43  & 42.41  & 42.55  & 41.88  & 38.35  & 38.17  & 39.80  & 39.07  & 40.63  & 40.92  & 39.54  & 44.38  & 35.54  \\
%\cmidrule{3-21}          &       & 0.942  & 0.869  & 0.919  & 0.940  & 0.956  & 0.942  & 0.977  & 0.981  & 0.980  & 0.971  & 0.946  & 0.964  & 0.960  & 0.951  & 0.968  & 0.963  & 0.965  & 0.981  & 0.950  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CVF-SID} & 36.31  & 34.43  & 29.13  & 31.02  & 33.08  & 33.35  & 36.68  & 39.08  & 39.73  & 36.40  & 33.13  & 33.16  & 32.07  & 33.33  & 36.92  & 38.40  & 35.22  & 38.56  & 29.89  \\
%\cmidrule{3-21}          &       & 0.923  & 0.912  & 0.853  & 0.898  & 0.912  & 0.929  & 0.933  & 0.974  & 0.976  & 0.929  & 0.895  & 0.920  & 0.857  & 0.917  & 0.946  & 0.961  & 0.927  & 0.952  & 0.849  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{CycleISP} & 39.57  & 39.42  & 35.40  & 36.87  & 37.61  & 37.70  & 41.26  & 41.84  & 42.64  & 41.59  & 38.47  & 38.01  & 38.79  & 38.67  & 40.61  & 40.03  & 39.86  & 44.75  & 35.54  \\
%\cmidrule{3-21}          &       & 0.955  & 0.956  & 0.916  & 0.939  & 0.955  & 0.936  & 0.977  & 0.977  & 0.978  & 0.969  & 0.952  & 0.966  & 0.961  & 0.952  & 0.970  & 0.953  & 0.968  & 0.987  & 0.949  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DANet} & 39.55  & 39.43  & 37.17  & 38.63  & 41.49  & 38.92  & 41.59  & 42.59  & 42.83  & 41.70  & 37.91  & 38.17  & 39.23  & 38.74  & 41.58  & 41.54  & 39.58  & 44.03  & 36.21  \\
%\cmidrule{3-21}          &       & 0.953  & 0.956  & 0.953  & 0.969  & 0.977  & 0.960  & 0.979  & 0.985  & 0.979  & 0.977  & 0.963  & 0.970  & 0.964  & 0.962  & 0.980  & 0.976  & 0.972  & 0.989  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DBF} & /     & /     & 38.48  & 40.59  & 38.87  & 40.09  & 41.56  & 42.87  & 44.85  & 42.36  & 39.98  & 38.86  & 40.17  & 40.26  & 42.12  & 43.17  & 40.67  & 44.75  & 36.45  \\
%\cmidrule{3-21}          &       & /     & /     & 0.960  & 0.981  & 0.970  & 0.970  & 0.979  & 0.984  & 0.992  & 0.975  & 0.967  & 0.972  & 0.966  & 0.966  & 0.982  & 0.982  & 0.973  & 0.987  & 0.963  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DCDicL} & /     & /     & 36.61  & /     & 37.45  & 38.12  & 37.77  & 38.24  & 38.39  & 38.62  & 35.87  & 36.07  & 35.83  & 36.25  & 39.84  & 39.38  & 37.04  & 40.24  & 34.72  \\
%\cmidrule{3-21}          &       & /     & /     & 0.945  & /     & 0.972  & 0.965  & 0.970  & 0.977  & 0.990  & 0.968  & 0.968  & 0.975  & 0.956  & 0.971  & 0.984  & 0.976  & 0.969  & 0.980  & 0.955  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DeamNet} & 39.63  & 39.35  & 36.63  & /     & 37.70  & 36.93  & 40.90  & 40.86  & 41.22  & 39.72  & 33.67  & 36.40  & 37.87  & 35.07  & 40.25  & 38.92  & 39.56  & 40.52  & 34.61  \\
%\cmidrule{3-21}          &       & 0.953  & 0.955  & 0.936  & /     & 0.958  & 0.944  & 0.977  & 0.978  & 0.979  & 0.967  & 0.953  & 0.964  & 0.961  & 0.948  & 0.966  & 0.957  & 0.969  & 0.980  & 0.952  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DIDN} & 39.64  & 39.78  & 36.06  & /     & 37.36  & 38.24  & 40.74  & 41.68  & 42.35  & 41.17  & 38.15  & 37.87  & 38.27  & 38.58  & 40.03  & 40.32  & 39.73  & 44.07  & 35.28  \\
%\cmidrule{3-21}          &       & 0.953  & 0.958  & 0.946  & /     & 0.953  & 0.950  & 0.975  & 0.977  & 0.975  & 0.966  & 0.951  & 0.965  & 0.954  & 0.950  & 0.963  & 0.959  & 0.966  & 0.985  & 0.949  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DnCNN} & 37.90  & 37.73  & 37.47  & 39.32  & 38.51  & 40.01  & 40.81  & 41.91  & 44.16  & 41.57  & 39.92  & 38.72  & 39.34  & 40.22  & 42.03  & 42.12  & 40.26  & 43.97  & 36.30  \\
%\cmidrule{3-21}          &       & 0.943  & 0.941  & 0.954  & 0.974  & 0.966  & 0.971  & 0.972  & 0.979  & 0.991  & 0.969  & 0.962  & 0.973  & 0.964  & 0.969  & 0.983  & 0.977  & 0.970  & 0.984  & 0.960  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DPIR} & /     & /     & 38.30  & 40.33  & 38.93  & 40.77  & 41.94  & 42.62  & 45.36  & 42.78  & 40.35  & 39.17  & 40.80  & 40.80  & 42.86  & 42.86  & 40.96  & 45.76  & 36.61  \\
%\cmidrule{3-21}          &       & /     & /     & 0.961  & 0.979  & 0.970  & 0.974  & 0.978  & 0.982  & 0.993  & 0.977  & 0.969  & 0.975  & 0.966  & 0.970  & 0.985  & 0.980  & 0.974  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{DudeNet} & 33.18  & 27.55  & 36.03  & 37.44  & 39.92  & 38.18  & 39.94  & 41.13  & 42.97  & 41.06  & 38.63  & 37.83  & 39.09  & 38.58  & 40.73  & 40.63  & 39.71  & 43.34  & 35.44  \\
%\cmidrule{3-21}          &       & 0.810  & 0.645  & 0.933  & 0.953  & 0.973  & 0.955  & 0.972  & 0.977  & 0.988  & 0.971  & 0.962  & 0.969  & 0.962  & 0.961  & 0.976  & 0.969  & 0.972  & 0.985  & 0.955  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{FCCF} & 36.30  & 23.32  & 39.02  & 40.89  & 38.87  & 41.20  & 42.03  & 43.07  & 45.15  & 42.80  & 40.14  & 39.04  & 40.61  & 40.66  & 42.31  & 43.05  & 40.95  & 45.47  & 36.72  \\
%\cmidrule{3-21}          &       & 0.885  & 0.461  & 0.968  & 0.982  & 0.971  & 0.978  & 0.980  & 0.985  & 0.993  & 0.978  & 0.966  & 0.974  & 0.967  & 0.969  & 0.984  & 0.982  & 0.975  & 0.989  & 0.964  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{FFD-Net} & 37.61  & 38.27  & 37.67  & 39.73  & 38.76  & 40.28  & 41.67  & 42.55  & 44.77  & 42.44  & 40.05  & 38.96  & 40.60  & 40.50  & 42.43  & 42.44  & 40.75  & 45.71  & 36.47  \\
%\cmidrule{3-21}          &       & 0.942  & 0.948  & 0.956  & 0.977  & 0.970  & 0.973  & 0.977  & 0.982  & 0.992  & 0.976  & 0.967  & 0.974  & 0.964  & 0.971  & 0.984  & 0.979  & 0.973  & 0.990  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{IDR} & /     & /     & 34.26  & 36.18  & 36.28  & 36.44  & 39.33  & 40.31  & 40.94  & 39.74  & 37.38  & 37.39  & 38.30  & 38.15  & 39.68  & 38.22  & 38.01  & 43.15  & 34.64  \\
%\cmidrule{3-21}          &       & /     & /     & 0.877  & 0.923  & 0.925  & 0.910  & 0.955  & 0.962  & 0.961  & 0.935  & 0.927  & 0.957  & 0.938  & 0.944  & 0.951  & 0.913  & 0.941  & 0.978  & 0.929  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{InvDN} & 39.57  & 39.28  & 34.55  & 36.33  & 35.94  & 38.01  & 38.95  & 40.09  & 42.03  & 40.02  & 33.32  & 37.00  & 36.64  & 37.66  & 40.06  & 40.98  & 39.10  & 40.74  & 34.15  \\
%\cmidrule{3-21}          &       & 0.952  & 0.955  & 0.937  & 0.953  & 0.947  & 0.952  & 0.965  & 0.973  & 0.978  & 0.960  & 0.930  & 0.965  & 0.939  & 0.955  & 0.966  & 0.971  & 0.964  & 0.969  & 0.935  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{IRCNN} & 34.78  & 33.50  & 37.26  & 37.25  & 37.49  & 39.66  & 41.24  & 41.85  & 43.89  & 41.78  & 39.91  & 38.63  & 40.14  & 40.12  & 41.87  & 41.86  & 40.26  & 44.38  & 36.22  \\
%\cmidrule{3-21}          &       & 0.907  & 0.887  & 0.954  & 0.956  & 0.956  & 0.970  & 0.978  & 0.981  & 0.991  & 0.973  & 0.969  & 0.972  & 0.965  & 0.969  & 0.983  & 0.977  & 0.972  & 0.988  & 0.961  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{MIRNet} & 39.88  & 39.55  & 36.06  & 37.25  & 37.49  & 38.10  & 40.72  & 41.68  & 42.76  & 41.05  & 38.28  & 37.80  & 38.60  & 38.55  & 40.28  & 40.46  & 39.73  & 43.66  & 35.42  \\
%\cmidrule{3-21}          &       & 0.956  & 0.957  & 0.942  & 0.956  & 0.956  & 0.952  & 0.975  & 0.978  & 0.980  & 0.968  & 0.954  & 0.967  & 0.959  & 0.952  & 0.966  & 0.964  & 0.967  & 0.983  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{MPRNet} & 39.82  & 39.57  & 35.94  & /     & 37.50  & 38.04  & 40.59  & 41.30  & 42.59  & 41.23  & 38.35  & 37.92  & 38.95  & 38.62  & 40.21  & 40.20  & 39.77  & 44.05  & 35.49  \\
%\cmidrule{3-21}          &       & 0.954  & 0.958  & 0.935  & /     & 0.954  & 0.946  & 0.974  & 0.974  & 0.978  & 0.969  & 0.952  & 0.966  & 0.960  & 0.949  & 0.965  & 0.960  & 0.967  & 0.986  & 0.951  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{NAFNet} & 38.36  & 40.15  & 34.39  & /     & 36.38  & 37.88  & 40.12  & 40.23  & 40.66  & 40.01  & 36.13  & 35.87  & 36.66  & 36.79  & 36.53  & 39.93  & 39.32  & 40.45  & 34.82  \\
%\cmidrule{3-21}          &       & 0.943  & 0.960  & 0.923  & /     & 0.947  & 0.954  & 0.973  & 0.943  & 0.936  & 0.962  & 0.919  & 0.927  & 0.948  & 0.927  & 0.884  & 0.951  & 0.966  & 0.924  & 0.948  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{NBNet} & 39.89  & 39.64  & 35.89  & /     & 37.37  & 38.32  & 40.95  & 41.91  & 42.92  & 41.17  & 38.02  & 37.87  & 37.79  & 38.45  & 40.51  & 40.45  & 39.73  & 43.96  & 35.37  \\
%\cmidrule{3-21}          &       & 0.955  & 0.958  & 0.935  & /     & 0.957  & 0.955  & 0.977  & 0.980  & 0.982  & 0.971  & 0.955  & 0.967  & 0.956  & 0.955  & 0.972  & 0.967  & 0.969  & 0.984  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Neigh2Neigh} & /     & /     & 34.47  & 35.65  & 37.10  & 36.59  & 40.22  & 40.41  & 41.29  & 41.24  & 38.13  & 37.94  & 39.71  & 38.50  & 39.63  & 38.05  & 39.17  & 44.49  & 35.30  \\
%\cmidrule{3-21}          &       & /     & /     & 0.883  & 0.907  & 0.942  & 0.908  & 0.967  & 0.960  & 0.966  & 0.958  & 0.940  & 0.961  & 0.956  & 0.936  & 0.952  & 0.919  & 0.958  & 0.984  & 0.944  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{NLNet} & /     & /     & 37.56  & 39.32  & 38.58  & 40.17  & 41.43  & 42.18  & 44.53  & 42.19  & 39.96  & 38.89  & 40.06  & 40.61  & 42.14  & 42.16  & 40.63  & 44.87  & 36.34  \\
%\cmidrule{3-21}          &       & /     & /     & 0.955  & 0.974  & 0.968  & 0.973  & 0.976  & 0.981  & 0.991  & 0.974  & 0.969  & 0.973  & 0.964  & 0.971  & 0.983  & 0.978  & 0.973  & 0.988  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Noise2Noise} & /     & /     & 33.55  & 34.67  & 35.91  & 35.28  & 38.88  & 39.07  & 39.34  & 39.26  & 36.81  & 36.99  & 38.04  & 37.21  & 38.00  & 36.35  & 37.67  & 42.59  & 34.44  \\
%\cmidrule{3-21}          &       & /     & /     & 0.850  & 0.874  & 0.913  & 0.875  & 0.950  & 0.940  & 0.938  & 0.931  & 0.919  & 0.948  & 0.936  & 0.916  & 0.924  & 0.876  & 0.936  & 0.975  & 0.926  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{PD-Denoising} & 38.40  & 33.99  & 35.85  & 37.13  & 37.13  & 37.12  & 40.85  & 41.38  & 41.13  & 41.05  & 37.72  & 37.57  & 39.03  & 38.01  & 39.18  & 39.64  & 38.80  & 43.73  & 35.05  \\
%\cmidrule{3-21}          &       & 0.943  & 0.896  & 0.924  & 0.944  & 0.944  & 0.921  & 0.974  & 0.974  & 0.966  & 0.959  & 0.935  & 0.956  & 0.948  & 0.929  & 0.948  & 0.946  & 0.955  & 0.981  & 0.940  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{PNGAN} & 39.38  & 39.81  & 38.44  & /     & 39.57  & 40.51  & 41.79  & 43.13  & 44.73  & 42.55  & 39.84  & 38.78  & 40.63  & 40.20  & 41.85  & 43.15  & 40.87  & 45.32  & 36.40  \\
%\cmidrule{3-21}          &       & 0.953  & 0.959  & 0.963  & /     & 0.974  & 0.974  & 0.979  & 0.985  & 0.992  & 0.977  & 0.964  & 0.970  & 0.969  & 0.962  & 0.981  & 0.982  & 0.974  & 0.988  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{R2R} & /     & /     & 36.32  & 38.11  & 38.57  & 38.71  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{3-21}          &       & /     & /     & 0.937  & 0.961  & 0.970  & 0.958  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Restormer} & 40.03  & 39.79  & 36.33  & /     & 37.66  & 38.29  & 41.10  & 41.84  & 42.49  & 41.47  & 38.42  & 38.08  & 39.05  & 38.77  & 40.13  & 40.53  & 39.56  & 44.19  & 35.65  \\
%\cmidrule{3-21}          &       & 0.956  & 0.959  & 0.941  & /     & 0.956  & 0.948  & 0.977  & 0.979  & 0.976  & 0.968  & 0.952  & 0.966  & 0.960  & 0.949  & 0.963  & 0.962  & 0.963  & 0.986  & 0.953  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{RIDNet} & 39.26  & 38.70  & 36.84  & 38.11  & 38.57  & 38.60  & 41.09  & 42.15  & 42.39  & 41.59  & 38.88  & 38.21  & 38.67  & 39.02  & 40.91  & 41.01  & 40.07  & 44.40  & 35.76  \\
%\cmidrule{3-21}          &       & 0.953  & 0.950  & 0.941  & 0.961  & 0.970  & 0.956  & 0.977  & 0.980  & 0.989  & 0.975  & 0.962  & 0.970  & 0.963  & 0.959  & 0.978  & 0.977  & 0.972  & 0.987  & 0.957  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{SADNet} & 39.59  & /     & 37.76  & 38.11  & 39.22  & 38.90  & 40.82  & 42.02  & 44.25  & 41.85  & 39.53  & 38.33  & 39.83  & 39.69  & 39.81  & 41.64  & 40.70  & 44.61  & 36.36  \\
%\cmidrule{3-21}          &       & 0.952  & /     & 0.952  & 0.961  & 0.972  & 0.965  & 0.976  & 0.980  & 0.992  & 0.975  & 0.965  & 0.970  & 0.965  & 0.963  & 0.965  & 0.979  & 0.974  & 0.988  & 0.962  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Self2Self} & /     & /     & 36.26  & 38.23  & /     & 39.49  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{3-21}          &       & /     & /     & 0.947  & 0.969  & /     & 0.963  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{Unet} & /     & /     & 36.95  & 38.96  & 38.05  & 39.62  & 40.40  & 41.36  & 43.58  & 41.12  & 39.35  & 38.25  & 38.94  & 39.95  & 41.32  & 41.70  & 39.51  & 43.17  & 36.09  \\
%\cmidrule{3-21}          &       & /     & /     & 0.943  & 0.971  & 0.962  & 0.967  & 0.968  & 0.977  & 0.989  & 0.968  & 0.963  & 0.971  & 0.959  & 0.968  & 0.979  & 0.974  & 0.966  & 0.981  & 0.958  \\
%\cmidrule{2-21}          & \multirow{2}[4]{*}{VDNet} & /     & /     & 35.86  & /     & 37.58  & 38.43  & 40.97  & 42.37  & 43.08  & 41.19  & 38.23  & 37.95  & 37.88  & 38.60  & 40.81  & 41.21  & 39.93  & 44.27  & 35.49  \\
%\cmidrule{3-21}          &       & /     & /     & 0.945  & /     & 0.957  & 0.955  & 0.976  & 0.983  & 0.983  & 0.970  & 0.956  & 0.968  & 0.956  & 0.956  & 0.973  & 0.970  & 0.970  & 0.984  & 0.953  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{tab:addlabel}%
%\end{table*}%
%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Average PSNR, SSIM values on real-world color image datasets. `/' means the results are not available due to high computational burden or other issues. `C: CANON', `F: FUJIFILM', `H: HUAWEI', `I: IPHONE', 'N: NIKON', `O: OPPO', `S: SONY', `X: XIAOMI'.}
  \scalebox{0.586}{
  \renewcommand{\arraystretch}{0.118}
    \begin{tabular}{ccccccccccccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Methods/Models}} & \multirow{2}[4]{*}{DnD} & \multirow{2}[4]{*}{SIDD} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multirow{2}[4]{*}{HighISO} & \multicolumn{13}{c}{IOCI} \\
    \cmidrule{9-21}    \multicolumn{2}{c}{} &       &       &       &       &       &       & C-100D & C-600D & C-5DMark4 & F-X100T & H-Honor6X & H-Mate40Pro & I-5S & I-6S & I-13 & N-D5300 & O-R11s & S-A6500 & X-MI8 \\
    \midrule
    /     & \# Images & 1000  & 1280  & 15    & 60    & 100   & 100   & 55    & 25    & 83    & 71    & 30    & 126   & 36    & 67    & 174   & 56    & 39    & 36    & 50 \\
    \midrule
    \multirow{168}[56]{*}{\shortstack[c]{Traditional \\ denoisers}} & \multirow{2}[4]{*}{LSCD} & /     & /     & 36.20  & 37.69  & 37.97  & 38.64  & 40.65  & 41.45  & /     & /     & 39.22  & /     & 39.84  & 39.53  & /     & 40.83  & /     & 44.34  & 35.86  \\
\cmidrule{3-21}          &       & /     & /     & 0.942  & 0.963  & 0.964  & 0.962  & 0.973  & 0.979  & /     & /     & 0.963  & /     & 0.963  & 0.963  & /     & 0.973  & /     & 0.987  & 0.957  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{GID} & 34.32  & 27.16  & 37.17  & 38.41  & 38.37  & 39.63  & 40.86  & 41.60  & 44.11  & 42.31  & 39.52  & 38.66  & 40.12  & 40.16  & 41.50  & 41.09  & 40.50  & 44.96  & 36.11  \\
\cmidrule{3-21}          &       & 0.817  & 0.634  & 0.946  & 0.963  & 0.967  & 0.967  & 0.974  & 0.979  & 0.989  & 0.975  & 0.965  & 0.972  & 0.964  & 0.967  & 0.979  & 0.973  & 0.973  & 0.989  & 0.960  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Bitonic} & 37.85  & 36.67  & 35.22  & 35.98  & 36.64  & 37.37  & 39.38  & 39.63  & 40.76  & 41.05  & 37.71  & 37.41  & 38.98  & 38.04  & 39.09  & 39.22  & 38.87  & 43.25  & 34.92  \\
\cmidrule{3-21}          &       & 0.936  & 0.933  & 0.925  & 0.931  & 0.940  & 0.943  & 0.959  & 0.952  & 0.965  & 0.964  & 0.940  & 0.956  & 0.947  & 0.939  & 0.952  & 0.954  & 0.959  & 0.979  & 0.941  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{LLRT} & 35.45  & 30.74  & 37.77  & 39.76  & 38.28  & 39.59  & 41.60  & 42.24  & 42.68  & 42.22  & 37.91  & 38.80  & 38.01  & 39.87  & 42.02  & 41.76  & 38.69  & 45.17  & 35.71  \\
\cmidrule{3-21}          &       & 0.897  & 0.766  & 0.957  & 0.977  & 0.970  & 0.972  & 0.977  & 0.983  & 0.992  & 0.975  & 0.969  & 0.973  & 0.965  & 0.971  & 0.984  & 0.979  & 0.972  & 0.989  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{MCWNNM } & 37.38  & 29.54  & 37.02  & 38.54  & 38.26  & 39.89  & 41.47  & 42.07  & 44.22  & 42.48  & 39.46  & 38.78  & 39.87  & 40.18  & 41.33  & 41.74  & 40.71  & 45.38  & 35.84  \\
\cmidrule{3-21}          &       & 0.929  & 0.888  & 0.950  & 0.967  & 0.965  & 0.970  & 0.977  & 0.979  & 0.988  & 0.976  & 0.961  & 0.971  & 0.957  & 0.963  & 0.976  & 0.975  & 0.973  & 0.990  & 0.952  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{TWSC } & 37.96  & /     & 37.90  & 39.66  & 38.62  & 40.62  & 41.65  & 42.52  & 44.94  & 42.26  & 38.71  & 38.81  & 38.77  & 40.12  & 41.71  & 42.23  & 40.65  & 45.49  & 35.40  \\
\cmidrule{3-21}          &       & 0.942  & /     & 0.959  & 0.976  & 0.967  & 0.975  & 0.977  & 0.982  & 0.992  & 0.973  & 0.945  & 0.972  & 0.938  & 0.962  & 0.980  & 0.975  & 0.972  & 0.990  & 0.939  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{WTR1} & /     & /     & 37.80  & 37.32  & 38.20  & 38.19  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{3-21}          &       & /     & /     & 0.958  & 0.944  & 0.965  & 0.940  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{M-SVD} & 37.45  & 33.51  & 37.63  & 39.36  & 38.57  & 40.27  & 41.81  & 42.55  & 44.39  & 42.68  & 39.99  & 38.93  & 40.78  & 40.52  & 41.72  & 42.18  & 40.73  & 45.71  & 36.37  \\
\cmidrule{3-21}          &       & 0.924  & 0.867  & 0.954  & 0.971  & 0.967  & 0.971  & 0.979  & 0.983  & 0.989  & 0.976  & 0.967  & 0.973  & 0.969  & 0.969  & 0.977  & 0.977  & 0.974  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{4DHOSVD} & 37.58  & 34.49  & 37.52  & 39.15  & 38.54  & 40.27  & 41.40  & 42.19  & 44.49  & 42.60  & 39.82  & 38.88  & 40.59  & 40.37  & 41.75  & 41.82  & 40.71  & 45.58  & 36.27  \\
\cmidrule{3-21}          &       & 0.929  & 0.911  & 0.956  & 0.973  & 0.968  & 0.973  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.965  & 0.967  & 0.980  & 0.977  & 0.974  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D1} & 38.04  & 35.00  & 37.58  & 39.21  & 38.60  & 40.11  & 41.58  & 42.40  & 44.43  & 42.53  & 39.93  & 38.84  & 40.56  & 40.41  & 41.93  & 42.29  & 40.62  & 45.58  & 36.24  \\
\cmidrule{3-21}          &       & 0.938  & 0.925  & 0.955  & 0.971  & 0.969  & 0.972  & 0.977  & 0.982  & 0.990  & 0.976  & 0.966  & 0.973  & 0.967  & 0.970  & 0.982  & 0.979  & 0.973  & 0.990  & 0.959  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D2} & 37.73  & 34.74  & 37.70  & 39.41  & 38.69  & 40.35  & 41.69  & 42.54  & 44.74  & 42.65  & 39.97  & 38.97  & 40.77  & 40.55  & 42.03  & 42.20  & 40.75  & 45.72  & 36.38  \\
\cmidrule{3-21}          &       & 0.934  & 0.922  & 0.957  & 0.975  & 0.970  & 0.974  & 0.978  & 0.984  & 0.992  & 0.977  & 0.967  & 0.974  & 0.967  & 0.969  & 0.983  & 0.979  & 0.974  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CBM3D\_best} & /     & /     & 38.01  & 39.80  & 38.82  & 40.65  & 42.08  & 42.89  & 45.08  & 43.14  & 40.45  & 39.23  & 41.21  & 41.12  & 42.42  & 42.79  & 40.92  & 45.84  & 36.76  \\
\cmidrule{3-21}          &       & /     & /     & 0.962  & 0.978  & 0.971  & 0.976  & 0.981  & 0.985  & 0.993  & 0.980  & 0.974  & 0.976  & 0.975  & 0.978  & 0.985  & 0.982  & 0.974  & 0.991  & 0.964  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CMSt-SVD} & 38.25  & 34.38  & 37.95  & 39.76  & 38.85  & 40.49  & 41.99  & 42.75  & 44.65  & 42.68  & 40.08  & 38.95  & 40.84  & 40.53  & 42.06  & 42.72  & 40.87  & 45.91  & 36.40  \\
\cmidrule{3-21}          &       & 0.940  & 0.900  & 0.959  & 0.976  & 0.971  & 0.974  & 0.979  & 0.984  & 0.991  & 0.977  & 0.967  & 0.973  & 0.967  & 0.967  & 0.982  & 0.980  & 0.974  & 0.991  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{NLH-CC} & 38.85  & /     & 38.49  & 39.86  & 38.36  & 40.29  & 41.77  & 42.72  & 43.66  & 42.80  & 38.84  & 38.31  & 40.44  & 39.94  & 41.13  & 43.25  & /     & 46.02  & 35.73  \\
\cmidrule{3-21}          &       & 0.953  & /     & 0.965  & 0.976  & 0.965  & 0.971  & 0.979  & 0.984  & 0.986  & 0.978  & 0.959  & 0.968  & 0.964  & 0.963  & 0.976  & 0.981  & /     & 0.991  & 0.955  \\
    \midrule
    \midrule
    \multirow{368}[148]{*}{\shortstack[c]{DNN \\ methods}} & \multirow{2}[4]{*}{AINDNet} & 39.77  & 39.08  & 36.14  & 37.19  & 37.33  & 38.00  & 38.54  & 39.33  & 39.49  & 38.50  & 36.53  & 36.24  & 36.93  & 36.83  & 37.27  & 38.11  & 37.44  & 40.17  & 34.65  \\
\cmidrule{3-21}          &       & 0.959  & 0.953  & 0.935  & 0.949  & 0.954  & 0.946  & 0.975  & 0.976  & 0.979  & 0.966  & 0.954  & 0.965  & 0.958  & 0.953  & 0.964  & 0.961  & 0.968  & 0.981  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{AP-BSN} & 37.29  & 35.97  & 35.44  & 36.76  & 36.99  & 38.26  & 40.23  & 41.29  & 42.72  & 41.40  & 37.87  & 37.62  & 37.47  & 38.29  & 40.83  & 40.86  & 39.55  & 43.73  & 34.37  \\
\cmidrule{3-21}          &       & 0.932  & 0.925  & 0.936  & 0.956  & 0.956  & 0.965  & 0.973  & 0.979  & 0.986  & 0.970  & 0.949  & 0.966  & 0.939  & 0.960  & 0.977  & 0.973  & 0.969  & 0.983  & 0.937  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Blind2Unblind} & /     & /     & 36.51  & 38.18  & 38.25  & 39.03  & 40.71  & 41.72  & 43.11  & 41.17  & 39.35  & 38.27  & 39.39  & 39.04  & 40.88  & 40.90  & 39.76  & 43.78  & 35.75  \\
\cmidrule{3-21}          &       & /     & /     & 0.935  & 0.958  & 0.968  & 0.962  & 0.974  & 0.981  & 0.990  & 0.970  & 0.967  & 0.971  & 0.962  & 0.958  & 0.976  & 0.970  & 0.971  & 0.986  & 0.956  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{BRDNet} & 33.80  & /     & 37.27  & 39.16  & 38.04  & 39.64  & 39.85  & 40.95  & 43.54  & 40.27  & 39.48  & 38.66  & 38.19  & 40.07  & 41.92  & 41.34  & 39.66  & 42.76  & 36.08  \\
\cmidrule{3-21}          &       & 0.897  & /     & 0.953  & 0.974  & 0.960  & 0.969  & 0.965  & 0.974  & 0.989  & 0.958  & 0.958  & 0.973  & 0.943  & 0.969  & 0.981  & 0.972  & 0.965  & 0.979  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{C2N} & 37.28  & /     & 37.02  & /     & 37.69  & 38.86  & 41.12  & 41.95  & 42.61  & 41.33  & 38.73  & 38.15  & 38.95  & 38.67  & 40.50  & 40.78  & 40.05  & 44.64  & 35.53  \\
\cmidrule{3-21}          &       & 0.924  & /     & 0.945  & /     & 0.958  & 0.960  & 0.976  & 0.980  & 0.980  & 0.966  & 0.954  & 0.965  & 0.956  & 0.945  & 0.977  & 0.964  & 0.970  & 0.987  & 0.952  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CBDNet} & 38.06  & 33.26  & 36.20  & 37.67  & 37.81  & 38.18  & 41.43  & 42.41  & 42.55  & 41.88  & 38.35  & 38.17  & 39.80  & 39.07  & 40.63  & 40.92  & 39.54  & 44.38  & 35.54  \\
\cmidrule{3-21}          &       & 0.942  & 0.869  & 0.919  & 0.940  & 0.956  & 0.942  & 0.977  & 0.981  & 0.980  & 0.971  & 0.946  & 0.964  & 0.960  & 0.951  & 0.968  & 0.963  & 0.965  & 0.981  & 0.950  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CVF-SID} & 36.31  & 34.43  & 29.13  & 31.02  & 33.08  & 33.35  & 36.68  & 39.08  & 39.73  & 36.40  & 33.13  & 33.16  & 32.07  & 33.33  & 36.92  & 38.40  & 35.22  & 38.56  & 29.89  \\
\cmidrule{3-21}          &       & 0.923  & 0.912  & 0.853  & 0.898  & 0.912  & 0.929  & 0.933  & 0.974  & 0.976  & 0.929  & 0.895  & 0.920  & 0.857  & 0.917  & 0.946  & 0.961  & 0.927  & 0.952  & 0.849  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{CycleISP} & 39.57  & 39.42  & 35.40  & 36.87  & 37.61  & 37.70  & 41.26  & 41.84  & 42.64  & 41.59  & 38.47  & 38.01  & 38.79  & 38.67  & 40.61  & 40.03  & 39.86  & 44.75  & 35.54  \\
\cmidrule{3-21}          &       & 0.955  & 0.956  & 0.916  & 0.939  & 0.955  & 0.936  & 0.977  & 0.977  & 0.978  & 0.969  & 0.952  & 0.966  & 0.961  & 0.952  & 0.970  & 0.953  & 0.968  & 0.987  & 0.949  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DANet} & 39.55  & 39.43  & 37.17  & 38.63  & 41.49  & 38.92  & 41.59  & 42.59  & 42.83  & 41.70  & 37.91  & 38.17  & 39.23  & 38.74  & 41.58  & 41.54  & 39.58  & 44.03  & 36.21  \\
\cmidrule{3-21}          &       & 0.953  & 0.956  & 0.953  & 0.969  & 0.977  & 0.960  & 0.979  & 0.985  & 0.979  & 0.977  & 0.963  & 0.970  & 0.964  & 0.962  & 0.980  & 0.976  & 0.972  & 0.989  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DBF} & /     & /     & 38.48  & 40.59  & 38.87  & 40.09  & 41.56  & 42.87  & 44.85  & 42.36  & 39.98  & 38.86  & 40.17  & 40.26  & 42.12  & 43.17  & 40.67  & 44.75  & 36.45  \\
\cmidrule{3-21}          &       & /     & /     & 0.960  & 0.981  & 0.970  & 0.970  & 0.979  & 0.984  & 0.992  & 0.975  & 0.967  & 0.972  & 0.966  & 0.966  & 0.982  & 0.982  & 0.973  & 0.987  & 0.963  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DCDicL} & /     & /     & 36.61  & /     & 37.45  & 38.12  & 37.77  & 38.24  & 38.39  & 38.62  & 35.87  & 36.07  & 35.83  & 36.25  & 39.84  & 39.38  & 37.04  & 40.24  & 34.72  \\
\cmidrule{3-21}          &       & /     & /     & 0.945  & /     & 0.972  & 0.965  & 0.970  & 0.977  & 0.990  & 0.968  & 0.968  & 0.975  & 0.956  & 0.971  & 0.984  & 0.976  & 0.969  & 0.980  & 0.955  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DeamNet} & 39.63  & 39.35  & 36.63  & /     & 37.70  & 36.93  & 40.90  & 40.86  & 41.22  & 39.72  & 33.67  & 36.40  & 37.87  & 35.07  & 40.25  & 38.92  & 39.56  & 40.52  & 34.61  \\
\cmidrule{3-21}          &       & 0.953  & 0.955  & 0.936  & /     & 0.958  & 0.944  & 0.977  & 0.978  & 0.979  & 0.967  & 0.953  & 0.964  & 0.961  & 0.948  & 0.966  & 0.957  & 0.969  & 0.980  & 0.952  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DIDN} & 39.64  & 39.78  & 36.06  & /     & 37.36  & 38.24  & 40.74  & 41.68  & 42.35  & 41.17  & 38.15  & 37.87  & 38.27  & 38.58  & 40.03  & 40.32  & 39.73  & 44.07  & 35.28  \\
\cmidrule{3-21}          &       & 0.953  & 0.958  & 0.946  & /     & 0.953  & 0.950  & 0.975  & 0.977  & 0.975  & 0.966  & 0.951  & 0.965  & 0.954  & 0.950  & 0.963  & 0.959  & 0.966  & 0.985  & 0.949  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DnCNN} & 37.90  & 37.73  & 37.47  & 39.32  & 38.51  & 40.01  & 40.81  & 41.91  & 44.16  & 41.57  & 39.92  & 38.72  & 39.34  & 40.22  & 42.03  & 42.12  & 40.26  & 43.97  & 36.30  \\
\cmidrule{3-21}          &       & 0.943  & 0.941  & 0.954  & 0.974  & 0.966  & 0.971  & 0.972  & 0.979  & 0.991  & 0.969  & 0.962  & 0.973  & 0.964  & 0.969  & 0.983  & 0.977  & 0.970  & 0.984  & 0.960  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DPIR} & /     & /     & 38.30  & 40.33  & 38.93  & 40.77  & 41.94  & 42.62  & 45.36  & 42.78  & 40.35  & 39.17  & 40.80  & 40.80  & 42.86  & 42.86  & 40.96  & 45.76  & 36.61  \\
\cmidrule{3-21}          &       & /     & /     & 0.961  & 0.979  & 0.970  & 0.974  & 0.978  & 0.982  & 0.993  & 0.977  & 0.969  & 0.975  & 0.966  & 0.970  & 0.985  & 0.980  & 0.974  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{DudeNet} & 33.18  & 27.55  & 36.03  & 37.44  & 39.92  & 38.18  & 39.94  & 41.13  & 42.97  & 41.06  & 38.63  & 37.83  & 39.09  & 38.58  & 40.73  & 40.63  & 39.71  & 43.34  & 35.44  \\
\cmidrule{3-21}          &       & 0.810  & 0.645  & 0.933  & 0.953  & 0.973  & 0.955  & 0.972  & 0.977  & 0.988  & 0.971  & 0.962  & 0.969  & 0.962  & 0.961  & 0.976  & 0.969  & 0.972  & 0.985  & 0.955  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{FCCF} & 36.30  & 23.32  & 39.02  & 40.89  & 38.87  & 41.20  & 42.03  & 43.07  & 45.15  & 42.80  & 40.14  & 39.04  & 40.61  & 40.66  & 42.31  & 43.05  & 40.95  & 45.47  & 36.72  \\
\cmidrule{3-21}          &       & 0.885  & 0.461  & 0.968  & 0.982  & 0.971  & 0.978  & 0.980  & 0.985  & 0.993  & 0.978  & 0.966  & 0.974  & 0.967  & 0.969  & 0.984  & 0.982  & 0.975  & 0.989  & 0.964  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{FFD-Net} & 37.61  & 38.27  & 37.67  & 39.73  & 38.76  & 40.28  & 41.67  & 42.55  & 44.77  & 42.44  & 40.05  & 38.96  & 40.60  & 40.50  & 42.43  & 42.44  & 40.75  & 45.71  & 36.47  \\
\cmidrule{3-21}          &       & 0.942  & 0.948  & 0.956  & 0.977  & 0.970  & 0.973  & 0.977  & 0.982  & 0.992  & 0.976  & 0.967  & 0.974  & 0.964  & 0.971  & 0.984  & 0.979  & 0.973  & 0.990  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{IDR} & /     & /     & 34.26  & 36.18  & 36.28  & 36.44  & 39.33  & 40.31  & 40.94  & 39.74  & 37.38  & 37.39  & 38.30  & 38.15  & 39.68  & 38.22  & 38.01  & 43.15  & 34.64  \\
\cmidrule{3-21}          &       & /     & /     & 0.877  & 0.923  & 0.925  & 0.910  & 0.955  & 0.962  & 0.961  & 0.935  & 0.927  & 0.957  & 0.938  & 0.944  & 0.951  & 0.913  & 0.941  & 0.978  & 0.929  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{InvDN} & 39.57  & 39.28  & 34.55  & 36.33  & 35.94  & 38.01  & 38.95  & 40.09  & 42.03  & 40.02  & 33.32  & 37.00  & 36.64  & 37.66  & 40.06  & 40.98  & 39.10  & 40.74  & 34.15  \\
\cmidrule{3-21}          &       & 0.952  & 0.955  & 0.937  & 0.953  & 0.947  & 0.952  & 0.965  & 0.973  & 0.978  & 0.960  & 0.930  & 0.965  & 0.939  & 0.955  & 0.966  & 0.971  & 0.964  & 0.969  & 0.935  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{IRCNN} & 34.78  & 33.50  & 37.26  & 37.25  & 37.49  & 39.66  & 41.24  & 41.85  & 43.89  & 41.78  & 39.91  & 38.63  & 40.14  & 40.12  & 41.87  & 41.86  & 40.26  & 44.38  & 36.22  \\
\cmidrule{3-21}          &       & 0.907  & 0.887  & 0.954  & 0.956  & 0.956  & 0.970  & 0.978  & 0.981  & 0.991  & 0.973  & 0.969  & 0.972  & 0.965  & 0.969  & 0.983  & 0.977  & 0.972  & 0.988  & 0.961  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{MIRNet} & 39.88  & 39.55  & 36.06  & 37.25  & 37.49  & 38.10  & 40.72  & 41.68  & 42.76  & 41.05  & 38.28  & 37.80  & 38.60  & 38.55  & 40.28  & 40.46  & 39.73  & 43.66  & 35.42  \\
\cmidrule{3-21}          &       & 0.956  & 0.957  & 0.942  & 0.956  & 0.956  & 0.952  & 0.975  & 0.978  & 0.980  & 0.968  & 0.954  & 0.967  & 0.959  & 0.952  & 0.966  & 0.964  & 0.967  & 0.983  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{MPRNet} & 39.82  & 39.57  & 35.94  & /     & 37.50  & 38.04  & 40.59  & 41.30  & 42.59  & 41.23  & 38.35  & 37.92  & 38.95  & 38.62  & 40.21  & 40.20  & 39.77  & 44.05  & 35.49  \\
\cmidrule{3-21}          &       & 0.954  & 0.958  & 0.935  & /     & 0.954  & 0.946  & 0.974  & 0.974  & 0.978  & 0.969  & 0.952  & 0.966  & 0.960  & 0.949  & 0.965  & 0.960  & 0.967  & 0.986  & 0.951  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{NAFNet} & 38.36  & 40.15  & 34.39  & /     & 36.38  & 37.88  & 40.12  & 40.23  & 40.66  & 40.01  & 36.13  & 35.87  & 36.66  & 36.79  & 36.53  & 39.93  & 39.32  & 40.45  & 34.82  \\
\cmidrule{3-21}          &       & 0.943  & 0.960  & 0.923  & /     & 0.947  & 0.954  & 0.973  & 0.943  & 0.936  & 0.962  & 0.919  & 0.927  & 0.948  & 0.927  & 0.884  & 0.951  & 0.966  & 0.924  & 0.948  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{NBNet} & 39.89  & 39.64  & 35.89  & /     & 37.37  & 38.32  & 40.95  & 41.91  & 42.92  & 41.17  & 38.02  & 37.87  & 37.79  & 38.45  & 40.51  & 40.45  & 39.73  & 43.96  & 35.37  \\
\cmidrule{3-21}          &       & 0.955  & 0.958  & 0.935  & /     & 0.957  & 0.955  & 0.977  & 0.980  & 0.982  & 0.971  & 0.955  & 0.967  & 0.956  & 0.955  & 0.972  & 0.967  & 0.969  & 0.984  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Neigh2Neigh} & /     & /     & 34.47  & 35.65  & 37.10  & 36.59  & 40.22  & 40.41  & 41.29  & 41.24  & 38.13  & 37.94  & 39.71  & 38.50  & 39.63  & 38.05  & 39.17  & 44.49  & 35.30  \\
\cmidrule{3-21}          &       & /     & /     & 0.883  & 0.907  & 0.942  & 0.908  & 0.967  & 0.960  & 0.966  & 0.958  & 0.940  & 0.961  & 0.956  & 0.936  & 0.952  & 0.919  & 0.958  & 0.984  & 0.944  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{NLNet} & /     & /     & 37.56  & 39.32  & 38.58  & 40.17  & 41.43  & 42.18  & 44.53  & 42.19  & 39.96  & 38.89  & 40.06  & 40.61  & 42.14  & 42.16  & 40.63  & 44.87  & 36.34  \\
\cmidrule{3-21}          &       & /     & /     & 0.955  & 0.974  & 0.968  & 0.973  & 0.976  & 0.981  & 0.991  & 0.974  & 0.969  & 0.973  & 0.964  & 0.971  & 0.983  & 0.978  & 0.973  & 0.988  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Noise2Noise} & /     & /     & 33.55  & 34.67  & 35.91  & 35.28  & 38.88  & 39.07  & 39.34  & 39.26  & 36.81  & 36.99  & 38.04  & 37.21  & 38.00  & 36.35  & 37.67  & 42.59  & 34.44  \\
\cmidrule{3-21}          &       & /     & /     & 0.850  & 0.874  & 0.913  & 0.875  & 0.950  & 0.940  & 0.938  & 0.931  & 0.919  & 0.948  & 0.936  & 0.916  & 0.924  & 0.876  & 0.936  & 0.975  & 0.926  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{PD-Denoising} & 38.40  & 33.99  & 35.85  & 37.13  & 37.13  & 37.12  & 40.85  & 41.38  & 41.13  & 41.05  & 37.72  & 37.57  & 39.03  & 38.01  & 39.18  & 39.64  & 38.80  & 43.73  & 35.05  \\
\cmidrule{3-21}          &       & 0.943  & 0.896  & 0.924  & 0.944  & 0.944  & 0.921  & 0.974  & 0.974  & 0.966  & 0.959  & 0.935  & 0.956  & 0.948  & 0.929  & 0.948  & 0.946  & 0.955  & 0.981  & 0.940  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{PNGAN} & 39.38  & 39.81  & 38.44  & /     & 39.57  & 40.51  & 41.79  & 43.13  & 44.73  & 42.55  & 39.84  & 38.78  & 40.63  & 40.20  & 41.85  & 43.15  & 40.87  & 45.32  & 36.40  \\
\cmidrule{3-21}          &       & 0.953  & 0.959  & 0.963  & /     & 0.974  & 0.974  & 0.979  & 0.985  & 0.992  & 0.977  & 0.964  & 0.970  & 0.969  & 0.962  & 0.981  & 0.982  & 0.974  & 0.988  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{R2R} & /     & /     & 36.32  & 38.11  & 38.57  & 38.71  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{3-21}          &       & /     & /     & 0.937  & 0.961  & 0.970  & 0.958  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Restormer} & 40.03  & 39.79  & 36.33  & /     & 37.66  & 38.29  & 41.10  & 41.84  & 42.49  & 41.47  & 38.42  & 38.08  & 39.05  & 38.77  & 40.13  & 40.53  & 39.56  & 44.19  & 35.65  \\
\cmidrule{3-21}          &       & 0.956  & 0.959  & 0.941  & /     & 0.956  & 0.948  & 0.977  & 0.979  & 0.976  & 0.968  & 0.952  & 0.966  & 0.960  & 0.949  & 0.963  & 0.962  & 0.963  & 0.986  & 0.953  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{RIDNet} & 39.26  & 38.70  & 36.84  & 38.11  & 38.57  & 38.60  & 41.09  & 42.15  & 42.39  & 41.59  & 38.88  & 38.21  & 38.67  & 39.02  & 40.91  & 41.01  & 40.07  & 44.40  & 35.76  \\
\cmidrule{3-21}          &       & 0.953  & 0.950  & 0.941  & 0.961  & 0.970  & 0.956  & 0.977  & 0.980  & 0.989  & 0.975  & 0.962  & 0.970  & 0.963  & 0.959  & 0.978  & 0.977  & 0.972  & 0.987  & 0.957  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{SADNet} & 39.59  & /     & 37.76  & 38.11  & 39.22  & 38.90  & 40.82  & 42.02  & 44.25  & 41.85  & 39.53  & 38.33  & 39.83  & 39.69  & 39.81  & 41.64  & 40.70  & 44.61  & 36.36  \\
\cmidrule{3-21}          &       & 0.952  & /     & 0.952  & 0.961  & 0.972  & 0.965  & 0.976  & 0.980  & 0.992  & 0.975  & 0.965  & 0.970  & 0.965  & 0.963  & 0.965  & 0.979  & 0.974  & 0.988  & 0.962  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Self2Self} & /     & /     & 36.26  & 38.23  & /     & 39.49  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{3-21}          &       & /     & /     & 0.947  & 0.969  & /     & 0.963  & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & /     & / \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{Unet} & /     & /     & 36.95  & 38.96  & 38.05  & 39.62  & 40.40  & 41.36  & 43.58  & 41.12  & 39.35  & 38.25  & 38.94  & 39.95  & 41.32  & 41.70  & 39.51  & 43.17  & 36.09  \\
\cmidrule{3-21}          &       & /     & /     & 0.943  & 0.971  & 0.962  & 0.967  & 0.968  & 0.977  & 0.989  & 0.968  & 0.963  & 0.971  & 0.959  & 0.968  & 0.979  & 0.974  & 0.966  & 0.981  & 0.958  \\
\cmidrule{2-21}          & \multirow{2}[4]{*}{VDNet} & /     & /     & 35.86  & /     & 37.58  & 38.43  & 40.97  & 42.37  & 43.08  & 41.19  & 38.23  & 37.95  & 37.88  & 38.60  & 40.81  & 41.21  & 39.93  & 44.27  & 35.49  \\
\cmidrule{3-21}          &       & /     & /     & 0.945  & /     & 0.957  & 0.955  & 0.976  & 0.983  & 0.983  & 0.970  & 0.956  & 0.968  & 0.956  & 0.956  & 0.973  & 0.970  & 0.970  & 0.984  & 0.953  \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_Results_Color_image_all}%
\end{table*}%


==> Table_color_all.tex <==
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Average PSNR, SSIM values and computational time of compared methods on CC15, Xu-100 and Kong-Image datasets. The average computational time is based on images of size $512 \times 512$. The best results are black bolded.}
%  \scalebox{0.83}{
%    \begin{tabular}{cccccccccccccccc}
%    \toprule
%    \multirow{2}[4]{*}{Method} & Dataset & CC15  & CC60  & Xu-100 & CANON 100D & CANON 600D & HUAWEI Honor6X & IPHONE 5S & IPHONE 6S & SONY A6500 & XIAOMI MI8 & OPPO R11s & FUJIFILM X100T & \multirow{2}[4]{*}{Implementation} & \multirow{2}[4]{*}{Time (s)} \\
%\cmidrule{2-14}          & \multicolumn{1}{l}{\# Images} & 15    & 60    & 100   & 55    & 25    & 30    & 36    & 67    & 36    & 50    & 39    & 71    &       &  \\
%    \midrule
%    \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{Noisy} & 33.41  & 34.51  & 35.97  & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{/} \\
%          &       & 0.8476  & 0.8712  & 0.9125  & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251  & 0.9356  & 0.9307  &       &  \\
%    \midrule
%    \multirow{28}[28]{*}{\shortstack[l]{DNN \\ methods}} & \multirow{2}[2]{*}{DnCNN} & 37.47  & 39.32  & 38.51  & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{3.28} \\
%          &       & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{FFD-Net} & 37.67  & 39.73  & 38.56  & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{1.99} \\
%          &       & 0.9563  & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBDNet} & 36.36  & 37.46  & 36.93  & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{3.58} \\
%          &       & 0.9294  & 0.9482  & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DBF} & 38.38  & 40.59  & 38.87  & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.32} \\
%          &       & 0.9644  & 0.9811  & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DIDN} & 36.04  & \multirow{2}[2]{*}{N/A} & 37.32  & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9456  &       & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{FCCF} & \textbf{39.04} & \textbf{40.89} & 38.85  & 41.91  & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.66} & \textbf{40.93} & \textbf{42.78} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{36.36} \\
%          &       & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & 0.9794  & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640} & \textbf{0.9747} & \textbf{0.9782} &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{NLNet} & 37.56  & 39.32  & 38.58  & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{49.98} \\
%          &       & 0.9554  & 0.9744  & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{Unet} & 36.95  & 38.96  & 38.05  & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{5.69} \\
%          &       & 0.9425  & 0.9708  & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{VDNet} & 35.86  & \multirow{2}[2]{*}{N/A} & 37.58  & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.21} \\
%          &       & 0.9454  &       & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{AINDNet} & 35.88  & 36.98  & 37.22  & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.29} \\
%          &       & 0.9113  & 0.9708  & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CycleISP} & 35.40  & 36.87  & 37.61  & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.38} \\
%          &       & 0.9158  & 0.9393  & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{RIDNet} & 36.83  & 38.11  & 38.57  & 41.08  & 42.18  & 38.88  & 38.69  & 39.02  & 44.40  & 35.75  & 40.08  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.06} \\
%          &       & 0.9406  & 0.9609  & 0.9702  & 0.9770  & 0.9801  & 0.9621  & 0.9627  & 0.9588  & 0.9873  & 0.9570  & 0.9719  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{SADNet} & 37.80  & \multirow{2}[2]{*}{N/A} & \textbf{39.30} & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.33} \\
%          &       & 0.9521  &       & \textbf{0.9725} & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DPIR} & 38.30  & 40.33  & 38.93  & \textbf{41.94} & 42.62  & \textbf{40.35} & \textbf{40.80} & \textbf{40.80} & 45.76  & 36.61  & \textbf{40.96} & \textbf{42.78} & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9608  & 0.9791  & 0.9700  & 0.9779  & 0.9819  & \textbf{0.9694} & 0.9661  & \textbf{0.9700} & 0.9895  & 0.9607  & 0.9741  & 0.9770  &       &  \\
%    \midrule
%    \midrule
%    \multirow{24}[24]{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{2}[2]{*}{LCSD} & 36.20  & 37.69  & 37.97  & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.45} \\
%          &       & 0.9339  & 0.9626  & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{LLRT} & 37.36  & 38.51  & 38.51  & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{>1000} \\
%          &       & 0.9559  & 0.9636  & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{GID} & 37.02  & 38.41  & 38.37  & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{38.88} \\
%          &       & 0.9459  & 0.9633  & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{MCWNNM} & 37.72  & 39.03  & 38.51  & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{228.16} \\
%          &       & 0.9568  & 0.9698  & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{NLH\_CC} & 38.49  & 39.86  & 38.36  & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & \textbf{46.00} & 35.73  & 40.69  & \textbf{42.80 } & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{51.86} \\
%          &       & 0.9647  & 0.9759  & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905} & 0.9552  & 0.9740  & 0.9776  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{TWSC} & 37.90  & 39.66  & 38.62  & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{368.68} \\
%          &       & 0.9592  & 0.9759  & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{M-SVD} & 37.62  & 39.27  & 38.56  & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{75.88} \\
%          &       & 0.9542  & 0.9705  & 0.9671  & 0.9788  & 0.9823  & 0.9671  & \textbf{0.9680} & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{4DHOSVD1} & 37.51  & 39.15  & 38.51  & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & \multirow{2}[2]{*}{Pure MATLAB} & \multirow{2}[2]{*}{86.69} \\
%          &       & 0.9559  & 0.9729  & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CMSt-SVD} & 37.95  & 39.75  & 38.82  & \textbf{41.99} & 42.75  & 40.08  & \textbf{40.84} & 40.53  & 45.89  & 36.40  & 40.85  & 42.68  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.18} \\
%          &       & 0.9588  & 0.9756  & 0.9694  & \textbf{0.9794} & 0.9840  & 0.9674  & 0.9668  & 0.9674  & 0.9903  & 0.9616  & 0.9743  & 0.9770  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D1} & 37.56  & 39.21  & 38.52  & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{0.95} \\
%          &       & 0.9562  & 0.9729  & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D2} & 37.70  & 39.41  & 38.69  & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{4.38} \\
%          &       & 0.9572  & 0.9740  & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D\_best} & 37.95  & 39.68  & 38.81  & \textbf{42.08 } & 42.89  & \textbf{40.48} & \textbf{41.25} & \textbf{41.16} & 45.81  & \textbf{36.66} & \textbf{40.89} & \textbf{43.14} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{4.38} \\
%          &       & 0.9621  & 0.9775  & 0.9712  & \textbf{0.9808} & 0.9851  & \textbf{0.9741} & \textbf{0.9758} & \textbf{0.9783} & 0.9904  & \textbf{0.9640} & 0.9742  & \textbf{0.9805} &       &  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_color_all}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet2'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Average PSNR, SSIM values and computational time (second) on four realistic color image datasets. The average time is calculated based on the PolyU dataset, and 'N/A' means the models can not handle certain size of images. The best results (excluding CBM3D\_best) are black bolded.}
%    \scalebox{0.806}{
%    \renewcommand{\arraystretch}{0.399}
%    \begin{tabular}{cccccccccccccccc}
%    \toprule
%    \multirow{3}[6]{*}{Method} & \multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multicolumn{9}{c}{IOCI}                                        & \multirow{3}[6]{*}{Implementation} & \multirow{3}[6]{*}{Time (s)} \\
%\cmidrule{6-14}          &       &       &       &       & CANON 100D & CANON 600D & HUAWEI Honor6X & IPHONE 5S & IPHONE 6S & SONY A6500 & XIAOMI MI8 & OPPO R11s & FUJIFILM X100T &       &  \\
%\cmidrule{2-14}          & \multicolumn{1}{l}{\# Images} & 15    & 60    & 100   & 55    & 25    & 30    & 36    & 67    & 36    & 50    & 39    & 71    &       &  \\
%    \midrule
%    \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{Noisy} & 33.41  & 34.51  & 35.97  & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{/} \\
%          &       & 0.8476  & 0.8712  & 0.9125  & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251  & 0.9356  & 0.9307  &       &  \\
%    \midrule
%    \multirow{32}[32]{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{2}[2]{*}{LCSD} & 36.20  & 37.69  & 37.97  & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.45} \\
%          &       & 0.9339  & 0.9626  & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{LLRT} & 37.36  & 38.51  & 38.51  & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{$>$1000} \\
%          &       & 0.9559  & 0.9636  & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{GID} & 37.02  & 38.41  & 38.37  & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{38.88} \\
%          &       & 0.9459  & 0.9633  & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{MCWNNM} & 37.72  & 39.03  & 38.51  & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{228.16} \\
%          &       & 0.9568  & 0.9698  & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{NLH} & 38.49  & 39.86  & 38.36  & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & 46.00  & 35.73  & 40.69  & 42.80  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{51.86} \\
%          &       & 0.9647  & 0.9759  & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & 0.9905  & 0.9552  & 0.9740  & 0.9776  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{TWSC} & 37.90  & 39.66  & 38.62  & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{368.68} \\
%          &       & 0.9592  & 0.9759  & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{M-SVD} & 37.62  & 39.27  & 38.56  & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{75.88} \\
%          &       & 0.9542  & 0.9705  & 0.9671  & 0.9788  & 0.9823  & 0.9671  & 0.9680  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{4DHOSVD} & 37.51  & 39.15  & 38.51  & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{80.69} \\
%          &       & 0.9559  & 0.9729  & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CMSt-SVD} & 37.95  & 39.75  & 38.82  & \textbf{41.99} & 42.75  & 40.08  & \textbf{40.84} & 40.53  & \textbf{45.89} & 36.40  & \textbf{40.85} & 42.68  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.18} \\
%          &       & 0.9588  & 0.9756  & 0.9694  & \textbf{0.9794} & 0.9840  & 0.9674  & 0.9668  & 0.9674  & \textbf{0.9903} & 0.9616  & 0.9743  & 0.9770  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D1} & 37.56  & 39.21  & 38.52  & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{0.95} \\
%          &       & 0.9562  & 0.9729  & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D2} & 37.70  & 39.41  & 38.69  & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{4.38} \\
%          &       & 0.9572  & 0.9740  & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D\_best} & 37.95  & 39.68  & 38.81  & \textbf{42.08} & 42.89  & \textbf{40.48} & \textbf{41.25} & \textbf{41.16} & \textbf{45.81} & \textbf{36.66} & \textbf{40.89} & \textbf{43.14} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{/} \\
%          &       & 0.9621  & 0.9775  & 0.9712  & \textbf{0.9808} & 0.9851  & \textbf{0.9741} & \textbf{0.9758} & \textbf{0.9783} & \textbf{0.9904} & \textbf{0.9640} & 0.9742  & \textbf{0.9805} &       &  \\
%    \midrule
%    \midrule
%    \multirow{52}[52]{*}{\shortstack[l]{DNN \\ methods}} & \multirow{2}[2]{*}{DnCNN} & 37.47  & 39.32  & 38.51  & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{3.28} \\
%          &       & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{FFDNet} & 37.68  & 39.73  & 38.56  & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{1.99} \\
%          &       & 0.9563  & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CBDNet} & 36.36  & 37.46  & 36.93  & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{3.58} \\
%          &       & 0.9294  & 0.9482  & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DBF} & 38.38  & 40.59  & 38.87  & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.32} \\
%          &       & 0.9644  & 0.9811  & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DIDN} & 36.04  & \multirow{2}[2]{*}{N/A} & 37.32  & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9456  &       & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{FCCF} & \textbf{39.04} & \textbf{40.89} & 38.85  & \textbf{41.91} & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.66 } & \textbf{40.93} & \textbf{42.78} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{36.36} \\
%          &       & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & \textbf{0.9794} & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640} & \textbf{0.9747} & \textbf{0.9782} &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{NLNet} & 37.56  & 39.32  & 38.58  & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{49.98} \\
%          &       & 0.9554  & 0.9744  & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{UDnet} & 36.95  & 38.96  & 38.05  & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{5.69} \\
%          &       & 0.9425  & 0.9708  & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{VDNet} & 35.86  & \multirow{2}[2]{*}{N/A} & 37.58  & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.21} \\
%          &       & 0.9454  &       & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{AINDNet} & 35.88  & 36.98  & 37.22  & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.29} \\
%          &       & 0.9113  & 0.9708  & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{CycleISP} & 35.40  & 36.87  & 37.61  & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.38} \\
%          &       & 0.9158  & 0.9393  & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{RIDNet} & 36.83  & 38.11  & 38.57  & 41.08  & 42.18  & 38.88  & 38.69  & 39.02  & 44.40  & 35.75  & 40.08  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.06} \\
%          &       & 0.9406  & 0.9609  & 0.9702  & 0.9770  & 0.9801  & 0.9621  & 0.9627  & 0.9588  & 0.9873  & 0.9570  & 0.9719  & 0.9750  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{SADNet} & 37.80  & \multirow{2}[2]{*}{N/A} & 39.30 & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.33} \\
%          &       & 0.9521  &       & 0.9725 & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DANet} & 37.17  & 38.63  & \textbf{41.76}  & 41.59  & 42.47  & 38.46  & 39.39  & 38.80  & 44.71  & 36.21  & 39.92  & 41.44  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.12} \\
%          &       & 0.9528  & 0.9694  & \textbf{0.9771}  & 0.9788  & 0.9833  & 0.9545  & 0.9661  & 0.9527  & 0.9874  & 0.9608  & 0.9673  & 0.9693  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{Self2Self} & 36.26 & 37.88 &	37.50 &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A}
% & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{$>$2000} \\
%          &       & 0.9466 & 0.9672 & 0.9801 &  &	 &  &  &  &  &  &  &  &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{MIRNet} & 36.06 & 37.25 &	37.49 &	40.72 & 41.68 &	38.28 &	38.60 &	38.55 &	43.66 &	35.42 &	39.73 &	41.05
% & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9416 & 0.9556 & 0.9556 & 0.9747 &	0.9777 & 0.9539 & 0.9591 & 0.9522 & 0.9834 & 0.9525 & 0.9670 & 0.9679 &       &  \\
%\cmidrule{2-16}          & \multirow{2}[2]{*}{DRUNet} & 38.30  & 40.33  & 38.93  & \textbf{41.94} & 42.62  & \textbf{40.35} & 40.80  & \textbf{40.80} & 45.76  & 36.61  & \textbf{40.96} & \textbf{42.78} & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
%          &       & 0.9608  & 0.9791  & 0.9700  & 0.9779  & 0.9819  & \textbf{0.9694} & 0.9661  & \textbf{0.9700} & 0.9895  & 0.9607  & 0.9741  & 0.9770  &       &  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_color_all}%
%\end{table*}%


\begin{table*}[htbp]
\tiny
  \centering
  \caption{Average PSNR, SSIM values and computational time (second) on four realistic color image datasets. The average time is calculated based on the PolyU dataset, and 'N/A' means the models can not handle certain size of images. The best results (excluding CBM3D\_best) are black bolded.}
    \scalebox{0.808}{
    \renewcommand{\arraystretch}{0.66}
    \begin{tabular}{cccccccccccccccc}
    \toprule
    \multirow{3}[6]{*}{Method} & \multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{CC15} & \multirow{2}[4]{*}{CC60} & \multirow{2}[4]{*}{PolyU} & \multicolumn{9}{c}{IOCI}                                        & \multirow{3}[6]{*}{Implementation} & \multirow{3}[6]{*}{Time (s)} \\
\cmidrule{6-14}          &       &       &       &       & CANON 100D & CANON 600D & HUAWEI Honor6X & IPHONE 5S & IPHONE 6S & SONY A6500 & XIAOMI MI8 & OPPO R11s & FUJIFILM X100T &       &  \\
\cmidrule{2-14}          & \multicolumn{1}{l}{\# Images} & 15    & 60    & 100   & 55    & 25    & 30    & 36    & 67    & 36    & 50    & 39    & 71    &       &  \\
    \midrule
    \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{Noisy} & 33.41  & 34.51  & 35.97  & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & \multirow{2}[2]{*}{/} & \multirow{2}[2]{*}{/} \\
          &       & 0.8476  & 0.8712  & 0.9125  & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251  & 0.9356  & 0.9307  &       &  \\
    \midrule
    \multirow{28}[28]{*}{\shortstack[l]{Traditional \\ denoisers}} & \multirow{2}[2]{*}{LCSD} & 36.20  & 37.69  & 37.97  & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.45} \\
          &       & 0.9339  & 0.9626  & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{LLRT} & 37.36  & 38.51  & 38.51  & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{$>$1000} \\
          &       & 0.9559  & 0.9636  & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{GID} & 37.02  & 38.41  & 38.37  & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{38.88} \\
          &       & 0.9459  & 0.9633  & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{MCWNNM} & 37.72  & 39.03  & 38.51  & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{228.16} \\
          &       & 0.9568  & 0.9698  & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{NLH} & 38.49  & 39.86  & 38.36  & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & \textbf{46.00}  & 35.73  & 40.69  & 42.80  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{51.86} \\
          &       & 0.9647  & 0.9759  & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905}  & 0.9552  & 0.9740  & 0.9776  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{TWSC} & 37.90  & 39.66  & 38.62  & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{368.68} \\
          &       & 0.9592  & 0.9759  & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{M-SVD} & 37.62  & 39.27  & 38.56  & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{75.88} \\
          &       & 0.9542  & 0.9705  & 0.9671  & 0.9788  & 0.9823  & 0.9671  & \textbf{0.9680}  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{4DHOSVD} & 37.51  & 39.15  & 38.51  & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & \multirow{2}[2]{*}{MATLAB} & \multirow{2}[2]{*}{80.69} \\
          &       & 0.9559  & 0.9729  & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CMSt-SVD} & 37.95  & 39.75  & 38.82  & \textbf{41.99} & 42.75  & 40.08  & \textbf{40.84} & 40.53  & 45.89 & 36.40  & 40.85 & 42.68  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{6.18} \\
          &       & 0.9588  & 0.9756  & 0.9694  & \textbf{0.9794} & 0.9840  & 0.9674  & 0.9668  & 0.9674  & 0.9903 & 0.9616  & 0.9743  & 0.9770  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D1} & 37.56  & 39.21  & 38.52  & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{0.95} \\
          &       & 0.9562  & 0.9729  & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D2} & 37.70  & 39.41  & 38.69  & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{4.38} \\
          &       & 0.9572  & 0.9740  & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CBM3D\_best} & 37.95  & 39.68  & 38.81  & {42.08} & 42.89  & {40.48} & {41.25} & {41.16} & {45.81} & {36.66} & {40.89} & {43.14} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{/} \\
          &       & 0.9621  & 0.9775  & 0.9712  & {0.9808} & 0.9851  & {0.9741} & {0.9758} & {0.9783} & {0.9904} & {0.9640} & 0.9742  & {0.9805} &       &  \\
    \midrule
    \midrule
    \multirow{43}[43]{*}{\shortstack[l]{DNN \\ methods}} & \multirow{2}[2]{*}{DnCNN} & 37.47  & 39.32  & 38.51  & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{3.28} \\
          &       & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{FFDNet} & 37.68  & 39.73  & 38.56  & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{1.99} \\
          &       & 0.9563  & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & \textbf{0.9707}  & 0.9901  & 0.9607  & 0.9733  & 0.9759  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CBDNet} & 36.36  & 37.46  & 36.93  & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{3.58} \\
          &       & 0.9294  & 0.9482  & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{DBF} & 38.38  & 40.59  & 38.87  & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.32} \\
          &       & 0.9644  & 0.9811  & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{DIDN} & 36.04  & \multirow{2}[2]{*}{N/A} & 37.32  & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
          &       & 0.9456  &       & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{FCCF} & \textbf{39.04} & \textbf{40.89} & 38.85  & \textbf{41.91} & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.66 } & \textbf{40.93} & \textbf{42.78} & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{36.36} \\
          &       & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & \textbf{0.9794} & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9888  & \textbf{0.9640} & \textbf{0.9747} & \textbf{0.9782} &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{NLNet} & 37.56  & 39.32  & 38.58  & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{49.98} \\
          &       & 0.9554  & 0.9744  & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & \textbf{0.9709}  & 0.9875  & 0.9617  & 0.9729  & 0.9739  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{UDnet} & 36.95  & 38.96  & 38.05  & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & \multirow{2}[2]{*}{MATLAB + MEX} & \multirow{2}[2]{*}{5.69} \\
          &       & 0.9425  & 0.9708  & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{VDNet} & 35.86  & \multirow{2}[2]{*}{N/A} & 37.58  & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.21} \\
          &       & 0.9454  &       & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{AINDNet} & 35.88  & 36.98  & 37.22  & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.18  & 34.49  & 37.20  & 38.50  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.29} \\
          &       & 0.9113  & 0.9305  & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{CycleISP} & 35.40  & 36.87  & 37.61  & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.38} \\
          &       & 0.9158  & 0.9393  & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{RIDNet} & 36.83  & 38.11  & 38.57  & 41.08  & 42.18  & 38.88  & 38.69  & 39.02  & 44.40  & 35.75  & 40.08  & 41.58  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{1.06} \\
          &       & 0.9406  & 0.9609  & 0.9702  & 0.9770  & 0.9801  & 0.9621  & 0.9627  & 0.9588  & 0.9873  & 0.9570  & 0.9719  & 0.9750  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{SADNet} & 37.80  & \multirow{2}[2]{*}{N/A} & 39.30 & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.33} \\
          &       & 0.9521  &       & 0.9725 & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{DANet} & 37.17  & 38.63  & \textbf{41.76}  & 41.59  & 42.47  & 38.46  & 39.39  & 38.80  & 44.71  & 36.21  & 39.92  & 41.44  & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.12} \\
          &       & 0.9528  & 0.9694  & \textbf{0.9771}  & 0.9788  & 0.9833  & 0.9545  & 0.9661  & 0.9527  & 0.9874  & 0.9608  & 0.9673  & 0.9693  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{Self2Self} & 36.26 & 37.88 &	37.66 &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A} &	\multirow{2}[2]{*}{N/A} & \multirow{2}[2]{*}{N/A}
 & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{$>$2000} \\
          &       & 0.9466 & 0.9672 & 0.9563 &  &	 &  &  &  &  &  &  &  &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{MIRNet} & 36.06 & 37.25 &	37.49 &	40.72 & 41.68 &	38.28 &	38.60 &	38.55 &	43.66 &	35.42 &	39.73 &	41.05
 & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
          &       & 0.9416 & 0.9556 & 0.9556 & 0.9747 &	0.9777 & 0.9539 & 0.9591 & 0.9522 & 0.9834 & 0.9525 & 0.9670 & 0.9679 &       &  \\
\cmidrule{2-16}          & \multirow{2}[2]{*}{DRUNet} & 38.30  & 40.33  & 38.93  & \textbf{41.94} & 42.62  & \textbf{40.35} & \textbf{40.80}  & \textbf{40.80} & 45.76  & 36.61  & \textbf{40.96} & \textbf{42.78} & \multirow{2}[2]{*}{Python + GPU} & \multirow{2}[2]{*}{0.18} \\
          &       & 0.9608  & 0.9791  & 0.9700  & 0.9779  & 0.9819  & \textbf{0.9694} & 0.9661  & 0.9700 & 0.9895  & 0.9607  & 0.9741  & 0.9770  &       &  \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_color_all}%
\end{table*}%




==> Table_color_all_psnr.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%\renewcommand{\arraystretch}{0.9}
%\tiny
%  \centering
%  \caption{Average PSNR and computational time of compared methods on CC15, Xu-100 and Kong-Image datasets. The average computational time is based on images of size $512 \times 512$.}
%  \scalebox{0.96}{
%    \begin{tabular}{cccccccccccccccc}
%    \toprule
%    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset}                                                                  & \multirow{2}[4]{*}{Implementation} & \multirow{2}[4]{*}{Time (s)} \\
%\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI &       &  \\
%    \midrule
%    \multicolumn{2}{c}{Noisy} & 33.41 & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & MATLAB + MEX & 1.99  \\
%    \midrule
%    \multirow{12}[24]{*}{Deep Network} & FFDNet & 37.67  & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & MATLAB + MEX & 3.58  \\
%\cmidrule{2-16}          & CBDNet & 36.36  & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & Python + GPU & 0.32  \\
%\cmidrule{2-16}          & DeepBoosting & 38.38  & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & Python + GPU & 0.18  \\
%\cmidrule{2-16}          & DIDN  & 36.04  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & Python + GPU & 0.98  \\
%\cmidrule{2-16}          & FCCF  & 39.04  & 40.89  & 38.85 & 41.91  & 43.07  & 40.11  & 40.39  & 40.65  & 45.38  & 36.67  & 40.93  & 42.78  & MATLAB + MEX & 49.98  \\
%\cmidrule{2-16}          & NLNet & 37.56  & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & MATLAB + MEX & 5.69  \\
%\cmidrule{2-16}          & Unet  & 36.95  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & Python + GPU & 0.21  \\
%\cmidrule{2-16}          & VDNet & 35.86  & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & Python + GPU & 1.29  \\
%\cmidrule{2-16}          & AINDNet & 35.88  & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & Python + GPU & 0.98  \\
%\cmidrule{2-16}          & CycleISP & 35.40  & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & Python + GPU & 0.38  \\
%\cmidrule{2-16}          & SADNet & 37.80  & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & Python + GPU & 0.33  \\
%\cmidrule{2-16}          & DnCNN & 37.47  & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & MATLAB + MEX & 3.28  \\
%    \midrule
%    \midrule
%    \multirow{12}[24]{*}{Gaussian} & LCSD  & 36.20  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & MATLAB + MEX & 6.45  \\
%\cmidrule{2-16}          & LLRT  & 37.36  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & Pure MATLAB & $>$1000 \\
%\cmidrule{2-16}          & GID   & 37.02  & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & Pure MATLAB  & 38.88  \\
%\cmidrule{2-16}          & MCWNNM & 37.72  & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & Pure MATLAB & 228.16  \\
%\cmidrule{2-16}          & NLH\_CC & 38.49  & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & 46.00  & 35.73  & 40.69  & 42.80  & MATLAB + MEX & 51.86  \\
%\cmidrule{2-16}          & TWSC  & 37.90  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & Pure MATLAB & 368.68  \\
%\cmidrule{2-16}          & CBM3D1 & 37.56  & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & MATLAB + MEX & 0.95  \\
%\cmidrule{2-16}          & CBM3D2 & 37.70  & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & MATLAB + MEX & 4.38  \\
%\cmidrule{2-16}          & M-SVD & 37.62  & 39.27 & 38.56 & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & Pure MATLAB & 4.38  \\
%\cmidrule{2-16}          & CBM3D\_best & 37.95  & 39.68 & 38.81 & 42.08 & 42.89 & 40.48 & 41.25 & 41.16 & 45.81 & 36.66  & 40.89  & 43.14  & Pure MATLAB & 75.88  \\
%\cmidrule{2-16}          & 4DHOSVD1 & 37.51  & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & Pure MATLAB & 86.69  \\
%\cmidrule{2-16}          & CMSt-SVD & 37.95  & 39.75 & 38.82 & 41.99  & 42.75  & 40.08  & 40.84  & 40.53  & 45.89  & 36.40  & 40.85  & 42.68  & MATLAB + MEX & 6.18  \\
%    \bottomrule
%    \end{tabular}}%
%  \label{Table_color_all_psnr}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Average PSNR values and computational time of compared methods on CC15, Xu-100 and Kong-Image datasets. The average computational time is based on images of size $512 \times 512$. The best results are black bolded.}
    \scalebox{0.96}{
    \renewcommand{\arraystretch}{0.69}
    \begin{tabular}{cccccccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset}                                                                  & \multirow{2}[4]{*}{Implementation} & \multirow{2}[4]{*}{Time (s)} \\
\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO& FUJIFILM &       &  \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 33.41 & 34.51  & 35.97 & 38.94  & 39.17  & 36.94  & 38.21  & 37.30  & 42.89  & 34.49  & 37.84  & 39.39  & MATLAB + MEX & 1.99  \\
    \midrule
    \multirow{12}[24]{*}{\shortstack[l]{Deep \\ Network}} & FFDNet & 37.67  & 39.73  & 38.56 & 41.67  & 42.55  & 40.05  & 40.60  & 40.49  & 45.71  & 36.47  & 40.75  & 42.44  & MATLAB + MEX & 3.58  \\
\cmidrule{2-16}          & CBDNet & 36.36  & 37.46  & 36.93 & 39.43  & 41.26  & 37.11  & 38.56  & 37.62  & 42.17  & 35.09  & 37.68  & 40.21  & Python + GPU & 0.32  \\
\cmidrule{2-16}          & DeepBoosting & 38.38  & 40.59  & 38.87 & 41.36  & 42.87  & 39.98  & 39.89  & 40.26  & 44.42  & 36.45  & 40.67  & 42.36  & Python + GPU & 0.18  \\
\cmidrule{2-16}          & DIDN  & 36.04  & N/A   & 37.32 & 40.66  & 41.58  & 38.09  & 38.22  & 38.50  & 43.89  & 35.25  & 39.66  & 41.17  & Python + GPU & 0.98  \\
\cmidrule{2-16}          & FCCF  & \textbf{39.04} & \textbf{40.89} & \textbf{38.85} & \textbf{41.91} & \textbf{43.07} & 40.11  & 40.39  & 40.65  & 45.38  & \textbf{36.67} & \textbf{40.93} & 42.78  & MATLAB + MEX & 49.98  \\
\cmidrule{2-16}          & NLNet & 37.56  & 39.32  & 38.58 & 41.43  & 42.18  & 39.96  & 40.06  & 40.61  & 44.84  & 36.34  & 40.63  & 42.19  & MATLAB + MEX & 5.69  \\
\cmidrule{2-16}          & Unet  & 36.95  & 38.96  & 38.05 & 40.40  & 41.36  & 39.35  & 38.94  & 39.95  & 43.15  & 36.09  & 39.51  & 41.12  & Python + GPU & 0.21  \\
\cmidrule{2-16}          & VDNet & 35.86  & N/A   & 37.58 & 40.97  & 42.37  & 38.23  & 37.88  & 38.60  & 44.27  & 35.49  & 39.93  & 41.19  & Python + GPU & 1.29  \\
\cmidrule{2-16}          & AINDNet & 35.88  & 36.98  & 37.22 & 38.28  & 39.21  & 36.53  & 36.68  & 36.83  & 40.17  & 34.49  & 37.20  & 38.50  & Python + GPU & 0.98  \\
\cmidrule{2-16}          & CycleISP & 35.40  & 36.87  & 37.61 & 41.24  & 41.79  & 38.43  & 38.69  & 38.60  & 44.71  & 35.50  & 39.85  & 41.58  & Python + GPU & 0.38  \\
\cmidrule{2-16}          & SADNet & 37.80  & N/A   & 39.3  & 40.74  & 42.03  & 39.55  & 39.91  & 39.72  & 44.69  & 36.38  & 40.72  & 41.91  & Python + GPU & 0.33  \\
\cmidrule{2-16}          & DnCNN & 37.47  & 39.32  & 38.51 & 40.81  & 41.91  & 39.92  & 39.34  & 40.22  & 43.94  & 36.30  & 40.26  & 41.57  & MATLAB + MEX & 3.28  \\
    \midrule
    \midrule
    \multirow{12}[24]{*}{\shortstack[l]{Traditional \\ Denoiser}} & LSCD  & 36.20  & 37.69 & 37.97 & 40.65  & 41.45  & 39.22  & 39.84  & 39.53  & 44.32  & 35.18  & 38.69  & 38.75  & MATLAB + MEX & 6.45  \\
\cmidrule{2-16}          & LLRT  & 37.36  & 38.51 & 38.51 & 41.84  & 42.53  & 39.54  & 40.02  & 39.72  & 45.71  & 34.93  & 36.63  & 39.19  & Pure MATLAB & $>$1000 \\
\cmidrule{2-16}          & GID   & 37.02  & 38.41 & 38.37 & 40.86  & 41.60  & 39.52  & 40.12  & 40.16  & 44.94  & 36.11  & 40.50  & 42.31  & Pure MATLAB & 38.88  \\
\cmidrule{2-16}          & MCWNNM & 37.72  & 39.03 & 38.51 & 41.47  & 42.07  & 39.46  & 39.87  & 40.18  & 45.37  & 35.84  & 40.71  & 42.48  & Pure MATLAB & 228.16  \\
\cmidrule{2-16}          & NLH\_CC & 38.49  & 39.86 & 38.36 & 41.77  & 42.72  & 38.84  & 40.44  & 39.94  & \textbf{46.00 } & 35.73  & 40.69  & 42.80  & MATLAB + MEX & 51.86  \\
\cmidrule{2-16}          & TWSC  & 37.90  & 39.66 & 38.62 & 41.65  & 42.52  & 39.71  & 40.27  & 40.12  & 45.48  & 35.41  & 40.71  & 42.22  & Pure MATLAB & 368.68  \\
\cmidrule{2-16}          & CBM3D1 & 37.56  & 39.21 & 38.52 & 41.71  & 42.50  & 39.93  & 40.56  & 40.45  & 45.56  & 36.30  & 40.62  & 42.53  & MATLAB + MEX & 0.95  \\
\cmidrule{2-16}          & CBM3D2 & 37.70  & 39.41 & 38.69 & 41.69  & 42.54  & 39.97  & 40.77  & 40.55  & 45.70  & 36.38  & 40.75  & 42.65  & MATLAB + MEX & 4.38  \\
\cmidrule{2-16}          & M-SVD & 37.62  & 39.27 & 38.56 & 41.81  & 42.54  & 39.94  & 40.66  & 40.35  & 45.69  & 36.24  & 40.69  & 42.52  & Pure MATLAB & 4.38  \\
\cmidrule{2-16}          & CBM3D\_best & 37.95  & 39.68 & \textbf{38.81} & \textbf{42.08} & 42.89 & \textbf{40.48} & \textbf{41.25} & \textbf{41.16} & \textbf{45.81} & \textbf{36.66} & \textbf{40.89} & \textbf{43.14} & MATLAB + mex & 75.88  \\
\cmidrule{2-16}          & 4DHOSVD1 & 37.51  & 39.15 & 38.51 & 41.41  & 42.14  & 39.82  & 40.68  & 40.36  & 45.56  & 36.17  & 40.69  & 42.47  & Pure MATLAB & 86.69  \\
\cmidrule{2-16}          & CMSt-SVD & 37.95  & 39.75 & \textbf{38.82} & \textbf{41.99} & 42.75  & 40.08  & 40.84  & 40.53  & \textbf{45.89} & 36.40  & \textbf{40.85} & 42.68  & MATLAB + MEX & 6.18  \\
    \bottomrule
    \end{tabular}}%
  \label{Table_color_all_psnr}%
\end{table*}%



==> Table_color_all_ssim.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Add caption}
%    \begin{tabular}{c|ccccccccccccc}
%    \multicolumn{2}{c}{\multirow{2}[3]{*}{Method}} & \multicolumn{12}{c}{Dataset} \\
%\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI \\
%    \midrule
%    \multicolumn{2}{c}{Noisy} & 0.8476 & 0.8712 & 0.9125 & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251 & 0.9356  & 0.9307  \\
%    \midrule
%    \multirow{12}[24]{*}{Deep Network} & FFD-Net & 0.9563 & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  \\
%\cmidrule{2-14}          & CBDNet & 0.9294 & 0.9482 & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  \\
%\cmidrule{2-14}          & DeepBoosting & 0.9644 & 0.9811 & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  \\
%\cmidrule{2-14}          & DIDN  & 0.9456 & N/A   & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  \\
%\cmidrule{2-14}          & FCCF  & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & 0.9794  & \textbf{0.9852 } & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640 } & \textbf{0.9747 } & 0.9782  \\
%\cmidrule{2-14}          & NLNet & 0.9554 & 0.9744 & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  \\
%\cmidrule{2-14}          & Unet  & 0.9425 & 0.9708 & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  \\
%\cmidrule{2-14}          & VDNet & 0.9454 & N/A   & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  \\
%\cmidrule{2-14}          & AINDNet & 0.9113 & 0.9708 & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  \\
%\cmidrule{2-14}          & CycleISP & 0.9158 & 0.9393 & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  \\
%\cmidrule{2-14}          & SADNet & 0.9521 & N/A   & 0.9725  & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  \\
%\cmidrule{2-14}          & DnCNN & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  \\
%    \midrule
%    \midrule
%    \multirow{12}[24]{*}{Gaussian Denoiser} & LCSD  & 0.9339 & 0.9626 & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  \\
%\cmidrule{2-14}          & LLRT  & 0.9559 & 0.9636 & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  \\
%\cmidrule{2-14}          & GID   & 0.9459 & 0.9633 & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  \\
%\cmidrule{2-14}          & MCWNNM & 0.9568 & 0.9698 & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  \\
%\cmidrule{2-14}          & NLH\_CC & 0.9647 & 0.9759 & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905 } & 0.9552  & 0.9740  & 0.9776  \\
%\cmidrule{2-14}          & TWSC  & 0.9592 & 0.9759 & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  \\
%\cmidrule{2-14}          & CBM3D1 & 0.9562 & 0.9729 & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  \\
%\cmidrule{2-14}          & CBM3D2 & 0.9572 & 0.974 & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  \\
%\cmidrule{2-14}          & M-SVD & 0.9542 & 0.9705 & 0.9671  & 0.9788  & 0.9823  & 0.9671  & 0.9680  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  \\
%\cmidrule{2-14}          & CBM3D\_best & 0.9621 & 0.9775 & \textbf{0.9712 } & \textbf{0.9808 } & \textbf{0.9851 } & \textbf{0.9741 } & \textbf{0.9758 } & \textbf{0.9783 } & \textbf{0.9904 } & \textbf{0.9640 } & 0.9742  & \textbf{0.9805 } \\
%\cmidrule{2-14}          & 4DHOSVD1 & 0.9559 & 0.9729 & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  \\
%\cmidrule{2-14}          & CMSt-SVD & 0.9588 & 0.9756 & 0.9694  & 0.9794  & 0.9840  & 0.9674  & 0.9668  & 0.9674  & \textbf{0.9903 } & 0.9616  & \textbf{0.9743 } & 0.9770  \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_color_all_ssim}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
\tiny
  \centering
    \caption{Average SSIM values of compared methods on CC15, Xu-100 and Kong-Image datasets. The best results are black bolded.}
    \renewcommand{\arraystretch}{0.69}
    \begin{tabular}{cccccccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{Method}} & \multicolumn{12}{c}{Dataset} \\
\cmidrule{3-14}    \multicolumn{2}{c}{} & CC15  & CC60  & Xu-100 & CAN 100D & CAN 600D & HUAWEI & IP 5S & IP 6S & SONY & XIAOMI & OPPO & FUJI \\
    \midrule
    \multicolumn{2}{c}{Noisy} & 0.8476 & 0.8712 & 0.9125 & 0.9482  & 0.9379  & 0.9185  & 0.9359  & 0.9143  & 0.9753  & 0.9251 & 0.9356  & 0.9307  \\
    \midrule
    \multirow{12}[24]{*}{Deep Network} & FFDNet & 0.9563 & 0.9770  & 0.9658  & 0.9768  & 0.9824  & 0.9669  & 0.9645  & 0.9707  & 0.9901  & 0.9607  & 0.9733  & 0.9759  \\
\cmidrule{2-14}          & CBDNet & 0.9294 & 0.9482 & 0.9457  & 0.9729  & 0.9788  & 0.9505  & 0.9586  & 0.9428  & 0.9819  & 0.9493  & 0.9601  & 0.9621  \\
\cmidrule{2-14}          & DeepBoosting & 0.9644 & 0.9811 & 0.9698  & 0.9765  & 0.9841  & 0.9669  & 0.9634  & 0.9660  & 0.9804  & 0.9631  & 0.9734  & 0.9751  \\
\cmidrule{2-14}          & DIDN  & 0.9456 & N/A   & 0.9523  & 0.9739  & 0.9760  & 0.9500  & 0.9535  & 0.9493  & 0.9840  & 0.9485  & 0.9647  & 0.9655  \\
\cmidrule{2-14}          & FCCF  & \textbf{0.9675} & \textbf{0.9819} & 0.9699  & 0.9794  & \textbf{0.9852} & 0.9656  & 0.9659  & 0.9680  & 0.9887  & \textbf{0.9640} & \textbf{0.9747} & 0.9782  \\
\cmidrule{2-14}          & NLNet & 0.9554 & 0.9744 & 0.9684  & 0.9759  & 0.9811  & 0.9687  & 0.9637  & 0.9709  & 0.9875  & 0.9617  & 0.9729  & 0.9739  \\
\cmidrule{2-14}          & Unet  & 0.9425 & 0.9708 & 0.9622  & 0.9683  & 0.9774  & 0.9631  & 0.9591  & 0.9683  & 0.9811  & 0.9582  & 0.9660  & 0.9675  \\
\cmidrule{2-14}          & VDNet & 0.9454 & N/A   & 0.9574  & 0.9763  & 0.9831  & 0.9555  & 0.9562  & 0.9556  & 0.9844  & 0.9530  & 0.9699  & 0.9701  \\
\cmidrule{2-14}          & AINDNet & 0.9113 & 0.9708 & 0.9460  & 0.9748  & 0.9759  & 0.9544  & 0.9581  & 0.9527  & 0.9812  & 0.9523  & 0.9676  & 0.9656  \\
\cmidrule{2-14}          & CycleISP & 0.9158 & 0.9393 & 0.9546  & 0.9766  & 0.9770  & 0.9515  & 0.9605  & 0.9518  & 0.9874  & 0.9489  & 0.9682  & 0.9688  \\
\cmidrule{2-14}          & SADNet & 0.9521 & N/A   & 0.9725  & 0.9758  & 0.9797  & 0.9646  & 0.9656  & 0.9626  & 0.9886  & 0.9620  & 0.9740  & 0.9752  \\
\cmidrule{2-14}          & DnCNN & 0.9537  & 0.9742  & 0.9663  & 0.9717  & 0.9790  & 0.9662  & 0.9639  & 0.9690  & 0.9840  & 0.9599  & 0.9736  & 0.9690  \\
    \midrule
    \midrule
    \multirow{12}[24]{*}{Gaussian Denoiser} & LSCD  & 0.9339 & 0.9626 & 0.9641  & 0.9732  & 0.9793  & 0.9633  & 0.9627  & 0.9625  & 0.9867  & 0.9560  & 0.9669  & 0.9440  \\
\cmidrule{2-14}          & LLRT  & 0.9559 & 0.9636 & 0.9707  & 0.9784  & 0.9816  & 0.9669  & 0.9676  & 0.9663  & 0.9899  & 0.9557  & 0.9687  & 0.9633  \\
\cmidrule{2-14}          & GID   & 0.9459 & 0.9633 & 0.9675  & 0.9743  & 0.9790  & 0.9653  & 0.9642  & 0.9670  & 0.9887  & 0.9599  & 0.9729  & 0.9750  \\
\cmidrule{2-14}          & MCWNNM & 0.9568 & 0.9698 & 0.9671  & 0.9774  & 0.9795  & 0.9610  & 0.9567  & 0.9628  & 0.9894  & 0.9516  & 0.9734  & 0.9757  \\
\cmidrule{2-14}          & NLH\_CC & 0.9647 & 0.9759 & 0.9655  & 0.9790  & 0.9841  & 0.9593  & 0.9644  & 0.9630  & \textbf{0.9905} & 0.9552  & 0.9740  & 0.9776  \\
\cmidrule{2-14}          & TWSC  & 0.9592 & 0.9759 & 0.9674  & 0.9767  & 0.9824  & 0.9651  & 0.9617  & 0.9619  & 0.9896  & 0.9385  & 0.9720  & 0.9728  \\
\cmidrule{2-14}          & CBM3D1 & 0.9562 & 0.9729 & 0.9676  & 0.9780  & 0.9827  & 0.9660  & 0.9666  & 0.9681  & 0.9897  & 0.9603  & 0.9725  & 0.9762  \\
\cmidrule{2-14}          & CBM3D2 & 0.9572 & 0.974 & 0.9695  & 0.9780  & 0.9836  & 0.9669  & 0.9668  & 0.9693  & 0.9902  & 0.9610  & 0.9737  & 0.9767  \\
\cmidrule{2-14}          & M-SVD & 0.9542 & 0.9705 & 0.9671  & 0.9788  & 0.9823  & 0.9671  & 0.9680  & 0.9660  & 0.9897  & 0.9606  & 0.9735  & 0.9750  \\
\cmidrule{2-14}          & CBM3D\_best & 0.9621 & 0.9775 & \textbf{0.9712} & \textbf{0.9808} & \textbf{0.9851} & \textbf{0.9741} & \textbf{0.9758} & \textbf{0.9783} & \textbf{0.9904} & \textbf{0.9640} & 0.9742  & \textbf{0.9805} \\
\cmidrule{2-14}          & 4DHOSVD1 & 0.9559 & 0.9729 & 0.9673  & 0.9771  & 0.9797  & 0.9658  & 0.9664  & 0.9671  & 0.9901  & 0.9600  & 0.9736  & 0.9753  \\
\cmidrule{2-14}          & CMSt-SVD & 0.9588 & 0.9756 & 0.9694  & 0.9794  & 0.9840  & 0.9674  & 0.9668  & 0.9674  & \textbf{0.9903} & 0.9616  & \textbf{0.9743} & 0.9770  \\
    \bottomrule
    \end{tabular}%
  \label{Table_color_all_ssim}%
\end{table*}%


==> Table_msi_psnr_ssim.tex <==
%% Table generated by Excel2LaTeX from sheet 'Origin'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Quantitative results comparison under i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$ on CAVE dataset.}
%    \begin{tabular}{cccccccccccccccccc}
%    \toprule
%    \multirow{2}[4]{*}{Methods} & \multicolumn{4}{c}{$\sigma$ = 10} & \multicolumn{4}{c}{$\sigma$ = 30} & \multicolumn{4}{c}{$\sigma$ = 50} & \multicolumn{4}{c}{$\sigma$ = 100} & \multirow{2}[4]{*}{Time (m)} \\
%\cmidrule{2-17}          & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   &  \\
%    \midrule
%    Noisy & 28.13  & 0.4371 & 236.40  & 0.7199 & 18.59  & 0.1069 & 676.01  & 1.0085 & 14.15 & 0.0475  & 1126.7 & 1.1461 & 8.13  & 0.0136  & 2253.4 & 1.3074  & / \\
%    \midrule
%    PARAFAC & 35.39  & 0.8759 & 108.78  & 0.2363 & 33.65  & 0.8294 & 125.13  & 0.3291 & 31.52 & 0.7393  & 154.19 & 0.4351 & 27.13  & 0.4637  & 250.68 & 0.6681  & 3.9 \\
%    \midrule
%    LRTA  & 41.36  & 0.9499 & 49.53  & 0.1718 & 36.06  & 0.8775 & 90.50  & 0.2446 & 33.52 & 0.8201  & 121.15 & 0.2897 & 30.06  & 0.7138  & 180.03 & 0.3649  & \textbf{0.5} \\
%    \midrule
%    LRMR  & 39.27  & 0.9094 & 64.81  & 0.3343 & 31.36  & 0.6451 & 157.65  & 0.6021 & 26.67 & 0.4000  & 264.28 & 0.7534 & 26.67  & 0.1850  & 469.26 & 0.9306  & / \\
%    \midrule
%    LLRGTV & 38.96  & 0.9384 & 71.54  & 0.2292 & 33.56  & 0.7862 & 122.45  & 0.4756 & 30.33 & 0.6375  & 172.22 & 0.6386 & 25.62  & 0.3917  & 288.78 & 0.8593  & 3.8 \\
%    \midrule
%    4DHOSVD1 & 45.43  & 0.9811 & 30.83  & 0.1084 & 39.78  & 0.9336 & 59.12  & 0.2272 & 36.82 & 0.8722  & 83.36 & 0.3385 & 32.66  & 0.7307  & 134.34 & 0.5599  & 4.9 \\
%    \midrule
%    BM4D1 & 42.76  & 0.9716  & 42.19  & 0.1585  & 37.13  & 0.9235  & 82.33  & 0.2910  & 34.55  & 0.8803  & 109.43  & 0.3591  & 31.17  & 0.7763  & 158.83  & 0.4751  & 2.1 \\
%    \midrule
%    BM4D2 & 44.61  & 0.9784 & 33.32  & 0.1289 & 38.80  & 0.9283 & 65.23  & 0.2579 & 35.90  & 0.8685  & 91.19 & 0.3557 & 31.84  & 0.7197  & 144.91 & 0.5160  & 8.8 \\
%    \midrule
%    TDL   & 44.41  & 0.9797 & 34.32  & 0.1048 & 39.07  & 0.9493 & 63.18  & 0.1493 & 36.46 & 0.9171  & 85.24 & 0.2008 & 32.92  & 0.8284  & 128.15 & 0.3132  & 0.9 \\
%    \midrule
%    ISTReg & 45.77  & 0.9802 & 30.53  & 0.1086 & 40.51  & 0.9488 & 53.05  & 0.1374 & 37.75 & 0.9271  & 70.16 & 0.1619 & 33.01  & 0.8648  & 120.77 & 0.2376  & / \\
%    \midrule
%    FastHyDe & 42.87  & 0.9763 & 42.90  & 0.1398 & 37.22  & 0.9151 & 81.44  & 0.3123 & 34.56 & 0.8471  & 108.75 & 0.4395 & 30.62  & 0.6717  & 168.92 & 0.6096  & 0.8 \\
%    \midrule
%    HSI-DeCNN & 41.40  & 0.9624 & 52.04  & 0.1523 & 37.57  & 0.9247  & 78.28 & 0.1959  & 35.49  & 0.8947  & 98.54 & 0.2141  & 32.51  & 0.8309  & 136.16 & 0.2748  & 56.8 \\
%    \midrule
%    LLRT  & \textbf{46.60} & \textbf{0.9868} & \textbf{26.75} & \textbf{0.0842} & \textbf{41.49} & \textbf{0.9681} & \textbf{48.50} & \textbf{0.1221} & \textbf{38.65} & \textbf{0.9482} & 67.56 & \textbf{0.1551} & \textbf{35.39} & \textbf{0.9154} & \textbf{99.37} & \textbf{0.1962} & 43.8 \\
%    \midrule
%    MSt-SVD & 45.20  & 0.9814 & 32.05  & 0.1064 & 40.23  & 0.9530  & 56.26  & 0.1737 & 37.73 & 0.9285  & 75.03 & 0.2231 & 34.20  & 0.8800  & 115.24 & 0.3142  & 1.5 \\
%    \midrule
%    LTDL  & 45.90  & 0.9859  & 29.06  & 0.0925 & 41.20  & 0.9644  & 49.73  & 0.1301 & \textbf{38.63 } & 0.9459  & \textbf{66.68 } & 0.1650  & 34.87  & 0.9015  & 103.65  & 0.2353  & 60.2 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_msi_psnr_ssim}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Origin'
\begin{table*}[ht]
\tiny
  \centering
  \caption{Comparison of quantitative results and computational time (minutes) under i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$ on CAVE dataset.}
  \renewcommand{\arraystretch}{0.918}
    \begin{tabular}{cccccccccccccccccc}
    \toprule
    \multirow{2}[4]{*}{Methods} & \multicolumn{4}{c}{$\sigma$ = 10} & \multicolumn{4}{c}{$\sigma$ = 30} & \multicolumn{4}{c}{$\sigma$ = 50} & \multicolumn{4}{c}{$\sigma$ = 100} & \multirow{2}[4]{*}{Time (m)} \\
\cmidrule{2-17}          & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   &  \\
    \midrule
    Noisy & 28.13  & 0.4371 & 236.40  & 0.7199 & 18.59  & 0.1069 & 676.01  & 1.0085 & 14.15 & 0.0475  & 1126.7 & 1.1461 & 8.13  & 0.0136  & 2253.4 & 1.3074  & / \\
    \midrule
    PARAFAC & 35.39  & 0.8759 & 108.78  & 0.2363 & 33.65  & 0.8294 & 125.13  & 0.3291 & 31.52 & 0.7393  & 154.19 & 0.4351 & 27.13  & 0.4637  & 250.68 & 0.6681  & 3.9 \\
    \midrule
    LRTA  & 41.36  & 0.9499 & 49.53  & 0.1718 & 36.06  & 0.8775 & 90.50  & 0.2446 & 33.52 & 0.8201  & 121.15 & 0.2897 & 30.06  & 0.7138  & 180.03 & 0.3649  & \textbf{0.5} \\
    \midrule
    LRMR  & 39.27  & 0.9094 & 64.81  & 0.3343 & 31.36  & 0.6451 & 157.65  & 0.6021 & 26.67 & 0.4000  & 264.28 & 0.7534 & 26.67  & 0.1850  & 469.26 & 0.9306  & 4.1 \\
    \midrule
    LLRGTV & 38.96  & 0.9384 & 71.54  & 0.2292 & 33.56  & 0.7862 & 122.45  & 0.4756 & 30.33 & 0.6375  & 172.22 & 0.6386 & 25.62  & 0.3917  & 288.78 & 0.8593  & 3.8 \\
    \midrule
    4DHOSVD1 & 45.43  & 0.9811 & 30.83  & 0.1084 & 39.78  & 0.9336 & 59.12  & 0.2272 & 36.82 & 0.8722  & 83.36 & 0.3385 & 32.66  & 0.7307  & 134.34 & 0.5599  & 4.9 \\
    \midrule
    BM4D1 & 42.76  & 0.9716  & 42.19  & 0.1585  & 37.13  & 0.9235  & 82.33  & 0.2910  & 34.55  & 0.8803  & 109.43  & 0.3591  & 31.17  & 0.7763  & 158.83  & 0.4751  & 2.1 \\
    \midrule
    BM4D2 & 44.61  & 0.9784 & 33.32  & 0.1289 & 38.80  & 0.9283 & 65.23  & 0.2579 & 35.90 & 0.8685  & 91.19 & 0.3557 & 31.84  & 0.7197  & 144.91 & 0.5160  & 8.8 \\
    \midrule
    TDL   & 44.41  & 0.9797 & 34.32  & 0.1048 & 39.07  & 0.9493 & 63.18  & 0.1493 & 36.46 & 0.9171  & 85.24 & 0.2008 & 32.92  & 0.8284  & 128.15 & 0.3132  & 0.9 \\
    \midrule
    ITSReg & 45.77  & 0.9802 & 30.53  & 0.1086 & 40.51  & 0.9488 & 53.05  & 0.1374 & 37.75 & 0.9271  & 70.16 & 0.1619 & 33.01  & 0.8648  & 120.77 & 0.2376  & 5.2 \\
    \midrule
    FastHyDe & 42.87  & 0.9763 & 42.90  & 0.1398 & 37.22  & 0.9151 & 81.44  & 0.3123 & 34.56 & 0.8471  & 108.75 & 0.4395 & 30.62  & 0.6717  & 168.92 & 0.6096  & 0.8 \\
    \midrule
    HSI-SDeCNN & 41.40  & 0.9624 & 52.04  & 0.1523 & 37.57  & 0.9247  & 78.28 & 0.1959  & 35.49  & 0.8947  & 98.54 & 0.2141  & 32.51  & 0.8309  & 136.16 & 0.2748  & 0.98 \\
    \midrule
    QRNN3D & 40.36  & 0.9672  & 65.31  & 0.1926  & 38.48  & 0.9496  & 76.21  & 0.2320  & 37.02  & 0.9314  & 87.15  & 0.2741  & 30.33  & 0.7128  & 172.68  & 0.5161  & 0.01  \\
    \midrule
    LLRT  & \textbf{46.60} & 0.9868 & \textbf{26.75} & \textbf{0.0842} & 41.49  & 0.9681 & 48.50 & \textbf{0.1221} & 38.65 & 0.9482  & 67.56 & \textbf{0.1551} & \textbf{35.39} & \textbf{0.9154} & \textbf{99.37} & \textbf{0.1962} & 43.8 \\
    \midrule
    MSt-SVD & 45.20  & 0.9814 & 32.05  & 0.1064 & 40.23  & 0.9530  & 56.26  & 0.1737 & 37.73 & 0.9285  & 75.03 & 0.2231 & 34.20  & 0.8800  & 115.24 & 0.3142  & 1.5 \\
    \midrule
    NGMeet & \textbf{46.58} & \textbf{0.9881} & 27.27  & 0.0853 & \textbf{41.60} & \textbf{0.9692} & \textbf{48.14} & 0.1238 & \textbf{38.88} & \textbf{0.9507} & \textbf{65.64} & 0.1616  & 34.97  & 0.9072  & 101.98 & 0.2506  & 4.6 \\
    \midrule
    LTDL  & 45.90  & 0.9859  & 29.06  & 0.0925 & 41.20  & 0.9644  & 49.73  & 0.1301 & 38.63  & 0.9459  & 66.68  & 0.1650  & 34.87  & 0.9015  & 103.65  & 0.2353  & 60.2 \\
    \bottomrule
    \end{tabular}%
  \label{Table_msi_psnr_ssim}%
\end{table*}%



==> Table_number_cameras_comparsion.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Changes of the proposed IOCI dataset for real-world image denoising.}
  \scalebox{0.95}{
    \begin{tabular}{cccc}
    \toprule
    Version & Number of camera devices & Number of scenes & Number of images \\
    \midrule
    Previous (TPAMI-2020-11-1630) & 9     & 106   & 289 \\
    \midrule
    Current manuscript & \textbf{13} & \textbf{169} & \textbf{409} \\
    \bottomrule
    \end{tabular}}%
  \label{Table_number_cameras_comparsion}%
\end{table}%


==> Table_number_methods_comparison.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Difference in the number of methods and datasets between previous and current versions.}
    \begin{tabular}{ccc}
    \toprule
    Version & Number of compared methods/models & Number of datasets \\
    \midrule
    Previous (TPAMI-2020-11-1630) & 58    & 8 \\
    \midrule
    Current manuscript & \textbf{96}    & \textbf{18} \\
    \bottomrule
    \end{tabular}%
  \label{Table_number_methods_comparison}%
\end{table}%


==> Table_supp_SIDD_validation_test.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet2'
%\begin{table*}[htbp]
%  \centering
%  \caption{Add caption}
%    \begin{tabular}{cccccccccccccccccccccc}
%    \toprule
%    \multirow{2}[4]{*}{PSNR} & \multicolumn{6}{c}{\textcolor[rgb]{ 1,  0,  0}{\textbf{Traditional Methods}}} & \multicolumn{15}{c}{\textcolor[rgb]{ 0,  .439,  .753}{\textbf{Deep learning methods}}} \\
%\cmidrule{2-22}          & Bitonic & CBM3D1 & CBM3D2 & CMS-TSVD & NLH\_CC & AINDNet & CBDNet & CycleISP & DANet & DeamNet & DIDN  & InvDN & MIRNet & MPRNet & NAFNet & NBNet & PD-Denoising & PNGAN & Restormer & RIDNet & VDIR \\
%    \midrule
%    Validation &       & 35.07  & 34.80  & 34.26  &       & 39.08  & 38.35  & 39.52  & 39.54  & 39.47  & 40.04  & 39.32  & 39.68  & 39.71  & 40.21  & 39.76  & 33.99  & 40.07  & 39.93  & 38.78  & 39.37  \\
%    \midrule
%    Test  &       & 35.00  & 34.74  & 34.38  &       & 39.08  & 33.26  & 39.35  & 39.78  & 39.35  & 39.78  & 39.28  & 39.55  & 39.57  & 40.15  & 39.64  & 33.99  & 39.81  & 39.79  & 38.70  & 39.26 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_supp_SIDD_validation_test}%
%\end{table*}%
%

%% Table generated by Excel2LaTeX from sheet 'Sheet2'
%\begin{table*}[htbp]
%\tiny
%  \centering
%  \caption{Add caption}
%  \scalebox{0.83}{
%    \begin{tabular}{ccccccccccccccccccccc}
%    \toprule
%    \multirow{2}[4]{*}{PSNR} & \multicolumn{4}{c}{Traditional denoisers} & \multicolumn{16}{c}{DNN methods} \\
%\cmidrule{2-21}          & Bitonic & CBM3D2 & CMSt-SVD & NLH\_CC & AINDNet & CBDNet & CycleISP & DANet & DeamNet & DIDN  & InvDN & MIRNet & MPRNet & NAFNet & NBNet & PD-Denoising & PNGAN & Restormer & RIDNet & VDIR \\
%    \midrule
%    Validation &       & 34.80  & 34.26  &       & 39.08  & 38.35  & 39.52  & 39.54  & 39.47  & 40.04  & 39.32  & 39.68  & 39.71  & 40.21  & 39.76  & 33.99  & 40.07  & 39.93  & 38.78  & 39.37  \\
%    \midrule
%    Test  &       & 34.74  & 34.38  &       & 39.08  & 33.26  & 39.35  & 39.78  & 39.35  & 39.78  & 39.28  & 39.55  & 39.57  & 40.15  & 39.64  & 33.99  & 39.81  & 39.79  & 38.70  & 39.26 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_supp_SIDD_validation_test}}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[htbp]
\tiny
  \centering
  \caption{Average PSNR value of compared methods on the validation and test data of the SIDD datasets.}
  \scalebox{0.908}{
    \begin{tabular}{ccccccccccccccccccc}
    \toprule
    \multirow{2}[4]{*}{PSNR} & \multicolumn{4}{c|}{Traditional denoisers} & \multicolumn{14}{c}{DNN methods} \\
\cmidrule{2-19}          & Bitonic & CBM3D2 & CMSt-SVD & NLHCC & AINDNet & CycleISP & DANet & DeamNet & DIDN  & InvDN & MIRNet & MPRNet & NAFNet & NBNet & PNGAN & Restormer & RIDNet & VDIR \\
    \midrule
    Validation & 36.46  & 34.80  & 34.26  & 35.18  & 39.06  & 39.52  & 39.54  & 39.47  & 40.04  & 39.32  & 39.68  & 39.71  & 40.21  & 39.76  & 40.07  & 39.93  & 38.78  & 39.37  \\
    \midrule
    Test  & 36.68  & 34.74  & 34.38  & 35.31  & 39.08  & 39.35  & 39.78  & 39.35  & 39.78  & 39.28  & 39.55  & 39.57  & 40.15  & 39.64  & 39.81  & 40.02  & 38.70  & 39.26 \\
    \midrule
    Difference & 0.22  & 0.06  & 0.12  & 0.13  & 0.02  & 0.17  & 0.24  & 0.12  & 0.26  & 0.04  & 0.13  & 0.14  & 0.06  & 0.12  & 0.26  & 0.14  & 0.08  & 0.11  \\
    \bottomrule
    \end{tabular}%
  \label{Table_supp_SIDD_validation_test}}%
\end{table*}%





==> Table_video_psnr_ssim.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet4'
%\begin{table}[htbp]
%\scriptsize
%  \centering
%  \caption{Add caption}
%  \scalebox{0.92}{
%    \begin{tabular}{ccccccc}
%    \toprule
%    \multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{Metric} & \multicolumn{5}{c}{Method} \\
%\cmidrule{3-7}          &       & Noisy & Fastdvdnet & Vnlnet & CVMStSVD & VBM4D \\
%    \midrule
%    \multirow{2}[4]{*}{HUAWEI\_BC} & PSNR  & 38.11  & 41.26  & 41.35  & 40.80  & 41.19  \\
%\cmidrule{2-7}          & SSIM  & 0.9593  & 0.9857  & 0.9868  & 0.9834  & 0.9830  \\
%    \midrule
%    \multirow{2}[4]{*}{HUAWEI\_FC} & PSNR  & 35.58  & 38.03  & 38.79  & 38.71  & 38.76  \\
%\cmidrule{2-7}          & SSIM  & 0.9413  & 0.9776  & 0.9809  & 0.9780  & 0.9785  \\
%    \midrule
%    \multirow{2}[4]{*}{OPPO\_BC} & PSNR  & 32.06  & 33.05  & 33.56  & 33.44  & 33.26  \\
%\cmidrule{2-7}          & SSIM  & 0.9071  & 0.9476  & 0.9544  & 0.9508  & 0.9456  \\
%    \midrule
%    \multirow{2}[4]{*}{OPPO\_FC} & PSNR  & 36.90  & 39.06  & 40.11  & 39.66  & 39.56  \\
%\cmidrule{2-7}          & SSIM  & 0.9447  & 0.9751  & 0.9823  & 0.9791  & 0.9785  \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_video_psnr_ssim}%
%\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet4'
%\begin{table}[htbp]
%\scriptsize
%  \centering
%  \caption{PSNR and SSIM values of compared methods on real-world color video dataset. Average time per frame is also included. The best results are bolded. 'FC' and 'BC' represent front camera and back camera, respectively.}
%  \scalebox{0.88}{
%  \renewcommand{\arraystretch}{0.99}
%    \begin{tabular}{cccccc}
%    \toprule
%    \multirow{2}[4]{*}{Dataset} & \multicolumn{5}{c}{Method} \\
%\cmidrule{2-6}          & Noisy & FastDVDNet & VNLNet & CVMSt-SVD & VBM4D1 \\
%    \midrule
%    \multirow{2}[4]{*}{HUAWEI\_BC} & 38.11  & \textbf{41.26} & \textbf{41.35} & 40.80  & 41.19  \\
%\cmidrule{2-6}          & 0.9593  & 0.9857  & \textbf{0.9868} & 0.9834  & 0.9830  \\
%    \midrule
%    \multirow{2}[4]{*}{HUAWEI\_FC} & 35.58  & 38.03  & \textbf{38.79} & \textbf{38.71} & \textbf{38.76} \\
%\cmidrule{2-6}          & 0.9413  & 0.9776  & \textbf{0.9809} & 0.9780  & 0.9785  \\
%    \midrule
%    \multirow{2}[4]{*}{OPPO\_BC} & 32.06  & 33.05  & \textbf{33.56} & \textbf{33.44} & 33.26  \\
%\cmidrule{2-6}          & 0.9071  & 0.9476  & \textbf{0.9544} & 0.9508  & 0.9456  \\
%    \midrule
%    \multirow{2}[4]{*}{OPPO\_FC} & 36.90  & 39.06  & \textbf{40.11} & 39.66  & 39.56  \\
%\cmidrule{2-6}          & 0.9447  & 0.9751  & \textbf{0.9823} & 0.9791  & 0.9785  \\
%    \midrule
%    Implementation & /     & GPU   & GPU   & MEX   & MEX \\
%    \midrule
%    Time/Frame (s) & /     & \textbf{0.08}  & 0.66  & 1.86  & 1.09 \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{Table_video_psnr_ssim}%
%\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[htbp]
\scriptsize
  \centering
  \caption{PSNR and SSIM values of compared methods on real-world color video dataset. Average time per frame is also included. The best results are bolded. 'FC' and 'BC' represent front camera and back camera, respectively.}
  \scalebox{0.89}{
  \renewcommand{\arraystretch}{0.99}
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}[4]{*}{Dataset} & \multicolumn{5}{c}{Method} \\
\cmidrule{2-6}          & Noisy & CVMSt-SVD & VBM4D1 & FastDVDNet & VNLNet \\
    \midrule
    \multirow{2}[4]{*}{HUAWEI\_BC} & 38.11  & 40.80  & 41.19  & \textbf{41.26} & \textbf{41.35} \\
\cmidrule{2-6}          & 0.9593  & 0.9834  & 0.9830  & 0.9857  & \textbf{0.9868} \\
    \midrule
    \multirow{2}[4]{*}{HUAWEI\_FC} & 35.58  & \textbf{38.71} & \textbf{38.76} & 38.03  & \textbf{38.79} \\
\cmidrule{2-6}          & 0.9413  & 0.9780  & 0.9785  & 0.9776  & \textbf{0.9809} \\
    \midrule
    \multirow{2}[4]{*}{OPPO\_BC} & 32.06  & \textbf{33.44} & 33.26  & 33.05  & \textbf{33.56} \\
\cmidrule{2-6}          & 0.9071  & 0.9508  & 0.9456  & 0.9476  & \textbf{0.9544} \\
    \midrule
    \multirow{2}[4]{*}{OPPO\_FC} & 36.90  & 39.66  & 39.56  & 39.06  & \textbf{40.11} \\
\cmidrule{2-6}          & 0.9447  & 0.9791  & 0.9785  & 0.9751  & \textbf{0.9823} \\
    \midrule
    Implementation & /     & MEX   & MEX   & GPU   & GPU \\
    \midrule
    Time/Frame (s) & /     & 1.86  & 1.29  & \textbf{0.08}  & 0.66 \\
    \bottomrule
    \end{tabular}%
    }
  \label{Table_video_psnr_ssim}%
\end{table}%


